Exploring and Exploiting Decision Boundary Dynamics for Adversarial Robustness

The robustness of a deep classifier can be characterized by its margins: the decision boundary's distances to natural data points. However, it is unclear whether existing robust training methods effectively increase the margin for each vulnerable point during training. To understand this, we propose a continuous-time framework for quantifying the relative speed of the decision boundary with respect to each individual point. Through visualizing the moving speed of the decision boundary under Adversarial Training, one of the most effective robust training algorithms, a surprising moving-behavior is revealed: the decision boundary moves away from some vulnerable points but simultaneously moves closer to others, decreasing their margins. To alleviate these conflicting dynamics of the decision boundary, we propose Dynamics-aware Robust Training (DyART), which encourages the decision boundary to engage in movement that prioritizes increasing smaller margins. In contrast to prior works, DyART directly operates on the margins rather than their indirect approximations, allowing for more targeted and effective robustness improvement. Experiments on the CIFAR-10 and Tiny-ImageNet datasets verify that DyART alleviates the conflicting dynamics of the decision boundary and obtains improved robustness under various perturbation sizes compared to the state-of-the-art defenses. Our code is available at https://github.com/Yuancheng-Xu/Dynamics-Aware-Robust-Training.

==> A_continuous_workshop/Speed_unnormalized_time.tex <==
\begin{wrapfigure}{r}{0.43\textwidth}%[!t] % !htbp
    \centering
    \vspace{-2em}
    \begin{subfigure}[t]{0.2\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/VR_AT_acc_noWithinCorrect}}
        \caption{\scriptsize{Test accuracy of AT}}
        \label{fig: AT_acc}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.2\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/AT_test_speed_time}}
        \caption{\scriptsize{Speed distribution of AT}}
        \label{fig: AT_speed_time}
    \end{subfigure}
    % \centering
    % \begin{subfigure}[t]{0.48\columnwidth}
    %     \centering
    %     \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/clean_acc}}
    %     \caption{\scriptsize{Test accuracy of NT}}
    %     \label{fig: clean_acc}
    % \end{subfigure}%
    % \hfill
    % \begin{subfigure}[t]{0.48\columnwidth}
    %     \centering
    %     \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/clean_test_speed_time}}
    %     \caption{\scriptsize{Speed distribution of NT}}
    %     \label{fig: clean_speed_time}
    % \end{subfigure}%
    \vspace{-0.9em}
    \caption{Speed distribution on the test set during AT. In Figure~\ref{fig: AT_speed_time}, % and Figure~\ref{fig: clean_speed_time}, 
    the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. }
    \label{fig: speed_time_all}
    \vspace{-1em}
\end{wrapfigure}

==> A_continuous_workshop/a1_speed_derivation.tex <==
\section{Proof of the closed-form expression for the speed 
in Equation \ref{eq: expression_for_speed}
} \label{app: closed_expression_speed}

In this section, our goal is to prove the closed-form expression~\eqref{eq: expression_for_speed} and provide further discussions. We first provide two preliminary lemmas and present the mathematical assumptions. Then we rigorously derive the closed-form expression. Finally, we discuss more about the expression and its assumptions. 

\begin{lemma} \label{lemma: norm_pq_app}
For $1\leq p \leq \infty$ and let $q$ satisfies $1/q+1/p=1$. Let $a$ be any fixed vector. Then 
\begin{equation*} 
    \left\|\nabla_x \left\|x-a\right\|_p\right\|_q = 1
\end{equation*}
\end{lemma}

\begin{proof}
Without loss of generality, assume $a$ is the zero vector. Write the $k$-th component of $x$ as $x_k$.

\emph{Case 1: $1\leq p < \infty$}

By calculation, $\frac{\partial \|x\|_p}{\partial x_k} = (\frac{|x_k|}{\|x\|_p})^{p-1}\cdot \sign (x_k)$. Since $q = \frac{p}{p-1}$, we have that 
\begin{equation*}
\begin{aligned}
\sum_k |\frac{\partial \|x\|_p}{\partial x_k}|^{q} &= \sum_k  |(\frac{|x_k|}{\|x\|_p})^{p-1}\cdot \sign (x_k)|^{\frac{p}{p-1}} \\
&= \sum_k \frac{|x_k|^p}{\|x\|_p^p} \\
&= 1
\end{aligned}
\end{equation*}

Therefore, $\left\|\nabla_x \left\|x\right\|_p\right\|_q = (\sum_k |\frac{\partial \|x\|_p}{\partial x_k}|^{q})^{1/q} = 1$.

\emph{Case 2: $p = \infty$}

In this case, $\nabla_x \|x\|_\infty$ is a one-hot vector (with the one being the position of the element of $x$ with the largest absolute value). Therefore, $\left\|\nabla_x \left\|x\right\|_{\infty}\right\|_1$ = 1. 

\end{proof}

The following lemma deals with the optimality condition for $p = \infty$. Special care needs to be taken since $L_\infty$ norm is not a differentiable function.

\begin{lemma} \label{lemma: Linf_optimality_app}
If $\hat{x}$ is a local optimum of the constrained optimization problem where $a$ is any fixed vector with $\phi(a) > 0$: 
\begin{equation*} \label{eq: closest_linf_app}
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
    \hat{x} = \argmin_{z} \|x-a\|_\infty \quad \textrm{s.t.}  \quad \phi(x) = 0.
\end{equation*}
Assume that $\phi$ is differentiable at point $\hat{x}$. Denote the coordinates set $\mathcal{J} = \{j: |\hat{x}_j - a_j| = \|\hat{x}-a\|_\infty\}$. Denote the $k$-th component of $\nabla_x \phi(\hat{x})$ as $\nabla_x \phi(\hat{x})_k$. Then (a) for $j \in \mathcal{J}$, $\nabla_x \phi(\hat{x})_j$ and $\hat{x}_j - a_j$ have opposite signs; (b) for $k\notin \mathcal{J}$, $\nabla_x \phi(\hat{x})_k = 0$. 
\end{lemma}

\begin{remark*}
If $\phi(a)<0$, then (a) for $j \in \mathcal{J}$, $\nabla_x \phi(\hat{x})_j$ and $\hat{x}_j - a_j$ have the same sign; (b) for $k\notin \mathcal{J}$, $\nabla_x \phi(\hat{x})_k = 0$.
\end{remark*}

\begin{proof}
\emph{(a)}
Consider the perturbation $\hat{x}(\epsilon) = \hat{x} + (0,\cdots,\epsilon_{j_1},\cdots,\epsilon_{j_m},\cdots,0)$ where $\mathcal{J} = \{j_1,\cdots,j_m\}$ and $\epsilon$ is a $m$ dimensional vector with $j$-th component $\epsilon_j$. Since $\phi(a)>0$ and $\hat{x}$ is a local optimum, $\|x-a\|_\infty < \|\hat{x}-a\|_\infty$ imply $\phi(x) > 0$ if $x$ is sufficiently close to $\hat{x}$. Therefore, if every $\epsilon_{j_i}$ is chosen so that $|\hat{x}_{j_i} + \epsilon_{j_i} - a_{j_i}| < |\hat{x}_{j_i} - a_{j_i}|$ (that is, $\epsilon_{j_i}$ has different sign from $\hat{x}_{j_i} - a_{j_i}$) and $\|\epsilon\|$ sufficiently small, then $\|\hat{x}(\epsilon) - a\| < \|\hat{x}-a\|$ and thus $\phi(\hat{x}(\epsilon))>0$. 

On the other hand, by Taylor expansion and the fact that $\phi(\hat{x})=0$, we have that 

\begin{equation*}
    \phi(\hat{x}(\epsilon)) = \sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j + \mathcal{O}(\|\epsilon\|^2)
\end{equation*}

Therefore, $\sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j > 0$ for any such $\epsilon$. By taking other $\epsilon_k \to 0$ if necessary, we obtain that $\forall j \in \mathcal{J}$, $\nabla \phi(\hat{x})_j \epsilon_j \geq 0$, where $\epsilon_j$ has different sign from $\hat{x}_{j} - a_{j}$. Therefore, $\nabla \phi(\hat{x})_j$ and $\hat{x}_{j} - a_{j}$ have different signs. 


\emph{(b)}
Take any $k \notin \mathcal{J}$ and consider the perturbation $\hat{x}(\epsilon) = \hat{x} + (0,\cdots,\epsilon_{j_1},\cdots,\epsilon_k,\cdots,\epsilon_{j_k},\cdots,0)$ where $\epsilon=(\epsilon_{j_1},\cdots,\epsilon_k,\cdots,\epsilon_{j_k})$. Choose any $\epsilon$ so that $\|\epsilon\|$ is sufficiently small, each $\epsilon_{j_i}$ has the opposite sign of $\hat{x}_{j_i} - a_{j_i}$ and $\epsilon_k$ small enough (which can be positive or negative), we have that $\phi(\hat{x}(\epsilon)) > 0$ since $\|\hat{x}(\epsilon) - a\|_\infty < \|\hat{x}-a\|_\infty$. By Taylor expansion, $\sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j + \epsilon_k \nabla_x \phi(\hat{x})_k > 0$ for any such $\epsilon$. By taking $\epsilon_j \to 0$ and using the fact that $\epsilon_k$ can be positive or negative, we conclude that $\nabla_x \phi(\hat{x})_k = 0$.

\end{proof}


Now we are ready to derive the closed-form expression of the speed. We first provide the full assumptions, then derive the expression, and finally we will discuss more about the assumptions. We will write $\hat{x}_i(t)$ as $\hat{x}_i$ when the indication is clear. 
\begin{assumption} \label{assumption: differentible}
Suppose that $(x_i,y_i)$ is correctly classified by $f_{\theta(t)}$ in some time interval $t \in I$ and $\hat{x}_i(t)$ is a locally closest boundary point in the sense that for any $t\in I$, it is the local optimum of the following:
\begin{equation*} 
    \hat{x}_i(t) = \argmin\nolimits_{\hat{x}} \|\hat{x}-x_i\|_p \quad \textrm{s.t.}  \quad \phi^{y_i}(\hat{x},\theta(t)) = 0.
\end{equation*}
Assume that in the time interval $I$: (a) $\hat{x}_i(t)$ is differentiable in $t$; (b) $\phi^{y_i}$ is differentiable at point $\hat{x}_i(t)$ and at the current parameter $\theta(t)$.
\end{assumption}


\begin{proposition*}[Closed-form expression of the speed $s(x_i,t)$] For $1 \leq p \leq \infty$ and under the Assumption~\ref{assumption: differentible}, define the (local) speed according to $\hat{x}_i(t)$ in Assumption~\ref{assumption: differentible} as $s(x_i,t) = \frac{d}{dt}\|\hat{x}_i(t) - x_i\|_p$, we have the following:

\begin{equation*} 
    s(x_i,t) = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)
\end{equation*}
where $q$ satisfies that $1/q+1/p=1$. In particular, $q=2$ when $p=2$ and $q=1$ when $p=\infty$.
\end{proposition*}

\begin{proof}
\emph{Case 1: $1\leq p < \infty$}

To compute $ s(x_i,t) = \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_2$, we need to characterize the curve of the closest boundary point $\hat{x}_i(t)$, where two key points stand out. First, $\hat{x}_i(t)$ is on the decision boundary $\Gamma_y (t)$ and thus  $\phi^y(\hat{x}_i(t),\theta(t)) = 0$ for all $t \in I$. By taking the time derivative on both sides, we obtain the level set equation \citep{osher2004level,aghasi2011parametric}

\begin{equation} \label{eq: LF_app}
	\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\cdot \hat{x}_i'(t) + \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) = 0
\end{equation}

Second, $\hat{x}_i(t)$ is the optimal solution of constrained optimization \eqref{eq: closest_pt}. Therefore, we have the following optimality condition:

\begin{equation} \label{eq: optimality_app}
    \nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t)) + \lambda(t)\nabla_x\|\hat{x}_i(t)-x_i\|_p = 0
\end{equation}

Since $x_i$ is correctly classified, $\phi^{y_i}(x_i) > 0$. Since $\hat{x}_i(t)$ is the closest point to $x_i$ whose $\phi^{y_i}$ value is zero, $\lambda(t) >0$. By taking the $L_q$ norm in Equation~\eqref{eq: optimality_app} and using Lemma~\ref{lemma: norm_pq_app}, we obtain that $\lambda(t) = \|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q$.

Now, we derive $s(x_i,t)$ as follows:

\begin{equation*}
\begin{aligned}
    s(x_i,t) &= \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_p  \\
    & = \nabla_x\|\hat{x}_i(t)-x_i\|_p \cdot \hat{x}_i'(t) \\
    & = -\frac{1}{\lambda} \nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t)) \cdot \hat{x}_i'(t) && \text{(By the optimality condition~\eqref{eq: optimality_app})} \\
    & = \frac{1}{\lambda} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) && \text{(By the level set equation~\eqref{eq: LF_app})}\\
    & = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x \phi^{y}(\hat{x}_i(t),\theta(t))\|_q}  
\end{aligned}
\end{equation*}

\emph{Case 2: $p = \infty$}

Note that since $L_\infty$ is not differentiable, the optimality condition in Equation~\eqref{eq: optimality_app} does not hold anymore. 

Denote the $j$-th component of $\hat{x}_i(t)$ and $x_i$ as $\hat{x}_{ij}(t)$ and $x_{ij}$. Let $\mathcal{J} = \{j: |\hat{x}_{ij}(t) - x_{ij}| = \|\hat{x}_i(t)-x_i\|_\infty\}$. By Lemma~\ref{lemma: Linf_optimality_app}, $s(x_i,t) = \frac{d}{dt}|\hat{x}_{ij}(t) - x_{ij}| = \hat{x}_{ij}^{'}(t) \sign (\hat{x}_{ij}(t)-x_{ij}) = - \hat{x}_{ij}^{'}(t) \sign (\nabla_x\phi^{y_i}(\hat{x}_{i})_j)$ for all $j \in \mathcal{J}$. Therefore, by Equation~\eqref{eq: LF_app} and Lemma~\ref{lemma: Linf_optimality_app}

\begin{equation*}
\begin{aligned}
- \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) &= \nabla_x \phi^{y_i}(\hat{x})\cdot \hat{x}_i'(t)\\
&= \sum_{j \in \mathcal{J}} \nabla_x \phi^{y_i}(\hat{x}_i)_j\cdot \hat{x}_{ij}'(t) \\
&= \sum_{j \in \mathcal{J}} - \nabla_x \phi^{y_i}(\hat{x}_i)_j \cdot \frac{s(x_i,t)}{\sign (\nabla_x\phi^{y}(\hat{x}_{i})_j)} \\
&= - \sum_{j \in \mathcal{J}} |\nabla_x\phi^{y_i}(\hat{x}_{i})_j| \cdot s(x_i,t)
\end{aligned}
\end{equation*}

Therefore, $s(x_i,t) = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\sum_{j \in \mathcal{J}} |\nabla_x\phi^{y_i}(\hat{x}_{i})_j|} = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x\phi^{y_i}(\hat{x}_{i})\|_1}$, where the last equality follows from Lemma~\ref{lemma: Linf_optimality_app} that the components of $\nabla_x \phi^{y_i}(\hat{x}_i)$ are zeros if they are not in $\mathcal{J}$.
 
\end{proof}

\subsection*{Discussions on the assumptions}
Assumption~\ref{assumption: differentible} has several points that need to be explained further.

First, we only require that $\hat{x}_i(t)$ is a local closest boundary point. This is important because in practice when an algorithm for searching the closest boundary point is used (e.g. FAB), a local solution is the best one can hope for due to the non-convex nature of the optimization problem. When $\hat{x}_i(t)$ is a local solution, the speed should be interpreted as how fast the distance changes around that local solution. In this case, although $\hat{x}_i$ is not the globally closest adversarial example, the local speed around $\hat{x}_i$ still has much information on the relative movement of the decision boundary w.r.t. $x_i$, especially when the distance  $\|\hat{x}_i - x_i\|$ is relatively small and the input space is a high-dimensional space (e.g. pixel space). 

Second, we require that $\hat{x}_i(t)$ is a differentiable curve in time interval $I$. Note that if we constrain $\hat{x}_i(t)$ to be the global closest boundary point, $\hat{x}_i$ is unlikely to be differential for a large time interval $I$, especially in high dimensional space. This is because as the decision boundary moves. the closest point might switch from one point to another point that is very far away abruptly. Fortunately, this problem is alleviated because our derived closed-form expression still works when $\hat{x}_i(t)$ is a locally closest boundary point. Note that however, due to the \textit{topological change} of the decision boundary, it still can happen that $\hat{x}_i(t)$ stops existing (and thus stops being differentiable) at some time point, when typically the speed will go to infinity. From a mathematical point of view, this is related to \textit{shock} in partial differential equation (PDE) theories. More exploration on this is left to future work. In this work, we only consider the speed of the decision boundary at each discrete time step.


==> A_continuous_workshop/a2_method_details.tex <==
\section{Algorithms} \label{app: algo}

\subsection{Details of the optimization problem \ref{eq:opt_for_weight}} \label{app: opt_for_weight}

In this section, we provide details of the optimization problem~\eqref{eq:opt_for_weight} by specifying the coefficients of this quadratic programming concretely using the neural network gradients $\nabla_x \phi^{y_i}(\hat{x}_i)$ and  $\nabla_\theta \phi^{y_i}(\hat{x}_i)$.

\subsubsection{The dependency between the weights and the speed}

First, we give the details of $\mathbf{s}(\mathbf{c})$, i.e. how the weights $\mathbf{c} = (c_1,\cdots, c_m)^{T}$ (linearly) determines the speed $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$. Recall that the dimension of the parameters $\theta$ is $p$, and the number of points in $\mathcal{B}_\theta^{+}$ is $m$. 

% theta'
\paragraph{The update rule $\theta'$} The weights $\mathbf{c}$ determines the update rule $\theta_k'$ as follows. We write $\theta'_k$ as $\theta' = \sum_{i\in \mathcal{B}_\theta^{+}}c_i\nabla_\theta \phi^{y_i}(\hat{x}_i) + z$, where the step index $k$ is omitted and $z$ includes terms that do not depend on the weights $\mathbf{c}$. In this paper, we use SGD with momentum and weight decay (which is commonly used in AT methods) and thus the relationship between $\theta'$ and the loss function is given by
% Equation~\eqref{eq: theta prime momentum weight decay general}

\begin{equation} \label{eq: theta prime momentum weight decay general}
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{aligned}
    \theta'_k &= -\nabla_\theta L(\theta_{k})  - \lambda_w \theta_{k}- \lambda_m b_{k}
\end{aligned}
\end{equation}

which can be interpreted as the un-normalized update direction of $\theta$ at step $k$. In this case, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$, where $\lambda_c$, $\lambda_w$ and $\lambda_m$ are coefficients for the clean loss, weight decay and momentum. 


% V(c)
\paragraph{The speed $\mathbf{s}(\mathbf{c})$} The weights $\mathbf{c}$ determines the speed $\mathbf{s}(\mathbf{c})$ through $\theta'$ as follows. By Equation~\eqref{eq: expression_for_speed}, $s(x_i) = \alpha_i \nabla_\theta \phi^{y_i}(\hat{x}_i)\cdot\theta'$ where $\alpha_i = \frac{1}{\|\nabla_x\phi^{y_i}(\hat{x}_i)\|_q}$. To expand it, we have 

\begin{equation*}
    s(x_i) =  \alpha_i \nabla_\theta \phi^{y_i}(\hat{x}_i)\cdot (\sum_{i\in \mathcal{B}_\theta^{+}}c_i\nabla_\theta \phi^{y_i}(\hat{x}_i) + z)
\end{equation*}
Now we express $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$ with $\mathbf{c}$ using the above equation in matrix form. Denote $A\in \mathbb{R}^{p\times m}$ as the matrix whose i-th column is $\nabla_\theta\phi^{y_i}(\hat{x}_i,y_i)$, $i = 1,\cdots,m$.  Also denote $\alpha \in \mathbb{R}^{m\times m}$ a diagonal matrix whose i-th diagonal element is $\alpha_i$. Then we have the following 

\begin{equation} \label{eq: s_c_app}
    \mathbf{s}(\mathbf{c}) =  \alpha A^{T} A \mathbf{c} + \alpha A^{T} z
\end{equation}

\subsubsection{The coefficients of problem \ref{eq:opt_for_weight}}

We give the coefficients of the quadratic programming problem~\eqref{eq:opt_for_weight} in matrix forms. 

We write all the optimization variables in a single vectors $\mathbf{w} = (c_1,\cdots,c_m,\mu)$.
By Equation~\eqref{eq: s_c_app}, we have that $\mathbf{s}(\mathbf{c}) - \mu \mathbf{g} = \alpha A^{T} A \mathbf{c} + \alpha A^{T} z - \mu \mathbf{g} = M\mathbf{w} + \alpha A^{T} z$, where $M \in \mathbb{R}^{m\times (m+1)}$ whose first $m$ columns are equal to the matrix $\alpha A^{T} A$ and the last column is equal to $-\mathbf{g}$. Therefore, the optimization problem~\eqref{eq:opt_for_weight} is rewritten as the follows:   

\begin{equation} \label{eq: opt_for_weight_withMu_detail_app}
\begin{aligned}
\min_{\mathbf{w}} \quad & \mathbf{w}^{T}M^{T}M\mathbf{w} + 2\mathbf{w}^{T}(M^{T}\alpha A^{T}z)  \\
\textrm{s.t.} & \quad 
\begin{bmatrix}
    1 &\cdots & 1 & 0
\end{bmatrix}\mathbf{w} = 1, \mathbf{w} \geq 0   \\
\end{aligned}    
\end{equation}

In summary, the details of the optimization problem~\eqref{eq:opt_for_weight} to obtain the weights $\mathbf{c} = (c_1,\cdots,c_m)$ are given by optimization problem~\ref{eq: opt_for_weight_withMu_detail_app}, where $\mathbf{w} = (c_1,\cdots,c_m,\mu)$, 
$M = \begin{bmatrix}
  \alpha A^{T}A 
  & \rvline & -\mathbf{g}
\end{bmatrix}$, 
$A = \begin{bmatrix}
  \nabla_\theta \phi^{y_1}(\hat{x}_1) & \cdots & \nabla_\theta \phi^{y_m}(\hat{x}_m) 
\end{bmatrix}$,
$
\alpha = \text{diag}(\alpha_1,\cdots,\alpha_m)
$,
$\alpha_i = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i)\|_q}$, and $z$ is the terms in $\theta'$ that do not depend on $\mathbf{c}$ (for example, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$ when SGD with momentum and weight decays is used). The problem~\eqref{eq: opt_for_weight_withMu_detail_app} is a quadratic programming problem with $m+1$ variables, which can be solved efficiently. 


\subsubsection{An alternative to problem \ref{eq:opt_for_weight}}
Here we present an alternative optimization problem to problem~\eqref{eq:opt_for_weight}, which is slightly more efficient since it corresponds to a quadratic problem of size $m$, instead of $m+1$ as in problem~\eqref{eq:opt_for_weight}. The alternative is given as follows:

\begin{equation} \label{eq:opt_for_weight_withoutMu_app}
\begin{aligned}
\min_{\mathbf{c}}\min_{\mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} c_i = 1, \quad c_i\geq0   \\
\end{aligned}
\end{equation}

The difference of problem~\eqref{eq:opt_for_weight_withoutMu_app} and the problem  problem~\eqref{eq:opt_for_weight} is that the former omit the constraint on $\mu$ to be positive. However, their optimal $\mathbf{c}$ are the same if the optimal $\mu$ is positive for the alternative optimization problem~\eqref{eq:opt_for_weight_withoutMu_app}. We find that in our experiments, the solved $\mu$ is always positive for the alternative problem~\eqref{eq:opt_for_weight_withoutMu_app} and thus these two optimization problems are equivalent. Due to its slightly better efficiency, we use the alternative formulation~\eqref{eq:opt_for_weight_withoutMu_app} instead of the formulation~\eqref{eq:opt_for_weight}.   We now give the details of the alternative optimization problem.


We use the following lemma:

\begin{lemma*}
\begin{equation*}
    \min_{\mu} \|x-\mu \mathbf{g}\|_2^2 = \|E_\mathbf{g} x\|_2^2 
\end{equation*}
where $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$.
\end{lemma*}

Therefore, $\min_{\mu}\|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 = \|E_\mathbf{g} \mathbf{s}(\mathbf{c})\|_2^2$. By Equation~\eqref{eq: s_c_app} that we have derived in the last section, $\mathbf{s}(\mathbf{c}) = \alpha A^{T} A \mathbf{c} + \alpha A^{T} z $. Therefore, $\min_{\mathbf{c}}\min_{\mu}  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 = \min_{\mathbf{c}}\|E_\mathbf{g} \mathbf{s}(\mathbf{c})\|_2^2 = \min_{\mathbf{c}}\|E_\mathbf{g} ( \alpha A^{T} A \mathbf{c} + \alpha A^{T} z)\|_2^2$, which corresponds to the following constrained quadratic programming problem:

\begin{equation} \label{eq: opt_for_weight_withoutMu_detail_app}
\begin{aligned}
\min_{\mathbf{c}} \quad & \mathbf{c}^{T}K_1^{T}K_1\mathbf{c} + 2\mathbf{c}^{T}(K_1^{T}K_2)  \\
\textrm{s.t.} & \quad \sum_{i}c_i = 1, \mathbf{c} \geq 0   \\
\end{aligned}    
\end{equation}

where $K_1 = E_\mathbf{g}\alpha A^{T}A, K_2 = E_\mathbf{g}\alpha A^{T}z$. 

In summary, the alternative scheme \eqref{eq:opt_for_weight_withoutMu_app} is given by the quadratic problem \eqref{eq: opt_for_weight_withoutMu_detail_app}, where $K_1 = E_\mathbf{g}\alpha A^{T}A, K_2 = E_\mathbf{g}\alpha A^{T}z$, $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$, $A = \begin{bmatrix}
  \nabla_\theta \phi^{y_1}(\hat{x}_1) & \cdots & \nabla_\theta \phi^{y_m}(\hat{x}_m) 
\end{bmatrix}$,
$
\alpha = \text{diag}(\alpha_1,\cdots,\alpha_m)
$,
$\alpha_i = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i)\|_q}$, and $z$ is the terms in $\theta'$ that do not depend on $\mathbf{c}$ (for example, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$ when SGD with momentum and weight decays is used). The problem~\eqref{eq: opt_for_weight_withoutMu_detail_app} is a quadratic programming problem in $m$ variables, which can be solved efficiently. 



\subsection{Workflow of \algoName} \label{app: algo_pseudo}
We present the pseudocode of our proposed \algoName in Algorithm~\ref{alg: main algo}.
\input{\texhome/algo} 


\section{Optimality condition in practice} \label{app: optimality}
Either computing the speed of the decision boundary or reverse engineering an update rule to achieve some desirable dynamics (like what \algoName does) requires the computation of the closest boundary point $\hat{x}$ for the correctly classified data point $(x,y)$, where we omit the subscript $i$ in this section. As discussed in Appendix~\ref{app: closed_expression_speed}, it suffices to find the local closest boundary point in order for the closed-form expression~\eqref{eq: expression_for_speed} for the speed to be valid. 

In this section, we will explain how to check the quality of the found $\hat{x}$ for the constrained optimization problem~\ref{eq: closest_pt} in practice. We will also give a simple analysis on how FAB\citep{croce2020minimally}, the algorithm we use in our implementation, solves the problem~\ref{eq: closest_pt} in practice. In this paper, we focus on $p = 2$ and $p = \infty$. 

The key points of analyzing $\hat{x}$ are that $\phi^{y}(\hat{x}) = 0$ and the KKT condition of problem~\ref{eq: closest_pt}.

\emph{Case 1: $p=2$}

In this case, the KKT condition is given by $\nabla_x \phi^{y}(\hat{x}) + \lambda (\hat{x} - x) = 0$ for some $\lambda > 0$ (since $\phi^{y}(x) >0$). In other words, $\frac{\nabla_x \phi^{y}(\hat{x})}{\|\nabla_x \phi^{y}(\hat{x})\|} \cdot \frac{x-\hat{x}}{\|x-\hat{x}\|} = 1$. In practice, we check the following two conditions (a) $|\phi(\hat{x})| \leq 0.1$; (b) $\frac{\nabla_x \phi^{y}(\hat{x})}{\|\nabla_x \phi^{y}(\hat{x})\|} \cdot \frac{x-\hat{x}}{\|x-\hat{x}\|} > 0.8$. In our experiments, we find that FAB with iterations greater than 10 can reliably find $\hat{x}$ satisfying these two conditions. In all of our experiments when $p=2$, including computing the speed for various methods (e.g. AT) and the implementation of \algoName, we only use those high-quality closest boundary points that satisfy these two conditions and discard the rest. We observe in our experiments that FAB can find high-quality closest boundary points for over 90\% of the correctly classified data points. 

\emph{Case 2: $p=\infty$}

In this case, we consider the optimality condition given in Lemma~\ref{lemma: Linf_optimality_app} of Appendix~\ref{app: closed_expression_speed}. Denote $\#B$ the number of points in the set $B$. Using the notation $\mathcal{J} = \{j: |\hat{x}_j - x_j| = \|\hat{x}-x\|_\infty\}$ and $\mathcal{J}^{C}$ the complement set of $\mathcal{J}$, we check the following conditions in practice: (a) $|\phi(\hat{x})| \leq 0.1$; (b) $\frac{\#\{j\in\mathcal{J}: \nabla_x \phi^{y}(\hat{x})_j (\hat{x}_j - x_j) \leq 0\}}{\#\mathcal{J}} > 0.9$; (c) $\frac{\#\{k\notin J: |\nabla_x \phi^{y}(\hat{x})_k| < 0.1 \}}{\#\mathcal{J}^C} > 0.8$. Note the unlike $p=2$, the optimality conditions for $p=\infty$ are on each coordinate of $\hat{x}$, which is more difficult to satisfy. We observe in our experiments that FAB with 60 iterations can find high-quality closest boundary points for about 85\% of the correctly classified points. However, when only 15 iterations are used, condition (3) is barely satisfied for all of the found boundary points (the first two conditions are still satisfied). In our visualizations of dynamics of the decision boundary for various methods in $L_\infty$ setting in Appendix~\ref{app: more_dynamics}, we use 60 iterations for FAB and only use high-quality closest boundary points, so that the visualization results are accurate. In our implementation of \algoName, we omit the condition (3) and only use 15 iterations for FAB for efficiency. 

Designing faster and more reliable methods to solve the constrained optimization problem~\ref{eq: closest_pt}, especially when $p = \infty$, is left for future work. 

==> A_continuous_workshop/a3_experiment.tex <==
\section{Experiments}\label{app: exp}
In this section, we provide experimental details and further results of \algoName along with other state-of-the-art defense methods. 
\subsection{Detailed experimental settings} \label{app: exp_settings}

\paragraph{Basic training setting} 
In all experiments on CIFAR-10 in this section, we use the Wide Residual Networks  \citep{zagoruyko2016wide} with depth 28 and width factor 4 (WRN-28-4), which is also used in previous works \citep{Ding2020MMA}. We replace the batch normalization (BN) layers with group normalization (GN) \citep{wu2018group} layers so that the decision boundary is the same at training and test time. This is necessary for \algoName since it uses the closest boundary points during training, which should be also on the decision boundary in the evaluation mode. For other baselines, we find that replacing BN with GN has negligible effect on the robustness performance. We use stochastic gradient descent with momentum 0.9 and weight decay 0.0005, which is suggested in \citep{pang2020bag}. We train 100 epochs in total with batch size 128. The learning rate begins at 0.1 and is decayed by a factor of 10 at the 50th and 75th epoch. The first 10 epochs of \algoName is the burn-in period, where only the clean loss is used. To alleviate robust overfitting \citep{rice2020overfitting}, early stopping is performed on a validation set of size 2000 in all experiments, where the model with the highest robust accuracy under projected gradient descent (PGD) attacks \citep{madry2017towards} with 20 steps (PGD-20) is chosen. All experiments are run on two NVIDIA GeForce RTX 2080 Ti GPU. 

\paragraph{Per-sample gradient} During implementation of the expression for speed in Equation~\eqref{eq: expression_for_speed} and also \algoName, we need to compute the per-sample gradient $\nabla_\theta \phi^{y_i}(\hat{x}_i,\theta)$ for every correctly classified point $x_i$. We use the Opacus package \citep{opacus} for computing per-sample gradients in parallel. Also, another reason why we replace BN with GN is because Opacus does not support BN for computing per-sample gradients.   


\paragraph{Evaluation protocol}
We evaluate our proposed method and baselines under $L_2/L_\infty$-norm constrained perturbation. The final robust accuracy is reported on the full test set against PGD-40 attack as well as AutoAttack (AA) \citep{croce2020reliable}, which uses an ensemble of selected strong attacks. Note that although AA is considered stronger and serves as a more reliable measure of robustness, we still include PGD attack results since it can happen that some methods performs well against PGD attack, but not against AA. In all experiments we find that AA gives lower robust accuracy than PGD attack. Therefore, we refer to the robust accuracy against AA, instead of PGD, when comparing performance among different defense methods. For all methods, we choose the hyperparameters to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. In addition, we evaluate on larger perturbation thresholds to better examine the robustness of the model against larger unknown perturbation thresholds. 

\textbf{Compared baselines and their hyperparameters}\quad
The baseline defense methods include: (1) standard adversarial training (AT) \citep{madry2017towards} which trains on the worst case adversarial examples generated by 10-step PGD (PGD-10) on the cross-entropy loss. The perturbation threshold is $0.5$ in $L_2$ setting, and $\frac{8}{255}$ in $L_\infty$ setting. The step size of PGD is $\frac{15}{255}$  in $L_2$ setting and $\frac{2}{255}$ in $L_\infty$ setting; the training setting follows Rice et al.\footnote{\href{https://github.com/locuslab/robust_overfitting}{Robust Overfitting's Github}}  \citep{rice2020overfitting}. (2) TRADES \footnote{\href{https://github.com/yaodongyu/TRADES}{TRADES's Github}}\citep{zhang2019theoretically} which trades off between the clean and robust accuracy. The perturbation threshold is $0.5$ in $L_2$ setting, and $\frac{8}{255}$ in $L_\infty$ setting. The step size of PGD-10 is $\frac{15}{255}$  in $L_2$ setting and $0.007$ in $L_\infty$ setting ; The regularization constant beta (or 1/lambda) is set to  6. (3) MMA  \footnote{\href{https://github.com/BorealisAI/mma_training}{MMA's Github}}  \citep{Ding2020MMA} which trains on the closest adversarial examples (closest boundary points) with uniform weights. 
% Since MMA is the most related to \algoName, we report four hyperparamter settings. MMA-1 in $L_2$ setting uses MaxEps = $1$; MMA-2 in $L_2$ setting uses MaxEps = $2$; MMA-3 in $L_\infty$ setting uses MaxEps = $\frac{20}{255}$; MMA-4 in $L_\infty$ setting uses MaxEps = $\frac{32}{255}$; 
The MaxEps is set to $1$ in $L_2$ setting and $\frac{32}{255}$ in $L_\infty$ setting. 
(4) GAIRAT \footnote{\href{https://github.com/zjfheart/Geometry-aware-Instance-reweighted-Adversarial-Training}{GAIRAT's Github}} \citep{zhang2021geometryaware}  which reweights adversarial examples using the least perturbation steps. We only evaluate GAIRAT under $L_\infty$ setting since it does not have $L_2$ implementation in the codebase. The perturbation length is $\frac{8}{255}$ with step size $0.007$ using PGD-10 and the 'tanh' weight assignment function is used. 


\subsubsection*{Hyperparameters of \algoName} 

We use the ratio function with $g(0) = 1, g(r_0) = 0, g(r_1) = - g_1$ with $g_1 \geq 0 $ and linearly interpolate them when $0\leq r \leq r_1$. When $r>r_1$, $g(r)$ was set to the constant $-g_1$. If $g_1 > 0$, it means that \algoName pulls back the decision boundary towards $x_i$ if its robust radius $R(x_i)$ is larger than $r_1$. We allow $g$ to be negative when $r > r_1$ since we experimentally find that this could help improve both the clean accuracy and robust accuracy under small perturbation lengths in some settings. This is because it helps reduce the variance of the robust radius distribution by eliminating robust radii that are unnecessarily large. When $g(R(x_i)) < 0 $, the weight $c_i$ is constrained to be non-positive since the decision boundary at $\hat{x}_i$ needs to be pulled back. In particular, we solve the following modified version of the optimization problem~\eqref{eq:opt_for_weight}:

\begin{equation} \label{eq:opt_for_weight_negative}
\begin{aligned}
\min_{\mathbf{c}, \mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} |c_i| = 1, \quad c_i g(R(x_i))\geq0, \quad \mu \geq 0    \\
\end{aligned}
\end{equation}

The optimization problem~\eqref{eq:opt_for_weight_negative} above is still a quadratic programming problem with the same objective function as the original problem~\eqref{eq:opt_for_weight}, whose details are given in Appendix~\ref{app: opt_for_weight}. The only difference is in the constraints, where  problem~\eqref{eq:opt_for_weight_negative} requires the weight to be non-positive if its $g$ value is negative, and the absolute values of the weights sum up to one. 

To achieve the best robust accuracy under $\epsilon = 0.5$ in the $L_2$ setting, we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = 0.4$. To achieve the best robust accuracy under $\epsilon = \frac{8}{255}$ in the $L_\infty$ setting, we set $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = 0.4$. We use FAB with 15 iterations to approximate the closest boundary points in both $L_2$ and $L_\infty$ setting. 


\subsection{Further experimental results}\label{app: further_exp_results}

\paragraph{Comparing with baselines} We first present results where the hyperparameters of $\algoName$ are chosen to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. That is , we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = 0.4$ in $L_2$ setting and  $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = 0.4$ in  $L_\infty$ setting. The results are given in Table~\ref{table: performance_L2_more_eps_app} and Table~\ref{table: performance_Linf_more_eps_app}. In the $L_2$ case, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. In the $L_\infty$ case, \algoName obtains both higher clean accuracy and robust accuracy than AT, MMA and GAIRAT. We observe that the robust accuracy under AA is much lower than PGD for GAIRAT and MMA, which may be due to obfuscated gradient \citep{AthalyeC018}. On the other hand, the performance gap between PGD and AA is relatively small for \algoName. When compared with TRADES, \algoName shows higher clean accuracy and comparable robust accuracy under larger $\epsilon$, although \algoName has lower robust accuracy when $\epsilon = \frac{8}{255}$. This is partially due to the higher difficulty of approximating the closest boundary points in the $L_\infty$ case, and a better algorithm for this is left for future work. 


\input{\texhome/appendix_experiments/tab_L2_moreEps}
\input{\texhome/appendix_experiments/tab_Linf_moreEps}

\paragraph{Effect of ratio function and clean loss coefficient} We study the effect of hyperparameters $r_0, r_1, g_1$ of the ratio function $g$, as well as the clean loss coefficient $\lambda_c$ in the loss function $
	L_\theta(\mathcal{B}) =  -\sum\nolimits_{i\in \mathcal{B}^{+}_\theta}c_i \phi^{y_i}(\hat{x}_i) + \lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}l(x_i,y_i) 
	$. We only show the robust accuracy results against AA since it gives a more accurate estimation of the robustness. The results are shown in Table~\ref{table: performance_L2_ours_ablation} and Table~\ref{table: performance_Linf_ours_ablation}, where several observations can be made. Firstly, we observe that when the ratio function $g$ is fixed, a smaller $\lambda_c$ tends to result in better robustness performance against all perturbation thresholds, though the clean accuracy is lower. This indicates a trade-off between the robust and clean accuracy. Secondly, when $\lambda_c$ is fixed, a flatter ratio function $g$ (with larger $r_0$) will result in higher robust accuracy under larger perturbation lengths,  but could hurt the robust accuracy under smaller perturbation lengths. Thirdly, using a positive $g_1$ when $r_0$ is relatively large (such as $2$ in $L_2$ case and $\frac{32}{255}$ in $L_\infty$ case) could improve the robust accuracy under smaller perturbation lengths (such as $0.5$ in $L_2$ case and $\frac{8}{255}$ in $L_\infty$ case) but decrease the robust accuracy under larger perturbation lengths. In this case, \algoName controls the decision boundary so that if it is very far from the natural data, it will move closer. This helps reduce the variance of the robust radius distribution, decrease the proportion of unnecessarily robust points and thus improve the robust accuracy under small perturbation thresholds. 

\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-1em}
    \centering
    \begin{subfigure}[b]{0.26\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\texhome/experiment_fig/ratio_function}}
        \vspace{-1.5em}
        \caption{Ratio function}
        \label{sfig: performance_ratio_function}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\texhome/experiment_fig/radius_distribution}}
        \vspace{-1.5em}
        \caption{radius distribution}
        \label{sfig: performance_radius_distribution}
    \end{subfigure}
    \vspace{-0.3em}
    \caption{Different choices of the ratio function $g$ and the corresponding radius distributions when using \algoName.
    }
\vspace{-1.2em}
\end{wrapfigure}

\textbf{Ratio function controls the robust radius distribution}\quad 
Instead of using a pre-defined perturbation length to control the robustness level, \algoName uses all of the closest boundary points, 
% with respect to all correctly classified data points during training
including those that are relatively far from the original ones. The ratio function $g$ controls the robustness level: if $g$ decays more slowly, \algoName will encourage robustness improvement even when the robust radius is large, and thus the model is robust to larger perturbation thresholds. On the other hand, if $g$ decays fast, the improvement on the non-robust points will be encouraged more. To verify this, we fix $\lambda_c = 2$ in the $L_2$ norm setting and train on $g(r) = 1 - r/k$ when $r\leq k$ and $g(r)=0$ otherwise, for different $k$'s as shown in Figure~\ref{sfig: performance_ratio_function}. For these trained models, we use FAB (with 40 iterations) to compute the robust radius distributions for the correctly classified points from the test set,
% We discard the low-quality boundary points that do not satisfy the optimality condition of equation $\eqref{eq: closest_pt}$. 
which are shown in Figure~\ref{sfig: performance_radius_distribution}.
We can see that when $g$ decays slower, the robust radius distribution within correctly classified points spreads out more and tends to be more robust. Note that the overall robust accuracy is the product of the robust accuracy within correct points and the clean accuracy. We find that although a flatter $g$ leads to better robust accuracy within correct points, it decreases the clean accuracy. This shows that improving the robustness of points with large robust radii could harm the clean accuracy. Therefore, there is a trade-off between the robustness and clean accuracy, which is balanced by $\lambda_c$ and the choice of $g$.





\input{\texhome/appendix_experiments/tab_L2_ours_ablation}
\input{\texhome/appendix_experiments/tab_Linf_ours_ablation}


==> A_continuous_workshop/a4_more_dynamics.tex <==
\newpage
\section{Further results of dynamics} \label{app: more_dynamics}
In this section, we present more visualizations and further analysis of the dynamics of the decision boundary during the training process. 

\subsection{Dynamics and robustness improvement}
In this section, we demonstrate a strong correlation between the speed of the decision boundary and the improvement of robust accuracy over time. 

\textbf{Experiment setting}\quad We train a ResNet-18 \citep{he2016deep} on CIFAR-10 using 10-step PGD under $L_2$ perturbation with $\epsilon=0.5$ from a naturally pretrained model and evaluate it using 20-step PGD.
Figure~\ref{fig: interpretation_acc} shows the test clean and robust accuracy, as well as the \textit{robust accuracy within correct points}: the proportion of robust data points within correctly classified ones, which is computed by the ratio between the robust accuracy and clean accuracy.
We consider the robust accuracy within correct points since the speed is only defined for correctly classified ones.
We will experimentally examine the correlation between the robust accuracy within correct points and the dynamic speed of the decision boundary.

\input{\texhome/fig_interpret_test}

\textbf{Dynamics and robustness improvement}\quad We choose 512 points from the test set and at each iteration, we compute the robust radii and speed for correctly classified points. We omit those points whose radii are larger than $1$, which are considered very robust under $\epsilon=0.5$. 
For every iteration, we normalize the speed values to have the maximum absolute value 1 for better visualization of their relative magnitude.
The result is shown in Figure~\ref{fig: interpretation_VR_test_scatter}.
The set of points 
$\mathcal{S}_{\mathsf{g}} = \{x_i: R(x_i)<0.5, s(x_i)>0\}$
(top left corner) can be viewed as vulnerable but are being improved, whereas points in
$\mathcal{S}_{\mathsf{b}} = \{x_i: 0.5<R(x_i)<1, s(x_i)<0\}$
(bottom right corner) can be considered as robust but are being compromised. Observe that at the start of training (e.g. iteration 5 and 30), the proportion  of $\mathcal{S}_{\mathsf{g}}$, denoted as $p(\mathcal{S}_{\mathsf{g}})$, is relatively large and $p(\mathcal{S}_{\mathsf{b}})$ is relatively small. At the same time, the robust accuracy within correct points increases drastically, as shown in figure \ref{fig: interpretation_acc}. At the later stage (e.g. iteration 200), $p(\mathcal{S}_{\mathsf{g}})$ decreases and $p(\mathcal{S}_{\mathsf{b}})$ increases, and the robustness improvement slows down. In order to capture the robustness improvement using dynamics, we compute $p(\mathcal{S}_{\mathsf{g}}) - p(\mathcal{S}_{\mathsf{b}})$ which is shown in Figure~\ref{fig: interpretation_acc_d}, along with the time derivative of the robust accuracy within correct points. We observe that both of them show the same pattern, indicating the strong correlation between the dynamics of the decision boundary and the robustness improvement during AT.

\subsection{Further analysis of dynamics}
In this section, we present the un-normalized speed (raw speed values) in Figure~\ref{fig: AT_speed_time_app_all}, where the 20\% quantile, median and 80\% quantile of the speed distribution at each iteration are shown. We observe that at the start of the training (first 100 iterations) where the robust accuracy improves drastically, the speed distribution is mostly positive. Later,  when the robustness improvement slows down, the speed distribution is centered around zero. Also, notice that the variance of the speed distribution is never vanishing: the decision boundary always moves towards some data points while moving away from others. This indicates that adversarial training methods do not converge, since the decision boundary does not stop moving. Despite the constant movement of the decision boundary, the average adversarial loss does converge. Therefore, the dynamics of the decision boundary w.r.t. each data point provides more information than an average of the surrogate loss. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/VR_AT_acc}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: AT_acc_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/AT_test_speed_time}}
        \caption{\scriptsize{Speed distribution and iterations}}
        \label{fig: AT_speed_time_app}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during AT. In Figure~\ref{fig: AT_speed_time_app}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. }
    \label{fig: AT_speed_time_app_all}
    %\vspace{-1em}
\end{figure}


\paragraph{Natural training}
To compare with the non-converging behaviour of adversarial training methods, we present the dynamics during natural training in Figure~\ref{fig: clean_speed_time_app_all}, where the robust accuracy stays at zero. This can be viewed as the final stage of the natural training since the clean accuracy does not increase significantly anymore. We observe that the speed distribution of the decision boundary is effectively zero. This indicates that natural training does converge in the following sense: the clean accuracy does not change and moreover, the decision boundary around every correctly classified point does not move anymore. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/clean_acc}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: clean_acc_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/clean_test_speed_time}}
        \caption{\scriptsize{Speed distribution and iterations}}
        \label{fig: clean_speed_time_app}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during natural training. In Figure~\ref{fig: clean_speed_time_app}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. Observe that the speed is almost zero during natural training, indicating that natural training eventually does not move the decision boundary around correctly classified points.}
    \label{fig: clean_speed_time_app_all}
    %\vspace{-1em}
\end{figure}

\subsection{Dynamics in the \texorpdfstring{$L_\infty$}{} setting }

Here we present the visualization of the speed in the $L_\infty$ setting. We use FAB with 60 iterations and only choose the closest boundary points with high quality according to Appendix~\ref{app: optimality}. We use AT with $\epsilon = \frac{8}{255}$ and \algoName with $r_0=\frac{32}{255}, g_1 = 0, \lambda_c = 1$. The speed-radius distribution on the training batches of three chosen iterations for both methods are shown in Figure~\ref{fig: AT_linf_VR_trainBatch_app} and Figure~\ref{fig: ours_linf_VR_trainBatch_app}. We can draw a similar conclusion as in the $L_2$ case: conflicting dynamics of the decision boundary exists for AT during training, since there is a significant proportion of vulnerable points (with $R(x_i) \leq \frac{8}{255}$) with negative speed values. On the other hand, \algoName can alleviate this conflict and encourage robustness improvement on more vulnerable points by assigning larger speed values to them. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/AT_batch_Linf_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
        \label{fig: AT_linf_VR_trainBatch_scatter_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/AT_batch_Linf_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: AT_linf_VR_trainBatch_hist_app}
    \end{subfigure}%
    \caption{Radius-speed plot of AT on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations in $L_\infty$ setting. Proportion of points with negative speed for these iterations are 31\%, 45\% and 46\% respectively.}
    \label{fig: AT_linf_VR_trainBatch_app}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/ours_batch_Linf_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of \algoName on the training batch}}
        \label{fig: ours_linf_VR_trainBatch_scatter_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/ours_batch_Linf_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: ours_linf_VR_trainBatch_hist_app}
    \end{subfigure}%
    \caption{Radius-speed plot of \algoName on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations in $L_\infty$ setting. Proportion of points with negative speed for these iterations are below 3\%.}
    \label{fig: ours_linf_VR_trainBatch_app}
\end{figure}

==> A_continuous_workshop/a5_related_work.tex <==
\section{More related Work}\label{sec:related_work_app}

\textbf{Controlling parameterized surface}\quad 
The decision boundary can be viewed as a parameterized surface in the input space. Controlling such surface has been studied in image segmentation\citep{li2011level,aghasi2011parametric} and shape modelling\citep{chen2019learning,park2019deepsdf}. As for adversarial training, the authors of \citep{Atzmon2019control} propose to maximize the distance between each data point and some point on the decision boundary, which is not the closest one. On the other hand, we study the movement of the decision boundary w.r.t. each data point by analyzing its closest boundary point, which is directly related to the 
robust radius. 

\textbf{Comparisons with related adversarial training methods}\quad 
There are several defense techniques including gradient regularization \citep{moosavi2019robustness,tramer2017ensemble}, certified denfense\citep{cohen2019certified,wong2018provable,balunovic2019adversarial} and adversarial training \citep{madry2017towards,zhang2019theoretically,gowal2020uncovering,wang2019improving,zhang2020attacks}, where the last one is the most related to this work. 
In particular, MMA\citep{Ding2020MMA} trains on the closest boundary points, which is similar to \algoName. However, MMA adopts uniform weights and thus does not consider the vulnerability difference among the points. On the other hand, weighted adversarial training methods \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware} assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. 

==> A_continuous_workshop/algo.tex <==
%%% wrapping algorithm inside a figure environment, so that we can adjust the spacing around it using \vspace{}

\begin{figure}[!htbp]
\vspace{-1em}
\centering
\begin{algorithm}[H] 
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{\algoNameFull (\algoName)}
\label{alg: main algo}
\begin{algorithmic}[1]
% \hspace*{\algorithmicindent} \textbf{Input:} 
\REQUIRE The training data set, ratio function $g$, norm type $p$, clean loss strength $\lambda_c$, number of epochs $T$ and number of batches $M$. $\mathcal{A}(x,y)$ denotes the approximate closest boundary point returned by an algorithm $\mathcal{A}$ (e.g. FAB) on the correctly classified data point $(x,y)$.  
% \hspace*{\algorithmicindent} \textbf{Output:} 
\ENSURE adversarially robust network $f_\theta$
\FOR{epoch = $1,\cdots,T$}
    \FOR{mini-batch = $1,\cdots,M$}
        \STATE Sample a mini-batch $\mathcal{B} = \{(x_i,y_i\}_{i=1}^{n}$
        \STATE Make predictions on $\mathcal{B}$ and find correctly classified points $\mathcal{B}_{\theta}^{+}$
        \FOR{$(x_i,y_i)\in \mathcal{B}_{\theta}^{+}$ (in parallel)}
            \STATE Find the approximate closest boundary point $\hat{x}_i = \mathcal{A}(x_i,y_i)$ as in \eqref{eq: closest_pt}
            \STATE Compute the robust radius $R(x_i) = \|\hat{x}_i - x_i\|_p$
            \STATE Calculate the ratio value $g(R(x_i))$
        \ENDFOR
        \STATE Solve the optimization problem \eqref{eq:opt_for_weight} for weights $c_i$ for $i \in \mathcal{B}_{\theta}^{+}$ 
        \STATE Update $\theta$ using the loss function $
	L_\theta(\mathcal{B}) =  -\sum\nolimits_{i\in \mathcal{B}^{+}_\theta}c_i \phi^{y_i}(\hat{x}_i) + \lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}l(x_i,y_i) 
	$
        % $\theta \gets \theta - \eta(\sum_{i\in B_1^{\text{adv}}}c_i\nabla_\theta l(\hat{x}_i,y_i)  + \lambda_c\sum_{i\in B}\frac{1}{N}\nabla_\theta l(x_i,y_i))$
    \ENDFOR
\ENDFOR

% \Function{ComputeWeight}{$x,y$} \Comment{{\small{return the summation of two variables}}}
%   \STATE $z = x + y$
%   \STATE \textbf{Return} $z$ 
% \EndFunction
\end{algorithmic}
\end{algorithm}
\vspace{-1em}
\end{figure}




==> A_continuous_workshop/experiment_fig/Our_batch_hist.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 100}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0930522158741951) rectangle (axis cs:0.130964314592326,0.0101324841380119);
\draw[draw=none,fill=color0] (axis cs:0,0.0101324841380119) rectangle (axis cs:0.523857258369306,0.113317184150219);
\draw[draw=none,fill=color0] (axis cs:0,0.1133171916008) rectangle (axis cs:0.654821525679423,0.216501891613007);
\draw[draw=none,fill=color0] (axis cs:0,0.216501891613007) rectangle (axis cs:0.785785887553959,0.319686591625214);
\draw[draw=none,fill=color0] (axis cs:0,0.319686591625214) rectangle (axis cs:1.83350040429257,0.422871291637421);
\draw[draw=none,fill=color0] (axis cs:0,0.422871291637421) rectangle (axis cs:1.44060746051559,0.526055991649628);
\draw[draw=none,fill=color0] (axis cs:0,0.526055991649628) rectangle (axis cs:0.654821572961632,0.629240691661835);
\draw[draw=none,fill=color0] (axis cs:0,0.629240691661835) rectangle (axis cs:1.17867883133094,0.732425391674042);
\draw[draw=none,fill=color0] (axis cs:0,0.732425391674042) rectangle (axis cs:1.30964314592326,0.835610091686249);
\draw[draw=none,fill=color0] (axis cs:0,0.835610091686249) rectangle (axis cs:1.17867883133094,0.938794791698456);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 500}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0894175097346306) rectangle (axis cs:0.325926569166786,0.0128550156950951);
\draw[draw=none,fill=color0] (axis cs:0,0.0128550156950951) rectangle (axis cs:0.325926569166786,0.115127541124821);
\draw[draw=none,fill=color0] (axis cs:0,0.11512752622366) rectangle (axis cs:1.19506408694488,0.217400044202805);
\draw[draw=none,fill=color0] (axis cs:0,0.217400074005127) rectangle (axis cs:1.52099065611167,0.319672584533691);
\draw[draw=none,fill=color0] (axis cs:0,0.319672584533691) rectangle (axis cs:2.49877072768424,0.421945095062256);
\draw[draw=none,fill=color0] (axis cs:0,0.421945095062256) rectangle (axis cs:1.73827528882382,0.52421760559082);
\draw[draw=none,fill=color0] (axis cs:0,0.52421760559082) rectangle (axis cs:1.08642205551489,0.626490116119385);
\draw[draw=none,fill=color0] (axis cs:0,0.626490116119385) rectangle (axis cs:0.760494995642261,0.728762686252594);
\draw[draw=none,fill=color0] (axis cs:0,0.728762686252594) rectangle (axis cs:0.108642205551489,0.831035196781158);
\draw[draw=none,fill=color0] (axis cs:0,0.831035196781158) rectangle (axis cs:0.217284411102978,0.933307707309723);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 1000}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0245624426752329) rectangle (axis cs:0.373517160888316,0.0699288472533226);
\draw[draw=none,fill=color0] (axis cs:0,0.069928839802742) rectangle (axis cs:0.87153997335234,0.164420127868652);
\draw[draw=none,fill=color0] (axis cs:0,0.164420127868652) rectangle (axis cs:1.24505720296105,0.258911430835724);
\draw[draw=none,fill=color0] (axis cs:0,0.258911430835724) rectangle (axis cs:1.6185741086022,0.353402733802795);
\draw[draw=none,fill=color0] (axis cs:0,0.353402733802795) rectangle (axis cs:1.12055130595537,0.447894036769867);
\draw[draw=none,fill=color0] (axis cs:0,0.447894036769867) rectangle (axis cs:1.49406840794049,0.542385339736938);
\draw[draw=none,fill=color0] (axis cs:0,0.542385339736938) rectangle (axis cs:1.86758668799003,0.636876583099365);
\draw[draw=none,fill=color0] (axis cs:0,0.636876583099365) rectangle (axis cs:0.747034203970246,0.731367886066437);
\draw[draw=none,fill=color0] (axis cs:0,0.731367945671082) rectangle (axis cs:0.622528503308539,0.825859248638153);
\draw[draw=none,fill=color0] (axis cs:0,0.825859189033508) rectangle (axis cs:0.622528503308539,0.92035049200058);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\end{groupplot}

\draw ({$(current bounding box.south west)!-0.01!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\LARGE{Speed}};
\end{tikzpicture}


==> A_continuous_workshop/experiment_fig/Our_batch_scatter.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 100}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.139259457588196 0.87974089384079
0.421387225389481 0.505936861038208
0.497758567333221 0.281495809555054
0.192086070775986 0.694953858852386
0.976208627223969 0.0887730941176414
0.553409993648529 0.440094947814941
0.439580053091049 0.442619472742081
0.968777179718018 0.246498510241508
0.879478633403778 0.321859002113342
0.927507281303406 0.132060289382935
0.725531160831451 0.677463829517365
0.250144422054291 0.624903559684753
0.282028943300247 0.938794791698456
0.392061352729797 0.590279817581177
0.226367816329002 0.709937810897827
0.253683537244797 0.509217083454132
0.264158725738525 0.527510821819305
0.143192574381828 0.847660481929779
0.0656776130199432 0.856230556964874
0.512509167194366 0.468835383653641
0.452651411294937 0.452691107988358
0.96679413318634 -0.0930522158741951
0.457594335079193 0.362852275371552
0.818558394908905 0.210012018680573
0.0865476429462433 0.760084748268127
0.92186176776886 0.419143319129944
0.229736253619194 0.822469353675842
0.454779326915741 0.55412769317627
0.569496870040894 0.675950586795807
0.605530679225922 0.753823578357697
0.756329953670502 0.356041789054871
0.449440777301788 0.525765717029572
0.401755213737488 0.489267826080322
0.729974925518036 0.641091227531433
0.864565491676331 0.158966660499573
0.569140493869781 0.492613941431046
0.195144489407539 0.906790733337402
0.607923448085785 0.39532533288002
0.704999208450317 0.15942719578743
0.83390611410141 0.280181169509888
0.655198633670807 0.403607189655304
0.58749520778656 0.285376042127609
0.645855844020844 0.349601417779922
0.147765323519707 0.784916758537292
0.640424787998199 0.415896952152252
0.516849458217621 0.365468591451645
0.552274227142334 0.3888900578022
0.628182530403137 0.356706947088242
0.450512319803238 0.634923756122589
0.660074591636658 0.393710017204285
0.116237349808216 0.841611802577972
0.560958743095398 0.501353740692139
0.950110077857971 0.0379549711942673
0.189407855272293 0.777242183685303
0.17595100402832 0.903630018234253
0.808530151844025 0.284991264343262
0.142146334052086 0.782856583595276
0.755055904388428 0.250042021274567
0.383216202259064 0.92495208978653
0.0799809321761131 0.819203019142151
0.261886149644852 0.78420078754425
0.554071724414825 0.41170459985733
0.932360053062439 0.0142253050580621
0.0659285113215446 0.894612729549408
0.150298565626144 0.690214574337006
0.263341963291168 0.644734263420105
0.123858392238617 0.710014164447784
0.447123974561691 0.581269323825836
0.839296758174896 0.0896879211068153
0.46270939707756 0.211884632706642
0.185274988412857 0.767150223255157
0.398056268692017 0.772571265697479
0.542429447174072 0.403975188732147
0.61186957359314 0.46583878993988
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 500}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.776936888694763 0.249753534793854
0.386116743087769 0.406365096569061
0.174472793936729 0.521653413772583
0.805141091346741 0.933307707309723
0.440240800380707 0.551619172096252
0.591361165046692 0.133534938097
0.455250889062881 0.401996105909348
0.332143425941467 0.372915893793106
0.467637568712234 0.814061284065247
0.724299252033234 0.130848690867424
0.158043280243874 0.647002637386322
0.566194474697113 0.347332745790482
0.473153501749039 0.482004195451736
0.267547637224197 0.527089238166809
0.71589583158493 0.430038511753082
0.658745765686035 0.457427114248276
0.144467324018478 0.657042145729065
0.422516047954559 0.367061853408813
0.78759354352951 0.379683077335358
0.370047807693481 0.349326610565186
0.131544753909111 0.42074191570282
0.590262830257416 0.158686131238937
0.888246536254883 0.231273204088211
0.985404491424561 0.173878386616707
0.404500156641006 0.519400238990784
0.335165202617645 0.72149384021759
0.23070877790451 0.558023869991302
0.436972916126251 0.331318795681
0.644021034240723 0.0856519564986229
0.630360901355743 0.435541301965714
0.447283953428268 0.239694103598595
0.180275335907936 0.505020081996918
0.510656476020813 0.335002541542053
0.405353397130966 0.287605851888657
0.464257538318634 0.453973650932312
0.303507149219513 0.453528463840485
0.311053872108459 0.504680037498474
0.690726935863495 0.261621564626694
0.170168474316597 0.674301147460938
0.388627707958221 0.569280743598938
0.561706483364105 0.616437673568726
0.448287129402161 0.329984992742538
0.162112429738045 0.625538289546967
0.247905418276787 0.34765100479126
0.495826065540314 0.558913290500641
0.703568994998932 0.673902451992035
0.25944322347641 0.407854646444321
0.677498459815979 0.390358507633209
0.402255445718765 0.240773573517799
0.329665958881378 0.497239798307419
0.689209342002869 0.216121166944504
0.936314046382904 0.426470637321472
0.0554389469325542 0.885870456695557
0.63409698009491 0.330398440361023
0.935300230979919 0.17045946419239
0.35245755314827 0.348024547100067
0.23744623363018 0.559127688407898
0.323607683181763 0.559788584709167
0.0888271629810333 0.495435357093811
0.127962559461594 0.374380618333817
0.468316853046417 0.234871447086334
0.158229857683182 0.637133896350861
0.716919124126434 0.129116103053093
0.144968807697296 0.523131608963013
0.849043250083923 0.0959296450018883
0.975417494773865 0.011977213434875
0.0905567705631256 0.728091776371002
0.403979033231735 0.260361164808273
0.202995106577873 0.577884078025818
0.182661727070808 0.340855956077576
0.98902815580368 0.225347593426704
0.693903625011444 0.238435164093971
0.587247252464294 0.324716359376907
0.190335050225258 0.475275486707687
0.786740481853485 0.152153328061104
0.426211625337601 0.371549278497696
0.177270129323006 0.292735397815704
0.736927688121796 0.246110171079636
0.446727216243744 0.363649725914001
0.449692755937576 0.485296905040741
0.345438122749329 0.340099722146988
0.8830726146698 0.00464663049206138
0.56570303440094 0.28088241815567
0.805004954338074 0.189938649535179
0.262816816568375 0.33413490653038
0.717803835868835 0.107261158525944
0.864565908908844 0.293800443410873
0.878847897052765 -0.0894175097346306
0.606184422969818 0.199088245630264
0.59554123878479 0.170070052146912
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 1000}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.57584023475647 0.338832080364227
0.225332260131836 0.623566269874573
0.968862056732178 0.346817523241043
0.311254441738129 0.513589560985565
0.568746745586395 0.515619337558746
0.366963326931 0.513030588626862
0.41833233833313 0.463166058063507
0.556143522262573 0.361476302146912
0.529341161251068 0.54360020160675
0.205069601535797 0.647709488868713
0.908150136470795 0.0687245801091194
0.710321962833405 0.378976941108704
0.898783683776855 0.167049989104271
0.161436930298805 0.74740469455719
0.479314923286438 0.819670855998993
0.0888834595680237 0.627499997615814
0.309117376804352 0.631774067878723
0.302228063344955 0.392113834619522
0.614017605781555 0.154380187392235
0.695720970630646 0.465875148773193
0.75020694732666 0.134846374392509
0.874695301055908 0.0960765555500984
0.498199701309204 0.408374339342117
0.710412740707397 0.193369522690773
0.336726933717728 0.338454991579056
0.538124024868011 0.0865073874592781
0.0881228446960449 0.633062362670898
0.771107912063599 0.309533357620239
0.369485050439835 0.374647527933121
0.319801241159439 0.614099442958832
0.744711935520172 0.0975610539317131
0.19185908138752 0.430443435907364
0.269707530736923 0.774192214012146
0.131259053945541 0.855269432067871
0.491700023412704 0.629065930843353
0.671019077301025 0.30482617020607
0.420025080442429 0.478932470083237
0.585492372512817 0.299596399068832
0.361166208982468 0.542346000671387
0.859290421009064 0.120165780186653
0.346621990203857 0.14356492459774
0.131627649068832 0.92035049200058
0.115172833204269 0.535668432712555
0.199532762169838 0.629831790924072
0.200127780437469 0.605798184871674
0.589739680290222 0.321029216051102
0.73112541437149 0.253543674945831
0.598318040370941 0.211257830262184
0.280894696712494 0.91473114490509
0.713802218437195 0.280924409627914
0.347708225250244 0.593869745731354
0.965838074684143 0.537938714027405
0.383636444807053 0.447239965200424
0.935863971710205 0.203516334295273
0.14890643954277 0.680480480194092
0.0562681667506695 0.802294194698334
0.749043345451355 0.179575711488724
0.423711746931076 0.486505329608917
0.844658136367798 0.166071742773056
0.661024570465088 0.563995838165283
0.54025536775589 0.434267282485962
0.565700888633728 0.227442294359207
0.520568788051605 0.592914402484894
0.131979018449783 0.673773288726807
0.876122951507568 0.00479763699695468
0.535711050033569 0.318562299013138
0.345073401927948 0.585593223571777
0.226624682545662 0.70534759759903
0.560894787311554 0.332505911588669
0.278737008571625 0.508535087108612
0.486066699028015 0.266474425792694
0.970355808734894 -0.0245624426752329
0.276687234640121 0.543783009052277
0.643745064735413 0.479749530553818
0.661679565906525 0.178459644317627
0.28415521979332 0.55865490436554
0.292061328887939 0.422659397125244
0.562201738357544 0.833523273468018
0.294146001338959 0.838525772094727
0.0868585333228111 0.749682188034058
0.510356962680817 0.273927867412567
0.669389963150024 0.297383904457092
0.678594410419464 0.222954750061035
0.17401809990406 0.670224070549011
0.25044584274292 0.683681547641754
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!-0.02!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=0.0
]{\LARGE{Radius}};
\draw ({$(current bounding box.south west)!-0.01!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\LARGE{Speed}};
\end{tikzpicture}


==> A_continuous_workshop/experiment_fig/radius_distribution.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, font=\large},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\Large{radius}},
xmin=0, xmax=5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=0.906499451926922,
ytick style={color=black}
]
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.00012119859457016,0) rectangle (axis cs:0.144508928060532,0.411766890524049);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.5}
\addlegendentry{k=1}

\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.14450891315937,0) rectangle (axis cs:0.28889662027359,0.545705991157668);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.28889662027359,0) rectangle (axis cs:0.433284342288971,0.678114247219903);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.433284342288971,0) rectangle (axis cs:0.577672064304352,0.792153776379909);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.577672064304352,0) rectangle (axis cs:0.722059786319733,0.848025492008637);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.722059786319733,0) rectangle (axis cs:0.866447508335114,0.863332811358974);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.866447448730469,0) rectangle (axis cs:1.01083517074585,0.80286923135731);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.01083517074585,0) rectangle (axis cs:1.15522289276123,0.677348881252386);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.15522289276123,0) rectangle (axis cs:1.29961061477661,0.492130317113316);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.29961061477661,0) rectangle (axis cs:1.44399833679199,0.347476149252637);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.44399833679199,0) rectangle (axis cs:1.58838605880737,0.222721496547395);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.58838605880737,0) rectangle (axis cs:1.73277378082275,0.114039529160006);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.73277378082275,0) rectangle (axis cs:1.87716150283813,0.0711790349790643);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.87716150283813,0) rectangle (axis cs:2.02154922485352,0.0336761025707401);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.02154922485352,0) rectangle (axis cs:2.1659369468689,0.0137765874153028);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.1659369468689,0) rectangle (axis cs:2.31032466888428,0.00612292774013456);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.31032466888428,0) rectangle (axis cs:2.45471239089966,0.00306146387006728);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.45471239089966,0) rectangle (axis cs:2.59910011291504,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.59910011291504,0) rectangle (axis cs:2.74348783493042,0.000765365967516821);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.74348783493042,0) rectangle (axis cs:2.8878755569458,0.00153073193503364);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.000629313290119171,0) rectangle (axis cs:0.20014876127243,0.432014092923934);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,fill opacity=0.5}
\addlegendentry{k=2}

\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.200148746371269,0) rectangle (axis cs:0.399668157100677,0.495429042647959);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.399668216705322,0) rectangle (axis cs:0.599187612533569,0.536761979920304);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.599187612533569,0) rectangle (axis cs:0.798707067966461,0.541291536028653);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.798707127571106,0) rectangle (axis cs:0.998226583003998,0.557711467560902);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.998226523399353,0) rectangle (axis cs:1.1977459192276,0.537894469506224);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.19774580001831,0) rectangle (axis cs:1.39726531505585,0.44616904075973);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.39726543426514,0) rectangle (axis cs:1.59678483009338,0.392946065091915);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.59678483009338,0) rectangle (axis cs:1.79630422592163,0.330097342865398);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.79630422592163,0) rectangle (axis cs:1.99582374095917,0.250828534335736);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.99582386016846,0) rectangle (axis cs:2.19534301757812,0.186847664203475);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.19534301757812,0) rectangle (axis cs:2.39486265182495,0.127962110361838);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.39486265182495,0) rectangle (axis cs:2.5943820476532,0.0883279339399694);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.59438228607178,0) rectangle (axis cs:2.79390168190002,0.037369510513064);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.79390144348145,0) rectangle (axis cs:2.99342083930969,0.0232143928944791);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.99342107772827,0) rectangle (axis cs:3.19294047355652,0.015853731732815);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.19294023513794,0) rectangle (axis cs:3.39245963096619,0.00566204704743393);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.39245963096619,0) rectangle (axis cs:3.59197926521301,0.00283102014074863);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.59197950363159,0) rectangle (axis cs:3.79149889945984,0.00169861411423018);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.79149866104126,0) rectangle (axis cs:3.99101805686951,0.00113240940948679);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.000650271773338318,0) rectangle (axis cs:0.263168036937714,0.371470997289431);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,fill opacity=0.5}
\addlegendentry{k=3}

\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.263167977333069,0) rectangle (axis cs:0.525685787200928,0.460623984346566);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.525685787200928,0) rectangle (axis cs:0.788203477859497,0.476833788422071);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.788203477859497,0) rectangle (axis cs:1.05072128772736,0.44576509553637);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.05072128772736,0) rectangle (axis cs:1.31323897838593,0.450718245713403);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.31323885917664,0) rectangle (axis cs:1.57575666904449,0.396685908250042);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.57575678825378,0) rectangle (axis cs:1.83827447891235,0.303930884971575);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.83827447891235,0) rectangle (axis cs:2.10079216957092,0.247647387754617);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.10079193115234,0) rectangle (axis cs:2.36330962181091,0.213427021446706);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.36330986022949,0) rectangle (axis cs:2.62582778930664,0.157143381512121);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.62582778930664,0) rectangle (axis cs:2.88834547996521,0.10806431465656);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.88834524154663,0) rectangle (axis cs:3.1508629322052,0.075645020259592);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.15086317062378,0) rectangle (axis cs:3.41338086128235,0.0481786736177164);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.41338086128235,0) rectangle (axis cs:3.6758987903595,0.0220631108713293);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.67589855194092,0) rectangle (axis cs:3.93841624259949,0.01350803933207);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.93841648101807,0) rectangle (axis cs:4.20093441009521,0.0103561540824607);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.20093441009521,0) rectangle (axis cs:4.46345186233521,0.00405241548002493);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.46345186233521,0) rectangle (axis cs:4.72596979141235,0.00135080270640792);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.7259693145752,0) rectangle (axis cs:4.98848676681519,0.00135080516000831);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.98848724365234,0) rectangle (axis cs:5.25100517272949,0.00045026756880264);
\addplot [semithick, red, opacity=0.5, dashed, forget plot]
table {%
0.5 0
0.5 0.906499451926922
};
\end{axis}

\end{tikzpicture}


==> A_continuous_workshop/experiment_fig/ratio_function.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
% \tiny, \scriptsize, \small, \large, \Large, \LARGE, \huge, \Huge, \HUGE
\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, font=\large},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\Large{radius}},
xmin=-0.260499999765307, xmax=5.25049999998882,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\Large{$g$}},
ymin=-0.0504999995231628, ymax=1.06049998998642,
% ymin=0, ymax=1.06049998998642,
ytick style={color=black}
]
\addplot [line width=3pt, color0]
table {%
-0.00999999977648258 1.00999999046326
0.0406060665845871 0.959393918514252
0.0912121310830116 0.908787846565247
0.141818180680275 0.858181834220886
0.19242425262928 0.807575762271881
0.243030324578285 0.756969690322876
0.293636381626129 0.706363618373871
0.344242453575134 0.655757546424866
0.394848525524139 0.605151474475861
0.445454597473145 0.554545402526855
0.49606066942215 0.50393933057785
0.546666741371155 0.453333258628845
0.597272753715515 0.402727246284485
0.647878885269165 0.352121114730835
0.698484897613525 0.301515102386475
0.749090969562531 0.250909030437469
0.799697041511536 0.200302958488464
0.850303113460541 0.149696886539459
0.900909185409546 0.0990908145904541
0.951515197753906 0.0484848022460938
1.00212132930756 0
1.05272734165192 0
1.10333347320557 0
1.15393948554993 0
1.20454549789429 0
1.25515151023865 0
1.3057576417923 0
1.35636365413666 0
1.40696978569031 0
1.45757579803467 0
1.50818181037903 0
1.55878794193268 0
1.60939407348633 0
1.66000008583069 0
1.71060621738434 0
1.7612122297287 0
1.81181836128235 0
1.86242437362671 0
1.91303038597107 0
1.96363651752472 0
2.01424264907837 0
2.06484866142273 0
2.11545467376709 0
2.16606092453003 0
2.21666693687439 0
2.26727294921875 0
2.31787896156311 0
2.36848497390747 0
2.41909098625183 0
2.46969699859619 0
2.52030301094055 0
2.57090926170349 0
2.62151527404785 0
2.67212128639221 0
2.72272729873657 0
2.77333354949951 0
2.82393932342529 0
2.87454533576965 0
2.92515134811401 0
2.97575759887695 0
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=1}
\addplot [line width=3pt, color1]
table {%
-0.00999999977648258 1.00499999523163
0.0406060665845871 0.979696989059448
0.0912121310830116 0.954393923282623
0.141818180680275 0.929090917110443
0.19242425262928 0.903787851333618
0.243030324578285 0.878484845161438
0.293636381626129 0.853181838989258
0.344242453575134 0.827878773212433
0.394848525524139 0.802575707435608
0.445454597473145 0.777272701263428
0.49606066942215 0.751969695091248
0.546666741371155 0.726666629314423
0.597272753715515 0.701363623142242
0.647878885269165 0.676060557365417
0.698484897613525 0.650757551193237
0.749090969562531 0.625454545021057
0.799697041511536 0.600151479244232
0.850303113460541 0.574848413467407
0.900909185409546 0.549545407295227
0.951515197753906 0.524242401123047
1.00212132930756 0.498939335346222
1.05272734165192 0.473636329174042
1.10333347320557 0.448333263397217
1.15393948554993 0.423030257225037
1.20454549789429 0.397727251052856
1.25515151023865 0.372424244880676
1.3057576417923 0.347121179103851
1.35636365413666 0.321818172931671
1.40696978569031 0.296515107154846
1.45757579803467 0.271212100982666
1.50818181037903 0.245909094810486
1.55878794193268 0.220606029033661
1.60939407348633 0.195302963256836
1.66000008583069 0.169999957084656
1.71060621738434 0.144696891307831
1.7612122297287 0.119393885135651
1.81181836128235 0.0940908193588257
1.86242437362671 0.0687878131866455
1.91303038597107 0.0434848070144653
1.96363651752472 0.0181817412376404
2.01424264907837 0
2.06484866142273 0
2.11545467376709 0
2.16606092453003 0
2.21666693687439 0
2.26727294921875 0
2.31787896156311 0
2.36848497390747 0
2.41909098625183 0
2.46969699859619 0
2.52030301094055 0
2.57090926170349 0
2.62151527404785 0
2.67212128639221 0
2.72272729873657 0
2.77333354949951 0
2.82393932342529 0
2.87454533576965 0
2.92515134811401 0
2.97575759887695 0
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=2}
\addplot [line width=3pt, color2]
table {%
-0.00999999977648258 1.00333333015442
0.0406060665845871 0.986464619636536
0.0912121310830116 0.969595968723297
0.141818180680275 0.952727258205414
0.19242425262928 0.935858607292175
0.243030324578285 0.918989896774292
0.293636381626129 0.902121186256409
0.344242453575134 0.88525253534317
0.394848525524139 0.868383824825287
0.445454597473145 0.851515114307404
0.49606066942215 0.834646463394165
0.546666741371155 0.817777752876282
0.597272753715515 0.800909101963043
0.647878885269165 0.78404039144516
0.698484897613525 0.767171680927277
0.749090969562531 0.750303030014038
0.799697041511536 0.733434319496155
0.850303113460541 0.716565608978271
0.900909185409546 0.699696898460388
0.951515197753906 0.682828307151794
1.00212132930756 0.665959596633911
1.05272734165192 0.649090886116028
1.10333347320557 0.632222175598145
1.15393948554993 0.615353465080261
1.20454549789429 0.598484873771667
1.25515151023865 0.581616163253784
1.3057576417923 0.564747452735901
1.35636365413666 0.547878742218018
1.40696978569031 0.531010031700134
1.45757579803467 0.514141440391541
1.50818181037903 0.497272729873657
1.55878794193268 0.480404019355774
1.60939407348633 0.463535308837891
1.66000008583069 0.446666657924652
1.71060621738434 0.429797947406769
1.7612122297287 0.412929236888885
1.81181836128235 0.396060526371002
1.86242437362671 0.379191875457764
1.91303038597107 0.362323224544525
1.96363651752472 0.345454514026642
2.01424264907837 0.328585803508759
2.06484866142273 0.311717092990875
2.11545467376709 0.294848442077637
2.16606092453003 0.277979671955109
2.21666693687439 0.26111102104187
2.26727294921875 0.244242370128632
2.31787896156311 0.227373659610748
2.36848497390747 0.21050500869751
2.41909098625183 0.193636357784271
2.46969699859619 0.176767647266388
2.52030301094055 0.159898996353149
2.57090926170349 0.143030226230621
2.62151527404785 0.126161575317383
2.67212128639221 0.109292924404144
2.72272729873657 0.092424213886261
2.77333354949951 0.0755555033683777
2.82393932342529 0.0586869120597839
2.87454533576965 0.0418182015419006
2.92515134811401 0.0249495506286621
2.97575759887695 0.00808078050613403
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=3}
\addplot [line width=3pt, red, opacity=0.5, forget plot]
table {%
-0.260499999765307 -2.77555756156289e-17
5.25049999998882 -2.77555756156289e-17
};
\addplot [line width=3pt, red, opacity=0.5, dashed, forget plot]
table {%
0.5 -0.0504999995231629
0.5 1.06049998998642
};
\end{axis}

\end{tikzpicture}


==> A_continuous_workshop/fig_intepret_train.tex <==
\begin{wrapfigure}{r}{0.43\textwidth}%[!t] % !htbp
\vspace{-1.8em}
    \resizebox{\linewidth}{!}{\input{\texhome/Intepretation_fig/AT_batch_scatter}}
    \vspace{-1.8em}
    % \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
    \caption{Radius-speed plot of AT on the training batches of three iterations. Proportions of points with negative speed  are $33.71\%$ at iteration 5, $34.29\%$ at iteration 30 and $39.87\%$ at iteration 200.}
    \label{fig: interpretation_VR_trainBatch_all}
    \vspace{-1.5em}
\end{wrapfigure}

==> A_continuous_workshop/fig_interpret_test.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.21\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/VR_AT_acc.tex}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: interpretation_acc}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.55\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/AT_test_scatter}}
        \caption{\scriptsize{Radius-speed plot of AT on the test data points}}
        \label{fig: interpretation_VR_test_scatter}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/VR_AT_approx_d}}
        \caption{\scriptsize{Robustness improvement 
        }}
        \label{fig: interpretation_acc_d}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Figure \ref{fig: interpretation_VR_test_scatter} shows the radius-speed plot on a fixed set of points in the test set for three iterations. Figure \ref{fig: interpretation_acc_d} shows the time derivative of the robust accuracy within correct points and its approximation using the dynamics statistics $p(\mathcal{S}_{\mathsf{g}}) - p(\mathcal{S}_{\mathsf{b}})$.}
    \label{fig: interpretation_VR_test_all}
    %\vspace{-1em}
\end{figure}

==> A_continuous_workshop/s0_abstract.tex <==
The adversarial robustness of a deep classifier can be measured by the \textit{robust radii}:
the decision boundary's distances to natural data points. 
However, it is unclear whether current adversarial training (AT) methods effectively improves the robust radius for each individual vulnerable point. To understand this, we propose a continuous-time framework that studies the relative speed of the decision boundary with respect to each individual point. 
Through visualizing the speed, a surprising conflicting moving-behavior is revealed: the decision boundary under AT moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones. To alleviate this \textit{conflicting dynamics} of the decision boundary, we propose \textit{\algoNameFull} (\algoName) which directly controls the decision boundary to move away from the training data points. Moreover, in order to further encourage the robustness improvement for more vulnerable points, \algoName controls the decision boundary to move faster away from points with smaller robust radii, achieving customized manipulation of the decision boundary. 
As a result, \algoName achieves fairer robustness to individuals, leading to better overall robustness under limited model capacity. 
Experiments verify that \algoName alleviates the conflicting dynamics and obtains improved robustness compared with the state-of-the-art defenses.





% for abstract submission

% The adversarial robustness of a deep classifier can be measured by the robust radii: the decision boundary's distances to natural data points. However, it is unclear whether current adversarial training (AT) methods effectively improves the robust radius for each individual vulnerable point. To understand this, we propose a continuous-time framework that studies the relative speed of the decision boundary with respect to each individual point. Through visualizing the speed, a surprising conflicting moving-behavior is revealed: the decision boundary under AT moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones. To alleviate this conflicting dynamics of the decision boundary, we propose Dynamical Customized Adversarial Training (Dyna-CAT) which directly controls the decision boundary to move away from the training data points. Moreover, in order to further encourage the robustness improvement for more vulnerable points, Dyna-CAT controls the decision boundary to move faster away from points with smaller robust radii, achieving customized manipulation of the decision boundary. As a result, Dyna-CAT achieves fairer robustness to individuals, leading to better overall robustness under limited model capacity. Experiments verify that Dyna-CAT alleviates the conflicting dynamics and obtains improved robustness compared with the state-of-the-art defenses.

==> A_continuous_workshop/s1_intro.tex <==
\section{Introduction}\label{sec:intro}

% Deep neural networks have been successfully deployed in a wide range of applications~\citep{krizhevsky2012imagenet,goodfellow2014generative,he2016deep,collobert2008unified}. 
% However, they have been shown to be susceptible to adversarial examples, leading to issues in security-critical applications such as autonomous driving and medicine~\citep{szegedy2013intriguing,nguyen2015deep}.  
% To alleviate this problem, adversarial training (AT)~\citep{madry2017towards,shafahi2019adversarial,zhang2019theoretically,gowal2020uncovering} was proposed and is one of the most prevalent methods against adversarial attacks. 
% Specifically, AT aims to find the worst-case adversarial examples based on some surrogate loss and adds them to the training dataset in order to improve robustness. 

\begin{wrapfigure}{r}{0.44\textwidth}%[!t]
\vspace{-3em}
    \centering
    % \begin{subfigure}[t]{0.3\textwidth}
    %     \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-1.pdf}
    %     \caption{The decision boundary, vulnerable points (solid) and robust points (hollow).}
    % \label{sfig:demo1}
    % \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.215\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-2.pdf}
        \caption{Conflicting dynamics} %moving-behavior of the decision boundary after one step of update.}
    \label{sfig:demo2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.215\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-3.pdf}
        \caption{Continuous movement} % of decision boundary.}
    \label{sfig:demo3}
    \end{subfigure}
    \vspace{-0.5em}
    \caption{The movement of the decision boundary. Red triangles and green circles are data points from two classes. %Figure~\ref{sfig:demo1} shows the vulnerability difference among the data points: some are closer to the decision boundary, whereas some are farther from it. 
    In Figure~\ref{sfig:demo2}, the decision boundary after an update 
    moves away from some vulnerable points (made more robust) but simultaneously moves closer to other vulnerable ones (made less robust), which is conflicting. 
    Figure~\ref{sfig:demo3} shows the corresponding continuous movement of the decision boundary.}
    \label{fig:demos}
     \vspace{-1.5em}
\end{wrapfigure}
Deep neural network classifiers are shown to be susceptible to adversarial perturbations \citep{szegedy2013intriguing}, which are human-imperceptible noise maliciously designed to fool the classifiers. Geometrically, there exists such adversarial perturbations since the robust radii, i.e. the distances between the decision boundary and natural data points, are too small. Adversarial training (AT) \cite{madry2017towards} is among the most successful defenses against adversarial perturbations. 
 % However, it has been shown that (even over-parameterized) neural networks, which can perfectly fit natural data in standard training~\citep{zhang2021understanding}, still have insufficient model capacity for fitting adversarial training data~\citep{zhang2021geometryaware}. 
% In order to carefully utilize the limited model capacity to fit the neighborhoods of more important data points,
% weighted adversarial training methods~\citep{zhang2021geometryaware, zeng2020adversarial,liu2021probabilistic} exploit the fact that data points have different vulnerability.  
% As shown in Figure~\ref{sfig:demo1}, some data points have smaller robustness radii, i.e., distances to the decision boundary, and are considered more vulnerable. 
% As shown in figure \yc{demo 1: static figure: only different RR}, some data has a smaller robust radius, i.e. its distance to the decision boundary, and is considered more vulnerable. 
% Therefore, weighted AT methods assign larger weights to adversarial examples whose natural counterparts have smaller robust radii estimated by the least perturbation steps \citep{zhang2021geometryaware} or the logit margin \citep{zeng2020adversarial,liu2021probabilistic}. 
% Despite up-weighting the surrogate loss on points with smaller robust radii, these weighted AT methods still do not directly increase the robust radii of each individual vulnerable point. 
% In addition, they only train on adversarial examples within an pre-defined universal perturbation threshold for all data points, which is likely sub-optimal due to the difference in vulnerability among points. 
% Therefore, it is unclear whether the learning algorithm is effectively improving the robust radius for each vulnerable point. 
% Geometrically, we are interested to know if the decision boundary moves away from the data points, especially the vulnerable ones. 
However, since AT does not directly increase the robust radius of each individual point, there can exist conflicting dynamics of the decision boundary as illustrated in Figure~\ref{sfig:demo2}:  it moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones during training. 
This motivates us to ask:



% In addition, they control the level of robustness by pre-defining the perturbation length $\epsilon$ and all of the points used for training are within $\epsilon$ distance from the original points, in regardless o
% However, this is sub-optimal because different points have different robustness and the model is unlikely to be robust to a more diverse attack budget.\yc{Some new sentences for varying $\epsilon$} 

\textbf{Question 1}\quad \textit{Given an training algorithm, how to analyze the dynamics of the decision boundary with respect to the data points?}\quad To answer this, we propose a continuous-time framework that studies the instantaneous movement of the decision boundary as shown in Figure~\ref{sfig:demo3}. Specifically, we define the relative speed of the decision boundary w.r.t. a point to be the time derivative of its robust radius, which can be interpreted as the speed of its closest adversarial example moving away from it. We show that the speed can be derived from the training algorithm using a closed-form expression. 
Using the proposed framework, we numerically compute the speed of the decision boundary w.r.t. data points for AT. As shown in Figure~\ref{fig: interpretation_VR_trainBatch_all},
We observe that a significant proportion of vulnerable points has negative speed, indicating the existence of the aforementioned conflicting dynamics (Figure~\ref{sfig:demo2},\ref{sfig:demo3}) of the decision boundary.
% across data points is a prevalent phenomenon, although it cannot be observed using averaged statistics such as robust accuracy or an average of a surrogate loss. 
On the other hand, a desirable dynamics should satisfy that the decision boundary moves away from the vulnerable points. Moreover, the speed should be larger for points with smaller robust radii to encourage the robustness improvement on vulnerable points. 
This leads to the question:
% This leads to another question:

\textbf{Question 2}\quad \textit{How to design algorithms to achieve desirable dynamics of the decision boundary?}\quad 
To this end, we propose \textit{\algoNameFull (\algoName)}, which explicitly controls the decision boundary to move away from the data points and moreover, faster from the points with smaller robust radii. Such control is possible since we can derive the dynamics of the decision boundary given a training algorithm, which enables us to reverse engineer the training scheme to achieve the desirable dynamics. 
% Specifically, \algoName adopts a weighted loss on the closest boundary points, where the weights are reverse engineered to realize the 
% % desirable 
% dynamics. 
Unlike previous weighted AT methods~\citep{zhang2021geometryaware, zeng2020adversarial,liu2021probabilistic} which directly assign larger weights to more vulnerable points, \algoName designs the weights so that the robustness improvement of vulnerable points is faster. 
% In addition, instead of pre-defining a uniform perturbation length for training as in AT, \algoName trains on the closest boundary points to take into account of the robust radius of each point. Consequently, \algoName is naturally robust to more diverse attacking budget $\epsilon$'s, whereas previous weighted AT methods are trained to be robust to a pre-defined $\epsilon$.
We experimentally show that \algoName realizes the desirable dynamics and achieves improved robustness performance. 
% on diverse attacking budgets. 


\textbf{Summary of contributions.} \textbf{(1)} We propose a continuous-time framework to study the relative speed of the decision boundary w.r.t. each individual data point and provide its closed-form expression.
\textbf{(2)} We visualize the speed of the decision boundary for AT and identify the conflicting dynamics of the decision boundary. 
\textbf{(3)} We propose Dynamical Adversarial Training (\algoName) which controls the decision boundary to move faster from more vulnerable points.
% with smaller robust radii. 
We experimentally show that \algoName alleviates the conflicting dynamics and obtains improved robustness over state-of-the-art defenses.  



==> A_continuous_workshop/s2_prelim.tex <==
% \section{Preliminaries} \label{sec:prelim}
% \subsection{Notations and definitions}

% \textbf{Notations and definitions}\quad
% We consider a classification task with inputs $x \in \mathcal{X}$ and labels $y\in\mathcal{Y} = \{1,2,...,K\}$.
% Let $\{x_i,y_i\}_{i=1}^N$ be all training data of size $N$. A deep classifier parameterized by $ \theta $ is denoted by $f_{\theta}(x) = \argmax_{c\in\mathcal{Y}}z_{\theta}^c(x)$ where $z_{\theta}^c(x)$ is the logit for class $c$. 
% % Denote $z_\theta(x)$ to be the vector of logits for all classes. 
% Denote the logit margin of class $ y $ as $ \phi^{y}_{\theta}(x) = z_{\theta}^y(x) - \max_{y'\neq y} z_{\theta}^{y'}(x) $. In the paper, we will use $\phi^{y}_\theta(x)$ and $\phi^{y}(x,\theta)$ interchangeably. Observe that $ x $ is classified as  $ y $ if and only if $ \phi^{y}_{\theta}(x) > 0 $. Therefore,  the zero level set of $ \phi^{y}_{\theta}(x) $, denoted by $ \Gamma_y=\{x: \phi^{y}_{\theta}(x) = 0\} $, is the decision boundary for class $ y $. Denote $\|\cdot\|_p$ the $L_p$ norm.
% with $1 \leq p \leq \infty$.
% For a correctly classified point $(x,y)$, its robust radius $R_\theta(x)$ is defined to be the distance from $x$ to the decision boundary for class $y$. That is,
% % \setlength\abovedisplayskip{0pt}
% % \setlength\belowdisplayskip{0pt}
% \begin{equation} \label{eq: robustness_radius}
%     R_\theta(x) = \min_{\hat{x}} \|\hat{x}-x\|_p \quad \textrm{s.t.}  \quad \phi_\theta^y(\hat{x}) = 0
% \end{equation}
% where $\|\cdot\|_p$ is the $L_p$ norm with $1\leq p \leq \infty$.


% \subsection{Continuous-time formulation}

% \textbf{Continuous-time formulation}\quad
% In this paper, we will use the continuous-time formulation for the optimization on the parameters $\theta$, which allows us to study the instantaneous movement of the decision boundary. Let $\theta'(t)$ be the continuous-time description of a training algorithm, which consists of a loss function $L$ and an optimization scheme. To derive the discrete counterpart $\theta'_k$ of $\theta'(t)$ at iteration $k$ given a training algorithm, we use the relationship $\theta'_k :=\frac{\theta_{k+1} - \theta_{k}}{\gamma}$, where $\gamma$ is the learning rate. 
% For example, consider the commonly used stochastic gradient descent (SGD) with momentum ($\lambda_m$) and weight decay  ($\lambda_w$) given by
% \begin{equation} \label{eq: SGD_momentum_weightDecay shorter}
% % \setlength\abovedisplayskip{1pt}
% % \setlength\belowdisplayskip{1pt}
% \begin{aligned}
%     b_{k+1} = \nabla_\theta L(\theta_{k}) +  \lambda_w \theta_{k} + \lambda_m b_{k}, \quad 
%     \theta_{k+1} = \theta_{k} - \gamma b_{k+1}
% \end{aligned}
% \end{equation}
% where $b_0 = 0$ and $b_k$'s are the intermediate variables. In this case, $\theta'_k$ is given by 

% \begin{equation} \label{eq: theta prime momentum weight decay general}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
% \begin{aligned}
%     \theta'_k &= -\nabla_\theta L(\theta_{k})  - \lambda_w \theta_{k}- \lambda_m b_{k} %\fhc{?}\text{\yc{What is unclear?}}
% \end{aligned}
% \end{equation}

% which can be interpreted as the un-normalized update direction of $\theta$ at step $k$. 

==> A_continuous_workshop/s3_dynamics4DB.tex <==
\section{Dynamics of the decision boundary} \label{sec: dynamics_of_bdr}
In this section, we study the relative speed of the decision boundary in continuous time and visualize the speed of AT for further insights. We consider a classification task with inputs $x \in \mathcal{X}$ and labels $y\in\mathcal{Y} = \{1,2,...,K\}$.
Let $\{x_i,y_i\}_{i=1}^N$ be all training data of size $N$. A deep classifier parameterized by $ \theta $ is denoted by $f_{\theta}(x) = \argmax_{c\in\mathcal{Y}}z_{\theta}^c(x)$ where $z_{\theta}^c(x)$ is the logit for class $c$. 
% Denote $z_\theta(x)$ to be the vector of logits for all classes. 
Denote the logit margin of class $ y $ as $ \phi^{y}_{\theta}(x) = z_{\theta}^y(x) - \max_{y'\neq y} z_{\theta}^{y'}(x) $. In the paper, we will use $\phi^{y}_\theta(x)$ and $\phi^{y}(x,\theta)$ interchangeably. Observe that $ x $ is classified as  $ y $ if and only if $ \phi^{y}_{\theta}(x) > 0 $. Therefore,  the zero level set of $ \phi^{y}_{\theta}(x) $, denoted by $ \Gamma_y=\{x: \phi^{y}_{\theta}(x) = 0\} $, is the decision boundary for class $ y $. Denote $\|\cdot\|_p$ the $L_p$ norm.

\vspace{-0.5em}
\subsection{Speed of the decision boundary}
\vspace{-0.5em}
For a correctly classified example $(x_i,y_i)$, we would like to capture the movement of the decision boundary $\Gamma_{y_i} (t) = \{x:\phi^{y_i}(x,\theta(t)) = 0\}$ w.r.t. $x_i$ as $t$ varies continuously. Therefore, we consider its closest boundary point:


\begin{definition}[Curve of the closest boundary point $\hat{x}_i(t)$] \label{def: closest_pt}
Suppose that $(x_i,y_i)$ is correctly classified by $f_{\theta(t)}$ in some time interval $t \in I$. Define the curve of the closest boundary point $\hat{x}_i(\cdot): I \to \mathcal{X}$ as
\begin{equation} \label{eq: closest_pt}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
    \hat{x}_i(t) = \argmin\nolimits_{\hat{x}} \|\hat{x}-x_i\|_p \quad \textrm{s.t.}  \quad \phi^{y_i}(\hat{x},\theta(t)) = 0.
\end{equation}
Define the robust radius of $x_i$ at time $t$ to be $R(x_i,t) = \|\hat{x}_i(t)-x_i\|_p $.
%\fhc{we need to explain $l_p$ norm. For example, how to choose $p$. Or what values can $p$ take?}\yc{added an explanation in prelim section.}
\end{definition}

\begin{wrapfigure}{r}{0.3\columnwidth}
% \begin{figure}[!t] % [!htbp]
 \vspace{-4em}
    \centering
    \includegraphics[width=0.245\columnwidth]{Intepretation_fig/AT_Dynamics-derivation.pdf}
    \vspace{-1.0em}
    \caption{Curve of the closest boundary point $\hat{x}(t)$ (in blue) of the data point $x$.}
    \label{fig:curve}
\vspace{-1em}
% \end{figure}
\end{wrapfigure}
An example of the curve of the closest boundary point is depicted in Figure~\ref{fig:curve}.
To understand how the distance between the decision boundary $\Gamma_{y_i} (t)$ and $x_i$ changes, it suffices to focus on the curve of the closest boundary point $\hat{x}_i(t)$. We define the speed of the decision boundary to be the time derivative of the robust radius as follows:

\begin{definition}[Speed of the decision boundary $s(x_i,t)$] \label{def: speed_of_bdr}
Under the setting of definition \ref{def: closest_pt}, define the relative speed of the decision boundary w.r.t. $x_i$ as $s(x_i,t) = \frac{d}{dt} R(x_i,t) = \frac{d}{dt}  \|\hat{x}_i(t)-x_i\|_p$.
\end{definition}

Note that the speed $s(x_i,t) > 0$ means that the robustness improves for $x_i$ at time $t$, which is desirable during adversarial training. The next proposition gives a closed-form expression for the speed given a continuous description $\theta'(t)$ of the training algorithm.

\begin{proposition}[Closed-form expression of the speed] For $1 \leq p \leq \infty$,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}   
\begin{equation} \label{eq: expression_for_speed}
    s(x_i,t) = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q} 
\end{equation}
where $q$ satisfies that $1/q+1/p=1$. In particular, $q=2$ when $p=2$ and $q=1$ when $p=\infty$.
\end{proposition}

\paragraph{Remark}
The main assumption for Equation~\eqref{eq: expression_for_speed} is the local differentiability of $\phi^{y_i}(\cdot,\theta(t))$ at $\hat{x}_i(t)$. The full assumptions and proof are left to Appendix~\ref{app: closed_expression_speed}. 
% The key points of proving Equation~\eqref{eq: expression_for_speed} include the level set equation \citep{osher2004level,aghasi2011parametric} and the optimality condition for optimization problem~\eqref{eq: closest_pt}. 
Special care has been taken for $p=\infty$ since $L_\infty$ norm is not differentiable.

According to Equation~\eqref{eq: expression_for_speed}, the speed $s(x_i,t_0) $ is positive at time $t_0$ when $\nabla_\theta \phi^{y_i} (\hat{x}_i(t_0),\theta(t_0)) \cdot \theta'(t_0) >0$, i.e. the value of $\phi^{y_i}(\hat{x}_i(t_0))$ increases. This means that the boundary point $\hat{x}_i(t_0)$ will be correctly classified after the update. 
Also, the magnitude of the speed tends to be larger if $\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q$ is smaller, i.e. the margin function $\phi^{y_i}$ is flatter around $\hat{x}_i(t)$. 
In the remaining part of the paper, we will denote $s(x_i,t)$ and $R(x_i,t)$ as $s(x_i)$ and $R(x_i)$ when the indication is clear.
% \textbf{Computing the closest boundary point:} 
To implement the Equation~\eqref{eq: expression_for_speed} in practice, we need to compute the closest boundary point $\hat{x}_i(t)$. We use the Fast Adaptive Boundary Attack (FAB) \citep{croce2020minimally} to approximate $\hat{x}_i(t)$. 
% Note that here FAB only serves as an algorithm to approximate $\hat{x}_i(t)$, and can be decoupled from the remaining part of the framework. In our experiments we find that given enough number of iterations, FAB can reliably find the local optimum of Equation~\eqref{eq: closest_pt} where the expression for speed in Equation~\eqref{eq: expression_for_speed} is still valid. We give more details of how to check the local optimality condition of Equation~\eqref{eq: closest_pt} and the performance of FAB in Appendix~\ref{app: optimality}. 


\subsection{Dynamics of adversarial training} \label{ssec: Dynamics of adversarial training}
\input{\texhome/Speed_unnormalized_time}
We numerically compute the speed of the decision boundary to understand the dynamics during AT.
%More analysis of the dynamics are left to Appendix~\ref{app: more_dynamics}. 
We train a ResNet-18 \citep{he2016deep} on CIFAR-10 using AT under $L_2$ perturbation with $\epsilon=0.5$, whose test clean and robust accuracy are shown in Figure~\ref{fig: AT_acc}. 
We choose 512 points from the test set and at each iteration we compute the robust radii and speed for correctly classified ones. 
% We omit those points whose robust radii are larger than 1, which are considered very robust under $\epsilon=0.5$. 
The speed distribution over time is shown in Figure~\ref{fig: AT_speed_time}. 
We can observe that at the start of training (the first 100 iterations), the speed distribution is mostly positive and the robust accuracy increases drastically. 
Later, the speed distribution is centered around zero and the robustness improvement slows down. %\fhc{shorten this paragraph.}

\input{\texhome/fig_intepret_train}
\textbf{Non-converging dynamics of AT}\quad
In Figure~\ref{fig: AT_speed_time} we find that the variance of the speed distribution is never vanishing: the decision boundary always moves towards some data points while moving away from others. This indicates that AT does not converge. Despite the constant movement of the decision boundary, the average adversarial loss does converge. Therefore, the dynamics of the decision boundary w.r.t. each data point provides more information than an average of the surrogate loss. 

%For comparison with AT, we adopt natural training (NT) whose test accuracy and speed distribution are shown in Figure~\ref{fig: clean_acc} and Figure~\ref{fig: clean_speed_time}. We observe that the speed distribution of the decision boundary during NT is effectively zero. This indicates that NT eventually does not move the decision boundary around correctly classified points anymore, which is different from AT. 

\textbf{Conflicting dynamics of AT}\quad Since the update of the parameters $\theta$ at each iteration is computed on one batch of the training data, we visualize the robust radii and speed on the training batch of each iteration in Figure~\ref{fig: interpretation_VR_trainBatch_all}. Observe that there is always a significant proportion of non-robust points (with $R(x_i)<0.5$) with negative speed, indicating the conflicting dynamics on the training batch. This is not desirable because ideally at each iteration, the vulnerable points in the training batch should be improved since the current update of $\theta$ is computed on them.
% \yc{This is also typical in other variants of AT, which is shown in appendix.} 
In Section~\ref{sec:dynamicalAT}, we will see that such conflicting dynamics can be alleviated: since the update rule has full access to the training batch, it is possible to design the update rule so that every vulnerable point in the training batch is made more robust. 
% We provide more analysis of the dynamics in Appendix~\ref{app: more_dynamics}. 







==> A_continuous_workshop/s4_dynamicalAT.tex <==
\vspace{-0.5em}
\section{\algoName: \algoNameFull}\label{sec:dynamicalAT}

To remedy the conflicting dynamics issue and encourage robustness improvement on more vulnerable points, we propose \algoNameFull (\algoName), which customizes the dynamics of the decision boundary for each data point. 
Ideally, the decision boundary should move away from each vulnerable point. Moreover, given the limited capacity of the neural networks, robustness improvement on more vulnerable points should be encouraged more. Therefore, the desirable dynamics should satisfy:  \textbf{Condition 1:} $s(x_i) > 0 $ when $R(x_i) < r_0$ for some threshold $r_0$. \textbf{Condition 2:} $s(x_i) \geq s(x_j)$ when $R(x_i) < R(x_j)$.
In particular, {Condition 2} considers customized manipulation of the decision boundary by encouraging smaller robust radii to improve faster. 
%The goal of \algoName is to approximate both conditions and thus achieving fairer robustness to each data point as well as better overall robustness.
% under the limited model capacity.

% In particular, \textbf{Condition 2} considers a customized manupulation of the decision boundary. When satisfied, it robustifies each individual vulnerable point\yc{..fairness; dyna-cat; customized..}. % rather than focusing on the average robustness (or more accurately (un)weighted average of surrogate robustness) as in most prior works. 
% Consequently, \textbf{Condition 2} achieves a fairer robustness to individuals, leading to better overall robustness under a limited model capacity as well. % \yc{Not quite accurate: Previous work focus on surrogate loss, weighted average. We focus on improving radius faster.}


To design such desirable dynamics, we introduce a \textit{ratio function} $g(r)$, a non-increasing function that satisfies $g(r) > 0$ when $r < r_0$ for some threshold $r_0$. 
At each iteration, the speed $s(x_i)$ of the decision boundary w.r.t. $x_i$ should be approximately proportional to $g(R(x_i))$. 
% In other words, $s(x_i) \approx \mu \cdot g(R(x_i))$ for some common scalar $\mu > 0$ for all data points. Since the effect of $g$ does not change if it is multiplied by a constant, we fix $g(0) = 1$. 
% \textbf{Controlling the robustness level with the ratio function}\quad Instead of using a pre-defined perturbation length to control the robustness level, \algoName uses all of the closest boundary points, 
% % with respect to all correctly classified data points during training
% including those that are relatively far from the original ones. The ratio function $g$ controls the robustness level: if $g$ decays more slowly, \algoName will encourage robustness improvement even when the robust radius is large, and thus the model is robust to larger perturbation thresholds. On the other hand, if $g$ decays fast, the improvement on the non-robust points will be encouraged more.
% % , so the model is unlikely to be able to withstand larger perturbation thresholds. 
% How to calculate the optimal $g$ is still an open question. Therefore, we heuristically design different $g'$s and discuss more about them in Section~\ref{sec:exp_effect} and Appendix~\ref{app: further_exp_results}.
% \subsection{\algoName: Realizing the desirable dynamics} \label{ssec: realizing_dynamics}
To customize the dynamics of the decision boundary for each data point, we propose to use a weighted average of loss on the closest boundary points and compute the weights to achieve the designed dynamics. 
Consider a batch $\mathcal{B}$ with size $n$ and denote $\mathcal{B}^{+}_\theta$ of size $m$ to be the set of correctly classified points in $\mathcal{B}$. We use the loss function
%\begin{equation} \label{eq: weighted loss general}
$
	L_\theta(\mathcal{B}) =  -\sum\nolimits_{i\in \mathcal{B}^{+}_\theta}c_i \phi^{y_i}(\hat{x}_i) + \lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}l(x_i,y_i) 
	$, 
%\end{equation}
where the first term is the weighted margin loss on the closest boundary points  with weights $\{c_i\}$ to be determined. The second term is the cross-entropy loss on natural examples.
By equation~\eqref{eq: expression_for_speed}, the speed $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$ is a linear function of the weights $\mathbf{c} = (c_1,\cdots, c_m)^{T}$, 
%in the following way: $\mathbf{c}$ determines the loss function above; the loss function, together with an optimization scheme, determines $\theta'(t)$; %(for example, by Equation~\ref{eq: theta prime momentum weight decay general}); finally, $\theta'(t)$ determines the speed $\mathbf{s}$ by the closed-form expression~\eqref{eq: expression_for_speed}. 
% Since these dependencies are all linear, 
% $\mathbf{s}$ is a linear function of $\mathbf{c}$, 
denoted by $\mathbf{s}(\mathbf{c})$. 


Our goal is to reverse engineer the weights $\mathbf{c}$ so that the speed $\mathbf{s}(\mathbf{c})$ approximates the designed dynamics specified by the ratio function $g$. Let the ratio values $\mathbf{g} = (g(R(x_1)),\cdots,g(R(x_{m})))^{T}$. 
% To approximate the desired dynamics given by $\mathbf{g}$, 
We solve the following optimization problem:
\vspace{-0.5em}
\begin{equation} \label{eq:opt_for_weight}
\setlength\abovedisplayskip{10pt}
\setlength\belowdisplayskip{2pt}
\min_{\mathbf{c}, \mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} c_i = 1, c_i\geq0, \mu \geq 0    
\end{equation}
where $\mu$ is a scalar so that the solved $\mathbf{s}(\mathbf{c})$ is approximately a multiple of $\mathbf{g}$.
The problem~\eqref{eq:opt_for_weight} is a quadratic programming problem with linear constraints of size $m+1$, which is convex and can be solved efficiently and reliably.
We find that the extra runtime of solving the problem~\eqref{eq:opt_for_weight} is negligible.
More details of \algoName are left to Appendix~\ref{app: algo} and Appendix~\ref{app: optimality}.

% We give the coefficient of this quadratic programming problem in Appendix~\ref{app: opt_for_weight}. % The pseudocode of \algoName is shown in Appendix~\ref{app: algo_pseudo}. 
% We also introduce a burn-in period where we only use the clean loss during the initial stage of the training to achieve a descent clean accuracy. This is necessary because the closest boundary points used by \algoName can only be found for correctly classified examples. 





% Let the ratio values $\mathbf{g} = (g(R(x_1)),\cdots,g(R(x_{m})))^{T}$ and $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$. 
% According to the speed expression \eqref{eq: expression_for_speed}, the expression of $\theta'_k$ in \eqref{eq: theta prime momentum weight decay general} and the loss function \eqref{eq: weighted loss general}, $\mathbf{s}$ is a linear function of the  weights $\mathbf{c}$ and we denote it as $\mathbf{s}(\mathbf{c})$. 

\textbf{Comparisons with related adversarial training methods}\quad 
Several existing adversarial training methods also leverage the vulnerability difference among data points. 
In particular, MMA\citep{Ding2020MMA} also trains on the closest boundary points, but it adopts uniform weights and thus does not necessarily improve robustness of every vulnerable point. On the other hand, weighted adversarial training methods
assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. 
% More related works are left to Appendix~\ref{sec:related_work_app}.




==> A_continuous_workshop/s5_related.tex <==
\section{Related Work}\label{sec:related}

\textbf{Controlling parameterized surface}\quad 
The decision boundary can be viewed as a parameterized surface in the input space. Controlling such surface has been studied in image segmentation\citep{li2011level,aghasi2011parametric} and shape modelling\citep{chen2019learning,park2019deepsdf}. As for adversarial training, the authors of \citep{Atzmon2019control} propose to maximize the distance between each data point and some point on the decision boundary, which is not the closest one. On the other hand, we study the movement of the decision boundary w.r.t. each data point by analyzing its closest boundary point, which is directly related to the 
robust radius. 

\textbf{Comparisons with related adversarial training methods}\quad 
There are several defense techniques including gradient regularization \citep{moosavi2019robustness,tramer2017ensemble}, certified denfense\citep{cohen2019certified,wong2018provable,balunovic2019adversarial} and adversarial training \citep{madry2017towards,zhang2019theoretically,gowal2020uncovering,wang2019improving,zhang2020attacks}, where the last one is the most related to this work. 
In particular, MMA\citep{Ding2020MMA} trains on the closest boundary points, which is similar to \algoName. However, MMA adopts uniform weights and thus does not consider the vulnerability difference among the points. On the other hand, weighted adversarial training methods \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware} assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. 



% so that an example with a larger logit margin value is viewed as more robust. However, a larger logit margin value does not necessarily correspond to a larger robust radius. 


==> A_continuous_workshop/s6_exp.tex <==
% \section{Experiments}\label{sec:exp}
% In this section, we empirically evaluate the proposed \algoName on the CIFAR-10 \citep{krizhevsky2009learning} dataset. We visualize its dynamics in Section~\ref{sec:exp_effect} and evaluate its robustness performance and compare it with several state-of-the-art baselines in Section~\ref{sec:exp_robust}. Implementation details are left to Appendix \ref{app: exp_settings}, including neural network architectures and training hyperparameters. 
% % Further experimental results are presented in Appendix \ref{app: further_exp_results}.


\begin{wrapfigure}{r}{0.4\textwidth}%[!t]
    \centering
     \vspace{-1.5em}
    \resizebox{0.4\textwidth}{!}{\input{\texhome/experiment_fig/Our_batch_scatter}}
    \vspace{-1.5em}
    \caption{Radius-speed plot of \algoName on the training batches for three randomly chosen iterations. Proportion of points with negative speed for these iterations are all below $2\%$.}
    \label{fig: performance_batch_VR_ours}
    \vspace{-1.0em}
\end{wrapfigure} 

\textbf{Realizing the desirable dynamics}\quad 
\algoName computes the weights to approximate the desirable dynamics by solving the optimization problem \eqref{eq:opt_for_weight}. To verify the quality of this approximation, we consider the $L_2$ norm constrained perturbation and choose the ratio function $g(r) = 1 - r$ when $r \leq 1$ and $g(r)=0$ otherwise. 
In Figure~\ref{fig: performance_batch_VR_ours}, we visualize the speed and robust radii of points in the training batches of three randomly chosen iterations.
We observe that the speed is positive for most of the points and is approximately a decreasing function of the robust radius, which is consistent with the design of $g$. 
By comparing with the conflicting dynamics of AT in Figure~\ref{fig: interpretation_VR_trainBatch_all}, we conclude that \algoName alleviates the conflicts and achieves the desirable dynamics during training. 
% \label{sec:exp_effect}





\input{\texhome/tab_L2_moreEps}
\textbf{Robustness evaluation}\quad 
%\label{sec:exp_robust}
%\textbf{Compared baselines}\quad
The baseline defense methods include: (1) standard adversarial training (AT) \citep{madry2017towards} which trains on the worst case adversarial examples; (2) TRADES \citep{zhang2019theoretically} which trades off between the clean and robust accuracy; (3) MMA \citep{Ding2020MMA} which trains on the closest adversarial examples with uniform weights.
%; (4) GAIRAT \citep{zhang2021geometryaware} which reweights adversarial examples based on the least perturbation steps. % Their hyperparameters are left to Appendix~\ref{app: exp_settings}. 
%\textbf{Evaluation protocol}\quad
% We evaluate \algoName and the baselines under $L_2$ and $L_\infty$ norm constrained perturbation. 
The final robust accuracy is reported on AutoAttack (AA) \citep{croce2020reliable}, which uses an ensemble of selected strong attacks. 
%We also include the results under PGD attack with 40 iterations in Appendix~\ref{app: further_exp_results}. 
For all methods, we choose the hyperparameters to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting. We also evaluate on larger perturbation thresholds to better examine the robustness of the models under larger unknown attack budgets.
As shown in Table~\ref{table: performance_L2_more_eps}, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. The full experimental settings and more experimental results are left to Appendix~\ref{app: exp}.
% against unknown perturbation strength.

% \textbf{Hyperparameters of \algoName}\quad 
% We use the ratio function with $g(0) = 1, g(r_0) = 0, g(r_1) = - g_1$ with $g_1 \geq 0 $ and linearly interpolate them when $0\leq r \leq r_1$. When $r>r_1$, $g(r)$ was set to the constant $-g_1$. We allow $g$ to be negative when $r > r_1$ because we experimentally find that 'pulling back' the decision boundary if it is too far away from data points could help improve both clean and robust accuracy. Choices of $r_0, r_1, g_1$ and other hyperparameters are left to Appendix~\ref{app: exp_settings}.


%\textbf{Performance}\quad 
% The main evaluation results are shown in Table \ref{table: performance_L2_more_eps} and Table \ref{table: performance_Linf_more_eps}. The full results and the ablation study on the effect of the ratio function are left to Appendix~\ref{app: further_exp_results}. In the $L_2$ case, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. In the $L_\infty$ case, \algoName obtains both higher clean accuracy and robust accuracy than AT, MMA and GAIRAT. We observe that GAIRAT achieves high robustness under PGD attacks (shown in Appendix~\ref{app: further_exp_results}) but has much lower robust accuracy under the stronger AA attack, which may be due to obfuscated gradient \citep{AthalyeC018}. On the other hand, the performance gap between PGD and AA is relatively small for \algoName. When compared with TRADES, \algoName shows higher clean accuracy and comparable robust accuracy under larger $\epsilon$, although \algoName has lower robust accuracy when $\epsilon = \frac{8}{255}$. This is partially due to the higher difficulty of approximating the closest boundary points in the $L_\infty$ case, and a better algorithm for this is left for future work. 

% \input{\texhome/tab_Linf_moreEps}
% \input{\texhome/tab_moreEps}

==> A_continuous_workshop/s7_conc.tex <==
\vspace{-0.5em}
\section{Conclusion and Discussion} \label{sec:conc}
% \vspace{-0.5em}
This paper has proposed a continuous-time framework to study the relative movement of the decision boundary w.r.t. each data point given an training algorithm. Using this framework, we reveal the non-converging and conflicting dynamics of AT. To alleviate the conflicts, we propose \algoName to control the decision boundary to move faster away from more vulnerable points, which shows promising results on robustness performance.
The future direction includes using the proposed framework to study the dynamics of other training algorithms for further insights.





==> A_continuous_workshop/tab_L2_moreEps.tex <==
\begin{wraptable}{r}{0.5\textwidth}%[!htbp]
\centering
\noindent
\vspace{-2em}
\caption{\scriptsize{Clean and robust accuracy on CIFAR-10 under $L_2$ attack}}
\resizebox{0.5\textwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=0.5$}  & {$\epsilon=1$} & {$\epsilon=1.5$}  & {$\epsilon=2$} \\
\midrule
AT & {$88.38 \pm 0.23$} & {$65.29 \pm 0.21$}  & {$33.71 \pm 0.16$}  & {$11.16 \pm 0.09$}  & {$2.4 \pm 0.17$}  & \\
TRADES & {$87.05 \pm 0.01$} & {$67.92 \pm 0.11 $}  & {$42.08 \pm 0.16$}  & {$19.33 \pm 0.38$} & {$6.62 \pm 0.16$}  & \\
MMA & {$\boldsymbol{88.40} \pm 0.14$} & {$65.62 \pm 0.23$}  & {$36.54 \pm 0.14$} & {$14.01 \pm 0.08$}  & {$3.49 \pm 0.10$}  & \\
\midrule
Ours & {$87.25 \pm 0.05$} & {$\boldsymbol{67.96} \pm 0.14$}   & {$\boldsymbol{43.48} \pm 0.23$}  & {$\boldsymbol{20.92} \pm 0.12$} & {$\boldsymbol{6.72} \pm 0.18$} &  \\
\bottomrule
\end{tabular}}
\label{table: performance_L2_more_eps}
\end{wraptable}

==> A_continuous_workshop/tab_Linf_moreEps.tex <==
\begin{table}[!htbp]
\vspace{-1em}
\centering
\noindent
\caption{{Clean and robust accuracy on CIFAR-10 under $L_\infty$ attack} }
\resizebox{\columnwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=\frac{8}{255}$} & {$\epsilon=\frac{12}{255}$} & {$\epsilon=\frac{16}{255}$} & {$\epsilon=\frac{20}{255}$} \\
\midrule
AT & {$83.25 \pm 0.17$} & {$45.75 \pm 0.15$} & {$26.38 \pm 0.14$} & {$12.34 \pm 0.17$} & {$4.89 \pm 0.11$}& \\
TRADES & {$83.54 \pm 0.08$} & {$\boldsymbol{47.18} \pm 0.11$}  & {$29.03 \pm 0.19$}& {$15.07 \pm 0.11$}  & {$\boldsymbol{6.78} \pm 0.06$} & \\
MMA & {$84.25 \pm 0.28$} & {$41.48 \pm 0.31$} & {$23.63 \pm 0.25$} & {$11.97 \pm 0.20$} &{$5.11 \pm 0.12$} & \\
GAIRAT & {$81.31 \pm 0.23$} & {$32.98 \pm 0.11$}& {$16.19 \pm 0.02$} & {$6.89 \pm 0.18$}  & {$2.57 \pm 0.07$} & \\
\midrule
Ours & {$\boldsymbol{85.13} \pm 0.13$} & {$46.47 \pm 0.18$}  & {$\boldsymbol{29.38} \pm 0.24$} & {$\boldsymbol{15.14} \pm 0.16$} & {$6.45 \pm 0.21$} & \\
\bottomrule
\end{tabular}}
\label{table: performance_Linf_more_eps}
\vspace{-1em}
\end{table}

==> ICLR_fig/AT_trainBatch_scatter_save.tex <==
% This file was created with tikzplotlib v0.10.1.
\pgfplotsset{scaled x ticks=false}
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\textbf{\Large{Naturally pretrained model}}},
x grid style={darkgray176},
xmin=0, xmax=0.0156862745098039,
xtick style={color=black},
% xtick={0,0.00784313725490196,0.0156862745098039},
xtick={0,0.00784313725490196,0.0156862745098039},
xticklabels={
  \(\displaystyle 0\),
  \(\displaystyle \frac{2}{255}\),
  \(\displaystyle \frac{4}{255}\)
},
y grid style={darkgray176},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
]
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, only marks]
table{%
x  y
0.00365513563156128 0.605594635009766
0.00130671262741089 -0.0589427873492241
0.00169408321380615 -0.345070779323578
0.00204837322235107 -0.619586765766144
0.00253874063491821 0.238536924123764
0.00160866975784302 0.639483451843262
0.00412929058074951 0.253036886453629
0.00132414698600769 -0.0763033553957939
0.000508546829223633 0.082988828420639
0.00128442049026489 -0.512788772583008
0.0013994574546814 -0.23567807674408
0.00204986333847046 0.235927268862724
0.00370496511459351 0.591313898563385
0.00144243240356445 -0.296937197446823
0.00272095203399658 0.057938851416111
0.00380492210388184 0.500588834285736
0.00121355056762695 0.0937552452087402
0.000508248805999756 0.461227506399155
0.00252401828765869 0.500977158546448
0.0058315098285675 0.286468863487244
0.0102527141571045 -0.333424836397171
0.00151592493057251 0.273176312446594
0.00289237499237061 0.0356715321540833
0.000670135021209717 0.296710997819901
0.00286799669265747 0.416187793016434
0.00423163175582886 0.29781785607338
0.00639420747756958 0.488814860582352
0.00381618738174438 -0.122778490185738
0.0039023756980896 0.283090800046921
0.00840854644775391 0.870968043804169
0.00304365158081055 0.624023377895355
0.00211650133132935 0.318257838487625
0.00190788507461548 0.140597447752953
0.00345897674560547 0.0910703614354134
0.00391268730163574 -0.198450520634651
0.00167614221572876 0.233509749174118
0.00183796882629395 0.228109285235405
0.00456094741821289 0.116979993879795
0.0010027289390564 0.242157712578773
0.00398576259613037 0.507651627063751
0.00392806529998779 -0.23045589029789
0.00346148014068604 0.182729840278625
0.00731205940246582 0.685366094112396
0.00440126657485962 -0.28048899769783
0.000771462917327881 0.0723515227437019
0.00243467092514038 0.391375303268433
0.00105792284011841 0.408040016889572
0.00056767463684082 0.234025448560715
0.00107598304748535 0.232879802584648
0.00310665369033813 -0.447581619024277
0.00261026620864868 -0.0730878189206123
0.00190842151641846 -0.0749514177441597
0.00116950273513794 0.370825201272964
0.00285583734512329 -0.296423405408859
0.00235158205032349 0.324640393257141
0.000541210174560547 -0.43024092912674
0.0034528374671936 0.71880978345871
0.00184226036071777 0.617101073265076
0.00801569223403931 0.708444178104401
};
\addplot [semithick, red, opacity=0.4]
table {%
0 0
0.0156862745098039 0
};
\addplot [semithick, red, opacity=0.4]
table {%
0.0313725490196078 -1
0.0313725490196078 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\textbf{\Large{Partially Robust model}}},
x grid style={darkgray176},
xmin=0, xmax=0.0627450980392157,
xtick style={color=black},
xtick={0,0.0313725490196078,0.0627450980392157},
xticklabels={
  \(\displaystyle 0\),
  \(\displaystyle \frac{8}{255}\),
  \(\displaystyle \frac{16}{255}\)
},
y grid style={darkgray176},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
]
\addplot [draw=steelblue31119180, fill=steelblue31119180, mark=*, only marks]
table{%
x  y
0.0120787620544434 0.674289047718048
0.00752228498458862 0.895295381546021
0.0173213481903076 -0.103290967643261
0.0173263549804688 0.56147962808609
0.0563383102416992 0.0265122763812542
0.00194507837295532 -0.103116601705551
0.0041617751121521 0.298849999904633
0.0335975289344788 -0.0617453046143055
0.0346554517745972 0.124957114458084
0.0227861404418945 0.63747650384903
0.0205302834510803 0.332097738981247
0.0143898129463196 -0.0305895339697599
0.0579545497894287 -0.0591495186090469
0.0093001127243042 0.355203866958618
0.000759243965148926 -0.266114711761475
0.0183109641075134 0.180211946368217
0.0407352447509766 -0.0738517940044403
0.0304546356201172 0.259497284889221
0.0371867418289185 -0.0665352717041969
0.0259443819522858 0.427894443273544
0.026517778635025 -0.0230144243687391
0.0311389565467834 -0.00789366196841002
0.0182619988918304 0.0811871364712715
0.0164907574653625 -0.302245914936066
0.0208012461662292 0.372285842895508
0.0014670193195343 0.0562338344752789
0.0134779810905457 0.023836636915803
0.0171606540679932 0.228304415941238
0.00991690158843994 -0.0616621002554893
0.00493943691253662 -0.414471715688705
0.050433337688446 0.634823799133301
0.0497239828109741 0.235450744628906
0.00920069217681885 0.143730089068413
0.0145842432975769 0.228869587182999
0.0177146196365356 -0.250288903713226
0.000945448875427246 0.379655569791794
0.0176169872283936 0.310396999120712
0.0166523456573486 0.299226760864258
0.0252554416656494 0.683125019073486
0.0343238115310669 -0.0856688097119331
0.0217269062995911 -0.0240955352783203
0.00842905044555664 0.530959784984589
0.0270448327064514 0.213502436876297
0.0280755162239075 -0.31022247672081
0.0262386798858643 -0.0468107014894485
0.0413601994514465 -0.155704766511917
0.0454379320144653 0.505486965179443
0.0109276175498962 0.69685685634613
0.0329769253730774 0.517087817192078
0.03421550989151 -0.0787589401006699
0.0500233173370361 0.50403243303299
0.0265262126922607 0.272267073392868
0.0481072664260864 -0.137751236557961
0.00505244731903076 0.0965651571750641
0.0374917984008789 0.30837070941925
0.0172470808029175 0.322719365358353
0.0201632976531982 -0.168686792254448
0.0406553745269775 0.249719142913818
0.0499173849821091 0.450171172618866
0.0134746432304382 0.0379396975040436
0.0510182976722717 0.341217041015625
0.0289039611816406 -0.00510647147893906
0.00889265537261963 -0.147434651851654
0.046957790851593 0.333819329738617
0.0246496200561523 0.388248592615128
0.0101080536842346 0.421099752187729
0.056393176317215 -0.110466592013836
0.0096631646156311 0.666519343852997
0.0141111016273499 0.836408674716949
0.0180205702781677 0.204066425561905
0.0288708806037903 0.507671892642975
0.0131513476371765 0.877965867519379
0.0109407901763916 0.164353460073471
0.026078462600708 -0.387259244918823
0.0281993746757507 0.141197517514229
0.0150520801544189 0.059478797018528
0.0396338105201721 -0.0353399328887463
0.0192951560020447 0.385244429111481
0.0115717649459839 -0.424117267131805
0.0351501107215881 0.0465284399688244
0.00839865207672119 -0.0405612736940384
0.00905865430831909 0.379240840673447
0.0472913980484009 0.425879597663879
0.00899308919906616 0.312629848718643
0.0528552532196045 0.132481917738914
0.0458186566829681 0.375701993703842
0.0128678977489471 0.202200084924698
0.0151546001434326 0.168911084532738
0.0261233448982239 0.318100243806839
0.0445794463157654 0.0455336906015873
0.0245963037014008 0.217880859971046
0.0188260674476624 -0.331865221261978
0.0342843532562256 -0.169293761253357
0.0296277403831482 0.0540156029164791
0.02399080991745 -0.21193128824234
0.0218909382820129 0.488309562206268
0.0598553903400898 -0.270011305809021
0.0387842655181885 0.187496706843376
0.0189304351806641 0.14123497903347
0.0244303345680237 0.231759086251259
0.0192072987556458 0.475536555051804
0.0339722037315369 0.282884567975998
0.039178192615509 0.356558591127396
0.0404327511787415 -0.076293833553791
0.0343047976493835 0.281413286924362
0.0100252628326416 0.115930676460266
0.0280327796936035 0.429253548383713
0.00663000345230103 -0.55614447593689
0.00852799415588379 0.604398906230927
0.0340432524681091 0.419088929891586
0.0121119618415833 0.0465480349957943
0.0159433484077454 0.311990886926651
0.041784405708313 -0.258487164974213
0.00211071968078613 -0.452877402305603
0.0122518539428711 0.313101291656494
0.0263164937496185 0.137401819229126
0.00725048780441284 0.630468130111694
0.0314773917198181 -0.350294560194016
0.0436456799507141 -0.564812242984772
0.0539036393165588 -0.0348610393702984
0.0409272909164429 0.364612460136414
0.0293255150318146 0.114148110151291
0.0023687481880188 0.40926268696785
0.00314748287200928 0.59053909778595
0.00759753584861755 0.342819541692734
0.00791352987289429 0.421508699655533
0.0438152551651001 -0.199223190546036
0.0423831939697266 0.298526108264923
0.0353854894638062 -0.135289192199707
0.0276824235916138 0.147400766611099
0.0337398052215576 0.267516672611237
0.0243437886238098 -0.214668199419975
0.00909298658370972 0.375927001237869
0.00669723749160767 -0.187032148241997
0.0173200368881226 -0.20353801548481
0.0195884704589844 0.345617085695267
0.0166680216789246 0.0796019956469536
0.0498999953269958 0.19355034828186
0.059927761554718 0.162762433290482
0.0561398267745972 0.53116512298584
0.0096169114112854 0.236524730920792
0.0207808613777161 0.337593674659729
0.00726032257080078 -0.0166352707892656
0.0478167533874512 -0.0436776056885719
0.0304744839668274 -0.24714033305645
0.0295634269714355 0.296645045280457
0.0163841843605042 -0.346481651067734
0.0356666743755341 -0.108997128903866
0.0613210201263428 0.713615596294403
0.0292864739894867 0.342380672693253
0.0381020307540894 0.0712453573942184
0.0249340534210205 0.145622923970222
0.0370959937572479 0.0832581073045731
0.00523161888122559 -0.0218310914933681
0.0357050895690918 0.015103773213923
};
\addplot [semithick, red, opacity=0.4]
table {%
1.38777878078145e-17 0
0.0627450980392157 0
};
\addplot [semithick, red, opacity=0.4]
table {%
0.0313725490196079 -1
0.0313725490196079 1
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)$}) node[
  scale=0.75,
  text=black,
  rotate=0.0,
  yshift=-0.5cm
]{\textbf{\LARGE{Radius}}};
\draw ({$(current bounding box.south west)!0!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.55!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\textbf{\LARGE{Speed}}};
\end{tikzpicture}


==> ICLR_fig/NotUsed_VR_bar_fromClean40.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.5)},
  anchor=east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={multiple stacked bar plot},
x grid style={darkgray176},
xlabel={radius interval},
xmin=-0.5, xmax=1.5,
xtick style={color=black},
xtick={0.166666666666667,1.16666666666667},
xticklabels={
  {\(\displaystyle [\frac{0}{255},\frac{4}{255}]\)},
  \(\displaystyle >\frac{4}{255}\)
},
y grid style={darkgray176},
ylabel={speed proportion},
ymin=0, ymax=1.08230772167444,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180,line width=0pt] (axis cs:-0.25,0) rectangle (axis cs:0.0833333333333333,0.15384615957737);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180,line width=0pt}
\addlegendentry{negative}

\draw[draw=none,fill=steelblue31119180,line width=0pt] (axis cs:0.75,0) rectangle (axis cs:1.08333333333333,0);
\draw[draw=none,fill=darkorange25512714,line width=0pt] (axis cs:-0.25,0.15384615957737) rectangle (axis cs:0.0833333333333333,1.0307692438364);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkorange25512714,line width=0pt}
\addlegendentry{positive}



% \node [draw,fill=white] at (rel axis cs: 0.3,0.8) {\shortstack[l]{
% \ref{p4} ours \\
% \ref{p5} AT \\}};% xyc

\addlegendimage{empty legend}
   \addplot {sqrt(x)}; 
   \addplot {ln(x)}; 

   \addlegendentry{\hspace{-.6cm}\textbf{A title}}
   \addlegendentry{$\sqrt{x}$}
   \addlegendentry{$\ln{x}$}


\draw[draw=none,fill=darkorange25512714,line width=0pt] (axis cs:0.75,0) rectangle (axis cs:1.08333333333333,0.0307692307978868);
\draw[draw=none,fill=steelblue31119180,line width=0pt,postaction={pattern=fivepointed stars}] (axis cs:0.0833333333333333,0) rectangle (axis cs:0.416666666666667,0.292307704687119);
\draw[draw=none,fill=steelblue31119180,line width=0pt,postaction={pattern=fivepointed stars}] (axis cs:1.08333333333333,0) rectangle (axis cs:1.41666666666667,0.0307692307978868);
\draw[draw=none,fill=darkorange25512714,line width=0pt,postaction={pattern=fivepointed stars}] (axis cs:0.0833333333333333,0.292307704687119) rectangle (axis cs:0.416666666666667,1.03076925873756);
\draw[draw=none,fill=darkorange25512714,line width=0pt,postaction={pattern=fivepointed stars}] (axis cs:1.08333333333333,0) rectangle (axis cs:1.41666666666667,0);
\draw[draw=none,fill=gray] (axis cs:-0.4,0) rectangle (axis cs:0.4,0);
\draw[draw=none,fill=gray,postaction={pattern=fivepointed stars}] (axis cs:-0.4,0) rectangle (axis cs:0.4,0);
\end{axis}

\end{tikzpicture}



==> ICLR_fig/NotUsed_VR_bar_fromTrades90.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
title={proportion of positive and negative speed},
x grid style={darkgray176},
xlabel={radius interval},
xmin=-0.5, xmax=3.5,
xtick style={color=black},
xtick={0.166666666666667,1.16666666666667,2.16666666666667,3.16666666666667},
xticklabels={
  {\(\displaystyle [\frac{0}{255},\frac{4}{255}]\)},
  {\(\displaystyle [\frac{4}{255},\frac{8}{255}]\)},
  {\(\displaystyle [\frac{8}{255},\frac{12}{255}]\)},
  \(\displaystyle >\frac{12}{255}\)
},
y grid style={darkgray176},
ylabel={speed proportion},
ymin=0, ymax=0.309137061238289,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180,line width=0pt] (axis cs:-0.25,0) rectangle (axis cs:0.0833333333333333,0.0355329960584641);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180,line width=0pt}
\addlegendentry{negative}

\draw[draw=none,fill=steelblue31119180,line width=0pt] (axis cs:0.75,0) rectangle (axis cs:1.08333333333333,0.0812182724475861);
\draw[draw=none,fill=steelblue31119180,line width=0pt] (axis cs:1.75,0) rectangle (axis cs:2.08333333333333,0.0507614202797413);
\draw[draw=none,fill=steelblue31119180,line width=0pt] (axis cs:2.75,0) rectangle (axis cs:3.08333333333333,0.162436544895172);
\draw[draw=none,fill=darkorange25512714,line width=0pt] (axis cs:-0.25,0.0355329960584641) rectangle (axis cs:0.0833333333333333,0.243654817342758);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkorange25512714,line width=0pt}
\addlegendentry{positive}

\draw[draw=none,fill=darkorange25512714,line width=0pt] (axis cs:0.75,0.0812182724475861) rectangle (axis cs:1.08333333333333,0.284263953566551);
\draw[draw=none,fill=darkorange25512714,line width=0pt] (axis cs:1.75,0.0507614202797413) rectangle (axis cs:2.08333333333333,0.177664969116449);
\draw[draw=none,fill=darkorange25512714,line width=0pt] (axis cs:2.75,0.162436544895172) rectangle (axis cs:3.08333333333333,0.294416233897209);
\draw[draw=none,fill=steelblue31119180,line width=0pt,postaction={pattern=north west lines}] (axis cs:0.0833333333333333,0) rectangle (axis cs:0.416666666666667,0.0710659921169281);
\draw[draw=none,fill=steelblue31119180,line width=0pt,postaction={pattern=north west lines}] (axis cs:1.08333333333333,0) rectangle (axis cs:1.41666666666667,0.101522840559483);
\draw[draw=none,fill=steelblue31119180,line width=0pt,postaction={pattern=north west lines}] (axis cs:2.08333333333333,0) rectangle (axis cs:2.41666666666667,0.0761421322822571);
\draw[draw=none,fill=steelblue31119180,line width=0pt,postaction={pattern=north west lines}] (axis cs:3.08333333333333,0) rectangle (axis cs:3.41666666666667,0.147208124399185);
\draw[draw=none,fill=darkorange25512714,line width=0pt,postaction={pattern=north west lines}] (axis cs:0.0833333333333333,0.0710659921169281) rectangle (axis cs:0.416666666666667,0.243654817342758);
\draw[draw=none,fill=darkorange25512714,line width=0pt,postaction={pattern=north west lines}] (axis cs:1.08333333333333,0.101522840559483) rectangle (axis cs:1.41666666666667,0.284263961017132);
\draw[draw=none,fill=darkorange25512714,line width=0pt,postaction={pattern=north west lines}] (axis cs:2.08333333333333,0.0761421322822571) rectangle (axis cs:2.41666666666667,0.17766497284174);
\draw[draw=none,fill=darkorange25512714,line width=0pt,postaction={pattern=north west lines}] (axis cs:3.08333333333333,0.147208124399185) rectangle (axis cs:3.41666666666667,0.29441624879837);
\end{axis}

\end{tikzpicture}


==> Intepretation_fig/old_figs/VR_AT_batch.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 5, acc :0.05},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.350645005702972 -0.357723206281662
0.032988291233778 -0.486761838197708
0.330953687429428 -0.0590110011398792
0.100467517971992 0.0715076699852943
0.137557923793793 0.0219248458743095
0.811247408390045 0.121164225041866
0.103034511208534 -0.0297818537801504
0.189304903149605 -0.116679713129997
0.113716632127762 0.445871919393539
0.416331261396408 0.204105973243713
0.519475936889648 -0.151445850729942
0.203828752040863 0.312905430793762
0.0601491741836071 0.338853299617767
0.255471736192703 0.328302353620529
0.103730417788029 -0.116220876574516
0.0261005666106939 0.150126472115517
0.0501029565930367 -0.262186378240585
0.756886839866638 0.524324417114258
0.267878472805023 0.368259400129318
0.251713901758194 0.546439170837402
0.457593888044357 -0.271094143390656
0.183898970484734 0.392179191112518
0.119350478053093 0.571984052658081
0.0769779458642006 0.090003177523613
0.234430804848671 0.404512196779251
0.0562266372144222 -0.0791343525052071
0.127323001623154 0.513573050498962
0.0684164762496948 0.155859962105751
0.204327255487442 -0.0880387648940086
0.0645019561052322 0.0647444948554039
0.172217562794685 -0.143741816282272
0.131110936403275 0.288698792457581
0.21003420650959 0.109185792505741
0.146040111780167 0.0116304159164429
0.18724325299263 0.23796221613884
0.402036100625992 0.424848705530167
0.0992129817605019 -0.115779370069504
0.0562263764441013 -0.0420425161719322
0.326883912086487 -0.4439677298069
0.0436937250196934 0.667995870113373
0.305925846099854 -0.384215444326401
0.4162437915802 0.285722553730011
0.322295606136322 0.592745840549469
0.124569460749626 0.142490103840828
0.0926206409931183 -0.0949237495660782
0.0212574880570173 0.125102773308754
0.114094875752926 0.559446692466736
0.0737206488847733 0.0302012991160154
0.237461552023888 0.528270363807678
0.148140102624893 0.463552862405777
0.22330729663372 0.840555489063263
0.438821166753769 0.371557235717773
0.0766104534268379 0.0580061078071594
0.0959797948598862 0.0672186464071274
0.36248654127121 0.196665167808533
0.085233598947525 -0.342096537351608
0.59651643037796 0.346522748470306
0.654286801815033 -0.246374428272247
0.246844440698624 0.930977880954742
0.351297229528427 -0.818039834499359
0.271543473005295 -0.192875057458878
0.299106121063232 -0.123107925057411
0.286141693592072 0.169598326086998
0.240220785140991 0.515935957431793
0.183167889714241 -0.0634122639894485
0.147648617625237 -0.190516233444214
0.213482320308685 -0.152524769306183
0.264887064695358 0.160409674048424
0.136962324380875 0.129906058311462
0.299153000116348 0.162912800908089
0.0348413102328777 -0.366237670183182
0.179535657167435 0.292125195264816
0.148379668593407 -0.55539745092392
0.0826730877161026 0.0902420654892921
0.582082092761993 -0.309556901454926
0.249333426356316 0.108124680817127
0.174837186932564 0.246677726507187
0.136317983269691 0.409960836172104
0.0430640690028667 0.281636446714401
0.189717635512352 0.296601206064224
0.18142831325531 0.189988970756531
0.0504078157246113 -0.126064315438271
0.110103860497475 0.0838920250535011
0.38933926820755 -0.252994567155838
0.289481431245804 0.349475681781769
0.496591567993164 0.946863353252411
0.0347103402018547 0.349300503730774
0.120276190340519 0.241603434085846
0.207154765725136 0.196084141731262
0.20856636762619 -0.233816146850586
0.0994263216853142 0.41433984041214
0.270468384027481 0.26143005490303
0.176049172878265 0.106662437319756
0.0437592342495918 0.155652359127998
0.212465986609459 0.137116283178329
0.189470648765564 -0.045875396579504
0.0878495946526527 -0.199956953525543
0.21386706829071 -0.152641668915749
0.0727341994643211 0.779003083705902
0.0814841389656067 0.519287884235382
0.171644046902657 -0.288103848695755
0.148351356387138 0.212449431419373
0.130700752139091 0.0409677214920521
0.34176504611969 -0.617099225521088
0.347665637731552 0.250591725111008
0.254938453435898 0.335430234670639
0.0973600819706917 0.261321276426315
0.0686248242855072 -0.462053388357162
0.0941711738705635 0.0391701757907867
0.165108248591423 -0.0265249218791723
0.0409367121756077 -0.27935254573822
0.0858509838581085 0.259572058916092
0.125789448618889 0.0103885801509023
0.364816635847092 -0.659589767456055
0.149800792336464 0.182640925049782
0.0288141574710608 -0.416706055402756
0.206090658903122 -0.448603600263596
0.0811603590846062 -0.255574852228165
0.288149744272232 0.33720275759697
0.649249970912933 0.330084711313248
0.089029036462307 0.086382769048214
0.0948949903249741 -0.377299189567566
0.358723700046539 -0.096101701259613
0.342412024736404 0.202205181121826
0.149430453777313 0.121697001159191
0.0908585265278816 0.356336057186127
0.275557279586792 0.284507125616074
0.262685656547546 0.184394404292107
0.185031563043594 -0.160783991217613
0.0803507417440414 -0.314200878143311
0.118128083646297 -0.0714240521192551
0.234431535005569 0.229737654328346
0.193430423736572 -0.0780361667275429
0.205365285277367 0.228854045271873
0.0999405607581139 -0.140404060482979
0.169778659939766 0.428475022315979
0.22930084168911 -0.0904056057333946
0.229325965046883 -0.155608415603638
0.156088829040527 -0.392003059387207
0.171000882983208 0.194703713059425
0.301906079053879 -0.100361213088036
0.176634088158607 -0.184982344508171
0.277097702026367 -0.588073968887329
0.0953186973929405 0.417231619358063
0.157846078276634 0.133044868707657
0.277929663658142 0.187186434864998
0.114235885441303 0.0581273287534714
0.134568586945534 0.0143716912716627
0.163922965526581 0.329766780138016
0.117034330964088 0.131119087338448
0.161064058542252 0.779893279075623
0.367609441280365 0.535443723201752
0.367694854736328 0.400110304355621
0.284291207790375 0.154774934053421
0.156717449426651 0.336863994598389
0.125651076436043 -0.154326811432838
0.0964546650648117 0.29834195971489
0.0751386508345604 0.171300053596497
0.227249190211296 0.527051210403442
0.23503278195858 0.773120939731598
0.0959869176149368 0.174097582697868
0.0399644300341606 0.191198632121086
0.171021997928619 0.165892660617828
0.470004677772522 0.283311128616333
0.0916483700275421 0.249542698264122
0.168057933449745 0.473415672779083
0.327438145875931 0.155924648046494
0.107134126126766 -0.0887699350714684
0.150853589177132 0.204368457198143
0.125263407826424 0.343882769346237
0.216423183679581 -0.0628196448087692
0.124283783137798 0.210597082972527
0.0793389678001404 0.388988524675369
0.218459904193878 0.246756732463837
0.0969680771231651 0.165721446275711
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 30, acc :0.36},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.619149625301361 0.888363301753998
0.0992287844419479 -0.0746122151613235
0.276408791542053 0.50996196269989
0.0743011683225632 -0.0300678145140409
0.44954314827919 0.588335871696472
0.784701466560364 0.1615159958601
0.0723130851984024 -0.876141905784607
0.194621443748474 -0.147653311491013
0.077987365424633 -0.0414864383637905
0.348132640123367 0.306459754705429
0.588421523571014 0.807112097740173
0.155239924788475 0.103738911449909
0.486647814512253 0.511501848697662
0.453481465578079 -0.326330125331879
0.213571324944496 0.118983186781406
0.947776734828949 -0.0508342944085598
0.263468474149704 0.052522785961628
0.73992657661438 0.327501177787781
0.885561108589172 0.952053308486938
0.0441741719841957 0.262268513441086
0.0689827650785446 -0.194756671786308
0.132024422287941 0.0381546057760715
0.317432820796967 -0.631633281707764
0.28329011797905 0.0789422020316124
0.184335350990295 0.947141349315643
0.337990254163742 0.273077130317688
0.0604018792510033 0.362208843231201
0.113609164953232 -0.0655749440193176
0.42327344417572 0.0546469204127789
0.167218208312988 0.154221788048744
0.283691734075546 0.131770342588425
0.518378734588623 0.532950699329376
0.141578108072281 0.324249118566513
0.354207962751389 -0.209533154964447
0.502260267734528 0.255975484848022
0.293110609054565 -0.0105929933488369
0.489076048135757 -0.0156403835862875
0.59712678194046 -0.200137913227081
0.293781965970993 0.101877339184284
0.325056433677673 0.387288361787796
0.076129823923111 -0.371416985988617
0.0944776609539986 0.353510469198227
0.349228054285049 0.209271743893623
0.599030554294586 0.50484174489975
0.140048429369926 -0.0181178972125053
0.268550038337708 -0.0683050155639648
0.380881875753403 0.269654542207718
0.271197736263275 0.518267810344696
0.156889528036118 0.082746796309948
0.420875787734985 -0.10366690158844
0.156684398651123 -0.0166249331086874
0.583673000335693 0.0741156190633774
0.193766489624977 -0.346061766147614
0.34925302863121 0.825122892856598
0.260235190391541 -0.0351118557155132
0.441181480884552 0.0593037679791451
0.262469440698624 0.194318309426308
0.172139823436737 -0.0245782807469368
0.123639211058617 0.161980137228966
0.0450788624584675 0.161659225821495
0.342057585716248 0.118125483393669
0.765700340270996 -0.0245211645960808
0.188139691948891 0.0039767948910594
0.355153858661652 0.662798762321472
0.57869690656662 0.133868709206581
0.218011781573296 0.418633490800858
0.590532183647156 0.166880637407303
0.502491116523743 0.406870812177658
0.247952789068222 0.144148647785187
0.259017378091812 -0.0552391558885574
0.204664543271065 -0.391686379909515
0.46842148900032 0.640620112419128
0.769041359424591 -0.40487802028656
0.309852778911591 0.619339287281036
0.584691643714905 0.383913964033127
0.316296249628067 0.310224324464798
0.240607425570488 0.503841996192932
0.249369949102402 0.284216850996017
0.215093567967415 0.481251418590546
0.105120792984962 0.0773545205593109
0.388253301382065 0.354287713766098
0.283635139465332 0.548295438289642
0.19461452960968 -0.324431627988815
0.0511402301490307 0.0726238340139389
0.820546329021454 0.37612122297287
0.157271549105644 -0.812458038330078
0.0995548292994499 -0.0822097435593605
0.892615079879761 0.0380958653986454
0.240698829293251 0.226501479744911
0.092851884663105 -0.031473733484745
0.35888808965683 0.718474924564362
0.0629680678248405 -0.0286520849913359
0.24188195168972 0.499620646238327
0.0525473840534687 -0.00303523428738117
0.13897493481636 0.79558277130127
0.168637901544571 -0.210350051522255
0.651881396770477 0.0661248341202736
0.141339153051376 0.228474229574203
0.410384654998779 -0.0572669319808483
0.48826265335083 0.462841838598251
0.267695367336273 -0.18343597650528
0.422782212495804 0.647741973400116
0.1813013702631 -0.101537711918354
0.314691781997681 0.0689489990472794
0.148449346423149 0.227359145879745
0.413541913032532 0.527271449565887
0.0832350105047226 0.895080983638763
0.239014640450478 -0.00103274150751531
0.614172279834747 0.476278245449066
0.742042303085327 0.0760700926184654
0.199159517884254 -0.564290046691895
0.165275260806084 0.229595646262169
0.306859105825424 0.0486879572272301
0.0393349081277847 -0.139342069625854
0.472904622554779 0.485097676515579
0.0436616018414497 -0.184588357806206
0.312122702598572 -0.304411828517914
0.900634765625 0.373908847570419
0.215540260076523 0.204494565725327
0.223173350095749 -0.101794935762882
0.716811239719391 -0.116718426346779
0.0531153082847595 0.775596022605896
0.254649847745895 -0.272706568241119
0.361141890287399 0.468778043985367
0.260849148035049 0.0720051899552345
0.4657321870327 0.369934916496277
0.590206921100616 0.227232918143272
0.213428065180779 -0.242548286914825
0.224101990461349 0.524737179279327
0.0626158565282822 -0.300854176282883
0.363197654485703 0.445196032524109
0.107756420969963 0.0453313104808331
0.090922512114048 -0.149762168526649
0.295974344015121 0.237063005566597
0.237810462713242 0.150068715214729
0.0567120127379894 -0.0698353499174118
0.327143162488937 0.0311995819211006
0.135956883430481 0.589147627353668
0.245569184422493 0.0101377489045262
0.183352932333946 0.622481644153595
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 700, acc :0.66},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.689801454544067 -0.212765321135521
0.593709647655487 -0.661541998386383
0.541443943977356 0.163858488202095
0.408217698335648 0.167099431157112
0.228866264224052 0.22038197517395
0.102096810936928 -0.159865185618401
0.0479068197309971 0.148817285895348
0.58553159236908 0.609703242778778
0.535767495632172 0.511780321598053
0.877086818218231 -0.900572299957275
0.987158536911011 0.164092764258385
0.215921133756638 -0.176576241850853
0.178981497883797 0.205264329910278
0.730333983898163 -0.148238718509674
0.808446168899536 0.443064749240875
0.592310786247253 0.563195884227753
0.245124235749245 -0.329326629638672
0.811948657035828 0.138793870806694
0.135625883936882 -0.230562388896942
0.777814567089081 0.0166796389967203
0.171816572546959 -0.118321515619755
0.103339180350304 0.339708358049393
0.895827889442444 -0.322716653347015
0.702014625072479 -0.0435676388442516
0.56940770149231 -0.00891394354403019
0.386584222316742 -0.0557840317487717
0.553413510322571 0.26427760720253
0.653706848621368 -0.138313800096512
0.300156027078629 0.262248694896698
0.828290581703186 0.135777503252029
0.353922128677368 -0.624431014060974
0.0770003274083138 0.106573708355427
0.518802762031555 0.0281285252422094
0.752460181713104 0.115507684648037
0.798154413700104 0.20286850631237
0.821331024169922 0.306026071310043
0.411080181598663 -0.489523619413376
0.469866901636124 0.00978597160428762
0.321152687072754 0.137494087219238
0.22759148478508 -0.335720539093018
0.177372977137566 0.392431974411011
0.593092262744904 -0.649705946445465
0.435600608587265 0.251847714185715
0.284750282764435 0.0126855885609984
0.943131327629089 0.0533225610852242
0.56761234998703 0.321890771389008
0.511895895004272 -0.302614629268646
0.510650634765625 0.553082227706909
0.383196026086807 -0.349745690822601
0.860490024089813 0.283787578344345
0.359424978494644 0.588446795940399
0.640754282474518 0.221349820494652
0.975925862789154 -0.054689098149538
0.376894801855087 0.616307854652405
0.697652161121368 0.54290384054184
0.799412369728088 0.398022592067719
0.584270775318146 -0.18210756778717
0.758255779743195 -0.00682881660759449
0.902950525283813 0.295697867870331
0.42943087220192 -0.141662687063217
0.618948459625244 0.214959189295769
0.47428834438324 -0.108898587524891
0.472959756851196 -0.194146081805229
0.537133514881134 -0.51135516166687
0.740495562553406 0.393499344587326
0.604780972003937 0.189485758543015
0.341991007328033 -0.0231794454157352
0.867071807384491 -0.609186828136444
0.851353704929352 0.487200915813446
0.860606610774994 -0.169017747044563
0.89232075214386 0.20709440112114
0.758271515369415 -0.0775540396571159
0.293827503919601 -0.0349501520395279
0.137665495276451 -0.0536527335643768
0.2071832716465 0.0656734332442284
0.137557700276375 -0.387925982475281
0.562016665935516 -0.152189061045647
0.165530726313591 -0.536406815052032
0.185333624482155 0.444874227046967
0.476507902145386 -0.110809840261936
0.552840292453766 -0.481717586517334
0.124422013759613 -0.0421370938420296
0.720729947090149 -0.108860559761524
0.358562886714935 0.104559525847435
0.573173642158508 0.169043511152267
0.463675916194916 0.351596027612686
0.645137429237366 -0.160961881279945
0.273621022701263 -0.107030607759953
0.173978880047798 0.472541838884354
0.528478264808655 0.573837041854858
0.933867275714874 0.682271599769592
0.157988607883453 -0.184272632002831
0.152687832713127 -0.641091227531433
0.489222049713135 -0.551352441310883
0.564649522304535 -0.0339494943618774
0.956498980522156 -0.692932367324829
0.961239635944366 -0.620947360992432
0.403791844844818 -0.492436230182648
0.267133116722107 -0.570857584476471
0.980686902999878 0.215895161032677
0.87985360622406 -0.146546125411987
0.560641646385193 -0.170701742172241
0.973293960094452 0.238160997629166
0.152638882398605 0.47105398774147
0.16191491484642 -0.069906197488308
0.482714772224426 -0.242741569876671
0.761951982975006 0.209079846739769
0.240731343626976 0.494243651628494
0.499020010232925 -0.411942988634109
0.34525254368782 -0.00691070314496756
0.668302297592163 -0.176308006048203
0.574423730373383 -0.0884093269705772
0.688857555389404 0.224692434072495
0.742052733898163 -0.010528227314353
0.428939551115036 -0.305193394422531
0.0580147430300713 -0.00735436612740159
0.426440864801407 0.211718693375587
0.839732229709625 0.0878208354115486
0.515936970710754 0.170672819018364
0.115300729870796 0.432935744524002
0.612647533416748 -0.0895610824227333
0.118362128734589 -0.43669581413269
0.312649726867676 0.63465029001236
0.911286175251007 0.264877796173096
0.207927972078323 -0.100341863930225
0.542215287685394 -0.199132934212685
0.895475268363953 0.0232708640396595
0.621709287166595 0.0403514206409454
0.890581727027893 -0.67852109670639
0.701946020126343 -0.107988946139812
0.273480862379074 0.485845595598221
0.829027414321899 -0.0654142573475838
0.75367534160614 -0.100045658648014
0.881464123725891 -0.181556761264801
0.401667505502701 0.170745566487312
0.709093928337097 0.174355000257492
0.217891678214073 0.500052809715271
0.437098801136017 0.427840441465378
0.216918900609016 -0.018059529364109
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.01!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=south,
  text=black,
  rotate=0.0
]{Radius};
\draw ({$(current bounding box.south west)!0.02!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=west,
  text=black,
  rotate=90.0
]{Speed};
\end{tikzpicture}


==> Neurips/a1_speed_derivation.tex <==
\section{Proof of the closed-form expression for the speed 
in Equation \eqref{eq: expression_for_speed}
} \label{app: closed_expression_speed}

In this section, our goal is to prove the closed-form expression~\eqref{eq: expression_for_speed} and provide further discussions. We first provide two preliminary lemmas and present the mathematical assumptions. Then we rigorously derive the closed-form expression. Finally, we discuss more about the expression and its assumptions. 

\begin{lemma} \label{lemma: norm_pq_app}
For $1\leq p \leq \infty$ and let $q$ satisfies $1/q+1/p=1$. Let $a$ be any fixed vector. Then 
\begin{equation*} 
    \left\|\nabla_x \left\|x-a\right\|_p\right\|_q = 1
\end{equation*}
\end{lemma}

\begin{proof}
Without loss of generality, assume $a$ is the zero vector. Write the $k$-th component of $x$ as $x_k$.

\emph{Case 1: $1\leq p < \infty$}

By calculation, $\frac{\partial \|x\|_p}{\partial x_k} = (\frac{|x_k|}{\|x\|_p})^{p-1}\cdot \sign (x_k)$. Since $q = \frac{p}{p-1}$, we have that 
\begin{equation*}
\begin{aligned}
\sum_k |\frac{\partial \|x\|_p}{\partial x_k}|^{q} &= \sum_k  |(\frac{|x_k|}{\|x\|_p})^{p-1}\cdot \sign (x_k)|^{\frac{p}{p-1}} \\
&= \sum_k \frac{|x_k|^p}{\|x\|_p^p} \\
&= 1
\end{aligned}
\end{equation*}

Therefore, $\left\|\nabla_x \left\|x\right\|_p\right\|_q = (\sum_k |\frac{\partial \|x\|_p}{\partial x_k}|^{q})^{1/q} = 1$.

\emph{Case 2: $p = \infty$}

In this case, $\nabla_x \|x\|_\infty$ is a one-hot vector (with the one being the position of the element of $x$ with the largest absolute value). Therefore, $\left\|\nabla_x \left\|x\right\|_{\infty}\right\|_1$ = 1. 

\end{proof}

The following lemma deals with the optimality condition for $p = \infty$. Special care needs to be taken since $L_\infty$ norm is not a differentiable function.

\begin{lemma} \label{lemma: Linf_optimality_app}
Let $\hat{x}$ be a local optimum of the constrained optimization problem: 
\begin{equation*} \label{eq: closest_linf_app}
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
    \hat{x} = \argmin_{z} \|x-a\|_\infty \quad \textrm{s.t.}  \quad \phi(x) = 0,
\end{equation*}
where $a$ is any fixed vector with $\phi(a) > 0$.
Assume that $\phi$ is differentiable at point $\hat{x}$. Denote the coordinates set $\mathcal{J} = \{j: |\hat{x}_j - a_j| = \|\hat{x}-a\|_\infty\}$. Denote the $k$-th component of $\nabla_x \phi(\hat{x})$ as $\nabla_x \phi(\hat{x})_k$. Then (a) for $j \in \mathcal{J}$, $\nabla_x \phi(\hat{x})_j$ and $\hat{x}_j - a_j$ have opposite signs; (b) for $k\notin \mathcal{J}$, $\nabla_x \phi(\hat{x})_k = 0$. 
\end{lemma}

\begin{remark*}
If $\phi(a)<0$, then (a) for $j \in \mathcal{J}$, $\nabla_x \phi(\hat{x})_j$ and $\hat{x}_j - a_j$ have the same sign; (b) for $k\notin \mathcal{J}$, $\nabla_x \phi(\hat{x})_k = 0$.
\end{remark*}

\begin{proof}
\emph{(a)}
Consider the perturbation $\hat{x}(\epsilon) = \hat{x} + (0,\cdots,\epsilon_{j_1},\cdots,\epsilon_{j_m},\cdots,0)$ where $\mathcal{J} = \{j_1,\cdots,j_m\}$ and $\epsilon$ is a $m$ dimensional vector with $j$-th component $\epsilon_j$. Since $\phi(a)>0$ and $\hat{x}$ is a local optimum, $\|x-a\|_\infty < \|\hat{x}-a\|_\infty$ imply $\phi(x) > 0$ if $x$ is sufficiently close to $\hat{x}$. Therefore, if every $\epsilon_{j_i}$ is chosen so that $|\hat{x}_{j_i} + \epsilon_{j_i} - a_{j_i}| < |\hat{x}_{j_i} - a_{j_i}|$ (that is, $\epsilon_{j_i}$ has different sign from $\hat{x}_{j_i} - a_{j_i}$) and $\|\epsilon\|$ sufficiently small, then $\|\hat{x}(\epsilon) - a\| < \|\hat{x}-a\|$ and thus $\phi(\hat{x}(\epsilon))>0$. 

On the other hand, by Taylor expansion and the fact that $\phi(\hat{x})=0$, we have that 

\begin{equation*}
    \phi(\hat{x}(\epsilon)) = \sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j + \mathcal{O}(\|\epsilon\|^2)
\end{equation*}

Therefore, $\sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j > 0$ for any such $\epsilon$. By taking other $\epsilon_k \to 0$ if necessary, we obtain that $\forall j \in \mathcal{J}$, $\nabla \phi(\hat{x})_j \epsilon_j \geq 0$, where $\epsilon_j$ has different sign from $\hat{x}_{j} - a_{j}$. Therefore, $\nabla \phi(\hat{x})_j$ and $\hat{x}_{j} - a_{j}$ have different signs. 


\emph{(b)}
Take any $k \notin \mathcal{J}$ and consider the perturbation $\hat{x}(\epsilon) = \hat{x} + (0,\cdots,\epsilon_{j_1},\cdots,\epsilon_k,\cdots,\epsilon_{j_k},\cdots,0)$ where $\epsilon=(\epsilon_{j_1},\cdots,\epsilon_k,\cdots,\epsilon_{j_k})$. Choose any $\epsilon$ so that $\|\epsilon\|$ is sufficiently small, each $\epsilon_{j_i}$ has the opposite sign of $\hat{x}_{j_i} - a_{j_i}$ and $\epsilon_k$ small enough (which can be positive or negative), we have that $\phi(\hat{x}(\epsilon)) > 0$ since $\|\hat{x}(\epsilon) - a\|_\infty < \|\hat{x}-a\|_\infty$. By Taylor expansion, $\sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j + \epsilon_k \nabla_x \phi(\hat{x})_k > 0$ for any such $\epsilon$. By taking $\epsilon_j \to 0$ and using the fact that $\epsilon_k$ can be positive or negative, we conclude that $\nabla_x \phi(\hat{x})_k = 0$.

\end{proof}


Now we are ready to derive the closed-form expression of the speed. We first provide the full assumptions, then derive the expression, and finally we will discuss more about the assumptions. We will write $\hat{x}_i(t)$ as $\hat{x}_i$ when the indication is clear. 
\begin{assumption} \label{assumption: differentible}
Suppose that $(x_i,y_i)$ is correctly classified by $f_{\theta(t)}$ in some time interval $t \in I$ and $\hat{x}_i(t)$ is a locally closest boundary point in the sense that for any $t\in I$, it is the local optimum of the following:
\begin{equation*} 
    \hat{x}_i(t) = \argmin\nolimits_{\hat{x}} \|\hat{x}-x_i\|_p \quad \textrm{s.t.}  \quad \phi^{y_i}(\hat{x},\theta(t)) = 0.
\end{equation*}
Assume that in the time interval $I$: (a) $\hat{x}_i(t)$ is differentiable in $t$; (b) $\phi^{y_i}$ is differentiable at point $\hat{x}_i(t)$ and at the current parameter $\theta(t)$.
\end{assumption}


\begin{proposition*}[Closed-form expression of the speed $s(x_i,t)$] For $1 \leq p \leq \infty$ and under Assumption~\ref{assumption: differentible}, define the (local) speed according to $\hat{x}_i(t)$ in Assumption~\ref{assumption: differentible} as $s(x_i,t) = \frac{d}{dt}\|\hat{x}_i(t) - x_i\|_p$, we have the following:

\begin{equation*} 
    s(x_i,t) = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)
\end{equation*}
where $q$ satisfies that $1/q+1/p=1$. In particular, $q=2$ when $p=2$ and $q=1$ when $p=\infty$.
\end{proposition*}

\begin{proof}
\emph{Case 1: $1\leq p < \infty$}

To compute $ s(x_i,t) = \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_2$, we need to characterize the curve of the closest boundary point $\hat{x}_i(t)$, where two key points stand out. First, $\hat{x}_i(t)$ is on the decision boundary $\Gamma_y (t)$ and thus  $\phi^y(\hat{x}_i(t),\theta(t)) = 0$ for all $t \in I$. By taking the time derivative on both sides, we obtain the level set equation \citep{osher2004level,aghasi2011parametric}

\begin{equation} \label{eq: LF_app}
	\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\cdot \hat{x}_i'(t) + \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) = 0
\end{equation}

Second, $\hat{x}_i(t)$ is the optimal solution of constrained optimization \eqref{eq: closest_pt}. Therefore, we have the following optimality condition:

\begin{equation} \label{eq: optimality_app}
    \nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t)) + \lambda(t)\nabla_x\|\hat{x}_i(t)-x_i\|_p = 0
\end{equation}

Since $x_i$ is correctly classified, $\phi^{y_i}(x_i) > 0$. Since $\hat{x}_i(t)$ is the closest point to $x_i$ whose $\phi^{y_i}$ value is zero, $\lambda(t) >0$. By taking the $L_q$ norm in Equation~\eqref{eq: optimality_app} and using Lemma~\ref{lemma: norm_pq_app}, we obtain that $\lambda(t) = \|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q$.

Now, we derive $s(x_i,t)$ as follows:

\begin{equation*}
\begin{aligned}
    s(x_i,t) &= \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_p  \\
    & = \nabla_x\|\hat{x}_i(t)-x_i\|_p \cdot \hat{x}_i'(t) \\
    & = -\frac{1}{\lambda} \nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t)) \cdot \hat{x}_i'(t) && \text{(By the optimality condition~\eqref{eq: optimality_app})} \\
    & = \frac{1}{\lambda} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) && \text{(By the level set equation~\eqref{eq: LF_app})}\\
    & = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x \phi^{y}(\hat{x}_i(t),\theta(t))\|_q}  
\end{aligned}
\end{equation*}

\emph{Case 2: $p = \infty$}

Note that since $L_\infty$ is not differentiable, the optimality condition in Equation~\eqref{eq: optimality_app} does not hold anymore. 

Denote the $j$-th component of $\hat{x}_i(t)$ and $x_i$ as $\hat{x}_{ij}(t)$ and $x_{ij}$. Let $\mathcal{J} = \{j: |\hat{x}_{ij}(t) - x_{ij}| = \|\hat{x}_i(t)-x_i\|_\infty\}$. By Lemma~\ref{lemma: Linf_optimality_app}, $s(x_i,t) = \frac{d}{dt}|\hat{x}_{ij}(t) - x_{ij}| = \hat{x}_{ij}^{'}(t) \sign (\hat{x}_{ij}(t)-x_{ij}) = - \hat{x}_{ij}^{'}(t) \sign (\nabla_x\phi^{y_i}(\hat{x}_{i})_j)$ for all $j \in \mathcal{J}$. Therefore, by Equation~\eqref{eq: LF_app} and Lemma~\ref{lemma: Linf_optimality_app}

\begin{equation*}
\begin{aligned}
- \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) &= \nabla_x \phi^{y_i}(\hat{x})\cdot \hat{x}_i'(t)\\
&= \sum_{j \in \mathcal{J}} \nabla_x \phi^{y_i}(\hat{x}_i)_j\cdot \hat{x}_{ij}'(t) \\
&= \sum_{j \in \mathcal{J}} - \nabla_x \phi^{y_i}(\hat{x}_i)_j \cdot \frac{s(x_i,t)}{\sign (\nabla_x\phi^{y}(\hat{x}_{i})_j)} \\
&= - \sum_{j \in \mathcal{J}} |\nabla_x\phi^{y_i}(\hat{x}_{i})_j| \cdot s(x_i,t)
\end{aligned}
\end{equation*}

Therefore, $s(x_i,t) = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\sum_{j \in \mathcal{J}} |\nabla_x\phi^{y_i}(\hat{x}_{i})_j|} = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x\phi^{y_i}(\hat{x}_{i})\|_1}$, where the last equality follows from Lemma~\ref{lemma: Linf_optimality_app} that the components of $\nabla_x \phi^{y_i}(\hat{x}_i)$ are zeros if they are not in $\mathcal{J}$.
 
\end{proof}

\subsection*{Discussions on the assumptions}
Assumption~\ref{assumption: differentible} has several points that need to be explained further.

First, we only require that $\hat{x}_i(t)$ is a local closest boundary point. This is important because in practice when an algorithm for searching the closest boundary point is used (e.g. FAB), a local solution is the best one can hope for due to the non-convex nature of the optimization problem. When $\hat{x}_i(t)$ is a local solution, the speed should be interpreted as how fast the distance changes around that local solution. In this case, although $\hat{x}_i$ is not the globally closest adversarial example, the local speed around $\hat{x}_i$ still has much information on the relative movement of the decision boundary w.r.t. $x_i$, especially when the distance  $\|\hat{x}_i - x_i\|$ is relatively small and the input space is a high-dimensional space (e.g. pixel space). 

Second, we require that $\hat{x}_i(t)$ is a differentiable curve in time interval $I$. Note that if we constrain $\hat{x}_i(t)$ to be the global closest boundary point, $\hat{x}_i$ is unlikely to be differential for a large time interval $I$, especially in high dimensional space. This is because as the decision boundary moves. the closest point might switch from one point to another point that is very far away abruptly. Fortunately, this problem is alleviated because our derived closed-form expression still works when $\hat{x}_i(t)$ is a locally closest boundary point. Note that however, due to the \textit{topological change} of the decision boundary, it still can happen that $\hat{x}_i(t)$ stops existing (and thus stops being differentiable) at some time point, when typically the speed will go to infinity. From a mathematical point of view, this is related to \textit{shock} in partial differential equation (PDE) theories. More exploration on this is left to future work. In this work, we only consider the speed of the decision boundary at each discrete time step.


==> Neurips/a2_method_details.tex <==
\section{Algorithms}

\subsection{Details of the optimization problem \eqref{eq:opt_for_weight}} \label{app: opt_for_weight}

In this section, we provide details of the optimization problem~\eqref{eq:opt_for_weight} by specifying the coefficients of this quadratic programming concretely using the neural network gradients $\nabla_x \phi^{y_i}(\hat{x}_i)$ and  $\nabla_\theta \phi^{y_i}(\hat{x}_i)$.

\subsubsection{The dependency between the weights and the speed}

First, we give the details of $\mathbf{s}(\mathbf{c})$, i.e. how the weights $\mathbf{c} = (c_1,\cdots, c_m)^{T}$ (linearly) determines the speed $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$. Recall that the dimension of the parameters $\theta$ is $p$, and the number of points in $\mathcal{B}_\theta^{+}$ is $m$. 

% theta'
\paragraph{The update rule $\theta'$} The weights $\mathbf{c}$ determines the update rule $\theta_k'$ as follows. We write $\theta'_k$ as $\theta' = \sum_{i\in \mathcal{B}_\theta^{+}}c_i\nabla_\theta \phi^{y_i}(\hat{x}_i) + z$, where the step index $k$ is omitted and $z$ includes terms that do not depend on the weights $\mathbf{c}$. In this paper, we use SGD with momentum and weight decay (which is commonly used in AT methods) and thus the relationship between $\theta'$ and the loss function is given by Equation~\eqref{eq: theta prime momentum weight decay general}. In this case, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$, where $\lambda_c$, $\lambda_w$ and $\lambda_m$ are coefficients for the clean loss, weight decay and momentum. 


% V(c)
\paragraph{The speed $\mathbf{s}(\mathbf{c})$} The weights $\mathbf{c}$ determines the speed $\mathbf{s}(\mathbf{c})$ through $\theta'$ as follows. By Equation~\eqref{eq: expression_for_speed}, $s(x_i) = \alpha_i \nabla_\theta \phi^{y_i}(\hat{x}_i)\cdot\theta'$ where $\alpha_i = \frac{1}{\|\nabla_x\phi^{y_i}(\hat{x}_i)\|_q}$. To expand it, we have 

\begin{equation*}
    s(x_i) =  \alpha_i \nabla_\theta \phi^{y_i}(\hat{x}_i)\cdot (\sum_{i\in \mathcal{B}_\theta^{+}}c_i\nabla_\theta \phi^{y_i}(\hat{x}_i) + z)
\end{equation*}
Now we express $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$ with $\mathbf{c}$ using the above equation in matrix form. Denote $A\in \mathbb{R}^{p\times m}$ as the matrix whose i-th column is $\nabla_\theta\phi^{y_i}(\hat{x}_i,y_i)$, $i = 1,\cdots,m$.  Also denote $\alpha \in \mathbb{R}^{m\times m}$ a diagonal matrix whose i-th diagonal element is $\alpha_i$. Then we have the following 

\begin{equation} \label{eq: s_c_app}
    \mathbf{s}(\mathbf{c}) =  \alpha A^{T} A \mathbf{c} + \alpha A^{T} z
\end{equation}

\subsubsection{The coefficients of problem \eqref{eq:opt_for_weight}}

We give the coefficients of the quadratic programming problem~\eqref{eq:opt_for_weight} in matrix forms. 

We write all the optimization variables in a single vectors $\mathbf{w} = (c_1,\cdots,c_m,\mu)$.
By Equation~\eqref{eq: s_c_app}, we have that $\mathbf{s}(\mathbf{c}) - \mu \mathbf{g} = \alpha A^{T} A \mathbf{c} + \alpha A^{T} z - \mu \mathbf{g} = M\mathbf{w} + \alpha A^{T} z$, where $M \in \mathbb{R}^{m\times (m+1)}$ whose first $m$ columns are equal to the matrix $\alpha A^{T} A$ and the last column is equal to $-\mathbf{g}$. Therefore, the optimization problem~\eqref{eq:opt_for_weight} is rewritten as the follows:   

\begin{equation} \label{eq: opt_for_weight_withMu_detail_app}
\begin{aligned}
\min_{\mathbf{w}} \quad & \mathbf{w}^{T}M^{T}M\mathbf{w} + 2\mathbf{w}^{T}(M^{T}\alpha A^{T}z)  \\
\textrm{s.t.} & \quad 
\begin{bmatrix}
    1 &\cdots & 1 & 0
\end{bmatrix}\mathbf{w} = 1, \mathbf{w} \geq 0   \\
\end{aligned}    
\end{equation}

In summary, the details of the optimization problem~\eqref{eq:opt_for_weight} to obtain the weights $\mathbf{c} = (c_1,\cdots,c_m)$ are given by optimization problem~\ref{eq: opt_for_weight_withMu_detail_app}, where $\mathbf{w} = (c_1,\cdots,c_m,\mu)$, 
$M = \begin{bmatrix}
  \alpha A^{T}A 
  & \rvline & -\mathbf{g}
\end{bmatrix}$, 
$A = \begin{bmatrix}
  \nabla_\theta \phi^{y_1}(\hat{x}_1) & \cdots & \nabla_\theta \phi^{y_m}(\hat{x}_m) 
\end{bmatrix}$,
$
\alpha = \text{diag}(\alpha_1,\cdots,\alpha_m)
$,
$\alpha_i = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i)\|_q}$, and $z$ is the terms in $\theta'$ that do not depend on $\mathbf{c}$ (for example, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$ when SGD with momentum and weight decays is used). The problem~\eqref{eq: opt_for_weight_withMu_detail_app} is a quadratic programming problem with $m+1$ variables, which can be solved efficiently. 


\subsubsection{An alternative to problem \eqref{eq:opt_for_weight}}
Here we present an alternative optimization problem to problem~\eqref{eq:opt_for_weight}, which is slightly more efficient since it corresponds to a quadratic problem of size $m$, instead of $m+1$ as in problem~\eqref{eq:opt_for_weight}. The alternative is given as follows:

\begin{equation} \label{eq:opt_for_weight_withoutMu_app}
\begin{aligned}
\min_{\mathbf{c}}\min_{\mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} c_i = 1, \quad c_i\geq0   \\
\end{aligned}
\end{equation}

The difference of problem~\eqref{eq:opt_for_weight_withoutMu_app} and the problem  problem~\eqref{eq:opt_for_weight} is that the former omit the constraint on $\mu$ to be positive. However, their optimal $\mathbf{c}$ are the same if the optimal $\mu$ is positive for the alternative optimization problem~\eqref{eq:opt_for_weight_withoutMu_app}. We find that in our experiments, the solved $\mu$ is always positive for the alternative problem~\eqref{eq:opt_for_weight_withoutMu_app} and thus these two optimization problems are equivalent. Due to its slightly better efficiency, we use the alternative formulation~\eqref{eq:opt_for_weight_withoutMu_app} instead of the formulation~\eqref{eq:opt_for_weight}.   We now give the details of the alternative optimization problem.


% We use the following lemma:

% \begin{lemma} Let $x,\mathbf{g}$ be two vectors. Then we have 
% \begin{equation*}
%     \min_{\mu} \|x-\mu \mathbf{g}\|_2^2 = \|E_\mathbf{g} x\|_2^2 
% \end{equation*}
% where $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$.
% \end{lemma}

Note that the inner minimization problem can be solved in closed form: $\min_{\mu}\|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 = \|E_\mathbf{g} \mathbf{s}(\mathbf{c})\|_2^2$ where $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$. By Equation~\eqref{eq: s_c_app} that we have derived in the last section, $\mathbf{s}(\mathbf{c}) = \alpha A^{T} A \mathbf{c} + \alpha A^{T} z $. Therefore, $\min_{\mathbf{c}}\min_{\mu}  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 = \min_{\mathbf{c}}\|E_\mathbf{g} \mathbf{s}(\mathbf{c})\|_2^2 = \min_{\mathbf{c}}\|E_\mathbf{g} ( \alpha A^{T} A \mathbf{c} + \alpha A^{T} z)\|_2^2$, which corresponds to the following constrained quadratic programming problem:

\begin{equation} \label{eq: opt_for_weight_withoutMu_detail_app}
\begin{aligned}
\min_{\mathbf{c}} \quad & \mathbf{c}^{T}K_1^{T}K_1\mathbf{c} + 2\mathbf{c}^{T}(K_1^{T}K_2)  \\
\textrm{s.t.} & \quad \sum_{i}c_i = 1, \mathbf{c} \geq 0   \\
\end{aligned}    
\end{equation}

where $K_1 = E_\mathbf{g}\alpha A^{T}A, K_2 = E_\mathbf{g}\alpha A^{T}z$. 

In summary, the alternative scheme \eqref{eq:opt_for_weight_withoutMu_app} is given by the quadratic problem \eqref{eq: opt_for_weight_withoutMu_detail_app}, where $K_1 = E_\mathbf{g}\alpha A^{T}A, K_2 = E_\mathbf{g}\alpha A^{T}z$, $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$, $A = \begin{bmatrix}
  \nabla_\theta \phi^{y_1}(\hat{x}_1) & \cdots & \nabla_\theta \phi^{y_m}(\hat{x}_m) 
\end{bmatrix}$,
$
\alpha = \text{diag}(\alpha_1,\cdots,\alpha_m)
$,
$\alpha_i = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i)\|_q}$, and $z$ is the terms in $\theta'$ that do not depend on $\mathbf{c}$ (for example, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$ when SGD with momentum and weight decays is used). The problem~\eqref{eq: opt_for_weight_withoutMu_detail_app} is a quadratic programming problem in $m$ variables, which can be solved efficiently. 



\subsection{Workflow of \algoName} \label{app: algo_pseudo}
We present the pseudocode of our proposed \algoName in Algorithm~\ref{alg: main algo}.
\input{algo} 


\section{Optimality condition in practice} \label{app: optimality}
Either computing the speed of the decision boundary or reverse engineering an update rule to achieve some desirable dynamics (like what \algoName does) requires the computation of the closest boundary point $\hat{x}$ for the correctly classified data point $(x,y)$, where we omit the subscript $i$ in this section. As discussed in Appendix~\ref{app: closed_expression_speed}, it suffices to find the local closest boundary point in order for the closed-form expression~\eqref{eq: expression_for_speed} for the speed to be valid. 

In this section, we will explain how to check the quality of the found $\hat{x}$ for the constrained optimization problem~\ref{eq: closest_pt} in practice. We will also give a simple analysis on how FAB\citep{croce2020minimally}, the algorithm we use in our implementation, solves the problem~\ref{eq: closest_pt} in practice. In this paper, we focus on $p = 2$ and $p = \infty$. 

The key points of analyzing $\hat{x}$ are that $\phi^{y}(\hat{x}) = 0$ and the KKT condition of problem~\ref{eq: closest_pt}.

\emph{Case 1: $p=2$}

In this case, the KKT condition is given by $\nabla_x \phi^{y}(\hat{x}) + \lambda (\hat{x} - x) = 0$ for some $\lambda > 0$ (since $\phi^{y}(x) >0$). In other words, $\frac{\nabla_x \phi^{y}(\hat{x})}{\|\nabla_x \phi^{y}(\hat{x})\|} \cdot \frac{x-\hat{x}}{\|x-\hat{x}\|} = 1$. In practice, we check the following two conditions (a) $|\phi(\hat{x})| \leq 0.1$; (b) $\frac{\nabla_x \phi^{y}(\hat{x})}{\|\nabla_x \phi^{y}(\hat{x})\|} \cdot \frac{x-\hat{x}}{\|x-\hat{x}\|} > 0.8$. In our experiments, we find that FAB with iterations greater than 10 can reliably find $\hat{x}$ satisfying these two conditions. In all of our experiments when $p=2$, including computing the speed for various methods (e.g. AT) and the implementation of \algoName, we only use those high-quality closest boundary points that satisfy these two conditions and discard the rest. We observe in our experiments that FAB can find high-quality closest boundary points for over 90\% of the correctly classified data points. 

\emph{Case 2: $p=\infty$}

In this case, we consider the optimality condition given in Lemma~\ref{lemma: Linf_optimality_app} of Appendix~\ref{app: closed_expression_speed}. Denote $\#B$ the number of points in the set $B$. Using the notation $\mathcal{J} = \{j: |\hat{x}_j - x_j| = \|\hat{x}-x\|_\infty\}$ and $\mathcal{J}^{C}$ the complement set of $\mathcal{J}$, we check the following conditions in practice: (a) $|\phi(\hat{x})| \leq 0.1$; (b) $\frac{\#\{j\in\mathcal{J}: \nabla_x \phi^{y}(\hat{x})_j (\hat{x}_j - x_j) \leq 0\}}{\#\mathcal{J}} > 0.9$; (c) $\frac{\#\{k\notin J: |\nabla_x \phi^{y}(\hat{x})_k| < 0.1 \}}{\#\mathcal{J}^C} > 0.8$. Note the unlike $p=2$, the optimality conditions for $p=\infty$ are on each coordinate of $\hat{x}$, which is more difficult to satisfy. We observe in our experiments that FAB with 60 iterations can find high-quality closest boundary points for about 85\% of the correctly classified points. However, when only 15 iterations are used, condition (3) is barely satisfied for all of the found boundary points (the first two conditions are still satisfied). In our visualizations of dynamics of the decision boundary for various methods in $L_\infty$ setting in Appendix~\ref{app: more_dynamics}, we use 60 iterations for FAB and only use high-quality closest boundary points, so that the visualization results are accurate. In our implementation of \algoName, we omit the condition (3) and only use 15 iterations for FAB for efficiency. 

Designing faster and more reliable methods to solve the constrained optimization problem~\ref{eq: closest_pt}, especially when $p = \infty$, is left for future work. 

==> Neurips/a3_experiment.tex <==



\section{Experiments}
In this section, we provide experimental details and further results of \algoName along with other state-of-the-art defense methods. 
\subsection{Detailed experimental settings} \label{app: exp_settings}

\paragraph{Basic training setting} 
In all experiments on CIFAR-10 in Section~\ref{sec:exp_robust}, we use the Wide Residual Networks  \citep{zagoruyko2016wide} with depth 28 and width factor 4 (WRN-28-4), which is also used in previous works \citep{Ding2020MMA}. We replace the batch normalization (BN) layers with group normalization (GN) \citep{wu2018group} layers so that the decision boundary is the same at training and test time. This is necessary for \algoName since it uses the closest boundary points during training, which should be also on the decision boundary in the evaluation mode. For other baselines, we find that replacing BN with GN has negligible effect on the robustness performance. We use stochastic gradient descent with momentum 0.9 and weight decay 0.0005, which is suggested in \citep{pang2020bag}. We train 100 epochs in total with batch size 128. The learning rate begins at 0.1 and is decayed by a factor of 10 at the 50th and 75th epoch. The first 10 epochs of \algoName is the burn-in period, where only the clean loss is used. To alleviate robust overfitting \citep{rice2020overfitting}, early stopping is performed on a validation set of size 2000 in all experiments, where the model with the highest robust accuracy under projected gradient descent (PGD) attacks \citep{madry2017towards} with 20 steps (PGD-20) is chosen. All experiments are run on two NVIDIA GeForce RTX 2080 Ti GPU. 

\paragraph{Per-sample gradient} During implementation of the expression for speed in Equation~\eqref{eq: expression_for_speed} and also \algoName, we need to compute the per-sample gradient $\nabla_\theta \phi^{y_i}(\hat{x}_i,\theta)$ for every correctly classified point $x_i$. We use the Opacus package \citep{opacus} for computing per-sample gradients in parallel. Also, another reason why we replace BN with GN is because Opacus does not support BN for computing per-sample gradients.   


\paragraph{Evaluation protocol}
We evaluate our proposed method and baselines under $L_2/L_\infty$-norm constrained perturbation. The final robust accuracy is reported on the full test set against PGD-40 attack as well as AutoAttack (AA) \citep{croce2020reliable}, which uses an ensemble of selected strong attacks. Note that although AA is considered stronger and serves as a more reliable measure of robustness, we still include PGD attack results since it can happen that some methods performs well against PGD attack, but not against AA. In all experiments we find that AA gives lower robust accuracy than PGD attack. Therefore, we refer to the robust accuracy against AA, instead of PGD, when comparing performance among different defense methods. For all methods, we choose the hyperparameters to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. In addition, we evaluate on larger perturbation thresholds to better examine the robustness of the model against larger unknown perturbation thresholds. 

\textbf{Compared baselines and their hyperparameters}\quad
The baseline defense methods include: (1) standard adversarial training (AT) \citep{madry2017towards} which trains on the worst case adversarial examples generated by 10-step PGD (PGD-10) on the cross-entropy loss. The perturbation threshold is $0.5$ in $L_2$ setting, and $\frac{8}{255}$ in $L_\infty$ setting. The step size of PGD is $\frac{15}{255}$  in $L_2$ setting and $\frac{2}{255}$ in $L_\infty$ setting; the training setting follows Rice et al.\footnote{\href{https://github.com/locuslab/robust_overfitting}{Robust Overfitting's Github}}  \citep{rice2020overfitting}. (2) TRADES \footnote{\href{https://github.com/yaodongyu/TRADES}{TRADES's Github}}\citep{zhang2019theoretically} which trades off between the clean and robust accuracy. The perturbation threshold is $0.5$ in $L_2$ setting, and $\frac{8}{255}$ in $L_\infty$ setting. The step size of PGD-10 is $\frac{15}{255}$  in $L_2$ setting and $0.007$ in $L_\infty$ setting ; The regularization constant beta (or 1/lambda) is set to  6. (3) MMA  \footnote{\href{https://github.com/BorealisAI/mma_training}{MMA's Github}}  \citep{Ding2020MMA} which trains on the closest adversarial examples (closest boundary points) with uniform weights. 
% Since MMA is the most related to \algoName, we report four hyperparamter settings. MMA-1 in $L_2$ setting uses MaxEps = $1$; MMA-2 in $L_2$ setting uses MaxEps = $2$; MMA-3 in $L_\infty$ setting uses MaxEps = $\frac{20}{255}$; MMA-4 in $L_\infty$ setting uses MaxEps = $\frac{32}{255}$; 
The MaxEps is set to $1$ in $L_2$ setting and $\frac{32}{255}$ in $L_\infty$ setting. 
(4) GAIRAT \footnote{\href{https://github.com/zjfheart/Geometry-aware-Instance-reweighted-Adversarial-Training}{GAIRAT's Github}} \citep{zhang2021geometryaware}  which reweights adversarial examples using the least perturbation steps. We only evaluate GAIRAT under $L_\infty$ setting since it does not have $L_2$ implementation in the codebase. The perturbation length is $\frac{8}{255}$ with step size $0.007$ using PGD-10 and the 'tanh' weight assignment function is used. (5) MAIL \footnote{\href{https://github.com/QizhouWang/MAIL}{MAIL's github}} \citep{liu2021probabilistic} which reweights adversarial examples using margin value. We only evaluate MAIL under $L_\infty$ setting since it does not have $L_2$ implementation in the codebase.(6) FAT \footnote{\href{https://github.com/zjfheart/Friendly-Adversarial-Training}{FAT's github}} \citep{zhang2020attacks} that exploits friendly adversarial data. We only evaluate FAT under $L_\infty$ setting since it does not have $L_2$ implementation in the codebase.


\subsubsection*{Hyperparameters of \algoName} 

We use the ratio function with $g(0) = 1, g(r_0) = 0, g(r_1) = - g_1$ with $g_1 \geq 0 $ and linearly interpolate them when $0\leq r \leq r_1$. When $r>r_1$, $g(r)$ was set to the constant $-g_1$. If $g_1 > 0$, it means that \algoName pulls back the decision boundary towards $x_i$ if its robust radius $R(x_i)$ is larger than $r_1$. We allow $g$ to be negative when $r > r_1$ since we experimentally find that this could help improve both the clean accuracy and robust accuracy under small perturbation lengths in some settings. This is because it helps reduce the variance of the robust radius distribution by eliminating robust radii that are unnecessarily large. When $g(R(x_i)) < 0 $, the weight $c_i$ is constrained to be non-positive since the decision boundary at $\hat{x}_i$ needs to be pulled back. In particular, we solve the following modified version of the optimization problem~\eqref{eq:opt_for_weight}:

\begin{equation} \label{eq:opt_for_weight_negative}
\begin{aligned}
\min_{\mathbf{c}, \mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} |c_i| = 1, \quad c_i g(R(x_i))\geq0, \quad \mu \geq 0    \\
\end{aligned}
\end{equation}

The optimization problem~\eqref{eq:opt_for_weight_negative} above is still a quadratic programming problem with the same objective function as the original problem~\eqref{eq:opt_for_weight}, whose details are given in Appendix~\ref{app: opt_for_weight}. The only difference is in the constraints, where  problem~\eqref{eq:opt_for_weight_negative} requires the weight to be non-positive if its $g$ value is negative, and the absolute values of the weights sum up to one. 

To achieve the best robust accuracy under $\epsilon = 0.5$ in the $L_2$ setting, we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = 0.4$. To achieve the best robust accuracy under $\epsilon = \frac{8}{255}$ in the $L_\infty$ setting, we set $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = 0.4$. We use FAB with 15 iterations to approximate the closest boundary points in both $L_2$ and $L_\infty$ setting. 


\subsection{Further experimental results}\label{app: further_exp_results}

\paragraph{Comparing with baselines} We first present results where the hyperparameters of $\algoName$ are chosen to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. That is , we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = 0.4$ in $L_2$ setting and  $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = 0.4$ in  $L_\infty$ setting. The results are given in Table~\ref{table: performance_L2_more_eps_app} and Table~\ref{table: performance_Linf_more_eps_app}. In the $L_2$ case, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. In the $L_\infty$ case, \algoName obtains both higher clean accuracy and robust accuracy than AT, MMA and GAIRAT. We observe that the robust accuracy under AA is much lower than PGD for GAIRAT and MMA, which may be due to obfuscated gradient \citep{AthalyeC018}. On the other hand, the performance gap between PGD and AA is relatively small for \algoName. When compared with TRADES, \algoName shows higher clean accuracy and comparable robust accuracy under larger $\epsilon$, although \algoName has lower robust accuracy when $\epsilon = \frac{8}{255}$. This is partially due to the higher difficulty of approximating the closest boundary points in the $L_\infty$ case, and a better algorithm for this is left for future work. 


\input{appendix_experiments/tab_L2_moreEps}
\input{appendix_experiments/tab_Linf_moreEps}

\paragraph{Effect of ratio function and clean loss coefficient} We study the effect of hyperparameters $r_0, r_1, g_1$ of the ratio function $g$, as well as the clean loss coefficient $\lambda_c$ in the loss function~\eqref{eq: weighted loss general}. We only show the robust accuracy results against AA since it gives a more accurate estimation of the robustness. The results are shown in Table~\ref{table: performance_L2_ours_ablation} and Table~\ref{table: performance_Linf_ours_ablation}, where several observations can be made. Firstly, we observe that when the ratio function $g$ is fixed, a smaller $\lambda_c$ tends to result in better robustness performance against all perturbation thresholds, though the clean accuracy is lower. This indicates a trade-off between the robust and clean accuracy. Secondly, when $\lambda_c$ is fixed, a flatter ratio function $g$ (with larger $r_0$) will result in higher robust accuracy under larger perturbation lengths,  but could hurt the robust accuracy under smaller perturbation lengths. Thirdly, using a positive $g_1$ when $r_0$ is relatively large (such as $2$ in $L_2$ case and $\frac{32}{255}$ in $L_\infty$ case) could improve the robust accuracy under smaller perturbation lengths (such as $0.5$ in $L_2$ case and $\frac{8}{255}$ in $L_\infty$ case) but decrease the robust accuracy under larger perturbation lengths. In this case, \algoName controls the decision boundary so that if it is very far from the natural data, it will move closer. This helps reduce the variance of the robust radius distribution, decrease the proportion of unnecessarily robust points and thus improve the robust accuracy under small perturbation thresholds. 


\input{appendix_experiments/tab_L2_ours_ablation}
\input{appendix_experiments/tab_Linf_ours_ablation}


==> Neurips/a4_more_dynamics.tex <==
\section{Further results of dynamics} \label{app: more_dynamics}
In this section, we present more visualizations and further analysis of the dynamics of the decision boundary during the training process. 

\subsection{Further analysis of dynamics}
In Figure~\ref{fig: interpretation_VR_test_all} of Section~\ref{ssec: Dynamics of adversarial training}, we present the speed at chosen iterations where the maximum absolute value of the speed is normalized to 1 for better visualization of the conflicts. Now we present the un-normalized speed (raw speed values) in Figure~\ref{fig: AT_speed_time_app_all}, where the 20\% quantile, median and 80\% quantile of the speed distribution at each iteration are shown. We observe that at the start of the training (first 100 iterations) where the robust accuracy improves drastically, the speed distribution is mostly positive. Later,  when the robustness improvement slows down, the speed distribution is centered around zero. Also, notice that the variance of the speed distribution is never vanishing: the decision boundary always moves towards some data points while moving away from others. This indicates that adversarial training methods do not converge, since the decision boundary does not stop moving. Despite the constant movement of the decision boundary, the average adversarial loss does converge. Therefore, the dynamics of the decision boundary w.r.t. each data point provides more information than an average of the surrogate loss. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/VR_AT_acc}}
        \caption{Test accuracy}
        \label{fig: AT_acc_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/AT_test_speed_time}}
        \caption{Speed distribution and iterations}
        \label{fig: AT_speed_time_app}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during AT. In Figure~\ref{fig: AT_speed_time_app}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. }
    \label{fig: AT_speed_time_app_all}
    %\vspace{-1em}
\end{figure}


\paragraph{Natural training}
To compare with the non-converging behaviour of adversarial training methods, we present the dynamics during natural training in Figure~\ref{fig: clean_speed_time_app_all}, where the robust accuracy stays at zero. This can be viewed as the final stage of the natural training since the clean accuracy does not increase significantly anymore. We observe that the speed distribution of the decision boundary is effectively zero. This indicates that natural training does converge in the following sense: the clean accuracy does not change and moreover, the decision boundary around every correctly classified point does not move anymore. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/clean_acc}}
        \caption{Test accuracy}
        \label{fig: clean_acc_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/clean_test_speed_time}}
        \caption{Speed distribution and iterations}
        \label{fig: clean_speed_time_app}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during natural training. In Figure~\ref{fig: clean_speed_time_app}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. Observe that the speed is almost zero during natural training, indicating that natural training eventually does not move the decision boundary around correctly classified points.}
    \label{fig: clean_speed_time_app_all}
    %\vspace{-1em}
\end{figure}

\subsection{Dynamics in the \texorpdfstring{$L_\infty$}{} setting }

Here we present the visualization of the speed in the $L_\infty$ setting. We use FAB with 60 iterations and only choose the closest boundary points with high quality according to Appendix~\ref{app: optimality}. We use AT with $\epsilon = \frac{8}{255}$ and \algoName with $r_0=\frac{32}{255}, g_1 = 0, \lambda_c = 1$. The speed-radius distribution on the training batches of three chosen iterations for both methods are shown in Figure~\ref{fig: AT_linf_VR_trainBatch_app} and Figure~\ref{fig: ours_linf_VR_trainBatch_app}. We can draw a similar conclusion as in the $L_2$ case: conflicting dynamics of the decision boundary exists for AT during training, since there is a significant proportion of vulnerable points (with $R(x_i) \leq \frac{8}{255}$) with negative speed values. On the other hand, \algoName can alleviate this conflict and encourage robustness improvement on more vulnerable points by assigning larger speed values to them. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/AT_batch_Linf_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
        \label{fig: AT_linf_VR_trainBatch_scatter_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/AT_batch_Linf_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: AT_linf_VR_trainBatch_hist_app}
    \end{subfigure}%
    \caption{Radius-speed plot of AT on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations in $L_\infty$ setting. Proportion of points with negative speed for these iterations are 31\%, 45\% and 46\% respectively.}
    \label{fig: AT_linf_VR_trainBatch_app}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/ours_batch_Linf_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of \algoName on the training batch}}
        \label{fig: ours_linf_VR_trainBatch_scatter_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{appendix_experiments/ours_batch_Linf_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: ours_linf_VR_trainBatch_hist_app}
    \end{subfigure}%
    \caption{Radius-speed plot of \algoName on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations in $L_\infty$ setting. Proportion of points with negative speed for these iterations are below 3\%.}
    \label{fig: ours_linf_VR_trainBatch_app}
\end{figure}

==> Neurips/a5_limitation.tex <==
\section{Limitations}

The main limitations of \algoName arises from the usage of FAB attack to find the closest boundary points, as well as computing the per-sample gradient in order to reverse engineer the weights for training. 

Specifically, according to the original paper\citep{croce2020minimally}, the computational cost is two forward passes and one backward pass per iteration. For comparison, the cost of PGD is one forward pass and one backward, so they are about the same. However, due to the design of the autograd functionality of Pytorch, FAB is indeed slower, especially when the number of classes is large \cite{croce2020reliable}. This is because pytorch does not support computation of gradients of all logits w.r.t. inputs in one backward pass. FAB and our method will significantly speed up when this functionality is supported. 

As for the extra cost of per-sample gradient computation, we use the Opacus package to implement this, which allows efficient computation of per-sample gradient w.r.t. parameters. Note that in vanilla Pytorch, per-sample gradients w.r.t. parameters are also computed, but then aggregated and therefore are difficult to access. Therefore, computing per-sample gradient doesn't affect the computation speed, but it increases the memory. In our experiments we found that the memory is about 3-4 times as traditional adversarial training. 

How to efficiently scale up \algoName is left for future work. 

==> Neurips/algo.tex <==
%%% wrapping algorithm inside a figure environment, so that we can adjust the spacing around it using \vspace{}

\begin{figure}[!htbp]
\vspace{-1em}
\centering
\begin{algorithm}[H] 
\caption{\algoNameFull (\algoName)}
\label{alg: main algo}
\hspace*{\algorithmicindent} \textbf{Input:} 
The training data set, ratio function $g$, norm type $p$, clean loss strength $\lambda_c$, number of epochs $T$ and number of batches $M$. $\mathcal{A}(x,y)$ denotes the approximate closest boundary point returned by an algorithm $\mathcal{A}$ (e.g. FAB) on the correctly classified data point $(x,y)$.  \\
\hspace*{\algorithmicindent} \textbf{Output:} adversarially robust network $f_\theta$
\begin{algorithmic}[1]
\For{epoch = $1,\cdots,T$}
    \For{mini-batch = $1,\cdots,M$}
        \State Sample a mini-batch $\mathcal{B} = \{(x_i,y_i\}_{i=1}^{n}$
        \State Make predictions on $\mathcal{B}$ and find correctly classified points $\mathcal{B}_{\theta}^{+}$
        \For{$(x_i,y_i)\in \mathcal{B}_{\theta}^{+}$ (in parallel)}
            \State Find the approximate closest boundary point $\hat{x}_i = \mathcal{A}(x_i,y_i)$ as in \eqref{eq: closest_pt}
            \State Compute the robust radius $R(x_i) = \|\hat{x}_i - x_i\|_p$
            \State Calculate the ratio value $g(R(x_i))$
        \EndFor
        \State Solve the optimization problem \eqref{eq:opt_for_weight} for weights $c_i$ for $i \in \mathcal{B}_{\theta}^{+}$ 
        \State Update $\theta$ using the loss function \eqref{eq: weighted loss general}
        % $\theta \gets \theta - \eta(\sum_{i\in B_1^{\text{adv}}}c_i\nabla_\theta l(\hat{x}_i,y_i)  + \lambda_c\sum_{i\in B}\frac{1}{N}\nabla_\theta l(x_i,y_i))$
    \EndFor
\EndFor

% \Function{ComputeWeight}{$x,y$} \Comment{{\small{return the summation of two variables}}}
%   \State $z = x + y$
%   \State \textbf{Return} $z$ 
% \EndFunction
\end{algorithmic}
\end{algorithm}

\vspace{-1em}
\end{figure}


==> Neurips/fig_intepret_train.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/AT_batch_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
        \label{fig: interpretation_VR_trainBatch_scatter}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/AT_batch_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: interpretation_VR_trainBatch_hist}
    \end{subfigure}%
    \caption{Figure \ref{fig: interpretation_VR_trainBatch_scatter} shows the radius-speed plot on the training batches of three iterations. Figure \ref{fig: interpretation_VR_trainBatch_hist} shows the vertical histogram of the speed. Proportions of points with negative speed  are $33.71\%$ at iteration 5, $34.29\%$ at iteration 30 and $39.87\%$ at iteration 200.}
    \label{fig: interpretation_VR_trainBatch_all}
\end{figure}

% \begin{figure}[!htbp] % !htbp
%     \resizebox{\linewidth}{!}{\input{Intepretation_fig/AT_batch_scatter}}
%     %\vspace{-0.5em}
%     \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
%     \caption{Radius-speed plot of AT on the training batches of three iterations. Proportions of points with negative speed  are $33.71\%$ at iteration 5, $34.29\%$ at iteration 30 and $39.87\%$ at iteration 200.}
%     \label{fig: interpretation_VR_trainBatch_all}
% \end{figure}

==> Neurips/fig_interpret.tex <==


\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.79\columnwidth}
        \centering
     \resizebox{\textwidth}{!}{\input{Intepretation_fig/VR_AT_batch_w_hist}}
     \caption{R plot on the train batch}
     \label{fig: interpretation_VR_batch}
    \end{subfigure}
    \hfill
     \begin{subfigure}[t]{0.2\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{Intepretation_fig/VR_AT_acc.tex}}
    \caption{\small{Accuracy during training}}
    \label{fig: interpretation_acc}
    \end{subfigure}\\
    \hfill
    \begin{subfigure}[t]{0.79\columnwidth}
        \centering
        % \resizebox{1.0\textwidth}{!}{\input{Intepretation_fig/VR_AT_test}}
        \resizebox{\textwidth}{!}{\input{Intepretation_fig/VR_AT_test_w_hist}}
        % \vspace{-0.5em}
        \caption{\small{VR plot on the test set}}
        \label{fig: interpretation_VR_test}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.2\columnwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{Intepretation_fig/VR_AT_approx_d}}
        \caption{\small{Derivative of Accuracy during training}}
        \label{fig: interpretation_acc_d}
    \end{subfigure}
    \caption{Caption. \fhc{maybe we could put training VR plot here as well.} \yc{1. add a zero horizontal line 2. freq: 10 iteration until 3000 iterations}}
    \label{fig: interpretation_VR_test_all}
\end{figure}

==> Neurips/fig_interpret_test.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.21\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/VR_AT_acc.tex}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: interpretation_acc}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.55\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/AT_test_scatter}}
        \caption{\scriptsize{Radius-speed plot of AT on the test data points}}
        \label{fig: interpretation_VR_test_scatter}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/VR_AT_approx_d}}
        \caption{\scriptsize{Robustness improvement 
        }}
        \label{fig: interpretation_acc_d}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Figure \ref{fig: interpretation_VR_test_scatter} shows the radius-speed plot on a fixed set of points in the test set for three iterations. Figure \ref{fig: interpretation_acc_d} shows the time derivative of the robust accuracy within correct points and its approximation using the dynamics statistics $p(\mathcal{S}_{\mathsf{g}}) - p(\mathcal{S}_{\mathsf{b}})$.}
    \label{fig: interpretation_VR_test_all}
    %\vspace{-1em}
\end{figure}

==> Neurips/s0_abstract.tex <==
Adversarial Training (AT) is among the most effective methods for improving the adversarial robustness of deep neural networks. The robustness of a deep classifier can be measured by the \textit{robust radii}:
the decision boundary's distances to natural data points. However, it is unclear whether AT effectively improves the robust radius for each individual vulnerable point. To understand this, we propose a continuous-time framework that studies the relative speed of the decision boundary with respect to each individual point. Through visualizing the moving speed of the decision boundary, a surprising conflicting moving-behavior is revealed: the decision boundary under AT moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones. To alleviate this \textit{conflicting dynamics} of the decision boundary, we propose \textit{\algoNameFull} (\algoName) which directly controls the decision boundary to move away from the training data points. Moreover, in order to further encourage the robustness improvement for more vulnerable points, \algoName controls the decision boundary to move faster away from points with smaller robust radii, achieving customized manipulation of the decision boundary. Therefore, \algoName robustifies each individual vulnerable point rather than focusing on the average robustness. 
As a result, \algoName achieves fairer robustness to individuals, leading to better overall robustness under limited model capacity. Experiments verify that \algoName alleviates the conflicting dynamics of the decision boundary and obtains improved robustness compared with the state-of-the-art defenses.


%\yc{this sentence is not perfect}
% and thus significantly improves the robustness generalized to every point in the distribution. %\st{ to all points}.
% Specifically, the decision boundary is designed to move away faster from data points with smaller robustness radius, which encourages the robustness improvement on more vulnerable data. 
% Our experiments validate our theory and  demonstrate the efficacy of \algoName on the CIFAR-10 dataset w.r.t $L_2$ and $L_\infty$ robustness.

% through such personalized attendance to vulnerable points. 



% for abstract submission
% \newcommand{\algoName}{{\texttt{Dyna-CAT}}\xspace}
% \newcommand{\algoNameFull}{Dynamical Customized Adversarial Training\xspace}
% Adversarial Training (AT) is among the most effective methods for improving the adversarial robustness of deep neural networks. The robustness of a deep classifier can be measured by the \textit{robust radii}:
% the decision boundary's distances to natural data points. However, it is unclear whether AT effectively improves the robust radius for each individual vulnerable point. To understand this, we propose a continuous-time framework that studies the relative speed of the decision boundary with respect to each individual point. Through visualizing the moving speed of the decision boundary, a surprising conflicting moving-behavior is revealed: the decision boundary under AT moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones. To alleviate this \textit{conflicting dynamics} of the decision boundary, we propose \textit{Dynamical Customized Adversarial Training\xspace} ({\texttt{Dyna-CAT}}\xspace) which directly controls the decision boundary to move away from the training data points. Moreover, in order to further encourage the robustness improvement for more vulnerable points, {\texttt{Dyna-CAT}}\xspace controls the decision boundary to move faster away from points with smaller robust radii, achieving customized manipulation of the decision boundary. Therefore, {\texttt{Dyna-CAT}}\xspace robustifies each individual vulnerable point rather than focusing on the average robustness. As a result, {\texttt{Dyna-CAT}}\xspace achieves fairer robustness to individuals, leading to better overall robustness under limited model capacity. Experiments verify that {\texttt{Dyna-CAT}}\xspace alleviates the conflicting dynamics of the decision boundary and obtains improved robustness compared with the state-of-the-art defenses.

==> Neurips/s1_intro.tex <==
\section{Introduction}\label{sec:intro}

% \ys{OPTION 1:

% 1. deep neural nets are good but vulnerable

% 2. there are a lot of work for training robust models, among which AT is xxx (good), but has following issues (1) (2) (3)

% 3. to solve these challenges, we dive deeper into the essence of robust training: (define robust radius and its relation to AT). (why AT has the above issues) 

% 4. in contrast, our method xxx (figure)


% OPTION 2:

% 1. deep neural nets are good but vulnerable (what is adversarial attack)

% 2. define the goal of robust training: robust radius and why it matters

% 3. how existing methods (AT) fit into this formulation, and why they do not solve this method, (a little surprising empirical evidence; oscillation figure in interpretation section)

% 4. in contrast, our method xxx (figure) improves the robust radius in a principled way}

Deep neural networks have been successfully deployed in a wide range of applications~\citep{krizhevsky2012imagenet,goodfellow2014generative,he2016deep,collobert2008unified}. 
However, they have been shown to be susceptible to adversarial examples, leading to issues in security-critical applications such as autonomous driving and medicine~\citep{szegedy2013intriguing,nguyen2015deep}.  
To alleviate this problem, adversarial training (AT)~\citep{madry2017towards,shafahi2019adversarial,zhang2019theoretically,gowal2020uncovering} was proposed and is one of the most prevalent methods against adversarial attacks. 
Specifically, AT aims to find the worst-case adversarial examples based on some surrogate loss and adds them to the training dataset in order to improve robustness. 

% \ys{maybe first praise AT for their success?}
Although AT is among the most successful defenses against adversarial perturbations, it has been shown that (even over-parameterized) neural networks, which can perfectly fit natural data in standard training~\citep{zhang2021understanding}, still have insufficient model capacity for fitting adversarial training data~\citep{zhang2021geometryaware}. 
In order to carefully utilize the limited model capacity to fit the neighborhoods of more important data points,
%\fh{what does it mean to utilize the limited model capacity?}, 
weighted adversarial training methods~\citep{zhang2021geometryaware, zeng2020adversarial,liu2021probabilistic} exploit the fact that data points have different vulnerability.  
As shown in Figure~\ref{sfig:demo1}, some data points have smaller robustness radii, i.e., distances to the decision boundary, and are considered more vulnerable. 
% As shown in figure \yc{demo 1: static figure: only different RR}, some data has a smaller robust radius, i.e. its distance to the decision boundary, and is considered more vulnerable. 
Therefore, weighted AT methods assign larger weights to adversarial examples whose natural counterparts have smaller robust radii, which are estimated by the least number of steps to attack \citep{zhang2021geometryaware} or the logit margin \citep{zeng2020adversarial,liu2021probabilistic}. 

\begin{figure}[!t]
\vspace{-0.5em}
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-1.pdf}
        \caption{The decision boundary, vulnerable points (in solid) and robust points (in hollow).}
    \label{sfig:demo1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-2.pdf}
        \caption{Conflicting moving-behavior of the decision boundary after one step of update.}
    \label{sfig:demo2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-3.pdf}
        \caption{Continuous movement of decision boundary.}
    \label{sfig:demo3}
    \end{subfigure}
    \caption{The movement of the decision boundary. Red triangles and green circles are data points from two classes. Figure~\ref{sfig:demo1} shows the vulnerability difference among the data points: some are closer to the decision boundary, whereas some are farther from it. In Figure~\ref{sfig:demo2}, the decision boundary after an update 
    moves away from some vulnerable points (made more robust) but simultaneously moves closer to other vulnerable ones (made less robust). 
    Figure~\ref{sfig:demo3} describes the continuous movement of the decision boundary in Figure~\ref{sfig:demo2}.}
    \label{fig:demos}
    % \vspace{-1.5em}
\end{figure}

Despite up-weighting the surrogate loss on points with smaller robust radii, these weighted AT methods still do not directly increase the robust radii of each individual vulnerable point. 
% \fh{Shall we demonstrate here that why this is a problem experimentally?}\yc{This is discussed in next two paragraph.}
In addition, they only train on adversarial examples within an pre-defined universal perturbation threshold for all data points, which is likely sub-optimal due to the difference in vulnerability among points. Therefore, it is unclear whether the learning algorithm is effectively improving the robust radius for each vulnerable point. Geometrically, we are interested to know if the decision boundary moves away from the data points, especially the vulnerable ones. As illustrated in Figure~\ref{sfig:demo2}, 
there can exist conflicting dynamics of the decision boundary:  it moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones during training. This motivates us to ask:


% In addition, they control the level of robustness by pre-defining the perturbation length $\epsilon$ and all of the points used for training are within $\epsilon$ distance from the original points, in regardless o
% However, this is sub-optimal because different points have different robustness and the model is unlikely to be robust to a more diverse attack budget.\yc{Some new sentences for varying $\epsilon$} 

\textbf{Question 1}\quad \textit{Given an training algorithm, how to analyze the dynamics of the decision boundary with respect to the data points?}

To answer the above question, we propose a continuous-time framework that studies the instantaneous movement of the decision boundary as shown in Figure~\ref{sfig:demo3}. Specifically, we define the relative speed of the decision boundary w.r.t. a point to be the time derivative of its robust radius, which can be interpreted as the speed of its closest adversarial example moving away from it. We show that the speed can be derived from the training algorithm using a closed-form expression. 

Using the proposed framework, we numerically compute the speed of the decision boundary w.r.t. data points for AT. As shown in Figure~\ref{fig: interpretation_VR_trainBatch_all},
We observe that a significant proportion of vulnerable points has negative speed, indicating the existence of the aforementioned conflicting dynamics (Figure~\ref{sfig:demo2},\ref{sfig:demo3}) of the decision boundary.
% across data points is a prevalent phenomenon, although it cannot be observed using averaged statistics such as robust accuracy or an average of a surrogate loss. 
On the other hand, a desirable dynamics should satisfy that the decision boundary moves away from the vulnerable points. Moreover, the speed should be larger for points with smaller robust radii in order to encourage the robustness improvement on vulnerable points. 
This leads to another question:

\textbf{Question 2}\quad \textit{How to design algorithms to achieve desirable dynamics of the decision boundary?}

To this end, we propose \textit{\algoNameFull (\algoName)}, which explicitly controls the decision boundary to move away from the data points and moreover, faster from the points with smaller robust radii. Such control is possible since we can derive the dynamics of the decision boundary given a training algorithm, which enables us to reverse engineer the training scheme to achieve the desirable dynamics. Specifically, \algoName adopts a weighted loss on the closest boundary points, where the weights are reverse engineered to realize the desirable dynamics. 

Unlike previous weighted AT methods which directly assign larger weights to more vulnerable points but still cause conflicting dynamics, \algoName designs the weights so that the robustness improvement of vulnerable points is faster. In addition, instead of pre-defining a uniform perturbation length for training as in AT, \algoName trains on the closest boundary points and thus takes into account of the robust radius of each point. Consequently, \algoName is naturally robust to more diverse attacking budget $\epsilon$'s, whereas previous weighted AT methods are trained to be robust to a pre-defined $\epsilon$.
We experimentally demonstrate that \algoName realizes the desirable dynamics during training and achieves improved robustness performance on diverse attacking budgets. 


\textbf{Summary of contributions.} \textbf{(1)} We propose a continuous-time framework to study the relative speed of the decision boundary w.r.t. each individual data point and provide the closed-form expression for the speed. 
\textbf{(2)} We visualize the speed of the decision boundary for AT and identify the conflicting dynamics of the decision boundary. 
\textbf{(3)} We propose Dynamical Adversarial Training (\algoName) which controls the decision boundary to move faster from more vulnerable points with smaller robust radii. We experimentally demonstrate that \algoName alleviates the conflicting dynamics and obtains improved robustness over state-of-the-art defenses.  



==> Neurips/s2_prelim.tex <==
\section{Preliminaries} \label{sec:prelim}
\subsection{Notations and definitions}
\textbf{Data and model} \quad We consider a classification task with inputs $x \in \mathcal{X}$ of dimension $d$ and corresponding labels $y\in\mathcal{Y} = \{1,2,...,K\}$.
Let $\{x_i,y_i\}_{i=1}^N$ be all training data of size $N$. A neural network classifier parameterized by $ \theta $ of dimension $p$ is denoted by $f_{\theta}(x) = \argmax_{c\in\mathcal{Y}}z_{\theta}^c(x)$ where $z_{\theta}^c(x)$ is the logit for class $c$. Denote $z_\theta(x)$ to be the vector of logits for all classes. 

\textbf{Decision boundary} \quad Denote the logit margin of class $ y $ as $ \phi^{y}_{\theta}(x) = z_{\theta}^y(x) - \max_{y'\neq y} z_{\theta}^{y'}(x) $. In the paper, we will use $\phi^{y}_\theta(x)$ and $\phi^{y}(x,\theta)$ interchangeably. Observe that $ x $ is classified as  $ y $ if and only if $ \phi^{y}_{\theta}(x) > 0 $. Therefore,  the zero level set of $ \phi^{y}_{\theta}(x) $, denoted by $ \Gamma_y=\{x: \phi^{y}_{\theta}(x) = 0\} $, is the decision boundary for class $ y $. 
% and omit the superscript $y$ when the indication is clear in the context. 
For a correctly classified point $(x,y)$, its robust radius $R_\theta(x)$ is defined to be the distance from $x$ to the decision boundary for class $y$. That is,
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
\begin{equation} \label{eq: robustness_radius}
    R_\theta(x) = \min_{\hat{x}} \|\hat{x}-x\|_p \quad \textrm{s.t.}  \quad \phi_\theta^y(\hat{x}) = 0
\end{equation}
where $\|\cdot\|_p$ is the $L_p$ norm with $1\leq p \leq \infty$.

% \textbf{Adversarial examples} \quad An correctly classified $(x,y)$ is said to be non-robust under perturbation threshold $\epsilon$ if its distance to the decision boundary $R(x) \leq \epsilon$. In this case, there exists an adversarial example $x'$ with$\|x'-x\|_p\leq \epsilon$ and its prediction $f_\theta(x') \neq y$.  

% \paragraph{Measuring adversarial robustness} Let $h$ be an non-increasing function that measures the vulnerability of robustness radius $R(x)$. To measure the adversarial robustness, define the following 

% \begin{equation} \label{Direct loss}
%     L_1(\theta) = \mathbb{E}_{(x,y)\sim D}[h(R_\theta(x))\cdot \mathbbm{1} \{f_\theta(x) = y\} + \mathbbm{1} \{f_\theta(x) \neq y\}]
% \end{equation}

% Note that when $h$ is $h(r) = \mathbbm{1}\{r\leq\epsilon\}$, $L_1$ is exactly the robust error \citep{zhang2019theoretically} under the perturbation threshold $\epsilon$. Here we consider more general $h$. \yc{How does it fit into our story?}

\subsection{Adversarial training}
Traditional adversarial training (AT)~\citep{madry2017towards} adopts the following objective
% \begin{equation} \label{eq: AT}
%     \min_\theta \mathbb{E}_{(x,y)\sim D} \Big[\max_{\|x'-x\|\leq \epsilon} l(z_\theta(x'),y) \Big]  
% \end{equation}
\begin{align} 
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
     \min_\theta \frac{1}{N}\sum_{i=1}^{N}l(z_\theta(x'_i),y_i) %\label{eq: AT}
     \quad \text{ where }    x'_i = \argmax _{\|x'-x_i\|\leq \epsilon} l(z_\theta(x'),y_i) \label{eq: AT inner}
\end{align}
where $l$ is a suitable loss function (e.g. the cross-entropy loss). In other words, AT employs the worst-case adversarial data for updating the parameters. In practice, the projected gradient descent method (PGD) \citep{madry2017towards} is most commonly used for solving the inner maximization problem.

% Weighted adversarial training methods \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware} assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robustness radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to the robustness radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used so that the an example with larger logit margin value is viewed as more robust. However, a larger logit margin value does not necessarily correspond to a larger robustness radius. For example, it can happen that a clean example $x$ is very closed to the decision boundary in the input space $\mathcal{X}$, but still has a very large $\phi^y_\theta(x)>0$ because the gradient of $\phi_\theta^y$ with respect to the input might be large.

% Unlike traditional AT that trains on the worst-case adversarial examples, MMA \citep{Ding2020MMA} explicitly trains on the closest boundary point. However, since MMA adopts a simple average of the cross-entropy loss over a batch of closest boundary points, it is not guaranteed that the robust radii of every vulnerable point in the batch will be improved. 

% \begin{equation} \label{eq: weighted AT}
%     \min_\theta \sum_{i=1}^{N}c_il(z_\theta(x'_i),y_i)
% \end{equation}
% where $c_i$ is larger when $x_i$ is considered to have a smaller robust radius. 




\subsection{Continuous-time formulation}
In this paper, we will use the continuous-time formulation for the optimization on the parameters $\theta$, which allows us to study the instantaneous movement of the decision boundary in Section~\ref{sec: dynamics_of_bdr}.

Let $\theta'(t)$ be the continuous-time description of a training algorithm, which consists of two parts: a loss function $L$ and an optimization scheme. To derive the discrete counterpart $\theta'_k$ of $\theta'(t)$ at iteration $k$ given a training algorithm, we use the relationship $\theta'_k :=\frac{\theta_{k+1} - \theta_{k}}{\gamma}$, where $\gamma$ is the learning rate. 
For example, consider the commonly used stochastic gradient descent (SGD) with momentum ($\lambda_m$) and weight decay  ($\lambda_w$) given by
\begin{equation} \label{eq: SGD_momentum_weightDecay shorter}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
\begin{aligned}
    b_{k+1} = \nabla_\theta L(\theta_{k}) +  \lambda_w \theta_{k} + \lambda_m b_{k}, \quad \quad 
    \theta_{k+1} = \theta_{k} - \gamma b_{k+1}
\end{aligned}
\end{equation}
where $b_0 = 0$ and $b_k$'s are the intermediate variables. In this case, $\theta'_k$ is given by 

\begin{equation} \label{eq: theta prime momentum weight decay general}
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{aligned}
    \theta'_k &= -\nabla_\theta L(\theta_{k})  - \lambda_w \theta_{k}- \lambda_m b_{k} %\fhc{?}\text{\yc{What is unclear?}}
\end{aligned}
\end{equation}

which can be interpreted as the un-normalized update direction of $\theta$ at step $k$. 

==> Neurips/s3_dynamics4DB.tex <==
\section{Dynamics of the decision boundary} \label{sec: dynamics_of_bdr}
In this section, we will study the dynamics of the decision boundary in continuous time. We first define its speed with respect to each data point, and then provide a closed-form expression for the speed.
Finally, we visualize the speed of the decision boundary of AT and analyze its dynamics. 

\subsection{Speed of the decision boundary}
Consider a correctly classified clean example $(x_i,y_i)$. Our goal is to capture the movement of the decision boundary $\Gamma_{y_i} (t) = \{x:\phi^{y_i}(x,\theta(t)) = 0\}$ w.r.t. $x_i$ as $t$ varies continuously. To this end, we consider the curve of the closest boundary point $\hat{x}_i(t)$ on $\Gamma_{y_i} (t)$ to $x_i$:


\begin{definition}[Curve of the closest boundary point $\hat{x}_i(t)$] \label{def: closest_pt}
Suppose that $(x_i,y_i)$ is correctly classified by $f_{\theta(t)}$ in some time interval $t \in I$. Define the curve of the closest boundary point $\hat{x}_i(\cdot): I \to \mathcal{X}$ as
\begin{equation} \label{eq: closest_pt}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
    \hat{x}_i(t) = \argmin\nolimits_{\hat{x}} \|\hat{x}-x_i\|_p \quad \textrm{s.t.}  \quad \phi^{y_i}(\hat{x},\theta(t)) = 0.
\end{equation}
Define the robust radius of $x_i$ at time $t$ to be $R(x_i,t) = \|\hat{x}_i(t)-x_i\|_p $.
%\fhc{we need to explain $l_p$ norm. For example, how to choose $p$. Or what values can $p$ take?}\yc{added an explanation in prelim section.}
\end{definition}

\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-2.5em}
    \centering
    \includegraphics[width=0.3\columnwidth]{Intepretation_fig/AT_Dynamics-derivation.pdf}
    \vspace{-1.5em}
    \caption{Curve of the closest boundary point $\hat{x}(t)$ (in blue) of the data point $x$.}
    \label{fig:curve}
\vspace{-2em}
\end{wrapfigure}

An example of the curve of the closest boundary point is depicted in Figure~\ref{fig:curve}.
To understand how the distance between the decision boundary $\Gamma_{y_i} (t)$ and $x_i$ changes, it suffices to focus on the curve of the closest boundary point $\hat{x}_i(t)$. We define the speed of the decision boundary to be the time derivative of the robust radius as follows:

\begin{definition}[Speed of the decision boundary $s(x_i,t)$] \label{def: speed_of_bdr}
Under the setting of definition \ref{def: closest_pt}, define the speed of the decision boundary w.r.t. $x_i$ as $s(x_i,t) = \frac{d}{dt} R(x_i,t) = \frac{d}{dt}  \|\hat{x}_i(t)-x_i\|_p$.
% \begin{equation} \label{eq: speed_of_bdr}
%     s(x_i,t) = \frac{d}{dt} R(x_i,t)
% \end{equation}
\end{definition}

Note that the speed $s(x_i,t) > 0$ means that the robustness is improving for $x_i$ at time $t$, which is desirable during adversarial training. The following proposition gives a closed-form expression for the speed, given a training algorithm $\theta'(t)$.

\begin{proposition}[Closed-form expression of the speed $s(x_i,t)$] For $1 \leq p \leq \infty$,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}   
\begin{equation} \label{eq: expression_for_speed}
    s(x_i,t) = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)
\end{equation}
where $q$ satisfies that $1/q+1/p=1$. In particular, $q=2$ when $p=2$ and $q=1$ when $p=\infty$.
\end{proposition}

\paragraph{Remark}
The main assumption for Equation~\eqref{eq: expression_for_speed} is the local differentiability of $\phi^{y_i}(\cdot,\theta(t))$ at $\hat{x}_i(t)$.  The full assumptions, proof and discussions are left to Appendix~\ref{app: closed_expression_speed}. The key points of proving Equation~\eqref{eq: expression_for_speed} include the level set equation \citep{osher2004level,aghasi2011parametric} and the optimality condition for optimization problem~\eqref{eq: closest_pt}. Special care has been taken for $p=\infty$ since $L_\infty$ norm is not differentiable.

According to Equation~\eqref{eq: expression_for_speed}, the speed $s(x_i,t_0) $ is positive at time $t_0$ when $\nabla_\theta \phi^{y_i} (\hat{x}_i(t_0),\theta(t_0)) \cdot \theta'(t_0) >0$, i.e. the value of $\phi^{y_i}(\hat{x}_i(t_0))$ increases. This means that the boundary point $\hat{x}_i(t_0)$ will be correctly classified after the update. Also, the magnitude of the speed tends to be larger if $\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q$ is smaller, i.e. the margin function $\phi^{y_i}$ is flatter around $\hat{x}_i(t)$. In the remaining part of the paper, we will denote $s(x_i,t)$ and $R(x_i,t)$ as $s(x_i)$ and $R(x_i)$ when the indication is clear.

% \begin{Sproof}
% Here we provide a proof sketch for $p=2$. 
% To compute $ s(x_i,t) = \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_2$, we need to characterize the curve of the closest boundary point $\hat{x}_i(t)$, where two key points stand out. First, $\hat{x}_i(t)$ is on the decision boundary $\Gamma_y (t)$ and thus  $\phi^y(\hat{x}_i(t),\theta(t)) = 0$ for all $t \in I$. By taking the time derivative on both sides, we obtain the level set equation \citep{osher2004level,aghasi2011parametric}
% \begin{equation} \label{eq: LF}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
% 	\nabla_x \phi^{y}(\hat{x}_i(t),\theta(t))\cdot \hat{x}_i'(t) + \nabla_\theta \phi^{y} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) = 0
% \end{equation}
% Second, $\hat{x}_i(t)$ is the optimal solution of constrained optimization \eqref{eq: closest_pt}. Therefore, we have the following optimality condition:
% \begin{equation} \label{eq: optimality}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
%     \nabla_x \phi^{y}(\hat{x}_i(t),\theta(t)) + \lambda(t)\nabla_x\|\hat{x}_i(t)-x_i\|_p = 0
% \end{equation}
% where $p=2$ and the scalar function $\lambda(t) = \|\nabla_x \phi^{y}(\hat{x}_i(t),\theta(t))\|_2 > 0$. 
% Note that $s(x_i,t) = \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_2 = \nabla_x\|\hat{x}_i(t)-x_i\|_2 \cdot \hat{x}_i'(t)$. Therefore, by plugging in equation \eqref{eq: LF} and \eqref{eq: optimality}, we obtain the closed-form expression in equation \eqref{eq: expression_for_speed}.

% Note that since $L_\infty$ norm is not differentiable, the optimality condition in Equation \ref{eq: optimality} is not valid for $p=\infty$ and special care needs to be taken. We leave the proof for $p =\infty$ in the appendix \ref{app: closed_expression_speed}, along with the general case where $1 \leq p < \infty$.
% \end{Sproof}


\textbf{Computing the closest boundary point}\quad 
To implement the Equation~\eqref{eq: expression_for_speed} in practice, we need to compute the closest boundary point $\hat{x}_i(t)$. We use the Fast Adaptive Boundary Attack (FAB) \citep{croce2020minimally} to approximate $\hat{x}_i(t)$. Specifically, FAB iteratively makes projection to the linearly approximated decision boundary with a bias towards the original data point, so that the resulting boundary point is close to the original point $x_i$. Note that here FAB only serves as an algorithm to approximate $\hat{x}_i(t)$, and can be decoupled from the remaining part of the framework. While finding the global optimum of Equation~\eqref{eq: closest_pt} is difficult due to its non-convex nature, in our experiments we find that FAB can reliably find its local optimum given enough number of iterations. In this case, the expression for speed in Equation~\eqref{eq: expression_for_speed} is still valid. We give more details of how to check the local optimality condition of Equation~\eqref{eq: closest_pt} and the performance of FAB in Appendix~\ref{app: optimality}. 



% \paragraph{Continuous update rule $\theta'$} To specify $\theta'$ from an training algorithm, we use the relationship $\theta'_k =\frac{\theta_{k+1} - \theta_{k}}{\gamma}$ \yc{notation?} where $\gamma$ is the learning rate. Note that $\theta_{k+1} - \theta_{k}$ depends on both the training loss $L$ and the optimization method. In this paper, we adopt the commonly used gradient descent with momentum ($\lambda_m$) and weight decay  ($\lambda_w$) given by

% \begin{equation} \label{eq: SGD_momentum_weightDecay shorter}
% \begin{aligned}
%     b_{k+1} &= \nabla_\theta L(\theta_{k}) +  \lambda_w \theta_{k} + \lambda_m b_{k} \\
%     \theta_{k+1} &= \theta_{k} - \gamma b_{k+1}
% \end{aligned}
% \end{equation}

% when $k>1$ with $b_0 = 0$ and $b_k$'s are intermediate variables. In this case, $\theta'_k$ is given by 

% \begin{equation} \label{eq: theta prime momentum weight decay general}
% \begin{aligned}
%     \theta'_k &= -\nabla_\theta L(\theta_{k})  - \lambda_w \theta_{k}- \lambda_m b_{k}
% \end{aligned}
% \end{equation}


\subsection{Dynamics of adversarial training} \label{ssec: Dynamics of adversarial training}
In this section, we numerically compute the speed of the decision boundary during AT. We first show a strong correlation between the speed and the improvement of robust accuracy over time. Then we visualize the speed and identify the conflicting dynamics of the decision boundary in AT. More visualizations and analysis of the dynamics on other training methods are left to Appendix~\ref{app: more_dynamics}. 

\textbf{Experiment setting}\quad We train a ResNet-18 \citep{he2016deep} on CIFAR-10 using 10-step PGD under $L_2$ perturbation with $\epsilon=0.5$ from a naturally pretrained model and evaluate it using 20-step PGD.
% under the same $\epsilon$. 
% We replace the Batch Normalization (BN) layers with Group Normalization (GN) layers \citep{wu2018group} because BN causes the classifier to have different decision boundary in training and test mode. We found that replacing BN with GN has negligible effect on the robustness performance. 
Figure~\ref{fig: interpretation_acc} shows the test clean and robust accuracy, as well as the \textit{robust accuracy within correct points}: the proportion of robust data points within correctly classified ones, which is computed by the ratio between the robust accuracy and clean accuracy. %\yc{
We consider the robust accuracy within correct points since the speed is only defined for correctly classified ones.
%} 
We will experimentally examine the correlation between the robust accuracy within correct points and the dynamic.
% speed of the decision boundary.

\input{fig_interpret_test}
% \input{fig_interpret}

\textbf{Dynamics and robustness improvement}\quad We choose 512 points from the test set and at each iteration, we compute the robust radii and speed for correctly classified points. We omit those points whose radii are larger than $1$, which are considered very robust under $\epsilon=0.5$. 
For every iteration, we normalize the speed values to have the maximum absolute value 1 for better visualization of their relative magnitude.
The result is shown in Figure~\ref{fig: interpretation_VR_test_scatter}.
The set of points 
$\mathcal{S}_{\mathsf{g}} = \{x_i: R(x_i)<0.5, s(x_i)>0\}$
(top left corner) can be viewed as vulnerable but are being improved, whereas points in
$\mathcal{S}_{\mathsf{b}} = \{x_i: 0.5<R(x_i)<1, s(x_i)<0\}$
(bottom right corner) can be considered as robust but are being compromised. Observe that at the start of training (e.g. iteration 5 and 30), the proportion  of $\mathcal{S}_{\mathsf{g}}$, denoted as $p(\mathcal{S}_{\mathsf{g}})$, is relatively large and $p(\mathcal{S}_{\mathsf{b}})$ is relatively small. At the same time, the robust accuracy within correct points increases drastically, as shown in figure \ref{fig: interpretation_acc}. At the later stage (e.g. iteration 200), $p(\mathcal{S}_{\mathsf{g}})$ decreases and $p(\mathcal{S}_{\mathsf{b}})$ increases, and the robustness improvement slows down. In order to capture the robustness improvement using dynamics, we compute $p(\mathcal{S}_{\mathsf{g}}) - p(\mathcal{S}_{\mathsf{b}})$ which is shown in Figure~\ref{fig: interpretation_acc_d}, along with the time derivative of the robust accuracy within correct points. We observe that both of them show the same pattern, indicating the strong correlation between the dynamics of the decision boundary and the robustness improvement during AT.


\textbf{Conflicting dynamics}\quad Since the update of the parameters $\theta$ at each iteration is computed on one batch of the training data, we visualize the radii and speed on the training batch of each iteration in Figure~\ref{fig: interpretation_VR_trainBatch_all}. Observe that there is always a significant proportion of non-robust points (with $R(x_i)<0.5$) with negative speed, indicating the conflicting dynamics on the training batch. This is not desirable because ideally at each iteration, the vulnerable points in the training batch should be improved since the current update of $\theta$ is computed on them.
% \yc{This is also typical in other variants of AT, which is shown in appendix.} 
In Section~\ref{sec:dynamicalAT}, we will see that such conflicting dynamics can be avoided: since the update rule has full access to the training batch, it is possible to design the update rule so that every vulnerable point in the training batch is made more robust. 


\input{fig_intepret_train}




==> Neurips/s4_dynamicalAT.tex <==
% old method: Dyna-CAT (computationally expensive because of FAB for hard boundary; memory expensive because of reverse-engineering)
\section{\algoName: \algoNameFull}\label{sec:dynamicalAT}

To remedy the conflicting dynamics issue and encourage robustness improvement on more vulnerable points, we propose \algoNameFull (\algoName), which customizes the dynamics of the decision boundary for each data point. We first introduce the design of the desirable dynamics in Section~\ref{ssec: dynamics_design}, and then present the algorithm in Section~\ref{ssec: realizing_dynamics}.
 
\subsection{Design of desirable dynamics} \label{ssec: dynamics_design}


% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}

Ideally, the decision boundary should move away from each vulnerable point. Moreover, given the limited capacity of the neural networks, robustness improvement on more vulnerable points should be encouraged more. Therefore, the desirable dynamics should satisfy the following speed conditions: 
\begin{list}{$\rhd$}{\topsep=0.ex \leftmargin=0.3in \rightmargin=0.in \itemsep =0.0in}
    \item \textbf{Condition 1:} $s(x_i) > 0 $ when $R(x_i) < r_0$ for some threshold $r_0$. 
    \item \textbf{Condition 2:} $s(x_i) \geq s(x_j)$ when $R(x_i) < R(x_j)$.
\end{list}

In particular, \textbf{Condition 2} considers customized manipulation of the decision boundary by encouraging smaller robust radii to improve faster. The goal of \algoName is to approximate both conditions and thus achieving fairer robustness to each data point as well as better overall robustness.
% under the limited model capacity.

% In particular, \textbf{Condition 2} considers a customized manupulation of the decision boundary. When satisfied, it robustifies each individual vulnerable point\yc{..fairness; dyna-cat; customized..}. % rather than focusing on the average robustness (or more accurately (un)weighted average of surrogate robustness) as in most prior works. 
% Consequently, \textbf{Condition 2} achieves a fairer robustness to individuals, leading to better overall robustness under a limited model capacity as well. % \yc{Not quite accurate: Previous work focus on surrogate loss, weighted average. We focus on improving radius faster.}


To design such desirable dynamics, we introduce a \textit{ratio function} $g(r)$, a non-increasing function that satisfies $g(r) > 0$ when $r < r_0$ for some threshold $r_0$. 
At each iteration, the speed $s(x_i)$ of the decision boundary w.r.t. $x_i$ should be approximately proportional to $g(R(x_i))$. In other words, $s(x_i) \approx \mu \cdot g(R(x_i))$ for some common scalar $\mu > 0$ for all data points. Since the effect of $g$ does not change if it is multiplied by a constant, we fix $g(0) = 1$. 


\textbf{Controlling the robustness level with the ratio function}\quad Instead of using a pre-defined perturbation length to control the robustness level, \algoName uses all of the closest boundary points, 
% with respect to all correctly classified data points during training
including those that are relatively far from the original ones. The ratio function $g$ controls the robustness level: if $g$ decays more slowly, \algoName will encourage robustness improvement even when the robust radius is large, and thus the model is robust to larger perturbation thresholds. On the other hand, if $g$ decays fast, the improvement on the non-robust points will be encouraged more.
% , so the model is unlikely to be able to withstand larger perturbation thresholds. 
How to calculate the optimal $g$ is still an open question. Therefore, we heuristically design different $g'$s and discuss more about them in Section~\ref{sec:exp_effect} and Appendix~\ref{app: further_exp_results}.

\subsection{\algoName: Realizing the desirable dynamics} \label{ssec: realizing_dynamics}
In order to customize the dynamics of the decision boundary for each data point, we propose to use a weighted average of loss on the closest boundary points and compute the weights to achieve the designed dynamics. Consider a batch $\mathcal{B}$ with size $n$ and denote $\mathcal{B}^{+}_\theta$ of size $m$ to be the set of correctly classified points in $\mathcal{B}$. We use the following form for the loss function
\begin{equation} \label{eq: weighted loss general}
	L_\theta(\mathcal{B}) =  -\sum\nolimits_{i\in \mathcal{B}^{+}_\theta}c_i \phi^{y_i}(\hat{x}_i) + \lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}l(x_i,y_i) 
\end{equation}
where the first term is the weighted margin loss on the closest boundary points $\hat{x}_i$'s with weights $\{c_i\}$ to be determined. The second term is the average cross-entropy loss on natural data points.

The speed $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$ depends on the weights $\mathbf{c} = (c_1,\cdots, c_m)^{T}$ in the following way: $\mathbf{c}$ determines the loss function by Equation~\ref{eq: weighted loss general}; the loss function, together with an optimization scheme, determines $\theta'(t)$ (for example, by Equation~\ref{eq: theta prime momentum weight decay general}); finally, $\theta'(t)$ determines the speed $\mathbf{s}$ by the closed-form expression~\ref{eq: expression_for_speed}. Note that all of these dependencies are linear, and thus $\mathbf{s}$ is a linear function of $\mathbf{c}$, denoted by $\mathbf{s}(\mathbf{c})$. 


Our goal is to reverse engineer the weights $\mathbf{c}$ so that the speed $\mathbf{s}(\mathbf{c})$ approximates the designed dynamics specified by the ratio function $g$. Let the ratio values $\mathbf{g} = (g(R(x_1)),\cdots,g(R(x_{m})))^{T}$. To approximate the desired dynamics given by $\mathbf{g}$, we solve the following optimization problem:
\begin{equation} \label{eq:opt_for_weight}
\begin{aligned}
\min_{\mathbf{c}, \mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} c_i = 1, \quad c_i\geq0, \quad \mu \geq 0    \\
\end{aligned}
\end{equation}
% \vspace{-0.1em}
% \fhc{I feel this is hiding too much details by using $\mathbf{s}(\mathbf{c})$?}
% \yc{Write out the dependency}
where $\mu$ is a scalar so that the solved $\mathbf{s}(\mathbf{c})$ is approximately a multiple of $\mathbf{g}$.
The problem~\eqref{eq:opt_for_weight} is a quadratic programming problem with linear constraints of size $m+1$, which is convex and can be solved efficiently and reliably. 
According to our experiments, the extra runtime of solving this quadratic programming is negligible.
We give the coefficient of this quadratic programming problem in Appendix~\ref{app: opt_for_weight}. The pseudocode of \algoName is shown in Appendix~\ref{app: algo_pseudo}. We also introduce a burn-in period where we only use the clean loss during the initial stage of the training to achieve a descent clean accuracy. This is necessary because the closest boundary points used by \algoName can only be found for correctly classified examples. 

% \input{algo} 




% Let the ratio values $\mathbf{g} = (g(R(x_1)),\cdots,g(R(x_{m})))^{T}$ and $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$. 
% According to the speed expression \eqref{eq: expression_for_speed}, the expression of $\theta'_k$ in \eqref{eq: theta prime momentum weight decay general} and the loss function \eqref{eq: weighted loss general}, $\mathbf{s}$ is a linear function of the  weights $\mathbf{c}$ and we denote it as $\mathbf{s}(\mathbf{c})$. 





==> Neurips/s5_related.tex <==
\section{Related Work}\label{sec:related}

\textbf{Controlling parameterized surface}\quad 
The decision boundary can be viewed as a parameterized surface in the input space. Controlling such surface has been studied in image segmentation\citep{li2011level,aghasi2011parametric} and shape modelling\citep{chen2019learning,park2019deepsdf}. As for adversarial training, the authors of \citep{Atzmon2019control} propose to maximize the distance between each data point and some point on the decision boundary, which is not the closest one. On the other hand, we study the movement of the decision boundary w.r.t. each data point by analyzing its closest boundary point, which is directly related to the 
robust radius. 

\textbf{Comparisons with related adversarial training methods}\quad 
There are several defense techniques including gradient regularization \citep{moosavi2019robustness,tramer2017ensemble}, certified denfense\citep{cohen2019certified,wong2018provable,balunovic2019adversarial} and adversarial training \citep{madry2017towards,zhang2019theoretically,gowal2020uncovering,wang2019improving,zhang2020attacks}, where the last one is the most related to this work. 
In particular, MMA\citep{Ding2020MMA} trains on the closest boundary points, which is similar to \algoName. However, MMA adopts uniform weights and thus does not consider the vulnerability difference among the points. On the other hand, weighted adversarial training methods \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware} assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. 



% so that an example with a larger logit margin value is viewed as more robust. However, a larger logit margin value does not necessarily correspond to a larger robust radius. 


==> Neurips/s6_exp.tex <==
\section{Experiments}\label{sec:exp}
In this section, we empirically evaluate the effectiveness and performance of the proposed \algoName on the CIFAR-10 \citep{krizhevsky2009learning} dataset. In Section~\ref{sec:exp_effect}, we visualize the dynamics and the robust radius distribution for different designs of the ratio function $g$. In Section~\ref{sec:exp_robust}, we evaluate the robustness of \algoName and compare it with several state-of-the-art baselines. Implementation details are left to Appendix \ref{app: exp_settings}, including neural network architecture and training hyperparameters. 
% Further experimental results are presented in Appendix \ref{app: further_exp_results}.

\subsection{Effectiveness of \algoName}
\label{sec:exp_effect}
\textbf{Realizing the desirable dynamics}\quad \algoName computes the weights to approximate the desirable dynamics by solving the optimization problem \eqref{eq:opt_for_weight}. To verify the quality of this approximation, we consider the $L_2$ norm constrained perturbation and choose the ratio function $g(r) = 1 - r$ when $r \leq 1$ and $g(r)=0$ otherwise. 
In Figure~\ref{fig: performance_batch_VR_ours}, we visualize the speed and robust radii of points in the training batches of three randomly chosen iterations.
We observe that the speed is positive for most of the points and is approximately a decreasing function of the robust radius, which is consistent with the design of $g$. 
By comparing with the conflicting dynamics of AT in Figure~\ref{fig: interpretation_VR_trainBatch_all}, we conclude that \algoName alleviates the conflicts and achieves the desirable dynamics during training. 


\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{experiment_fig/Our_batch_scatter}}
        \caption{Radius-speed plot of \algoName %on the training batch
        }
        \label{sfig: performance_batch_VR_ours_scatter}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.52\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{experiment_fig/Our_batch_hist}}
        \caption{Histogram of speed}
        \label{sfig: performance_batch_VR_ours_hist}
    \end{subfigure}
    \vspace{-0.3em}
    \caption{Radius-speed plot of \algoName on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations. Proportion of points with negative speed for these iterations are all below $2\%$.}
    \label{fig: performance_batch_VR_ours}
\end{figure} 


\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-1em}
    \centering
    \begin{subfigure}[b]{0.26\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{experiment_fig/ratio_function}}
        \vspace{-1.5em}
        \caption{Ratio function}
        \label{sfig: performance_ratio_function}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{experiment_fig/radius_distribution}}
        \vspace{-1.5em}
        \caption{radius distribution}
        \label{sfig: performance_radius_distribution}
    \end{subfigure}
    \vspace{-0.3em}
    \caption{Different choices of the ratio function $g$ and the corresponding radius distributions when using \algoName.
    }
\vspace{-1.2em}
\end{wrapfigure}


\textbf{Ratio function controls the robust radius distribution}\quad 
\algoName uses the ratio function $g$ to control the robustness level. As discussed in Section~\ref{ssec: dynamics_design}, the trained model is expected to be robust to larger perturbation thresholds if $g$ decays slower. To verify this, we fix $\lambda_c = 2$ in the $L_2$ norm setting and train on $g(r) = 1 - r/k$ when $r\leq k$ and $g(r)=0$ otherwise, for different $k$'s as shown in Figure~\ref{sfig: performance_ratio_function}. For these trained models, we use FAB (with 40 iterations) to compute the robust radius distributions for the correctly classified points from the test set,
% We discard the low-quality boundary points that do not satisfy the optimality condition of equation $\eqref{eq: closest_pt}$. 
which are shown in Figure~\ref{sfig: performance_radius_distribution}.
We can see that when $g$ decays slower, the robust radius distribution within correctly classified points spreads out more and tends to be more robust. Note that the overall robust accuracy is the product of the robust accuracy within correct points and the clean accuracy. We find that although a flatter $g$ leads to better robust accuracy within correct points, it decreases the clean accuracy. This shows that improving the robustness of points with large robust radii could harm the clean accuracy. Therefore, there is a trade-off between the robustness and clean accuracy, which is balanced by $\lambda_c$ and the choice of $g$.


\subsection{Robustness Evaluation}
\label{sec:exp_robust}
\textbf{Compared baselines}\quad
The baseline defense methods include: (1) standard adversarial training (AT) \citep{madry2017towards} which trains on the worst case adversarial examples generated by PGD; (2) TRADES \citep{zhang2019theoretically} which trades off between the clean and robust accuracy; (3) MMA \citep{Ding2020MMA} which trains on the closest adversarial examples with uniform weights; (4) GAIRAT \citep{zhang2021geometryaware} which reweights adversarial examples based on the least perturbation steps. Their hyperparameters are left to Appendix~\ref{app: exp_settings}. 

\paragraph{Evaluation protocol}%\quad
We evaluate \algoName and the baselines under $L_2$ and $L_\infty$ norm constrained perturbation. The final robust accuracy is reported on AutoAttack (AA) \citep{croce2020reliable}, which uses an ensemble of selected strong attacks. We also include the results under PGD attack with 40 iterations in Appendix~\ref{app: further_exp_results}. For all methods, we choose the hyperparameters to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. We also evaluate on larger perturbation thresholds to better examine the robustness of the models.
% against unknown perturbation strength.

\paragraph{Hyperparameters of \algoName}%\quad 
We use the ratio function with $g(0) = 1, g(r_0) = 0, g(r_1) = - g_1$ with $g_1 \geq 0 $ and linearly interpolate them when $0\leq r \leq r_1$. When $r>r_1$, $g(r)$ was set to the constant $-g_1$. We allow $g$ to be negative when $r > r_1$ because we experimentally find that 'pulling back' the decision boundary if it is too far away from data points could help improve both clean and robust accuracy. Choices of $r_0, r_1, g_1$ and other hyperparameters are left to Appendix~\ref{app: exp_settings}.
% In the $L_2$ setting, we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = -0.4$. In the $L_\infty$ setting, we set $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = -0.4$.
% \fhc{Move to appendix, mention here that we have all details in appendix REF.}



\paragraph{Performance}%\quad 
The main evaluation results are shown in Table \ref{table: performance_L2_more_eps} and Table \ref{table: performance_Linf_more_eps}. The full results are left to Appendix~\ref{app: further_exp_results}. In the $L_2$ case, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. In the $L_\infty$ case, \algoName obtains both higher clean accuracy and robust accuracy than AT, MMA and GAIRAT. We observe that GAIRAT achieves high robustness under PGD attacks (shown in Appendix~\ref{app: further_exp_results}) but has much lower robust accuracy under the stronger AA attack, which may be due to obfuscated gradient \citep{AthalyeC018}. On the other hand, the performance gap between PGD and AA is relatively small for \algoName. When compared with TRADES, \algoName shows higher clean accuracy and comparable robust accuracy under larger $\epsilon$, although \algoName has lower robust accuracy when $\epsilon = \frac{8}{255}$. This is partially due to the higher difficulty of approximating the closest boundary points in the $L_\infty$ case, and a better algorithm for this is left for future work. 
\input{tab_L2_moreEps}
\input{tab_Linf_moreEps}
% \input{tab_moreEps}

==> Neurips/s7_conc.tex <==
\section{Conclusion and Discussion} \label{sec:conc}

This paper has proposed a continuous-time framework to study the moving speed of the decision boundary w.r.t. each individual data point. Under this framework, the conflicting dynamics of adversarial training methods is revealed, where the decision boundary moves away from some data points but moves closer to other points and harms their robustness. To alleviate the conflicts, we propose \algoNameFull (\algoName) to customize the dynamics of the decision boundary for each data point, so that the decision boundary moves faster away from more vulnerable points. Under the limited model capacity, \algoName shows promising results on robustness performance. The future direction includes (a) more efficient and reliable algorithms for finding the closest boundary points; (b) better design of the desirable dynamics; (c) combining \algoName with other state-of-the-art methods such as TRADES; (d) using the proposed framework of dynamics to study the convergence of AT and other training algorithms. 




==> Neurips/s8_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Appendix~\ref{app: closed_expression_speed}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{app: closed_expression_speed}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{app: exp_settings}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}{We only use standard datasets}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Neurips/save.tex <==
Based on previous adversarial training method, we consider the weighted adversarial loss as the following form
\begin{equation} \label{eq: weighted loss general soft}
	-L_\theta(S) =  q\left[\sum_{i\in H_\theta^{+}}c_i\phi_\theta(\tilde{x}_i,y_i) + \sum_{i\in S_{\theta}^{-}}c_0 \phi_\theta(x_i,y_i) \right] + (1-q)\sum_{i\in S}\frac{1}{N}\phi_\theta(x_i,y_i) 
\end{equation}

where $\{c_i\}_{i=1}^{m}$ is the weights on boundary points $x_i \in H_\theta^{+}$ and $c_0$ is the weight on points in $S_{\theta}^{-}$. They satisfy that $\sum_{i=1}^{m}c_i + nc_0 = 1$. We further assign $c_0 = \frac{1}{m+n}$. Note that $\phi_{\theta}$ here can be replaced with negative cross entropy loss, which is more similar to adversarial training notational wise. Also, we don't require the weight to be positive (this could be improved by solving the closest point in the feasible set, but speed is not ratioed anymore..). 

Therefore, $\theta'(t)$ is of the form
\begin{equation} \label{eq: theta prime GD}
	\theta'(t) =  q\left[\sum_{i\in H_\theta^{+}}c_i\nabla_\theta\phi_\theta(\tilde{x}_i,y_i) + \sum_{i\in S_{\theta}^{-}}c_0 \nabla_\theta\phi_\theta(x_i,y_i) \right] + (1-q)\sum_{i\in S}\frac{1}{N}\nabla_\theta\phi_\theta(x_i,y_i) 
\end{equation}

\subsection{Enforcing the speed ratio}
We would like to find $c = (c_1,\cdots, c_m)$ such that the corresponding $\theta'(t)$ results in the speed $D(\tilde{x}_i,x_i)$ obeying the ratio $g(r_i)$. Denote $\mathbf{g} = (g(r_1),\cdots,g(r_m))^{T}$ and let $\mathbf{D} = (D(\tilde{x}_1,x_1),\cdots,D(\tilde{x}_m,x_m))^{T}$, which depends on $\theta'$ and $c$.
We aim to solve the following linear system for $c$ and a dummy scalar $\mu$:

\begin{equation}
    \begin{cases}
      \mathbf{D} &= \mu\cdot \mathbf{g}, \quad  \\
		\mathbf{1}_{m}^{T}c &= 1 - nc_0
    \end{cases}
\end{equation}

Result: Denote the $p$ dimensional vector $z = (qc_0 + \frac{1-q}{N})\sum_{i\in S_\theta^{-}} \nabla_\theta \phi_\theta(x_i,y_i) + \frac{1-q}{N}\sum_{j\in S_\theta^{+}}\phi_\theta(x_j,y_j)$, which is the term without boundary point in equation \ref{eq: theta prime GD}. Denote $A\in \mathbb{R}^{p\times m}$ as the matrix whose i-th column is $\nabla_i\phi_\theta(\tilde{x}_i,x_i)$, $i = 1,\cdots,m$. Also denote $\alpha \in \mathbb{R}^{m\times m}$ a diagonal matrix whose i-th diagonal $\alpha_i$ satisfies $D(\tilde{x}_i,x_i) = \frac{(x_i-\tilde{x}_i) \cdot \nabla_{x}\phi(\tilde{x}_i)}{\|x_i-\tilde{x}_i\|\|\nabla_x \phi(\tilde{x}_i)\|^2 }\nabla_\theta \phi(\tilde{x}_i) \cdot \theta'(t) = \alpha_i \nabla_\theta \phi(\tilde{x}_i) \cdot \theta'(t)$. That is, $\alpha_i = \frac{(x_i-\tilde{x}_i) \cdot \nabla_{x}\phi(\tilde{x}_i)}{\|x_i-\tilde{x}_i\|\|\nabla_x \phi(\tilde{x}_i)\|^2 }$ in $l_2$ case and $\alpha_i = \frac{\sign(x_i-\tilde{x}_i)\cdot \nabla_x \phi(\tilde{x}_i)}{\|\nabla_x \phi(\tilde{x}_i)\|_{2}^{2}}$ in L-infinity case. Then

\begin{equation} \label{eq: weight eqn}
    \begin{cases}
      \mu &= \frac{q(1-nc_0) + \mathbf{1}_{m}^{T}(A^{T}A)^{-1}A^{T}z}{\mathbf{1}_{m}^{T}(A^{T}A)^{-1}\alpha^{-1}\mathbf{g}}  \\
		c &= \frac{1}{q}(A^{T}A)^{-1}(\mu\alpha^{-1}\mathbf{g}-A^{T}z)
    \end{cases}
\end{equation}

Note that when using stochastic optimization, $N$ is the batch size and $(A^{T}A)^{-1} \in \mathbb{R}^{m\times m}$ with $m<N$. In practice we find that $\mu > 0 $, meaning that the decision boundary is moving away from points in $H_\theta^{+}$.




Consider a correctly classified clean example $(x_i,y_i)$ and a point $x(t)\in \Gamma^{y_i}(t)$ near $x_i$. In order to characterize the speed of a point $x(t)$ moving away from $x_i$ in the $l_2$ norm, we define $s(x,x_i)$ as the projection of $v(x(t))$ onto the direction $\frac{x-x_i}{\|x-x_i\|_2}$, i.e. $s(x,x_i) = v(x) \cdot \frac{x-x_i}{\|x-x_i\|} = \frac{(x_i-x) \cdot \nabla_{x}\phi(x)}{\|x_i-x\|\|\nabla_x \phi(x)\|^2 }\nabla_\theta \phi(x) \cdot \theta'(t)$. To capture the dynamics of the decision boundary $\Gamma^{y_i}$ near the data $x_i$, we define the speed of the decision boundary w.r.t $x_i$ to be the speed $s(\hat{x}_i,x_i)$ of the closest point $\hat{x}_i \in \Gamma^{y_i}$. That is,

\begin{equation}\label{eq: V_bdr_L2}
 s(\hat{x}_i,x_i) = \frac{(x_i-\hat{x}_i) \cdot \nabla_{x}\phi(\hat{x}_i)}{\|x_i-\hat{x}_i\|\|\nabla_x \phi(\hat{x}_i)\|^2 }\nabla_\theta \phi(\hat{x}_i) \cdot \theta'(t)
\end{equation}
where

\begin{equation} \label{eq: closest_adv} 
	\hat{x}_i  = \argmin_{x\in \Gamma^{y_i}} \|x - x_i\|
\end{equation}

Note that when the $l_2$ norm is used, by the KKT condition and the fact that $\hat{x}_i$ is the closest adversarial example at current time $t$, we have that $ \nabla_x \phi(\tilde{x}_i,\theta(t)) = \lambda (\tilde{x}_i-x_i) $ with $ \lambda < 0 $. Therefore, the equation \ref{eq: V_bdr_L2} reduces to 

\begin{equation} \label{eq: V_bdr_L2_concise}
	s(\hat{x}_i,x_i) = \frac{1}{\|\nabla_x\phi(\hat{x}_i)\|_2} \nabla_\theta \phi(\hat{x}_i) \cdot \theta'(t)
\end{equation}

\yc{Explanation of the above formula?} As the following theorem shows, the speed $s(\hat{x}_i,x_i)$ of the decision boundary is the derivative of the robustness radius in $l_2$ norm w.r.t time $t$. 

% \begin{equation}\label{eq:effective V}
%  D(x,x_i) = v(x) \cdot \frac{x-x_i}{\|x-x_i\|} = \frac{(x_i-x) \cdot \nabla_{x}\phi(x)}{\|x_i-x\|\|\nabla_x \phi(x)\|^2 }\nabla_\theta \phi(x) \cdot \theta'(t)
% \end{equation}

% This can be interpreted as the signed length of the velocity vector $v(x,t)$ on the direction of $x - x_i$. If $ D(x,x_i)>0 $, the point $ x $ on the decision boundary $ \Gamma(t) $ is going away from $ x_i $, which is favored in adversarial training. On the other hand, a negative $ D(x,x_i)<0 $ means that $ x $ is going towards $ x_i $ and thus $ x_i $ might become less robust. Note that since $ \phi(x) = 0 $ and $ \phi(x_i) > 0 $, $ (x_i-x) \cdot \nabla_{x}\phi(x) $ is typically positive. Since adversarial training often makes $ \phi(x) $ larger (that is, fix x, $ \phi(x,\theta(t)) $ has positive derivative with respect to $ t $), $ \nabla_\theta \phi(x) \cdot \theta'(t) $ is also typically positive. Therefore, a good adversarial learning algorithm should result in positive $ D(x,x_i) $ for $ x\in \Gamma(t) $ around $ x_i $. \ys{I feel the logic does not flow naturally here. You said that adversarial training often results in positive speed, but then you claim that good adversarial training should result in positive speed. If they already often have positive speed, what are we promoting? When is adversarial training not getting positive speed?}


\begin{theorem} \yc{Informal, need smoothness assumption} Suppose that $(x_i,y_i)$ is correctly classified by $f_\theta(t)$. Denote $r(x_i,\theta(t)) = \min_{\phi^{y_i}(x,\theta(t))=0} \|x-x_i\|_2 = \|\hat{x}_i - x_i\|_2$ the $l_2$ robustness radius of $x_i$ for the current model parameterized by  $\theta(t)$. Then $\frac{d}{dt}r(x_i,\theta(t)) = s(\hat{x}_i,x_i)$. In the discrete time setting, if the parameter is updated by $\theta_{k+1} \leftarrow \theta_{k} + \eta\theta'(t)$, then  $r(x_i,\theta(k+1)) - r(x_i,\theta(k)) = \eta s(\hat{x}_i,x_i) + O(\eta^2) $. Equivalently, $\nabla_\theta d(x_i,y_i;\theta) = \frac{\nabla_\theta \phi(\hat{x}_i)}{\|\nabla_x\phi(\hat{x}_i)\|}$. \yc{Need to fix confusion of k and t; cite MMA on this?}
\end{theorem}

When the $l_\infty$ norm is used, we consider the closest point $\hat{x}_i$ in $l_\infty$ norm and and define the speed of the decision boundary w.r.t $x_i$ as the projection of $v(\hat{x}_i)$ onto the $i_{*}$ coordinate direction, where $i_{*} = \argmax_{j} |\nabla_x \phi(\hat{x}_i)|_j $ is the coordinate index where $\nabla_x \phi(\hat{x}_i)$ has the largest absolute value. Therefore, the speed of the decision boundary w.r.t $x_i$ is given by

\begin{equation} \label{eq: V_bdr_Linf}
	s(\hat{x}_i,x_i) = \frac{|\nabla_x \phi(\hat{x}_i)|_{i_*}}{\|\nabla_x\phi(\hat{x}_i)\|^{2}_2} \nabla_\theta \phi(\hat{x}_i) \cdot \theta'(t)
\end{equation}

\begin{theorem} \yc{same issue as before} Suppose that $(x_i,y_i)$ is correctly classified by $f_\theta(t)$. Denote $r(x_i,\theta(t)) = \min_{\phi^{y_i}(x,\theta(t))=0} \|x-x_i\|_\infty = \|\hat{x}_i - x_i\|_\infty$ the $l_\infty$ robustness radius of $x_i$ for the current model parametrized by  $\theta(t)$. Then $\frac{d}{dt}r(x_i,\theta(t)) = s(\hat{x}_i,x_i)$. In the discrete time setting, if the parameter is updated by $\theta_{k+1} \leftarrow \theta_{k} + \eta\theta'(t)$, then  $r(x_i,\theta(k+1)) - r(x_i,\theta(k)) = \eta s(\hat{x}_i,x_i) + O(\eta^2) $.  \yc{Maybe put organize two theorems as one}
\end{theorem}


% The downside of using the logit margin in adversarial training is that it only looks at two classes, while there might exist several adversarial classes for a clean example. To mitigate this, we consider the soft logit margin given by $\phi^{\text{SLM}}_{\theta}(x,y; \beta) =  z_{\theta}^c(x) - \frac{1}{\beta}log\sum_{c'\neq c}e^{\beta z_{\theta}^{c'}(x)}$. The relationship between the two is given by $\phi^{\text{LM}}_{\theta}(x,y)  -\frac{log(K-1)}{\beta} \leq \phi^{\text{SLM}}_{\theta}(x,y; \beta) \leq \phi^{\text{LM}}_{\theta}(x,y) $. Note that $\phi^{\text{SLM}}_{\theta}(x,y; \beta) > 0 $ means x is classified as class $c$, but not vice versa. Consider the soft decision boundary of class $y$ given by $ \Gamma^{\text{soft}}_y=\{x: \phi^{\text{SLM}}_{\theta}(x,y;\beta) = 0\} $. Notice that since $l_{\text{xent}}(z_{\theta}(x),y;\beta) = -log(\frac{e^{\beta z_\theta^y(x)}}{\sum_{y'\neq y}e^{\beta z_\theta^{y'}(x)}}) = log(1+e^{-\beta \phi^{\text{SLM}}_{\theta}(x,y; \beta)})$, the soft decision boundary is also the zero level set of the function $\phi_\theta(x,y;\beta) = log2 - l_{\textit{xent}}(z_{\theta}(x),y;\beta)$, with $\phi_\theta(x,y;\beta) > 0 $ if and only if $\phi^{\text{SLM}}_{\theta}(x,y;\beta) > 0$. In the following, the decision boundary refers to the soft decision boundary $ \Gamma=\{x: \phi_\theta(x,y) = 0\} $, with the superscript $y$ and the temperature $\beta$ omitted.

% \subsection{Level set equation}
% \yc{Motivation of using LF?}
% In this section, we aim to derive the velocity vector of an arbitrary point on the decision boundary by the level set equation. To fix idea, take $ x(t) \in \Gamma_{y}(t) $ and define its velocity as 

% \begin{equation} \label{eq: v_representation}
% 	v(x(t)) = F(x(t)) \cdot \frac{\nabla_x \phi^{y}(x(t),\theta(t))}{\|\nabla_x \phi^{y}(x(t),\theta(t))\|_{2}}
% \end{equation}

% where $ F(x(t)) $ is a scalar and $ \frac{\nabla_x \phi^{y}(x(t),\theta(t))}{\|\nabla_x \phi^{y}(x(t),\theta(t))\|_{2}} $ is the unit vector on the normal direction. Note that we only care about the normal direction because any other directions orthogonal to it will not move the decision boundary. The movement of $ \Gamma^{y}(t) $ is characterized by the velocity of every point on the curve, i.e. $ \{v(x(t)), x(t)\in \Gamma^{y}(t)\} $. 

% In order to obtain the velocity $ v(x(t)) $, note that since $ x(t) $ stays on $ \Gamma^{y}(t) $, we have that $\phi^{y}(x(t), \theta(t))  = 0$.
% % \begin{equation} \label{eq: LF_any_t}
% % 	\phi(x(t), \theta(t))  = 0, \quad \forall t
% % \end{equation}
% By taking derivative with respective to $ t $, we obtain the level set equation  

% \begin{equation} \label{eq: level set equation para}
% 	\nabla_x \phi^{y}(x(t),\theta(t))\cdot v(x(t)) + \nabla_\theta \phi^{y} (x(t),\theta(t)) \cdot \theta'(t) = 0
% \end{equation}

% by noting that $ v(x,t) = x'(t) $. By plugging the velocity representation in equation \ref{eq: v_representation} into equation \ref{eq: level set equation para}, we obtain that $ F(x,t) = -\frac{\nabla_\theta \phi \cdot \theta'(t) }{\|\nabla_x \phi(x)\|} $ and the velocity vector is given by
% \begin{equation}
% 	v(x,t) = - \frac{ \nabla_\theta \phi^{y} \cdot \theta'(t) }{\|\nabla_x \phi^{y}(x)\|} \cdot \frac{\nabla_x \phi^{y}(x)}{\|\nabla_x \phi^{y}(x)\|}
% \end{equation}

% where $ \theta'(t) $ is given by any first order training algorithm. \yc{Simpler notation? Omit y and t?}

% Although equation \ref{eq: level set equation para} gives the velocity for an arbitrary point on the decision boundary, it is still unclear how the decision boundary moves w.r.t the individual data $x_i$ during training, which we will elaborate on in the next section.


\subsection{Optimization}
In previous section, we compute the weight with the assumption that vanilla stochastic gradient descent is used. That is, when learning rate is very small and gradient descent is used, running the obtained weighted algorithm will cause the points on the current batch to have the preferred speed ratio. However, in practice people use other optimization method other than vanilla SGD. A concrete example would be SGD with momentum ($\lambda_m$) and weight decay ($\lambda_w$). The update rule is given by

\begin{equation} \label{eq: SGD_momentum_weightDecay}
\begin{aligned}
    g_k &= \nabla_\theta L(\theta_{k-1}) + \lambda_w \theta_{k-1}  \\
    b_k &= \lambda_m b_{k-1} + g_{k} \\
    \theta_{k} &= \theta_{k-1} - \gamma b_k
\end{aligned}
\end{equation}
when $k>1$ and $b_0 = 0$. More succinctly,

\begin{equation} \label{eq: SGD_momentum_weightDecay shorter}
\begin{aligned}
    b_k &= \lambda_m b_{k-1} + \nabla_\theta L(\theta_{k-1}) + \lambda_w \theta_{k-1} \\
    \theta_{k} &= \theta_{k-1} - \gamma b_k
\end{aligned}
\end{equation}

Therefore, $\theta'$ is given by 

\begin{equation} \label{eq: theta prime momentum weight decay}
\begin{aligned}
    \theta'(t) &= -\sum_{i\in H_\theta^{+}}c_i\nabla_\theta l(\hat{x}_i,y_i)  - \lambda_c\sum_{i\in S}\frac{1}{N}\nabla_\theta l(x_i,y_i) - \lambda_w \theta(t) - \lambda_m b_{t}
\end{aligned}
\end{equation}

Therefore, we need to use $z = - \lambda_c\sum_{i\in S}\frac{1}{N}\nabla_\theta l(x_i,y_i) - \lambda_w \theta(t) - \lambda_m b_{t}$ in solution \ref{eq: opt for weight detail} in order to calibrate for the use of SGD with momentum and weight decay. 



\section{Interpretation}
\subsection{Predicting robustness accuracy using speed}
As a proof of concept, we will see that the speed is indeed related to the improvement of robustness accuracy, and can serve as a measure of effectiveness of adversarial training.

The robustness accuracy improvement $a_{t+1}^{\text{robust}} - \text{acc}_t^{\text{robust}} = P(R_{t+1}>\epsilon) - P(R_t>\epsilon)$ can be approximated by $a_{t}^{\text{clean}}\cdot\{P(R_t<\epsilon,R_{t+1}>\epsilon) - P(R_t>\epsilon, R_{t+1}<\epsilon)\}$,where $a_{t}^{\text{clean}}$ is the current clean accuracy.

One approximation is $$a_{t}^{\text{clean}}\cdot\{P(R_t<\epsilon,V_t>0) - P(\epsilon'>R_t>\epsilon,V_t<0)\}$$, where only the sign of the speed is used. Another approximation is $$a_{t}^{\text{clean}}\cdot\{P(R_t<\epsilon,R_t + V_t \cdot \textit{lr} >\epsilon) - P(R_t>\epsilon,R_t + V_t \cdot \textit{lr} <\epsilon)\}$$
We should expect that they approximate the improvement of robustness accuracy. 

Note: In the implementation, the accuracy and  speed are computed every $T$ iterations. However, the speed $V_t$ is more related to the accuracy improvement at the current iteration $t$.

\section{Next}
\subsection{Findings and thoughts}

Speed and landscape through the course of training:
\begin{itemize}
    \item The speed gets larger as training goes on. There are two factors. The first one is that the landscape (the cross entropy landscape in the input space) becomes flatter. The second one is the next bullet point.
    \item The norm of gradient (or $\theta'$) gets larger as training goes on. One reason is that it is computed on less points. 
    \item Comparing speed across iterations gives us the speed of improvement on $H_\theta^{+}$ (which has different size every time). Even starting at the same $\theta$ using the same algorithm, different batch size will give different speed. Maybe $\frac{\theta'(t)}{\|\theta'(t)\|}$ (this also gets larger, since flatness of CE in the input space)
    \item Comparing speed on $H_\theta^{+}$ (training batch) does not tell us AT is harder or easier. 
\end{itemize}
\ys{Why doesn't a larger speed lead to a larger robust radius? Are there topological changes?
}

Hardness of AT using "speed":
\begin{itemize}
    \item Comparing speed among the whole distribution (training or testing) tells us the trade-off between the points. 
    \item We should come up with a measure that is kind of invariant to the scale of speed (since speed is going larger, but doesn't mean anything to harness of AT). For example, the sign of speed (although this is oversimplified I think). 
    \item Then what is a good measure (related to speed)?
\end{itemize}

% \paragraph{DAT improves the quality of robustness radius distribution} As discussed in section xx, imposing the desirable dynamics should help reduce the variance of the robustness radius distribution, decrease the proportion of very non-robust points and improve the overall robustness. To verify this, we track how the robustness radius distribution changes over time under $L_2$ case (since FAB is more reliable in $L_2$) for MMA and DAT. We use MMA since it claims that it is better at it than tradition AT. Specifically, we choose points from test data set and use FAB to compute the robustness radius at the end of each epoch. The change in distribution is shown in figure  \ref{fig: performance_radius_compare}

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=3cm]{example-image-a}
%     \caption{R histogram plot (for 5 time steps) for the test data. L2 for MMA and DAT}
%     \label{fig: performance_radius_compare}
% \end{figure}

% \yc{'DAT improves the quality of robustness radius distribution compared with AT' is not shown here anymore. Not fair comparison for AT.}

==> Neurips/tab_L2_moreEps.tex <==
\begin{table}[!htbp]
\centering
\noindent
\resizebox{\textwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=0.5$}  & {$\epsilon=1$} & {$\epsilon=1.5$}  & {$\epsilon=2$} \\
\midrule
AT & {$88.38 \pm 0.23$} & {$65.29 \pm 0.21$}  & {$33.71 \pm 0.16$}  & {$11.16 \pm 0.09$}  & {$2.4 \pm 0.17$}  & \\
TRADES & {$87.05 \pm 0.01$} & {$67.92 \pm 0.11 $}  & {$42.08 \pm 0.16$}  & {$19.33 \pm 0.38$} & {$6.62 \pm 0.16$}  & \\
MMA & {$\boldsymbol{88.40} \pm 0.14$} & {$65.62 \pm 0.23$}  & {$36.54 \pm 0.14$} & {$14.01 \pm 0.08$}  & {$3.49 \pm 0.10$}  & \\
\midrule
Ours & {$87.25 \pm 0.05$} & {$\boldsymbol{67.96} \pm 0.14$}   & {$\boldsymbol{43.48} \pm 0.23$}  & {$\boldsymbol{20.92} \pm 0.12$} & {$\boldsymbol{6.72} \pm 0.18$} &  \\
\bottomrule
\end{tabular}}
\caption{{Clean and robust accuracy on CIFAR-10 under $L_2$ attack}}
\label{table: performance_L2_more_eps}
\end{table}

==> Neurips/tab_Linf_moreEps.tex <==
% \begin{table}[!htbp]
% \centering
% \noindent
% \resizebox{\textwidth}{!}{\begin{tabular}{lSSSSSSSSSS}
% \centering
% & & \multicolumn{2}{c}{$\epsilon=\frac{8}{255}$} & \multicolumn{2}{c}{$\epsilon=\frac{12}{255}$} & \multicolumn{2}{c}{$\epsilon=\frac{16}{255}$} & \multicolumn{2}{c}{$\epsilon=\frac{20}{255}$} \\
% \cmidrule(r){3-4}\cmidrule(l){5-6}\cmidrule(l){7-8} \cmidrule(l){9-10}
% Defense & {Clean} & {AA}  & {PGD} & {AA}  & {PGD} & {AA}  & {PGD} & {AA}  & {PGD}\\
% \midrule
% AT & {$83.25 \pm 0.17$} & {$45.75 \pm 0.15$} & {$49.21 \pm 0.13$}  & {$26.38 \pm 0.14$} & {$30.41 \pm 0.19$} & {$12.34 \pm 0.17$} & {$15.73 \pm 0.12$} & {$4.89 \pm 0.11$} & {$7.35 \pm 0.14$} & \\
% TRADES & {$83.54 \pm 0.08$} & {$\boldsymbol{47.18} \pm 0.11$} & {$51.09 \pm 0.01$} & {$29.03 \pm 0.19$} & {$33.96 \pm 0.49$} & {$15.07 \pm 0.11$} & {$19.77 \pm 0.18$} & {$\boldsymbol{6.78} \pm 0.06$} & {$10.17 \pm 0.08$} & \\
% MMA & {$84.25 \pm 0.28$} & {$41.48 \pm 0.31$} & {$48.94 \pm 0.21$} & {$23.63 \pm 0.25$} & {$35.41 \pm 0.14$} & {$11.97 \pm 0.20$} & {$25.70 \pm 0.16$} & {$5.11 \pm 0.12$} & {$18.72 \pm 0.18$} & \\
% GAIRAT & {$81.31 \pm 0.23$} & {$32.98 \pm 0.11$} & {$58.72 \pm 0.52$} & {$16.19 \pm 0.02$} & {$41.29 \pm 0.52$} & {$6.89 \pm 0.18$} & {$25.16 \pm 0.08$} & {$2.57 \pm 0.07$} & {$12.95 \pm 0.29$} & \\
% \midrule
% Ours & {$\boldsymbol{85.13} \pm 0.13$} & {$46.47 \pm 0.18$} & {$47.86 \pm 0.22$}  & {$\boldsymbol{29.38} \pm 0.24$} & {$30.19 \pm 0.21$} & {$\boldsymbol{15.14} \pm 0.16$} & {$17.25 \pm 0.12$} & {$6.45 \pm 0.21$} & {$8.23 \pm 0.14$} & \\
% \bottomrule
% \end{tabular}}
% \caption{\small{Clean and robust accuracy on CIFAR-10 under $L_\infty$ attack} \yc{Maybe don't include ours-2 ours-3.} \fhc{Shall we move this table to appendix?}\yc{Only use AA; Put PGD in appendix and mention it in the main text}}
% \label{table: performance_Linf_more_eps}
% \end{table}
\begin{table}[!htbp]
\vspace{-2em}
\centering
\noindent
\resizebox{\textwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=\frac{8}{255}$} & {$\epsilon=\frac{12}{255}$} & {$\epsilon=\frac{16}{255}$} & {$\epsilon=\frac{20}{255}$} \\
\midrule
AT & {$83.25 \pm 0.17$} & {$45.75 \pm 0.15$} & {$26.38 \pm 0.14$} & {$12.34 \pm 0.17$} & {$4.89 \pm 0.11$}& \\
TRADES & {$83.54 \pm 0.08$} & {$\boldsymbol{47.18} \pm 0.11$}  & {$29.03 \pm 0.19$}& {$15.07 \pm 0.11$}  & {$\boldsymbol{6.78} \pm 0.06$} & \\
MMA & {$84.25 \pm 0.28$} & {$41.48 \pm 0.31$} & {$23.63 \pm 0.25$} & {$11.97 \pm 0.20$} &{$5.11 \pm 0.12$} & \\
GAIRAT & {$81.31 \pm 0.23$} & {$32.98 \pm 0.11$}& {$16.19 \pm 0.02$} & {$6.89 \pm 0.18$}  & {$2.57 \pm 0.07$} & \\
\midrule
Ours & {$\boldsymbol{85.13} \pm 0.13$} & {$46.47 \pm 0.18$}  & {$\boldsymbol{29.38} \pm 0.24$} & {$\boldsymbol{15.14} \pm 0.16$} & {$6.45 \pm 0.21$} & \\
\bottomrule
\end{tabular}}
\caption{{Clean and robust accuracy on CIFAR-10 under $L_\infty$ attack} }
\label{table: performance_Linf_more_eps}
\end{table}

==> Neurips/tab_moreEps.tex <==
\begin{table}[!htbp]

\centering
\noindent
\resizebox{\textwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=0.5$}  & {$\epsilon=1$} & {$\epsilon=1.5$}  & {$\epsilon=2$} \\
\midrule
AT & {$88.38 \pm 0.23$} & {$65.29 \pm 0.21$}  & {$33.71 \pm 0.16$}  & {$11.16 \pm 0.09$}  & {$2.4 \pm 0.17$}  & \\
TRADES & {$87.05 \pm 0.01$} & {$67.92 \pm 0.11 $}  & {$42.08 \pm 0.16$}  & {$19.33 \pm 0.38$} & {$6.62 \pm 0.16$}  & \\
MMA & {$\boldsymbol{88.40} \pm 0.14$} & {$65.62 \pm 0.23$}  & {$36.54 \pm 0.14$} & {$14.01 \pm 0.08$}  & {$3.49 \pm 0.10$}  & \\
\midrule
Ours & {$87.25 \pm 0.05$} & {$\boldsymbol{67.96} \pm 0.14$}   & {$\boldsymbol{43.48} \pm 0.23$}  & {$\boldsymbol{20.92} \pm 0.12$} & {$\boldsymbol{6.72} \pm 0.18$} &  \\
\bottomrule
\end{tabular}}
\caption{\small{Clean and robust accuracy on CIFAR-10 under $L_2$ attack} }

\centering
\noindent
\resizebox{\textwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=\frac{8}{255}$} & {$\epsilon=\frac{12}{255}$} & {$\epsilon=\frac{16}{255}$} & {$\epsilon=\frac{20}{255}$} \\
\midrule
AT & {$83.25 \pm 0.17$} & {$45.75 \pm 0.15$} & {$26.38 \pm 0.14$} & {$12.34 \pm 0.17$} & {$4.89 \pm 0.11$}& \\
TRADES & {$83.54 \pm 0.08$} & {$\boldsymbol{47.18} \pm 0.11$}  & {$29.03 \pm 0.19$}& {$15.07 \pm 0.11$}  & {$\boldsymbol{6.78} \pm 0.06$} & \\
MMA & {$84.25 \pm 0.28$} & {$41.48 \pm 0.31$} & {$23.63 \pm 0.25$} & {$11.97 \pm 0.20$} &{$5.11 \pm 0.12$} & \\
GAIRAT & {$81.31 \pm 0.23$} & {$32.98 \pm 0.11$}& {$16.19 \pm 0.02$} & {$6.89 \pm 0.18$}  & {$2.57 \pm 0.07$} & \\
\midrule
Ours & {$\boldsymbol{85.13} \pm 0.13$} & {$46.47 \pm 0.18$}  & {$\boldsymbol{29.38} \pm 0.24$} & {$\boldsymbol{15.14} \pm 0.16$} & {$6.45 \pm 0.21$} & \\
\bottomrule
\end{tabular}}
\caption{\small{Clean and robust accuracy on CIFAR-10 under $L_\infty$ attack} }
\label{table: performance_Linf_more_eps}
\end{table}

==> a0_Preliminary.tex <==
\section{Additional Preliminaries}\label{app:sec:prelim}
\subsection{Adversarial training}\label{app:subsec:at}
Traditional adversarial training (AT)~\citep{madry2017towards} adopts the following objective
% \begin{equation} \label{eq: AT}
%     \min_\theta \mathbb{E}_{(x,y)\sim D} \Big[\max_{\|x'-x\|\leq \epsilon} l(z_\theta(x'),y) \Big]  
% \end{equation}
\begin{align} 
% \setlength\abovedisplayskip{0pt}
% \setlength\belowdisplayskip{0pt}
     \min_\theta \frac{1}{N}\sum_{i=1}^{N}l(z_\theta(x'_i),y_i) %\label{eq: AT}
     \quad \text{ where }    x'_i = \argmax _{\|x'-x_i\|\leq \epsilon} l(z_\theta(x'),y_i) \label{eq: AT inner}
\end{align}
where $l$ is a suitable loss function (e.g. the cross-entropy loss). In other words, AT employs the worst-case adversarial data for updating the parameters. In practice, the projected gradient descent method (PGD) \citep{madry2017towards} is most commonly used for solving the inner maximization problem.

==> advML_workshop/Speed_unnormalized_time.tex <==
\begin{figure}[!t] % !htbp
    \centering
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/VR_AT_acc_noWithinCorrect}}
        \caption{\scriptsize{Test accuracy of AT}}
        \label{fig: AT_acc}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/AT_test_speed_time}}
        \caption{\scriptsize{Speed distribution of AT}}
        \label{fig: AT_speed_time}
    \end{subfigure}

    \centering
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/clean_acc}}
        \caption{\scriptsize{Test accuracy of NT}}
        \label{fig: clean_acc}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{\texhome/appendix_experiments/clean_test_speed_time}}
        \caption{\scriptsize{Speed distribution of NT}}
        \label{fig: clean_speed_time}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during AT and natural training (NT). In Figure~\ref{fig: AT_speed_time} and Figure~\ref{fig: clean_speed_time}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. }
    \label{fig: speed_time_all}
    \vspace{-2em}
\end{figure}

==> advML_workshop/a1_speed_derivation.tex <==
\section{Proof of the closed-form expression for the speed 
in Equation \eqref{eq: expression_for_speed}
} \label{app: closed_expression_speed}

In this section, our goal is to prove the closed-form expression~\eqref{eq: expression_for_speed} and provide further discussions. We first provide two preliminary lemmas and present the mathematical assumptions. Then we rigorously derive the closed-form expression. Finally, we discuss more about the expression and its assumptions. 

\begin{lemma} \label{lemma: norm_pq_app}
For $1\leq p \leq \infty$ and let $q$ satisfies $1/q+1/p=1$. Let $a$ be any fixed vector. Then 
\begin{equation*} 
    \left\|\nabla_x \left\|x-a\right\|_p\right\|_q = 1
\end{equation*}
\end{lemma}

\begin{proof}
Without loss of generality, assume $a$ is the zero vector. Write the $k$-th component of $x$ as $x_k$.

\emph{Case 1: $1\leq p < \infty$}

By calculation, $\frac{\partial \|x\|_p}{\partial x_k} = (\frac{|x_k|}{\|x\|_p})^{p-1}\cdot \sign (x_k)$. Since $q = \frac{p}{p-1}$, we have that 
\begin{equation*}
\begin{aligned}
\sum_k |\frac{\partial \|x\|_p}{\partial x_k}|^{q} &= \sum_k  |(\frac{|x_k|}{\|x\|_p})^{p-1}\cdot \sign (x_k)|^{\frac{p}{p-1}} \\
&= \sum_k \frac{|x_k|^p}{\|x\|_p^p} \\
&= 1
\end{aligned}
\end{equation*}

Therefore, $\left\|\nabla_x \left\|x\right\|_p\right\|_q = (\sum_k |\frac{\partial \|x\|_p}{\partial x_k}|^{q})^{1/q} = 1$.

\emph{Case 2: $p = \infty$}

In this case, $\nabla_x \|x\|_\infty$ is a one-hot vector (with the one being the position of the element of $x$ with the largest absolute value). Therefore, $\left\|\nabla_x \left\|x\right\|_{\infty}\right\|_1$ = 1. 

\end{proof}

The following lemma deals with the optimality condition for $p = \infty$. Special care needs to be taken since $L_\infty$ norm is not a differentiable function.

\begin{lemma} \label{lemma: Linf_optimality_app}
If $\hat{x}$ is a local optimum of the constrained optimization problem where $a$ is any fixed vector with $\phi(a) > 0$: 
\begin{equation*} \label{eq: closest_linf_app}
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
    \hat{x} = \argmin_{z} \|x-a\|_\infty \quad \textrm{s.t.}  \quad \phi(x) = 0.
\end{equation*}
Assume that $\phi$ is differentiable at point $\hat{x}$. Denote the coordinates set $\mathcal{J} = \{j: |\hat{x}_j - a_j| = \|\hat{x}-a\|_\infty\}$. Denote the $k$-th component of $\nabla_x \phi(\hat{x})$ as $\nabla_x \phi(\hat{x})_k$. Then (a) for $j \in \mathcal{J}$, $\nabla_x \phi(\hat{x})_j$ and $\hat{x}_j - a_j$ have opposite signs; (b) for $k\notin \mathcal{J}$, $\nabla_x \phi(\hat{x})_k = 0$. 
\end{lemma}

\begin{remark*}
If $\phi(a)<0$, then (a) for $j \in \mathcal{J}$, $\nabla_x \phi(\hat{x})_j$ and $\hat{x}_j - a_j$ have the same sign; (b) for $k\notin \mathcal{J}$, $\nabla_x \phi(\hat{x})_k = 0$.
\end{remark*}

\begin{proof}
\emph{(a)}
Consider the perturbation $\hat{x}(\epsilon) = \hat{x} + (0,\cdots,\epsilon_{j_1},\cdots,\epsilon_{j_m},\cdots,0)$ where $\mathcal{J} = \{j_1,\cdots,j_m\}$ and $\epsilon$ is a $m$ dimensional vector with $j$-th component $\epsilon_j$. Since $\phi(a)>0$ and $\hat{x}$ is a local optimum, $\|x-a\|_\infty < \|\hat{x}-a\|_\infty$ imply $\phi(x) > 0$ if $x$ is sufficiently close to $\hat{x}$. Therefore, if every $\epsilon_{j_i}$ is chosen so that $|\hat{x}_{j_i} + \epsilon_{j_i} - a_{j_i}| < |\hat{x}_{j_i} - a_{j_i}|$ (that is, $\epsilon_{j_i}$ has different sign from $\hat{x}_{j_i} - a_{j_i}$) and $\|\epsilon\|$ sufficiently small, then $\|\hat{x}(\epsilon) - a\| < \|\hat{x}-a\|$ and thus $\phi(\hat{x}(\epsilon))>0$. 

On the other hand, by Taylor expansion and the fact that $\phi(\hat{x})=0$, we have that 

\begin{equation*}
    \phi(\hat{x}(\epsilon)) = \sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j + \mathcal{O}(\|\epsilon\|^2)
\end{equation*}

Therefore, $\sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j > 0$ for any such $\epsilon$. By taking other $\epsilon_k \to 0$ if necessary, we obtain that $\forall j \in \mathcal{J}$, $\nabla \phi(\hat{x})_j \epsilon_j \geq 0$, where $\epsilon_j$ has different sign from $\hat{x}_{j} - a_{j}$. Therefore, $\nabla \phi(\hat{x})_j$ and $\hat{x}_{j} - a_{j}$ have different signs. 


\emph{(b)}
Take any $k \notin \mathcal{J}$ and consider the perturbation $\hat{x}(\epsilon) = \hat{x} + (0,\cdots,\epsilon_{j_1},\cdots,\epsilon_k,\cdots,\epsilon_{j_k},\cdots,0)$ where $\epsilon=(\epsilon_{j_1},\cdots,\epsilon_k,\cdots,\epsilon_{j_k})$. Choose any $\epsilon$ so that $\|\epsilon\|$ is sufficiently small, each $\epsilon_{j_i}$ has the opposite sign of $\hat{x}_{j_i} - a_{j_i}$ and $\epsilon_k$ small enough (which can be positive or negative), we have that $\phi(\hat{x}(\epsilon)) > 0$ since $\|\hat{x}(\epsilon) - a\|_\infty < \|\hat{x}-a\|_\infty$. By Taylor expansion, $\sum_{j\in\mathcal{J}} \nabla \phi(\hat{x})_j \epsilon_j + \epsilon_k \nabla_x \phi(\hat{x})_k > 0$ for any such $\epsilon$. By taking $\epsilon_j \to 0$ and using the fact that $\epsilon_k$ can be positive or negative, we conclude that $\nabla_x \phi(\hat{x})_k = 0$.

\end{proof}


Now we are ready to derive the closed-form expression of the speed. We first provide the full assumptions, then derive the expression, and finally we will discuss more about the assumptions. We will write $\hat{x}_i(t)$ as $\hat{x}_i$ when the indication is clear. 
\begin{assumption} \label{assumption: differentible}
Suppose that $(x_i,y_i)$ is correctly classified by $f_{\theta(t)}$ in some time interval $t \in I$ and $\hat{x}_i(t)$ is a locally closest boundary point in the sense that for any $t\in I$, it is the local optimum of the following:
\begin{equation*} 
    \hat{x}_i(t) = \argmin\nolimits_{\hat{x}} \|\hat{x}-x_i\|_p \quad \textrm{s.t.}  \quad \phi^{y_i}(\hat{x},\theta(t)) = 0.
\end{equation*}
Assume that in the time interval $I$: (a) $\hat{x}_i(t)$ is differentiable in $t$; (b) $\phi^{y_i}$ is differentiable at point $\hat{x}_i(t)$ and at the current parameter $\theta(t)$.
\end{assumption}


\begin{proposition*}[Closed-form expression of the speed $s(x_i,t)$] For $1 \leq p \leq \infty$ and under the Assumption~\ref{assumption: differentible}, define the (local) speed according to $\hat{x}_i(t)$ in Assumption~\ref{assumption: differentible} as $s(x_i,t) = \frac{d}{dt}\|\hat{x}_i(t) - x_i\|_p$, we have the following:

\begin{equation*} 
    s(x_i,t) = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)
\end{equation*}
where $q$ satisfies that $1/q+1/p=1$. In particular, $q=2$ when $p=2$ and $q=1$ when $p=\infty$.
\end{proposition*}

\begin{proof}
\emph{Case 1: $1\leq p < \infty$}

To compute $ s(x_i,t) = \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_2$, we need to characterize the curve of the closest boundary point $\hat{x}_i(t)$, where two key points stand out. First, $\hat{x}_i(t)$ is on the decision boundary $\Gamma_y (t)$ and thus  $\phi^y(\hat{x}_i(t),\theta(t)) = 0$ for all $t \in I$. By taking the time derivative on both sides, we obtain the level set equation \citep{osher2004level,aghasi2011parametric}

\begin{equation} \label{eq: LF_app}
	\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\cdot \hat{x}_i'(t) + \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) = 0
\end{equation}

Second, $\hat{x}_i(t)$ is the optimal solution of constrained optimization \eqref{eq: closest_pt}. Therefore, we have the following optimality condition:

\begin{equation} \label{eq: optimality_app}
    \nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t)) + \lambda(t)\nabla_x\|\hat{x}_i(t)-x_i\|_p = 0
\end{equation}

Since $x_i$ is correctly classified, $\phi^{y_i}(x_i) > 0$. Since $\hat{x}_i(t)$ is the closest point to $x_i$ whose $\phi^{y_i}$ value is zero, $\lambda(t) >0$. By taking the $L_q$ norm in Equation~\eqref{eq: optimality_app} and using Lemma~\ref{lemma: norm_pq_app}, we obtain that $\lambda(t) = \|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q$.

Now, we derive $s(x_i,t)$ as follows:

\begin{equation*}
\begin{aligned}
    s(x_i,t) &= \frac{d}{dt} \|\hat{x}_i(t)-x_i\|_p  \\
    & = \nabla_x\|\hat{x}_i(t)-x_i\|_p \cdot \hat{x}_i'(t) \\
    & = -\frac{1}{\lambda} \nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t)) \cdot \hat{x}_i'(t) && \text{(By the optimality condition~\eqref{eq: optimality_app})} \\
    & = \frac{1}{\lambda} \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) && \text{(By the level set equation~\eqref{eq: LF_app})}\\
    & = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x \phi^{y}(\hat{x}_i(t),\theta(t))\|_q}  
\end{aligned}
\end{equation*}

\emph{Case 2: $p = \infty$}

Note that since $L_\infty$ is not differentiable, the optimality condition in Equation~\eqref{eq: optimality_app} does not hold anymore. 

Denote the $j$-th component of $\hat{x}_i(t)$ and $x_i$ as $\hat{x}_{ij}(t)$ and $x_{ij}$. Let $\mathcal{J} = \{j: |\hat{x}_{ij}(t) - x_{ij}| = \|\hat{x}_i(t)-x_i\|_\infty\}$. By Lemma~\ref{lemma: Linf_optimality_app}, $s(x_i,t) = \frac{d}{dt}|\hat{x}_{ij}(t) - x_{ij}| = \hat{x}_{ij}^{'}(t) \sign (\hat{x}_{ij}(t)-x_{ij}) = - \hat{x}_{ij}^{'}(t) \sign (\nabla_x\phi^{y_i}(\hat{x}_{i})_j)$ for all $j \in \mathcal{J}$. Therefore, by Equation~\eqref{eq: LF_app} and Lemma~\ref{lemma: Linf_optimality_app}

\begin{equation*}
\begin{aligned}
- \nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t) &= \nabla_x \phi^{y_i}(\hat{x})\cdot \hat{x}_i'(t)\\
&= \sum_{j \in \mathcal{J}} \nabla_x \phi^{y_i}(\hat{x}_i)_j\cdot \hat{x}_{ij}'(t) \\
&= \sum_{j \in \mathcal{J}} - \nabla_x \phi^{y_i}(\hat{x}_i)_j \cdot \frac{s(x_i,t)}{\sign (\nabla_x\phi^{y}(\hat{x}_{i})_j)} \\
&= - \sum_{j \in \mathcal{J}} |\nabla_x\phi^{y_i}(\hat{x}_{i})_j| \cdot s(x_i,t)
\end{aligned}
\end{equation*}

Therefore, $s(x_i,t) = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\sum_{j \in \mathcal{J}} |\nabla_x\phi^{y_i}(\hat{x}_{i})_j|} = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x\phi^{y_i}(\hat{x}_{i})\|_1}$, where the last equality follows from Lemma~\ref{lemma: Linf_optimality_app} that the components of $\nabla_x \phi^{y_i}(\hat{x}_i)$ are zeros if they are not in $\mathcal{J}$.
 
\end{proof}

\subsection*{Discussions on the assumptions}
Assumption~\ref{assumption: differentible} has several points that need to be explained further.

First, we only require that $\hat{x}_i(t)$ is a local closest boundary point. This is important because in practice when an algorithm for searching the closest boundary point is used (e.g. FAB), a local solution is the best one can hope for due to the non-convex nature of the optimization problem. When $\hat{x}_i(t)$ is a local solution, the speed should be interpreted as how fast the distance changes around that local solution. In this case, although $\hat{x}_i$ is not the globally closest adversarial example, the local speed around $\hat{x}_i$ still has much information on the relative movement of the decision boundary w.r.t. $x_i$, especially when the distance  $\|\hat{x}_i - x_i\|$ is relatively small and the input space is a high-dimensional space (e.g. pixel space). 

Second, we require that $\hat{x}_i(t)$ is a differentiable curve in time interval $I$. Note that if we constrain $\hat{x}_i(t)$ to be the global closest boundary point, $\hat{x}_i$ is unlikely to be differential for a large time interval $I$, especially in high dimensional space. This is because as the decision boundary moves. the closest point might switch from one point to another point that is very far away abruptly. Fortunately, this problem is alleviated because our derived closed-form expression still works when $\hat{x}_i(t)$ is a locally closest boundary point. Note that however, due to the \textit{topological change} of the decision boundary, it still can happen that $\hat{x}_i(t)$ stops existing (and thus stops being differentiable) at some time point, when typically the speed will go to infinity. From a mathematical point of view, this is related to \textit{shock} in partial differential equation (PDE) theories. More exploration on this is left to future work. In this work, we only consider the speed of the decision boundary at each discrete time step.


==> advML_workshop/a2_method_details.tex <==
\section{Algorithms}

\subsection{Details of the optimization problem \eqref{eq:opt_for_weight}} \label{app: opt_for_weight}

In this section, we provide details of the optimization problem~\eqref{eq:opt_for_weight} by specifying the coefficients of this quadratic programming concretely using the neural network gradients $\nabla_x \phi^{y_i}(\hat{x}_i)$ and  $\nabla_\theta \phi^{y_i}(\hat{x}_i)$.

\subsubsection{The dependency between the weights and the speed}

First, we give the details of $\mathbf{s}(\mathbf{c})$, i.e. how the weights $\mathbf{c} = (c_1,\cdots, c_m)^{T}$ (linearly) determines the speed $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$. Recall that the dimension of the parameters $\theta$ is $p$, and the number of points in $\mathcal{B}_\theta^{+}$ is $m$. 

% theta'
\paragraph{The update rule $\theta'$} The weights $\mathbf{c}$ determines the update rule $\theta_k'$ as follows. We write $\theta'_k$ as $\theta' = \sum_{i\in \mathcal{B}_\theta^{+}}c_i\nabla_\theta \phi^{y_i}(\hat{x}_i) + z$, where the step index $k$ is omitted and $z$ includes terms that do not depend on the weights $\mathbf{c}$. In this paper, we use SGD with momentum and weight decay (which is commonly used in AT methods) and thus the relationship between $\theta'$ and the loss function is given by Equation~\eqref{eq: theta prime momentum weight decay general}. In this case, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$, where $\lambda_c$, $\lambda_w$ and $\lambda_m$ are coefficients for the clean loss, weight decay and momentum. 


% V(c)
\paragraph{The speed $\mathbf{s}(\mathbf{c})$} The weights $\mathbf{c}$ determines the speed $\mathbf{s}(\mathbf{c})$ through $\theta'$ as follows. By Equation~\eqref{eq: expression_for_speed}, $s(x_i) = \alpha_i \nabla_\theta \phi^{y_i}(\hat{x}_i)\cdot\theta'$ where $\alpha_i = \frac{1}{\|\nabla_x\phi^{y_i}(\hat{x}_i)\|_q}$. To expand it, we have 

\begin{equation*}
    s(x_i) =  \alpha_i \nabla_\theta \phi^{y_i}(\hat{x}_i)\cdot (\sum_{i\in \mathcal{B}_\theta^{+}}c_i\nabla_\theta \phi^{y_i}(\hat{x}_i) + z)
\end{equation*}
Now we express $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$ with $\mathbf{c}$ using the above equation in matrix form. Denote $A\in \mathbb{R}^{p\times m}$ as the matrix whose i-th column is $\nabla_\theta\phi^{y_i}(\hat{x}_i,y_i)$, $i = 1,\cdots,m$.  Also denote $\alpha \in \mathbb{R}^{m\times m}$ a diagonal matrix whose i-th diagonal element is $\alpha_i$. Then we have the following 

\begin{equation} \label{eq: s_c_app}
    \mathbf{s}(\mathbf{c}) =  \alpha A^{T} A \mathbf{c} + \alpha A^{T} z
\end{equation}

\subsubsection{The coefficients of problem \eqref{eq:opt_for_weight}}

We give the coefficients of the quadratic programming problem~\eqref{eq:opt_for_weight} in matrix forms. 

We write all the optimization variables in a single vectors $\mathbf{w} = (c_1,\cdots,c_m,\mu)$.
By Equation~\eqref{eq: s_c_app}, we have that $\mathbf{s}(\mathbf{c}) - \mu \mathbf{g} = \alpha A^{T} A \mathbf{c} + \alpha A^{T} z - \mu \mathbf{g} = M\mathbf{w} + \alpha A^{T} z$, where $M \in \mathbb{R}^{m\times (m+1)}$ whose first $m$ columns are equal to the matrix $\alpha A^{T} A$ and the last column is equal to $-\mathbf{g}$. Therefore, the optimization problem~\eqref{eq:opt_for_weight} is rewritten as the follows:   

\begin{equation} \label{eq: opt_for_weight_withMu_detail_app}
\begin{aligned}
\min_{\mathbf{w}} \quad & \mathbf{w}^{T}M^{T}M\mathbf{w} + 2\mathbf{w}^{T}(M^{T}\alpha A^{T}z)  \\
\textrm{s.t.} & \quad 
\begin{bmatrix}
    1 &\cdots & 1 & 0
\end{bmatrix}\mathbf{w} = 1, \mathbf{w} \geq 0   \\
\end{aligned}    
\end{equation}

In summary, the details of the optimization problem~\eqref{eq:opt_for_weight} to obtain the weights $\mathbf{c} = (c_1,\cdots,c_m)$ are given by optimization problem~\ref{eq: opt_for_weight_withMu_detail_app}, where $\mathbf{w} = (c_1,\cdots,c_m,\mu)$, 
$M = \begin{bmatrix}
  \alpha A^{T}A 
  & \rvline & -\mathbf{g}
\end{bmatrix}$, 
$A = \begin{bmatrix}
  \nabla_\theta \phi^{y_1}(\hat{x}_1) & \cdots & \nabla_\theta \phi^{y_m}(\hat{x}_m) 
\end{bmatrix}$,
$
\alpha = \text{diag}(\alpha_1,\cdots,\alpha_m)
$,
$\alpha_i = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i)\|_q}$, and $z$ is the terms in $\theta'$ that do not depend on $\mathbf{c}$ (for example, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$ when SGD with momentum and weight decays is used). The problem~\eqref{eq: opt_for_weight_withMu_detail_app} is a quadratic programming problem with $m+1$ variables, which can be solved efficiently. 


\subsubsection{An alternative to problem \eqref{eq:opt_for_weight}}
Here we present an alternative optimization problem to problem~\eqref{eq:opt_for_weight}, which is slightly more efficient since it corresponds to a quadratic problem of size $m$, instead of $m+1$ as in problem~\eqref{eq:opt_for_weight}. The alternative is given as follows:

\begin{equation} \label{eq:opt_for_weight_withoutMu_app}
\begin{aligned}
\min_{\mathbf{c}}\min_{\mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} c_i = 1, \quad c_i\geq0   \\
\end{aligned}
\end{equation}

The difference of problem~\eqref{eq:opt_for_weight_withoutMu_app} and the problem  problem~\eqref{eq:opt_for_weight} is that the former omit the constraint on $\mu$ to be positive. However, their optimal $\mathbf{c}$ are the same if the optimal $\mu$ is positive for the alternative optimization problem~\eqref{eq:opt_for_weight_withoutMu_app}. We find that in our experiments, the solved $\mu$ is always positive for the alternative problem~\eqref{eq:opt_for_weight_withoutMu_app} and thus these two optimization problems are equivalent. Due to its slightly better efficiency, we use the alternative formulation~\eqref{eq:opt_for_weight_withoutMu_app} instead of the formulation~\eqref{eq:opt_for_weight}.   We now give the details of the alternative optimization problem.


% We use the following lemma:

% \begin{lemma} Let $x,\mathbf{g}$ be two vectors. Then we have 
% \begin{equation*}
%     \min_{\mu} \|x-\mu \mathbf{g}\|_2^2 = \|E_\mathbf{g} x\|_2^2 
% \end{equation*}
% where $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$.
% \end{lemma}

Note that the inner minimization problem can be solved in closed form: $\min_{\mu}\|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 = \|E_\mathbf{g} \mathbf{s}(\mathbf{c})\|_2^2$ where $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$. By Equation~\eqref{eq: s_c_app} that we have derived in the last section, $\mathbf{s}(\mathbf{c}) = \alpha A^{T} A \mathbf{c} + \alpha A^{T} z $. Therefore, $\min_{\mathbf{c}}\min_{\mu}  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 = \min_{\mathbf{c}}\|E_\mathbf{g} \mathbf{s}(\mathbf{c})\|_2^2 = \min_{\mathbf{c}}\|E_\mathbf{g} ( \alpha A^{T} A \mathbf{c} + \alpha A^{T} z)\|_2^2$, which corresponds to the following constrained quadratic programming problem:

\begin{equation} \label{eq: opt_for_weight_withoutMu_detail_app}
\begin{aligned}
\min_{\mathbf{c}} \quad & \mathbf{c}^{T}K_1^{T}K_1\mathbf{c} + 2\mathbf{c}^{T}(K_1^{T}K_2)  \\
\textrm{s.t.} & \quad \sum_{i}c_i = 1, \mathbf{c} \geq 0   \\
\end{aligned}    
\end{equation}

where $K_1 = E_\mathbf{g}\alpha A^{T}A, K_2 = E_\mathbf{g}\alpha A^{T}z$. 

In summary, the alternative scheme \eqref{eq:opt_for_weight_withoutMu_app} is given by the quadratic problem \eqref{eq: opt_for_weight_withoutMu_detail_app}, where $K_1 = E_\mathbf{g}\alpha A^{T}A, K_2 = E_\mathbf{g}\alpha A^{T}z$, $E_{\mathbf{g}} = I - \frac{\mathbf{g}\mathbf{g}^{T}}{\mathbf{g}^{T}\mathbf{g}}$, $A = \begin{bmatrix}
  \nabla_\theta \phi^{y_1}(\hat{x}_1) & \cdots & \nabla_\theta \phi^{y_m}(\hat{x}_m) 
\end{bmatrix}$,
$
\alpha = \text{diag}(\alpha_1,\cdots,\alpha_m)
$,
$\alpha_i = \frac{1}{\|\nabla_x \phi^{y_i}(\hat{x}_i)\|_q}$, and $z$ is the terms in $\theta'$ that do not depend on $\mathbf{c}$ (for example, $z = -\lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}\nabla_\theta l(x_i,y_i)  - \lambda_w \theta_k - \lambda_m b_k$ when SGD with momentum and weight decays is used). The problem~\eqref{eq: opt_for_weight_withoutMu_detail_app} is a quadratic programming problem in $m$ variables, which can be solved efficiently. 



\subsection{Workflow of \algoName} \label{app: algo_pseudo}
We present the pseudocode of our proposed \algoName in Algorithm~\ref{alg: main algo}.
\input{\texhome/algo} 


\section{Optimality condition in practice} \label{app: optimality}
Either computing the speed of the decision boundary or reverse engineering an update rule to achieve some desirable dynamics (like what \algoName does) requires the computation of the closest boundary point $\hat{x}$ for the correctly classified data point $(x,y)$, where we omit the subscript $i$ in this section. As discussed in Appendix~\ref{app: closed_expression_speed}, it suffices to find the local closest boundary point in order for the closed-form expression~\eqref{eq: expression_for_speed} for the speed to be valid. 

In this section, we will explain how to check the quality of the found $\hat{x}$ for the constrained optimization problem~\ref{eq: closest_pt} in practice. We will also give a simple analysis on how FAB\citep{croce2020minimally}, the algorithm we use in our implementation, solves the problem~\ref{eq: closest_pt} in practice. In this paper, we focus on $p = 2$ and $p = \infty$. 

The key points of analyzing $\hat{x}$ are that $\phi^{y}(\hat{x}) = 0$ and the KKT condition of problem~\ref{eq: closest_pt}.

\emph{Case 1: $p=2$}

In this case, the KKT condition is given by $\nabla_x \phi^{y}(\hat{x}) + \lambda (\hat{x} - x) = 0$ for some $\lambda > 0$ (since $\phi^{y}(x) >0$). In other words, $\frac{\nabla_x \phi^{y}(\hat{x})}{\|\nabla_x \phi^{y}(\hat{x})\|} \cdot \frac{x-\hat{x}}{\|x-\hat{x}\|} = 1$. In practice, we check the following two conditions (a) $|\phi(\hat{x})| \leq 0.1$; (b) $\frac{\nabla_x \phi^{y}(\hat{x})}{\|\nabla_x \phi^{y}(\hat{x})\|} \cdot \frac{x-\hat{x}}{\|x-\hat{x}\|} > 0.8$. In our experiments, we find that FAB with iterations greater than 10 can reliably find $\hat{x}$ satisfying these two conditions. In all of our experiments when $p=2$, including computing the speed for various methods (e.g. AT) and the implementation of \algoName, we only use those high-quality closest boundary points that satisfy these two conditions and discard the rest. We observe in our experiments that FAB can find high-quality closest boundary points for over 90\% of the correctly classified data points. 

\emph{Case 2: $p=\infty$}

In this case, we consider the optimality condition given in Lemma~\ref{lemma: Linf_optimality_app} of Appendix~\ref{app: closed_expression_speed}. Denote $\#B$ the number of points in the set $B$. Using the notation $\mathcal{J} = \{j: |\hat{x}_j - x_j| = \|\hat{x}-x\|_\infty\}$ and $\mathcal{J}^{C}$ the complement set of $\mathcal{J}$, we check the following conditions in practice: (a) $|\phi(\hat{x})| \leq 0.1$; (b) $\frac{\#\{j\in\mathcal{J}: \nabla_x \phi^{y}(\hat{x})_j (\hat{x}_j - x_j) \leq 0\}}{\#\mathcal{J}} > 0.9$; (c) $\frac{\#\{k\notin J: |\nabla_x \phi^{y}(\hat{x})_k| < 0.1 \}}{\#\mathcal{J}^C} > 0.8$. Note the unlike $p=2$, the optimality conditions for $p=\infty$ are on each coordinate of $\hat{x}$, which is more difficult to satisfy. We observe in our experiments that FAB with 60 iterations can find high-quality closest boundary points for about 85\% of the correctly classified points. However, when only 15 iterations are used, condition (3) is barely satisfied for all of the found boundary points (the first two conditions are still satisfied). In our visualizations of dynamics of the decision boundary for various methods in $L_\infty$ setting in Appendix~\ref{app: more_dynamics}, we use 60 iterations for FAB and only use high-quality closest boundary points, so that the visualization results are accurate. In our implementation of \algoName, we omit the condition (3) and only use 15 iterations for FAB for efficiency. 

Designing faster and more reliable methods to solve the constrained optimization problem~\ref{eq: closest_pt}, especially when $p = \infty$, is left for future work. 

==> advML_workshop/a3_experiment.tex <==



\section{Experiments}
In this section, we provide experimental details and further results of \algoName along with other state-of-the-art defense methods. 
\subsection{Detailed experimental settings} \label{app: exp_settings}

\paragraph{Basic training setting} 
In all experiments on CIFAR-10 in Section~\ref{sec:exp_robust}, we use the Wide Residual Networks  \citep{zagoruyko2016wide} with depth 28 and width factor 4 (WRN-28-4), which is also used in previous works \citep{Ding2020MMA}. We replace the batch normalization (BN) layers with group normalization (GN) \citep{wu2018group} layers so that the decision boundary is the same at training and test time. This is necessary for \algoName since it uses the closest boundary points during training, which should be also on the decision boundary in the evaluation mode. For other baselines, we find that replacing BN with GN has negligible effect on the robustness performance. We use stochastic gradient descent with momentum 0.9 and weight decay 0.0005, which is suggested in \citep{pang2020bag}. We train 100 epochs in total with batch size 128. The learning rate begins at 0.1 and is decayed by a factor of 10 at the 50th and 75th epoch. The first 10 epochs of \algoName is the burn-in period, where only the clean loss is used. To alleviate robust overfitting \citep{rice2020overfitting}, early stopping is performed on a validation set of size 2000 in all experiments, where the model with the highest robust accuracy under projected gradient descent (PGD) attacks \citep{madry2017towards} with 20 steps (PGD-20) is chosen. All experiments are run on two NVIDIA GeForce RTX 2080 Ti GPU. 

\paragraph{Per-sample gradient} During implementation of the expression for speed in Equation~\eqref{eq: expression_for_speed} and also \algoName, we need to compute the per-sample gradient $\nabla_\theta \phi^{y_i}(\hat{x}_i,\theta)$ for every correctly classified point $x_i$. We use the Opacus package \citep{opacus} for computing per-sample gradients in parallel. Also, another reason why we replace BN with GN is because Opacus does not support BN for computing per-sample gradients.   


\paragraph{Evaluation protocol}
We evaluate our proposed method and baselines under $L_2/L_\infty$-norm constrained perturbation. The final robust accuracy is reported on the full test set against PGD-40 attack as well as AutoAttack (AA) \citep{croce2020reliable}, which uses an ensemble of selected strong attacks. Note that although AA is considered stronger and serves as a more reliable measure of robustness, we still include PGD attack results since it can happen that some methods performs well against PGD attack, but not against AA. In all experiments we find that AA gives lower robust accuracy than PGD attack. Therefore, we refer to the robust accuracy against AA, instead of PGD, when comparing performance among different defense methods. For all methods, we choose the hyperparameters to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. In addition, we evaluate on larger perturbation thresholds to better examine the robustness of the model against larger unknown perturbation thresholds. 

\textbf{Compared baselines and their hyperparameters}\quad
The baseline defense methods include: (1) standard adversarial training (AT) \citep{madry2017towards} which trains on the worst case adversarial examples generated by 10-step PGD (PGD-10) on the cross-entropy loss. The perturbation threshold is $0.5$ in $L_2$ setting, and $\frac{8}{255}$ in $L_\infty$ setting. The step size of PGD is $\frac{15}{255}$  in $L_2$ setting and $\frac{2}{255}$ in $L_\infty$ setting; the training setting follows Rice et al.\footnote{\href{https://github.com/locuslab/robust_overfitting}{Robust Overfitting's Github}}  \citep{rice2020overfitting}. (2) TRADES \footnote{\href{https://github.com/yaodongyu/TRADES}{TRADES's Github}}\citep{zhang2019theoretically} which trades off between the clean and robust accuracy. The perturbation threshold is $0.5$ in $L_2$ setting, and $\frac{8}{255}$ in $L_\infty$ setting. The step size of PGD-10 is $\frac{15}{255}$  in $L_2$ setting and $0.007$ in $L_\infty$ setting ; The regularization constant beta (or 1/lambda) is set to  6. (3) MMA  \footnote{\href{https://github.com/BorealisAI/mma_training}{MMA's Github}}  \citep{Ding2020MMA} which trains on the closest adversarial examples (closest boundary points) with uniform weights. 
% Since MMA is the most related to \algoName, we report four hyperparamter settings. MMA-1 in $L_2$ setting uses MaxEps = $1$; MMA-2 in $L_2$ setting uses MaxEps = $2$; MMA-3 in $L_\infty$ setting uses MaxEps = $\frac{20}{255}$; MMA-4 in $L_\infty$ setting uses MaxEps = $\frac{32}{255}$; 
The MaxEps is set to $1$ in $L_2$ setting and $\frac{32}{255}$ in $L_\infty$ setting. 
(4) GAIRAT \footnote{\href{https://github.com/zjfheart/Geometry-aware-Instance-reweighted-Adversarial-Training}{GAIRAT's Github}} \citep{zhang2021geometryaware}  which reweights adversarial examples using the least perturbation steps. We only evaluate GAIRAT under $L_\infty$ setting since it does not have $L_2$ implementation in the codebase. The perturbation length is $\frac{8}{255}$ with step size $0.007$ using PGD-10 and the 'tanh' weight assignment function is used. 


\subsubsection*{Hyperparameters of \algoName} 

We use the ratio function with $g(0) = 1, g(r_0) = 0, g(r_1) = - g_1$ with $g_1 \geq 0 $ and linearly interpolate them when $0\leq r \leq r_1$. When $r>r_1$, $g(r)$ was set to the constant $-g_1$. If $g_1 > 0$, it means that \algoName pulls back the decision boundary towards $x_i$ if its robust radius $R(x_i)$ is larger than $r_1$. We allow $g$ to be negative when $r > r_1$ since we experimentally find that this could help improve both the clean accuracy and robust accuracy under small perturbation lengths in some settings. This is because it helps reduce the variance of the robust radius distribution by eliminating robust radii that are unnecessarily large. When $g(R(x_i)) < 0 $, the weight $c_i$ is constrained to be non-positive since the decision boundary at $\hat{x}_i$ needs to be pulled back. In particular, we solve the following modified version of the optimization problem~\eqref{eq:opt_for_weight}:

\begin{equation} \label{eq:opt_for_weight_negative}
\begin{aligned}
\min_{\mathbf{c}, \mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} |c_i| = 1, \quad c_i g(R(x_i))\geq0, \quad \mu \geq 0    \\
\end{aligned}
\end{equation}

The optimization problem~\eqref{eq:opt_for_weight_negative} above is still a quadratic programming problem with the same objective function as the original problem~\eqref{eq:opt_for_weight}, whose details are given in Appendix~\ref{app: opt_for_weight}. The only difference is in the constraints, where  problem~\eqref{eq:opt_for_weight_negative} requires the weight to be non-positive if its $g$ value is negative, and the absolute values of the weights sum up to one. 

To achieve the best robust accuracy under $\epsilon = 0.5$ in the $L_2$ setting, we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = 0.4$. To achieve the best robust accuracy under $\epsilon = \frac{8}{255}$ in the $L_\infty$ setting, we set $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = 0.4$. We use FAB with 15 iterations to approximate the closest boundary points in both $L_2$ and $L_\infty$ setting. 


\subsection{Further experimental results}\label{app: further_exp_results}

\paragraph{Comparing with baselines} We first present results where the hyperparameters of $\algoName$ are chosen to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. That is , we set $\lambda_c = 2, r_0 = 2, r_1 = 3, g_1 = 0.4$ in $L_2$ setting and  $\lambda_c = 1, r_0 = \frac{32}{255}, r_1=\frac{48}{255}, g_1 = 0.4$ in  $L_\infty$ setting. The results are given in Table~\ref{table: performance_L2_more_eps_app} and Table~\ref{table: performance_Linf_more_eps_app}. In the $L_2$ case, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. In the $L_\infty$ case, \algoName obtains both higher clean accuracy and robust accuracy than AT, MMA and GAIRAT. We observe that the robust accuracy under AA is much lower than PGD for GAIRAT and MMA, which may be due to obfuscated gradient \citep{AthalyeC018}. On the other hand, the performance gap between PGD and AA is relatively small for \algoName. When compared with TRADES, \algoName shows higher clean accuracy and comparable robust accuracy under larger $\epsilon$, although \algoName has lower robust accuracy when $\epsilon = \frac{8}{255}$. This is partially due to the higher difficulty of approximating the closest boundary points in the $L_\infty$ case, and a better algorithm for this is left for future work. 


\input{\texhome/appendix_experiments/tab_L2_moreEps}
\input{\texhome/appendix_experiments/tab_Linf_moreEps}

\paragraph{Effect of ratio function and clean loss coefficient} We study the effect of hyperparameters $r_0, r_1, g_1$ of the ratio function $g$, as well as the clean loss coefficient $\lambda_c$ in the loss function~\eqref{eq: weighted loss general}. We only show the robust accuracy results against AA since it gives a more accurate estimation of the robustness. The results are shown in Table~\ref{table: performance_L2_ours_ablation} and Table~\ref{table: performance_Linf_ours_ablation}, where several observations can be made. Firstly, we observe that when the ratio function $g$ is fixed, a smaller $\lambda_c$ tends to result in better robustness performance against all perturbation thresholds, though the clean accuracy is lower. This indicates a trade-off between the robust and clean accuracy. Secondly, when $\lambda_c$ is fixed, a flatter ratio function $g$ (with larger $r_0$) will result in higher robust accuracy under larger perturbation lengths,  but could hurt the robust accuracy under smaller perturbation lengths. Thirdly, using a positive $g_1$ when $r_0$ is relatively large (such as $2$ in $L_2$ case and $\frac{32}{255}$ in $L_\infty$ case) could improve the robust accuracy under smaller perturbation lengths (such as $0.5$ in $L_2$ case and $\frac{8}{255}$ in $L_\infty$ case) but decrease the robust accuracy under larger perturbation lengths. In this case, \algoName controls the decision boundary so that if it is very far from the natural data, it will move closer. This helps reduce the variance of the robust radius distribution, decrease the proportion of unnecessarily robust points and thus improve the robust accuracy under small perturbation thresholds. 

\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-1em}
    \centering
    \begin{subfigure}[b]{0.26\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\texhome/experiment_fig/ratio_function}}
        \vspace{-1.5em}
        \caption{Ratio function}
        \label{sfig: performance_ratio_function}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{\texhome/experiment_fig/radius_distribution}}
        \vspace{-1.5em}
        \caption{radius distribution}
        \label{sfig: performance_radius_distribution}
    \end{subfigure}
    \vspace{-0.3em}
    \caption{Different choices of the ratio function $g$ and the corresponding radius distributions when using \algoName.
    }
\vspace{-1.2em}
\end{wrapfigure}

\textbf{Ratio function controls the robust radius distribution}\quad 
Here we provide further analysis on the effect of the ratio function $g$. \algoName uses the ratio function $g$ to control the robustness level. As discussed in Section~\ref{ssec: dynamics_design}, the trained model is expected to be robust to larger perturbation thresholds if $g$ decays slower. To verify this, we fix $\lambda_c = 2$ in the $L_2$ norm setting and train on $g(r) = 1 - r/k$ when $r\leq k$ and $g(r)=0$ otherwise, for different $k$'s as shown in Figure~\ref{sfig: performance_ratio_function}. For these trained models, we use FAB (with 40 iterations) to compute the robust radius distributions for the correctly classified points from the test set,
% We discard the low-quality boundary points that do not satisfy the optimality condition of equation $\eqref{eq: closest_pt}$. 
which are shown in Figure~\ref{sfig: performance_radius_distribution}.
We can see that when $g$ decays slower, the robust radius distribution within correctly classified points spreads out more and tends to be more robust. Note that the overall robust accuracy is the product of the robust accuracy within correct points and the clean accuracy. We find that although a flatter $g$ leads to better robust accuracy within correct points, it decreases the clean accuracy. This shows that improving the robustness of points with large robust radii could harm the clean accuracy. Therefore, there is a trade-off between the robustness and clean accuracy, which is balanced by $\lambda_c$ and the choice of $g$.





\input{\texhome/appendix_experiments/tab_L2_ours_ablation}
\input{\texhome/appendix_experiments/tab_Linf_ours_ablation}


==> advML_workshop/a4_more_dynamics.tex <==
\newpage
\section{Further results of dynamics} \label{app: more_dynamics}
In this section, we present more visualizations and further analysis of the dynamics of the decision boundary during the training process. 

\subsection{Dynamics and robustness improvement}
In this section, we demonstrate a strong correlation between the speed of the decision boundary and the improvement of robust accuracy over time. 

\textbf{Experiment setting}\quad We train a ResNet-18 \citep{he2016deep} on CIFAR-10 using 10-step PGD under $L_2$ perturbation with $\epsilon=0.5$ from a naturally pretrained model and evaluate it using 20-step PGD.
Figure~\ref{fig: interpretation_acc} shows the test clean and robust accuracy, as well as the \textit{robust accuracy within correct points}: the proportion of robust data points within correctly classified ones, which is computed by the ratio between the robust accuracy and clean accuracy.
We consider the robust accuracy within correct points since the speed is only defined for correctly classified ones.
We will experimentally examine the correlation between the robust accuracy within correct points and the dynamic speed of the decision boundary.

\input{\texhome/fig_interpret_test}

\textbf{Dynamics and robustness improvement}\quad We choose 512 points from the test set and at each iteration, we compute the robust radii and speed for correctly classified points. We omit those points whose radii are larger than $1$, which are considered very robust under $\epsilon=0.5$. 
For every iteration, we normalize the speed values to have the maximum absolute value 1 for better visualization of their relative magnitude.
The result is shown in Figure~\ref{fig: interpretation_VR_test_scatter}.
The set of points 
$\mathcal{S}_{\mathsf{g}} = \{x_i: R(x_i)<0.5, s(x_i)>0\}$
(top left corner) can be viewed as vulnerable but are being improved, whereas points in
$\mathcal{S}_{\mathsf{b}} = \{x_i: 0.5<R(x_i)<1, s(x_i)<0\}$
(bottom right corner) can be considered as robust but are being compromised. Observe that at the start of training (e.g. iteration 5 and 30), the proportion  of $\mathcal{S}_{\mathsf{g}}$, denoted as $p(\mathcal{S}_{\mathsf{g}})$, is relatively large and $p(\mathcal{S}_{\mathsf{b}})$ is relatively small. At the same time, the robust accuracy within correct points increases drastically, as shown in figure \ref{fig: interpretation_acc}. At the later stage (e.g. iteration 200), $p(\mathcal{S}_{\mathsf{g}})$ decreases and $p(\mathcal{S}_{\mathsf{b}})$ increases, and the robustness improvement slows down. In order to capture the robustness improvement using dynamics, we compute $p(\mathcal{S}_{\mathsf{g}}) - p(\mathcal{S}_{\mathsf{b}})$ which is shown in Figure~\ref{fig: interpretation_acc_d}, along with the time derivative of the robust accuracy within correct points. We observe that both of them show the same pattern, indicating the strong correlation between the dynamics of the decision boundary and the robustness improvement during AT.

\subsection{Further analysis of dynamics}
In this section, we present the un-normalized speed (raw speed values) in Figure~\ref{fig: AT_speed_time_app_all}, where the 20\% quantile, median and 80\% quantile of the speed distribution at each iteration are shown. We observe that at the start of the training (first 100 iterations) where the robust accuracy improves drastically, the speed distribution is mostly positive. Later,  when the robustness improvement slows down, the speed distribution is centered around zero. Also, notice that the variance of the speed distribution is never vanishing: the decision boundary always moves towards some data points while moving away from others. This indicates that adversarial training methods do not converge, since the decision boundary does not stop moving. Despite the constant movement of the decision boundary, the average adversarial loss does converge. Therefore, the dynamics of the decision boundary w.r.t. each data point provides more information than an average of the surrogate loss. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/VR_AT_acc}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: AT_acc_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/AT_test_speed_time}}
        \caption{\scriptsize{Speed distribution and iterations}}
        \label{fig: AT_speed_time_app}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during AT. In Figure~\ref{fig: AT_speed_time_app}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. }
    \label{fig: AT_speed_time_app_all}
    %\vspace{-1em}
\end{figure}


\paragraph{Natural training}
To compare with the non-converging behaviour of adversarial training methods, we present the dynamics during natural training in Figure~\ref{fig: clean_speed_time_app_all}, where the robust accuracy stays at zero. This can be viewed as the final stage of the natural training since the clean accuracy does not increase significantly anymore. We observe that the speed distribution of the decision boundary is effectively zero. This indicates that natural training does converge in the following sense: the clean accuracy does not change and moreover, the decision boundary around every correctly classified point does not move anymore. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/clean_acc}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: clean_acc_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/clean_test_speed_time}}
        \caption{\scriptsize{Speed distribution and iterations}}
        \label{fig: clean_speed_time_app}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Speed distribution on the test set during natural training. In Figure~\ref{fig: clean_speed_time_app}, the speed distribution at each iteration is shown. At every iteration, the median (solid line), 20\% quantile (lower light line) and 80\% quantile (upper light line) are shown to represent the speed distribution at that iteration. Observe that the speed is almost zero during natural training, indicating that natural training eventually does not move the decision boundary around correctly classified points.}
    \label{fig: clean_speed_time_app_all}
    %\vspace{-1em}
\end{figure}

\subsection{Dynamics in the \texorpdfstring{$L_\infty$}{} setting }

Here we present the visualization of the speed in the $L_\infty$ setting. We use FAB with 60 iterations and only choose the closest boundary points with high quality according to Appendix~\ref{app: optimality}. We use AT with $\epsilon = \frac{8}{255}$ and \algoName with $r_0=\frac{32}{255}, g_1 = 0, \lambda_c = 1$. The speed-radius distribution on the training batches of three chosen iterations for both methods are shown in Figure~\ref{fig: AT_linf_VR_trainBatch_app} and Figure~\ref{fig: ours_linf_VR_trainBatch_app}. We can draw a similar conclusion as in the $L_2$ case: conflicting dynamics of the decision boundary exists for AT during training, since there is a significant proportion of vulnerable points (with $R(x_i) \leq \frac{8}{255}$) with negative speed values. On the other hand, \algoName can alleviate this conflict and encourage robustness improvement on more vulnerable points by assigning larger speed values to them. 

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/AT_batch_Linf_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
        \label{fig: AT_linf_VR_trainBatch_scatter_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/AT_batch_Linf_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: AT_linf_VR_trainBatch_hist_app}
    \end{subfigure}%
    \caption{Radius-speed plot of AT on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations in $L_\infty$ setting. Proportion of points with negative speed for these iterations are 31\%, 45\% and 46\% respectively.}
    \label{fig: AT_linf_VR_trainBatch_app}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/ours_batch_Linf_scatter}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Radius-speed plot of \algoName on the training batch}}
        \label{fig: ours_linf_VR_trainBatch_scatter_app}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.52\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{\texhome/appendix_experiments/ours_batch_Linf_hist}}
        %\vspace{-0.5em}
        \caption{\scriptsize{Histogram of speed}}
        \label{fig: ours_linf_VR_trainBatch_hist_app}
    \end{subfigure}%
    \caption{Radius-speed plot of \algoName on the training batches and their corresponding vertical histograms of speed distribution for three randomly chosen iterations in $L_\infty$ setting. Proportion of points with negative speed for these iterations are below 3\%.}
    \label{fig: ours_linf_VR_trainBatch_app}
\end{figure}

==> advML_workshop/a5_related_work.tex <==
\section{More related Work}\label{sec:related_work_app}

\textbf{Controlling parameterized surface}\quad 
The decision boundary can be viewed as a parameterized surface in the input space. Controlling such surface has been studied in image segmentation\citep{li2011level,aghasi2011parametric} and shape modelling\citep{chen2019learning,park2019deepsdf}. As for adversarial training, the authors of \citep{Atzmon2019control} propose to maximize the distance between each data point and some point on the decision boundary, which is not the closest one. On the other hand, we study the movement of the decision boundary w.r.t. each data point by analyzing its closest boundary point, which is directly related to the 
robust radius. 

\textbf{Comparisons with related adversarial training methods}\quad 
There are several defense techniques including gradient regularization \citep{moosavi2019robustness,tramer2017ensemble}, certified denfense\citep{cohen2019certified,wong2018provable,balunovic2019adversarial} and adversarial training \citep{madry2017towards,zhang2019theoretically,gowal2020uncovering,wang2019improving,zhang2020attacks}, where the last one is the most related to this work. 
In particular, MMA\citep{Ding2020MMA} trains on the closest boundary points, which is similar to \algoName. However, MMA adopts uniform weights and thus does not consider the vulnerability difference among the points. On the other hand, weighted adversarial training methods \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware} assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. 

==> advML_workshop/algo.tex <==
%%% wrapping algorithm inside a figure environment, so that we can adjust the spacing around it using \vspace{}

\begin{figure}[!htbp]
\vspace{-1em}
\centering
\begin{algorithm}[H] 
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{\algoNameFull (\algoName)}
\label{alg: main algo}
\begin{algorithmic}[1]
% \hspace*{\algorithmicindent} \textbf{Input:} 
\REQUIRE The training data set, ratio function $g$, norm type $p$, clean loss strength $\lambda_c$, number of epochs $T$ and number of batches $M$. $\mathcal{A}(x,y)$ denotes the approximate closest boundary point returned by an algorithm $\mathcal{A}$ (e.g. FAB) on the correctly classified data point $(x,y)$.  
% \hspace*{\algorithmicindent} \textbf{Output:} 
\ENSURE adversarially robust network $f_\theta$
\FOR{epoch = $1,\cdots,T$}
    \FOR{mini-batch = $1,\cdots,M$}
        \STATE Sample a mini-batch $\mathcal{B} = \{(x_i,y_i\}_{i=1}^{n}$
        \STATE Make predictions on $\mathcal{B}$ and find correctly classified points $\mathcal{B}_{\theta}^{+}$
        \FOR{$(x_i,y_i)\in \mathcal{B}_{\theta}^{+}$ (in parallel)}
            \STATE Find the approximate closest boundary point $\hat{x}_i = \mathcal{A}(x_i,y_i)$ as in \eqref{eq: closest_pt}
            \STATE Compute the robust radius $R(x_i) = \|\hat{x}_i - x_i\|_p$
            \STATE Calculate the ratio value $g(R(x_i))$
        \ENDFOR
        \STATE Solve the optimization problem \eqref{eq:opt_for_weight} for weights $c_i$ for $i \in \mathcal{B}_{\theta}^{+}$ 
        \STATE Update $\theta$ using the loss function \eqref{eq: weighted loss general}
        % $\theta \gets \theta - \eta(\sum_{i\in B_1^{\text{adv}}}c_i\nabla_\theta l(\hat{x}_i,y_i)  + \lambda_c\sum_{i\in B}\frac{1}{N}\nabla_\theta l(x_i,y_i))$
    \ENDFOR
\ENDFOR

% \Function{ComputeWeight}{$x,y$} \Comment{{\small{return the summation of two variables}}}
%   \STATE $z = x + y$
%   \STATE \textbf{Return} $z$ 
% \EndFunction
\end{algorithmic}
\end{algorithm}

\vspace{-1em}
\end{figure}


==> advML_workshop/experiment_fig/Our_batch_hist.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 100}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0930522158741951) rectangle (axis cs:0.130964314592326,0.0101324841380119);
\draw[draw=none,fill=color0] (axis cs:0,0.0101324841380119) rectangle (axis cs:0.523857258369306,0.113317184150219);
\draw[draw=none,fill=color0] (axis cs:0,0.1133171916008) rectangle (axis cs:0.654821525679423,0.216501891613007);
\draw[draw=none,fill=color0] (axis cs:0,0.216501891613007) rectangle (axis cs:0.785785887553959,0.319686591625214);
\draw[draw=none,fill=color0] (axis cs:0,0.319686591625214) rectangle (axis cs:1.83350040429257,0.422871291637421);
\draw[draw=none,fill=color0] (axis cs:0,0.422871291637421) rectangle (axis cs:1.44060746051559,0.526055991649628);
\draw[draw=none,fill=color0] (axis cs:0,0.526055991649628) rectangle (axis cs:0.654821572961632,0.629240691661835);
\draw[draw=none,fill=color0] (axis cs:0,0.629240691661835) rectangle (axis cs:1.17867883133094,0.732425391674042);
\draw[draw=none,fill=color0] (axis cs:0,0.732425391674042) rectangle (axis cs:1.30964314592326,0.835610091686249);
\draw[draw=none,fill=color0] (axis cs:0,0.835610091686249) rectangle (axis cs:1.17867883133094,0.938794791698456);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 500}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0894175097346306) rectangle (axis cs:0.325926569166786,0.0128550156950951);
\draw[draw=none,fill=color0] (axis cs:0,0.0128550156950951) rectangle (axis cs:0.325926569166786,0.115127541124821);
\draw[draw=none,fill=color0] (axis cs:0,0.11512752622366) rectangle (axis cs:1.19506408694488,0.217400044202805);
\draw[draw=none,fill=color0] (axis cs:0,0.217400074005127) rectangle (axis cs:1.52099065611167,0.319672584533691);
\draw[draw=none,fill=color0] (axis cs:0,0.319672584533691) rectangle (axis cs:2.49877072768424,0.421945095062256);
\draw[draw=none,fill=color0] (axis cs:0,0.421945095062256) rectangle (axis cs:1.73827528882382,0.52421760559082);
\draw[draw=none,fill=color0] (axis cs:0,0.52421760559082) rectangle (axis cs:1.08642205551489,0.626490116119385);
\draw[draw=none,fill=color0] (axis cs:0,0.626490116119385) rectangle (axis cs:0.760494995642261,0.728762686252594);
\draw[draw=none,fill=color0] (axis cs:0,0.728762686252594) rectangle (axis cs:0.108642205551489,0.831035196781158);
\draw[draw=none,fill=color0] (axis cs:0,0.831035196781158) rectangle (axis cs:0.217284411102978,0.933307707309723);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 1000}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0245624426752329) rectangle (axis cs:0.373517160888316,0.0699288472533226);
\draw[draw=none,fill=color0] (axis cs:0,0.069928839802742) rectangle (axis cs:0.87153997335234,0.164420127868652);
\draw[draw=none,fill=color0] (axis cs:0,0.164420127868652) rectangle (axis cs:1.24505720296105,0.258911430835724);
\draw[draw=none,fill=color0] (axis cs:0,0.258911430835724) rectangle (axis cs:1.6185741086022,0.353402733802795);
\draw[draw=none,fill=color0] (axis cs:0,0.353402733802795) rectangle (axis cs:1.12055130595537,0.447894036769867);
\draw[draw=none,fill=color0] (axis cs:0,0.447894036769867) rectangle (axis cs:1.49406840794049,0.542385339736938);
\draw[draw=none,fill=color0] (axis cs:0,0.542385339736938) rectangle (axis cs:1.86758668799003,0.636876583099365);
\draw[draw=none,fill=color0] (axis cs:0,0.636876583099365) rectangle (axis cs:0.747034203970246,0.731367886066437);
\draw[draw=none,fill=color0] (axis cs:0,0.731367945671082) rectangle (axis cs:0.622528503308539,0.825859248638153);
\draw[draw=none,fill=color0] (axis cs:0,0.825859189033508) rectangle (axis cs:0.622528503308539,0.92035049200058);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\end{groupplot}

\draw ({$(current bounding box.south west)!-0.01!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\LARGE{Speed}};
\end{tikzpicture}


==> advML_workshop/experiment_fig/Our_batch_scatter.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 100}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.139259457588196 0.87974089384079
0.421387225389481 0.505936861038208
0.497758567333221 0.281495809555054
0.192086070775986 0.694953858852386
0.976208627223969 0.0887730941176414
0.553409993648529 0.440094947814941
0.439580053091049 0.442619472742081
0.968777179718018 0.246498510241508
0.879478633403778 0.321859002113342
0.927507281303406 0.132060289382935
0.725531160831451 0.677463829517365
0.250144422054291 0.624903559684753
0.282028943300247 0.938794791698456
0.392061352729797 0.590279817581177
0.226367816329002 0.709937810897827
0.253683537244797 0.509217083454132
0.264158725738525 0.527510821819305
0.143192574381828 0.847660481929779
0.0656776130199432 0.856230556964874
0.512509167194366 0.468835383653641
0.452651411294937 0.452691107988358
0.96679413318634 -0.0930522158741951
0.457594335079193 0.362852275371552
0.818558394908905 0.210012018680573
0.0865476429462433 0.760084748268127
0.92186176776886 0.419143319129944
0.229736253619194 0.822469353675842
0.454779326915741 0.55412769317627
0.569496870040894 0.675950586795807
0.605530679225922 0.753823578357697
0.756329953670502 0.356041789054871
0.449440777301788 0.525765717029572
0.401755213737488 0.489267826080322
0.729974925518036 0.641091227531433
0.864565491676331 0.158966660499573
0.569140493869781 0.492613941431046
0.195144489407539 0.906790733337402
0.607923448085785 0.39532533288002
0.704999208450317 0.15942719578743
0.83390611410141 0.280181169509888
0.655198633670807 0.403607189655304
0.58749520778656 0.285376042127609
0.645855844020844 0.349601417779922
0.147765323519707 0.784916758537292
0.640424787998199 0.415896952152252
0.516849458217621 0.365468591451645
0.552274227142334 0.3888900578022
0.628182530403137 0.356706947088242
0.450512319803238 0.634923756122589
0.660074591636658 0.393710017204285
0.116237349808216 0.841611802577972
0.560958743095398 0.501353740692139
0.950110077857971 0.0379549711942673
0.189407855272293 0.777242183685303
0.17595100402832 0.903630018234253
0.808530151844025 0.284991264343262
0.142146334052086 0.782856583595276
0.755055904388428 0.250042021274567
0.383216202259064 0.92495208978653
0.0799809321761131 0.819203019142151
0.261886149644852 0.78420078754425
0.554071724414825 0.41170459985733
0.932360053062439 0.0142253050580621
0.0659285113215446 0.894612729549408
0.150298565626144 0.690214574337006
0.263341963291168 0.644734263420105
0.123858392238617 0.710014164447784
0.447123974561691 0.581269323825836
0.839296758174896 0.0896879211068153
0.46270939707756 0.211884632706642
0.185274988412857 0.767150223255157
0.398056268692017 0.772571265697479
0.542429447174072 0.403975188732147
0.61186957359314 0.46583878993988
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 500}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.776936888694763 0.249753534793854
0.386116743087769 0.406365096569061
0.174472793936729 0.521653413772583
0.805141091346741 0.933307707309723
0.440240800380707 0.551619172096252
0.591361165046692 0.133534938097
0.455250889062881 0.401996105909348
0.332143425941467 0.372915893793106
0.467637568712234 0.814061284065247
0.724299252033234 0.130848690867424
0.158043280243874 0.647002637386322
0.566194474697113 0.347332745790482
0.473153501749039 0.482004195451736
0.267547637224197 0.527089238166809
0.71589583158493 0.430038511753082
0.658745765686035 0.457427114248276
0.144467324018478 0.657042145729065
0.422516047954559 0.367061853408813
0.78759354352951 0.379683077335358
0.370047807693481 0.349326610565186
0.131544753909111 0.42074191570282
0.590262830257416 0.158686131238937
0.888246536254883 0.231273204088211
0.985404491424561 0.173878386616707
0.404500156641006 0.519400238990784
0.335165202617645 0.72149384021759
0.23070877790451 0.558023869991302
0.436972916126251 0.331318795681
0.644021034240723 0.0856519564986229
0.630360901355743 0.435541301965714
0.447283953428268 0.239694103598595
0.180275335907936 0.505020081996918
0.510656476020813 0.335002541542053
0.405353397130966 0.287605851888657
0.464257538318634 0.453973650932312
0.303507149219513 0.453528463840485
0.311053872108459 0.504680037498474
0.690726935863495 0.261621564626694
0.170168474316597 0.674301147460938
0.388627707958221 0.569280743598938
0.561706483364105 0.616437673568726
0.448287129402161 0.329984992742538
0.162112429738045 0.625538289546967
0.247905418276787 0.34765100479126
0.495826065540314 0.558913290500641
0.703568994998932 0.673902451992035
0.25944322347641 0.407854646444321
0.677498459815979 0.390358507633209
0.402255445718765 0.240773573517799
0.329665958881378 0.497239798307419
0.689209342002869 0.216121166944504
0.936314046382904 0.426470637321472
0.0554389469325542 0.885870456695557
0.63409698009491 0.330398440361023
0.935300230979919 0.17045946419239
0.35245755314827 0.348024547100067
0.23744623363018 0.559127688407898
0.323607683181763 0.559788584709167
0.0888271629810333 0.495435357093811
0.127962559461594 0.374380618333817
0.468316853046417 0.234871447086334
0.158229857683182 0.637133896350861
0.716919124126434 0.129116103053093
0.144968807697296 0.523131608963013
0.849043250083923 0.0959296450018883
0.975417494773865 0.011977213434875
0.0905567705631256 0.728091776371002
0.403979033231735 0.260361164808273
0.202995106577873 0.577884078025818
0.182661727070808 0.340855956077576
0.98902815580368 0.225347593426704
0.693903625011444 0.238435164093971
0.587247252464294 0.324716359376907
0.190335050225258 0.475275486707687
0.786740481853485 0.152153328061104
0.426211625337601 0.371549278497696
0.177270129323006 0.292735397815704
0.736927688121796 0.246110171079636
0.446727216243744 0.363649725914001
0.449692755937576 0.485296905040741
0.345438122749329 0.340099722146988
0.8830726146698 0.00464663049206138
0.56570303440094 0.28088241815567
0.805004954338074 0.189938649535179
0.262816816568375 0.33413490653038
0.717803835868835 0.107261158525944
0.864565908908844 0.293800443410873
0.878847897052765 -0.0894175097346306
0.606184422969818 0.199088245630264
0.59554123878479 0.170070052146912
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 1000}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.57584023475647 0.338832080364227
0.225332260131836 0.623566269874573
0.968862056732178 0.346817523241043
0.311254441738129 0.513589560985565
0.568746745586395 0.515619337558746
0.366963326931 0.513030588626862
0.41833233833313 0.463166058063507
0.556143522262573 0.361476302146912
0.529341161251068 0.54360020160675
0.205069601535797 0.647709488868713
0.908150136470795 0.0687245801091194
0.710321962833405 0.378976941108704
0.898783683776855 0.167049989104271
0.161436930298805 0.74740469455719
0.479314923286438 0.819670855998993
0.0888834595680237 0.627499997615814
0.309117376804352 0.631774067878723
0.302228063344955 0.392113834619522
0.614017605781555 0.154380187392235
0.695720970630646 0.465875148773193
0.75020694732666 0.134846374392509
0.874695301055908 0.0960765555500984
0.498199701309204 0.408374339342117
0.710412740707397 0.193369522690773
0.336726933717728 0.338454991579056
0.538124024868011 0.0865073874592781
0.0881228446960449 0.633062362670898
0.771107912063599 0.309533357620239
0.369485050439835 0.374647527933121
0.319801241159439 0.614099442958832
0.744711935520172 0.0975610539317131
0.19185908138752 0.430443435907364
0.269707530736923 0.774192214012146
0.131259053945541 0.855269432067871
0.491700023412704 0.629065930843353
0.671019077301025 0.30482617020607
0.420025080442429 0.478932470083237
0.585492372512817 0.299596399068832
0.361166208982468 0.542346000671387
0.859290421009064 0.120165780186653
0.346621990203857 0.14356492459774
0.131627649068832 0.92035049200058
0.115172833204269 0.535668432712555
0.199532762169838 0.629831790924072
0.200127780437469 0.605798184871674
0.589739680290222 0.321029216051102
0.73112541437149 0.253543674945831
0.598318040370941 0.211257830262184
0.280894696712494 0.91473114490509
0.713802218437195 0.280924409627914
0.347708225250244 0.593869745731354
0.965838074684143 0.537938714027405
0.383636444807053 0.447239965200424
0.935863971710205 0.203516334295273
0.14890643954277 0.680480480194092
0.0562681667506695 0.802294194698334
0.749043345451355 0.179575711488724
0.423711746931076 0.486505329608917
0.844658136367798 0.166071742773056
0.661024570465088 0.563995838165283
0.54025536775589 0.434267282485962
0.565700888633728 0.227442294359207
0.520568788051605 0.592914402484894
0.131979018449783 0.673773288726807
0.876122951507568 0.00479763699695468
0.535711050033569 0.318562299013138
0.345073401927948 0.585593223571777
0.226624682545662 0.70534759759903
0.560894787311554 0.332505911588669
0.278737008571625 0.508535087108612
0.486066699028015 0.266474425792694
0.970355808734894 -0.0245624426752329
0.276687234640121 0.543783009052277
0.643745064735413 0.479749530553818
0.661679565906525 0.178459644317627
0.28415521979332 0.55865490436554
0.292061328887939 0.422659397125244
0.562201738357544 0.833523273468018
0.294146001338959 0.838525772094727
0.0868585333228111 0.749682188034058
0.510356962680817 0.273927867412567
0.669389963150024 0.297383904457092
0.678594410419464 0.222954750061035
0.17401809990406 0.670224070549011
0.25044584274292 0.683681547641754
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!-0.02!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=0.0
]{\LARGE{Radius}};
\draw ({$(current bounding box.south west)!-0.01!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\LARGE{Speed}};
\end{tikzpicture}


==> advML_workshop/experiment_fig/radius_distribution.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, font=\large},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\Large{radius}},
xmin=0, xmax=5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=0.906499451926922,
ytick style={color=black}
]
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.00012119859457016,0) rectangle (axis cs:0.144508928060532,0.411766890524049);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.5}
\addlegendentry{k=1}

\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.14450891315937,0) rectangle (axis cs:0.28889662027359,0.545705991157668);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.28889662027359,0) rectangle (axis cs:0.433284342288971,0.678114247219903);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.433284342288971,0) rectangle (axis cs:0.577672064304352,0.792153776379909);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.577672064304352,0) rectangle (axis cs:0.722059786319733,0.848025492008637);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.722059786319733,0) rectangle (axis cs:0.866447508335114,0.863332811358974);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.866447448730469,0) rectangle (axis cs:1.01083517074585,0.80286923135731);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.01083517074585,0) rectangle (axis cs:1.15522289276123,0.677348881252386);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.15522289276123,0) rectangle (axis cs:1.29961061477661,0.492130317113316);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.29961061477661,0) rectangle (axis cs:1.44399833679199,0.347476149252637);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.44399833679199,0) rectangle (axis cs:1.58838605880737,0.222721496547395);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.58838605880737,0) rectangle (axis cs:1.73277378082275,0.114039529160006);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.73277378082275,0) rectangle (axis cs:1.87716150283813,0.0711790349790643);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.87716150283813,0) rectangle (axis cs:2.02154922485352,0.0336761025707401);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.02154922485352,0) rectangle (axis cs:2.1659369468689,0.0137765874153028);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.1659369468689,0) rectangle (axis cs:2.31032466888428,0.00612292774013456);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.31032466888428,0) rectangle (axis cs:2.45471239089966,0.00306146387006728);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.45471239089966,0) rectangle (axis cs:2.59910011291504,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.59910011291504,0) rectangle (axis cs:2.74348783493042,0.000765365967516821);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.74348783493042,0) rectangle (axis cs:2.8878755569458,0.00153073193503364);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.000629313290119171,0) rectangle (axis cs:0.20014876127243,0.432014092923934);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,fill opacity=0.5}
\addlegendentry{k=2}

\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.200148746371269,0) rectangle (axis cs:0.399668157100677,0.495429042647959);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.399668216705322,0) rectangle (axis cs:0.599187612533569,0.536761979920304);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.599187612533569,0) rectangle (axis cs:0.798707067966461,0.541291536028653);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.798707127571106,0) rectangle (axis cs:0.998226583003998,0.557711467560902);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.998226523399353,0) rectangle (axis cs:1.1977459192276,0.537894469506224);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.19774580001831,0) rectangle (axis cs:1.39726531505585,0.44616904075973);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.39726543426514,0) rectangle (axis cs:1.59678483009338,0.392946065091915);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.59678483009338,0) rectangle (axis cs:1.79630422592163,0.330097342865398);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.79630422592163,0) rectangle (axis cs:1.99582374095917,0.250828534335736);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.99582386016846,0) rectangle (axis cs:2.19534301757812,0.186847664203475);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.19534301757812,0) rectangle (axis cs:2.39486265182495,0.127962110361838);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.39486265182495,0) rectangle (axis cs:2.5943820476532,0.0883279339399694);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.59438228607178,0) rectangle (axis cs:2.79390168190002,0.037369510513064);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.79390144348145,0) rectangle (axis cs:2.99342083930969,0.0232143928944791);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.99342107772827,0) rectangle (axis cs:3.19294047355652,0.015853731732815);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.19294023513794,0) rectangle (axis cs:3.39245963096619,0.00566204704743393);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.39245963096619,0) rectangle (axis cs:3.59197926521301,0.00283102014074863);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.59197950363159,0) rectangle (axis cs:3.79149889945984,0.00169861411423018);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.79149866104126,0) rectangle (axis cs:3.99101805686951,0.00113240940948679);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.000650271773338318,0) rectangle (axis cs:0.263168036937714,0.371470997289431);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,fill opacity=0.5}
\addlegendentry{k=3}

\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.263167977333069,0) rectangle (axis cs:0.525685787200928,0.460623984346566);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.525685787200928,0) rectangle (axis cs:0.788203477859497,0.476833788422071);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.788203477859497,0) rectangle (axis cs:1.05072128772736,0.44576509553637);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.05072128772736,0) rectangle (axis cs:1.31323897838593,0.450718245713403);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.31323885917664,0) rectangle (axis cs:1.57575666904449,0.396685908250042);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.57575678825378,0) rectangle (axis cs:1.83827447891235,0.303930884971575);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.83827447891235,0) rectangle (axis cs:2.10079216957092,0.247647387754617);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.10079193115234,0) rectangle (axis cs:2.36330962181091,0.213427021446706);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.36330986022949,0) rectangle (axis cs:2.62582778930664,0.157143381512121);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.62582778930664,0) rectangle (axis cs:2.88834547996521,0.10806431465656);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.88834524154663,0) rectangle (axis cs:3.1508629322052,0.075645020259592);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.15086317062378,0) rectangle (axis cs:3.41338086128235,0.0481786736177164);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.41338086128235,0) rectangle (axis cs:3.6758987903595,0.0220631108713293);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.67589855194092,0) rectangle (axis cs:3.93841624259949,0.01350803933207);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.93841648101807,0) rectangle (axis cs:4.20093441009521,0.0103561540824607);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.20093441009521,0) rectangle (axis cs:4.46345186233521,0.00405241548002493);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.46345186233521,0) rectangle (axis cs:4.72596979141235,0.00135080270640792);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.7259693145752,0) rectangle (axis cs:4.98848676681519,0.00135080516000831);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.98848724365234,0) rectangle (axis cs:5.25100517272949,0.00045026756880264);
\addplot [semithick, red, opacity=0.5, dashed, forget plot]
table {%
0.5 0
0.5 0.906499451926922
};
\end{axis}

\end{tikzpicture}


==> advML_workshop/experiment_fig/ratio_function.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
% \tiny, \scriptsize, \small, \large, \Large, \LARGE, \huge, \Huge, \HUGE
\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, font=\large},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\Large{radius}},
xmin=-0.260499999765307, xmax=5.25049999998882,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\Large{$g$}},
ymin=-0.0504999995231628, ymax=1.06049998998642,
% ymin=0, ymax=1.06049998998642,
ytick style={color=black}
]
\addplot [line width=3pt, color0]
table {%
-0.00999999977648258 1.00999999046326
0.0406060665845871 0.959393918514252
0.0912121310830116 0.908787846565247
0.141818180680275 0.858181834220886
0.19242425262928 0.807575762271881
0.243030324578285 0.756969690322876
0.293636381626129 0.706363618373871
0.344242453575134 0.655757546424866
0.394848525524139 0.605151474475861
0.445454597473145 0.554545402526855
0.49606066942215 0.50393933057785
0.546666741371155 0.453333258628845
0.597272753715515 0.402727246284485
0.647878885269165 0.352121114730835
0.698484897613525 0.301515102386475
0.749090969562531 0.250909030437469
0.799697041511536 0.200302958488464
0.850303113460541 0.149696886539459
0.900909185409546 0.0990908145904541
0.951515197753906 0.0484848022460938
1.00212132930756 0
1.05272734165192 0
1.10333347320557 0
1.15393948554993 0
1.20454549789429 0
1.25515151023865 0
1.3057576417923 0
1.35636365413666 0
1.40696978569031 0
1.45757579803467 0
1.50818181037903 0
1.55878794193268 0
1.60939407348633 0
1.66000008583069 0
1.71060621738434 0
1.7612122297287 0
1.81181836128235 0
1.86242437362671 0
1.91303038597107 0
1.96363651752472 0
2.01424264907837 0
2.06484866142273 0
2.11545467376709 0
2.16606092453003 0
2.21666693687439 0
2.26727294921875 0
2.31787896156311 0
2.36848497390747 0
2.41909098625183 0
2.46969699859619 0
2.52030301094055 0
2.57090926170349 0
2.62151527404785 0
2.67212128639221 0
2.72272729873657 0
2.77333354949951 0
2.82393932342529 0
2.87454533576965 0
2.92515134811401 0
2.97575759887695 0
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=1}
\addplot [line width=3pt, color1]
table {%
-0.00999999977648258 1.00499999523163
0.0406060665845871 0.979696989059448
0.0912121310830116 0.954393923282623
0.141818180680275 0.929090917110443
0.19242425262928 0.903787851333618
0.243030324578285 0.878484845161438
0.293636381626129 0.853181838989258
0.344242453575134 0.827878773212433
0.394848525524139 0.802575707435608
0.445454597473145 0.777272701263428
0.49606066942215 0.751969695091248
0.546666741371155 0.726666629314423
0.597272753715515 0.701363623142242
0.647878885269165 0.676060557365417
0.698484897613525 0.650757551193237
0.749090969562531 0.625454545021057
0.799697041511536 0.600151479244232
0.850303113460541 0.574848413467407
0.900909185409546 0.549545407295227
0.951515197753906 0.524242401123047
1.00212132930756 0.498939335346222
1.05272734165192 0.473636329174042
1.10333347320557 0.448333263397217
1.15393948554993 0.423030257225037
1.20454549789429 0.397727251052856
1.25515151023865 0.372424244880676
1.3057576417923 0.347121179103851
1.35636365413666 0.321818172931671
1.40696978569031 0.296515107154846
1.45757579803467 0.271212100982666
1.50818181037903 0.245909094810486
1.55878794193268 0.220606029033661
1.60939407348633 0.195302963256836
1.66000008583069 0.169999957084656
1.71060621738434 0.144696891307831
1.7612122297287 0.119393885135651
1.81181836128235 0.0940908193588257
1.86242437362671 0.0687878131866455
1.91303038597107 0.0434848070144653
1.96363651752472 0.0181817412376404
2.01424264907837 0
2.06484866142273 0
2.11545467376709 0
2.16606092453003 0
2.21666693687439 0
2.26727294921875 0
2.31787896156311 0
2.36848497390747 0
2.41909098625183 0
2.46969699859619 0
2.52030301094055 0
2.57090926170349 0
2.62151527404785 0
2.67212128639221 0
2.72272729873657 0
2.77333354949951 0
2.82393932342529 0
2.87454533576965 0
2.92515134811401 0
2.97575759887695 0
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=2}
\addplot [line width=3pt, color2]
table {%
-0.00999999977648258 1.00333333015442
0.0406060665845871 0.986464619636536
0.0912121310830116 0.969595968723297
0.141818180680275 0.952727258205414
0.19242425262928 0.935858607292175
0.243030324578285 0.918989896774292
0.293636381626129 0.902121186256409
0.344242453575134 0.88525253534317
0.394848525524139 0.868383824825287
0.445454597473145 0.851515114307404
0.49606066942215 0.834646463394165
0.546666741371155 0.817777752876282
0.597272753715515 0.800909101963043
0.647878885269165 0.78404039144516
0.698484897613525 0.767171680927277
0.749090969562531 0.750303030014038
0.799697041511536 0.733434319496155
0.850303113460541 0.716565608978271
0.900909185409546 0.699696898460388
0.951515197753906 0.682828307151794
1.00212132930756 0.665959596633911
1.05272734165192 0.649090886116028
1.10333347320557 0.632222175598145
1.15393948554993 0.615353465080261
1.20454549789429 0.598484873771667
1.25515151023865 0.581616163253784
1.3057576417923 0.564747452735901
1.35636365413666 0.547878742218018
1.40696978569031 0.531010031700134
1.45757579803467 0.514141440391541
1.50818181037903 0.497272729873657
1.55878794193268 0.480404019355774
1.60939407348633 0.463535308837891
1.66000008583069 0.446666657924652
1.71060621738434 0.429797947406769
1.7612122297287 0.412929236888885
1.81181836128235 0.396060526371002
1.86242437362671 0.379191875457764
1.91303038597107 0.362323224544525
1.96363651752472 0.345454514026642
2.01424264907837 0.328585803508759
2.06484866142273 0.311717092990875
2.11545467376709 0.294848442077637
2.16606092453003 0.277979671955109
2.21666693687439 0.26111102104187
2.26727294921875 0.244242370128632
2.31787896156311 0.227373659610748
2.36848497390747 0.21050500869751
2.41909098625183 0.193636357784271
2.46969699859619 0.176767647266388
2.52030301094055 0.159898996353149
2.57090926170349 0.143030226230621
2.62151527404785 0.126161575317383
2.67212128639221 0.109292924404144
2.72272729873657 0.092424213886261
2.77333354949951 0.0755555033683777
2.82393932342529 0.0586869120597839
2.87454533576965 0.0418182015419006
2.92515134811401 0.0249495506286621
2.97575759887695 0.00808078050613403
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=3}
\addplot [line width=3pt, red, opacity=0.5, forget plot]
table {%
-0.260499999765307 -2.77555756156289e-17
5.25049999998882 -2.77555756156289e-17
};
\addplot [line width=3pt, red, opacity=0.5, dashed, forget plot]
table {%
0.5 -0.0504999995231629
0.5 1.06049998998642
};
\end{axis}

\end{tikzpicture}


==> advML_workshop/fig_intepret_train.tex <==
\begin{figure}[!t] % !htbp
    \resizebox{\linewidth}{!}{\input{\texhome/Intepretation_fig/AT_batch_scatter}}
    %\vspace{-0.5em}
    % \caption{\scriptsize{Radius-speed plot of AT on the training batch}}
    \caption{Radius-speed plot of AT on the training batches of three iterations. At each iteration, the speed values are normalized to have the maximum absolute value 1 for better visualization of their relative magnitude. Proportions of negative speed are 
    % $33.71\%$ at iteration 5, $34.29\%$ at iteration 30 and $39.87\%$ at iteration 200.
    $33.71\%$, $34.29\%$ and $39.87\%$ at iteration 5, 30 and 200, respectively.}
    \label{fig: interpretation_VR_trainBatch_all}
    \vspace{-2em}
\end{figure}

==> advML_workshop/fig_interpret_test.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}[t]{0.21\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/VR_AT_acc.tex}}
        \caption{\scriptsize{Test accuracy}}
        \label{fig: interpretation_acc}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.55\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/AT_test_scatter}}
        \caption{\scriptsize{Radius-speed plot of AT on the test data points}}
        \label{fig: interpretation_VR_test_scatter}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Intepretation_fig/VR_AT_approx_d}}
        \caption{\scriptsize{Robustness improvement 
        }}
        \label{fig: interpretation_acc_d}
    \end{subfigure}%
    %\vspace{-0.5em}
    \caption{Figure \ref{fig: interpretation_VR_test_scatter} shows the radius-speed plot on a fixed set of points in the test set for three iterations. Figure \ref{fig: interpretation_acc_d} shows the time derivative of the robust accuracy within correct points and its approximation using the dynamics statistics $p(\mathcal{S}_{\mathsf{g}}) - p(\mathcal{S}_{\mathsf{b}})$.}
    \label{fig: interpretation_VR_test_all}
    %\vspace{-1em}
\end{figure}

==> advML_workshop/s0_abstract.tex <==
% Adversarial Training (AT) is among the most effective methods for improving the adversarial robustness of deep neural networks. 
The adversarial robustness of a deep classifier can be measured by the \textit{robust radii}:
the decision boundary's distances to natural data points. 
However, it is unclear whether current adversarial training (AT) methods effectively improves the robust radius for each individual vulnerable point. To understand this, we propose a continuous-time framework that studies the relative speed of the decision boundary with respect to each individual point. 
Through visualizing the speed, a surprising conflicting moving-behavior is revealed: the decision boundary under AT moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones. To alleviate this \textit{conflicting dynamics} of the decision boundary, we propose \textit{\algoNameFull} (\algoName) which directly controls the decision boundary to move away from the training data points. Moreover, in order to further encourage the robustness improvement for more vulnerable points, \algoName controls the decision boundary to move faster away from points with smaller robust radii, achieving customized manipulation of the decision boundary. 
% Therefore, \algoName robustifies each individual vulnerable point rather than focusing on the average robustness. 
As a result, \algoName achieves fairer robustness to individuals, leading to better overall robustness under limited model capacity. 
Experiments verify that \algoName alleviates the conflicting dynamics of the decision boundary and obtains improved robustness compared with the state-of-the-art defenses.





% for abstract submission
% The adversarial robustness of a deep classifier can be measured by the robust radii: the decision boundary's distances to natural data points.
% However, it is unclear whether current adversarial training (AT) methods effectively improves the robust radius for each individual vulnerable point. To understand this, we propose a continuous-time framework that studies the relative speed of the decision boundary with respect to each individual point. Through visualizing the speed, a surprising conflicting moving-behavior is revealed: the decision boundary under AT moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones. To alleviate this conflicting dynamics of the decision boundary, we propose Dynamical Customized Adversarial Training (Dyna-CAT) which directly controls the decision boundary to move away from the training data points. Moreover, in order to further encourage the robustness improvement for more vulnerable points, Dyna-CAT controls the decision boundary to move faster away from points with smaller robust radii, achieving customized manipulation of the decision boundary. As a result, Dyna-CAT achieves fairer robustness to individuals, leading to better overall robustness under limited model capacity. Experiments verify that Dyna-CAT alleviates the conflicting dynamics of the decision boundary and obtains improved robustness compared with the state-of-the-art defenses.

==> advML_workshop/s1_intro.tex <==
\section{Introduction}\label{sec:intro}

Deep neural networks have been successfully deployed in a wide range of applications~\citep{krizhevsky2012imagenet,goodfellow2014generative,he2016deep,collobert2008unified}. 
However, they have been shown to be susceptible to adversarial examples, leading to issues in security-critical applications such as autonomous driving and medicine~\citep{szegedy2013intriguing,nguyen2015deep}.  
To alleviate this problem, adversarial training (AT)~\citep{madry2017towards,shafahi2019adversarial,zhang2019theoretically,gowal2020uncovering} was proposed and is one of the most prevalent methods against adversarial attacks. 
Specifically, AT aims to find the worst-case adversarial examples based on some surrogate loss and adds them to the training dataset in order to improve robustness. 

% \ys{maybe first praise AT for their success?}
Although AT is among the most successful defenses against adversarial perturbations, it has been shown that (even over-parameterized) neural networks, which can perfectly fit natural data in standard training~\citep{zhang2021understanding}, still have insufficient model capacity for fitting adversarial training data~\citep{zhang2021geometryaware}. 
In order to carefully utilize the limited model capacity to fit the neighborhoods of more important data points,
%\fh{what does it mean to utilize the limited model capacity?}, 
weighted adversarial training methods~\citep{zhang2021geometryaware, zeng2020adversarial,liu2021probabilistic} exploit the fact that data points have different vulnerability.  
As shown in Figure~\ref{sfig:demo1}, some data points have smaller robustness radii, i.e., distances to the decision boundary, and are considered more vulnerable. 
% As shown in figure \yc{demo 1: static figure: only different RR}, some data has a smaller robust radius, i.e. its distance to the decision boundary, and is considered more vulnerable. 
Therefore, weighted AT methods assign larger weights to adversarial examples whose natural counterparts have smaller robust radii estimated by the least perturbation steps \citep{zhang2021geometryaware} or the logit margin \citep{zeng2020adversarial,liu2021probabilistic}. 

\begin{figure*}[!t]
\vspace{-0.5em}
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-1.pdf}
        \caption{The decision boundary, vulnerable points (solid) and robust points (hollow).}
    \label{sfig:demo1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-2.pdf}
        \caption{Conflicting moving-behavior of the decision boundary after one step of update.}
    \label{sfig:demo2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Intepretation_fig/AT_Dynamics-demo-3.pdf}
        \caption{Continuous movement of decision boundary.}
    \label{sfig:demo3}
    \end{subfigure}
    \caption{The movement of the decision boundary. Red triangles and green circles are data points from two classes. Figure~\ref{sfig:demo1} shows the vulnerability difference among the data points: some are closer to the decision boundary, whereas some are farther from it. In Figure~\ref{sfig:demo2}, the decision boundary after an update 
    moves away from some vulnerable points (made more robust) but simultaneously moves closer to other vulnerable ones (made less robust). 
    Figure~\ref{sfig:demo3} describes the continuous movement of the decision boundary in Figure~\ref{sfig:demo2}.}
    \label{fig:demos}
    % \vspace{-1.5em}
\end{figure*}

Despite up-weighting the surrogate loss on points with smaller robust radii, these weighted AT methods still do not directly increase the robust radii of each individual vulnerable point. 
In addition, they only train on adversarial examples within an pre-defined universal perturbation threshold for all data points, which is likely sub-optimal due to the difference in vulnerability among points. Therefore, it is unclear whether the learning algorithm is effectively improving the robust radius for each vulnerable point. Geometrically, we are interested to know if the decision boundary moves away from the data points, especially the vulnerable ones. As illustrated in Figure~\ref{sfig:demo2}, 
there can exist conflicting dynamics of the decision boundary:  it moves away from some vulnerable points but simultaneously moves closer to other vulnerable ones during training. This motivates us to ask:


% In addition, they control the level of robustness by pre-defining the perturbation length $\epsilon$ and all of the points used for training are within $\epsilon$ distance from the original points, in regardless o
% However, this is sub-optimal because different points have different robustness and the model is unlikely to be robust to a more diverse attack budget.\yc{Some new sentences for varying $\epsilon$} 

\textbf{Question 1}\quad \textit{Given an training algorithm, how to analyze the dynamics of the decision boundary with respect to the data points?}

To answer this, we propose a continuous-time framework that studies the instantaneous movement of the decision boundary as shown in Figure~\ref{sfig:demo3}. Specifically, we define the relative speed of the decision boundary w.r.t. a point to be the time derivative of its robust radius, which can be interpreted as the speed of its closest adversarial example moving away from it. We show that the speed can be derived from the training algorithm using a closed-form expression. 

Using the proposed framework, we numerically compute the speed of the decision boundary w.r.t. data points for AT. As shown in Figure~\ref{fig: interpretation_VR_trainBatch_all},
We observe that a significant proportion of vulnerable points has negative speed, indicating the existence of the aforementioned conflicting dynamics (Figure~\ref{sfig:demo2},\ref{sfig:demo3}) of the decision boundary.
% across data points is a prevalent phenomenon, although it cannot be observed using averaged statistics such as robust accuracy or an average of a surrogate loss. 
On the other hand, a desirable dynamics should satisfy that the decision boundary moves away from the vulnerable points. Moreover, the speed should be larger for points with smaller robust radii in order to encourage the robustness improvement on vulnerable points. 
This leads to another question:

\textbf{Question 2}\quad \textit{How to design algorithms to achieve desirable dynamics of the decision boundary?}

To this end, we propose \textit{\algoNameFull (\algoName)}, which explicitly controls the decision boundary to move away from the data points and moreover, faster from the points with smaller robust radii. Such control is possible since we can derive the dynamics of the decision boundary given a training algorithm, which enables us to reverse engineer the training scheme to achieve the desirable dynamics. Specifically, \algoName adopts a weighted loss on the closest boundary points, where the weights are reverse engineered to realize the 
% desirable 
dynamics. 

Unlike previous weighted AT methods which directly assign larger weights to more vulnerable points, \algoName designs the weights so that the robustness improvement of vulnerable points is faster. In addition, instead of pre-defining a uniform perturbation length for training as in AT, \algoName trains on the closest boundary points to take into account of the robust radius of each point. Consequently, \algoName is naturally robust to more diverse attacking budget $\epsilon$'s, whereas previous weighted AT methods are trained to be robust to a pre-defined $\epsilon$.
We experimentally demonstrate that \algoName realizes the desirable dynamics during training and achieves improved robustness performance on diverse attacking budgets. 


\textbf{Summary of contributions.} \textbf{(1)} We propose a continuous-time framework to study the relative speed of the decision boundary w.r.t. each individual data point and provide its closed-form expression.
\textbf{(2)} We visualize the speed of the decision boundary for AT and identify the conflicting dynamics of the decision boundary. 
\textbf{(3)} We propose Dynamical Adversarial Training (\algoName) which controls the decision boundary to move faster from more vulnerable points with smaller robust radii. We experimentally demonstrate that \algoName alleviates the conflicting dynamics and obtains improved robustness over state-of-the-art defenses.  



==> advML_workshop/s2_prelim.tex <==
\section{Preliminaries} \label{sec:prelim}
% \subsection{Notations and definitions}

\textbf{Notations and definitions}\quad
We consider a classification task with inputs $x \in \mathcal{X}$ and labels $y\in\mathcal{Y} = \{1,2,...,K\}$.
Let $\{x_i,y_i\}_{i=1}^N$ be all training data of size $N$. A deep classifier parameterized by $ \theta $ is denoted by $f_{\theta}(x) = \argmax_{c\in\mathcal{Y}}z_{\theta}^c(x)$ where $z_{\theta}^c(x)$ is the logit for class $c$. 
% Denote $z_\theta(x)$ to be the vector of logits for all classes. 
Denote the logit margin of class $ y $ as $ \phi^{y}_{\theta}(x) = z_{\theta}^y(x) - \max_{y'\neq y} z_{\theta}^{y'}(x) $. In the paper, we will use $\phi^{y}_\theta(x)$ and $\phi^{y}(x,\theta)$ interchangeably. Observe that $ x $ is classified as  $ y $ if and only if $ \phi^{y}_{\theta}(x) > 0 $. Therefore,  the zero level set of $ \phi^{y}_{\theta}(x) $, denoted by $ \Gamma_y=\{x: \phi^{y}_{\theta}(x) = 0\} $, is the decision boundary for class $ y $. Denote $\|\cdot\|_p$ the $L_p$ norm.
% with $1 \leq p \leq \infty$.
% For a correctly classified point $(x,y)$, its robust radius $R_\theta(x)$ is defined to be the distance from $x$ to the decision boundary for class $y$. That is,
% % \setlength\abovedisplayskip{0pt}
% % \setlength\belowdisplayskip{0pt}
% \begin{equation} \label{eq: robustness_radius}
%     R_\theta(x) = \min_{\hat{x}} \|\hat{x}-x\|_p \quad \textrm{s.t.}  \quad \phi_\theta^y(\hat{x}) = 0
% \end{equation}
% where $\|\cdot\|_p$ is the $L_p$ norm with $1\leq p \leq \infty$.


% \subsection{Continuous-time formulation}

\textbf{Continuous-time formulation}\quad
In this paper, we will use the continuous-time formulation for the optimization on the parameters $\theta$, which allows us to study the instantaneous movement of the decision boundary. Let $\theta'(t)$ be the continuous-time description of a training algorithm, which consists of a loss function $L$ and an optimization scheme. To derive the discrete counterpart $\theta'_k$ of $\theta'(t)$ at iteration $k$ given a training algorithm, we use the relationship $\theta'_k :=\frac{\theta_{k+1} - \theta_{k}}{\gamma}$, where $\gamma$ is the learning rate. 
For example, consider the commonly used stochastic gradient descent (SGD) with momentum ($\lambda_m$) and weight decay  ($\lambda_w$) given by
\begin{equation} \label{eq: SGD_momentum_weightDecay shorter}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
\begin{aligned}
    b_{k+1} = \nabla_\theta L(\theta_{k}) +  \lambda_w \theta_{k} + \lambda_m b_{k}, \quad 
    \theta_{k+1} = \theta_{k} - \gamma b_{k+1}
\end{aligned}
\end{equation}
where $b_0 = 0$ and $b_k$'s are the intermediate variables. In this case, $\theta'_k$ is given by 

\begin{equation} \label{eq: theta prime momentum weight decay general}
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}
\begin{aligned}
    \theta'_k &= -\nabla_\theta L(\theta_{k})  - \lambda_w \theta_{k}- \lambda_m b_{k} %\fhc{?}\text{\yc{What is unclear?}}
\end{aligned}
\end{equation}

% which can be interpreted as the un-normalized update direction of $\theta$ at step $k$. 

==> advML_workshop/s3_dynamics4DB.tex <==
\section{Dynamics of the decision boundary} \label{sec: dynamics_of_bdr}
In this section, we will study the dynamics of the decision boundary in continuous time by first defining its speed with respect to each data point and then providing a closed-form expression for the speed.
Finally, we visualize the speed of the decision boundary of AT and analyze its dynamics. 

\subsection{Speed of the decision boundary}
For a correctly classified example $(x_i,y_i)$, we would like to capture the movement of the decision boundary $\Gamma_{y_i} (t) = \{x:\phi^{y_i}(x,\theta(t)) = 0\}$ w.r.t. $x_i$ as $t$ varies continuously. Therefore, we consider its closest boundary point:



\begin{definition}[Curve of the closest boundary point $\hat{x}_i(t)$] \label{def: closest_pt}
Suppose that $(x_i,y_i)$ is correctly classified by $f_{\theta(t)}$ in some time interval $t \in I$. Define the curve of the closest boundary point $\hat{x}_i(\cdot): I \to \mathcal{X}$ as
\begin{equation} \label{eq: closest_pt}
% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}
    \hat{x}_i(t) = \argmin\nolimits_{\hat{x}} \|\hat{x}-x_i\|_p \quad \textrm{s.t.}  \quad \phi^{y_i}(\hat{x},\theta(t)) = 0.
\end{equation}
Define the robust radius of $x_i$ at time $t$ to be $R(x_i,t) = \|\hat{x}_i(t)-x_i\|_p $.
%\fhc{we need to explain $l_p$ norm. For example, how to choose $p$. Or what values can $p$ take?}\yc{added an explanation in prelim section.}
\end{definition}

% \begin{wrapfigure}{r}{0.3\textwidth}
\begin{figure}[!t] % [!htbp]
% \vspace{-2.5em}
    \centering
    \includegraphics[width=0.5\columnwidth]{Intepretation_fig/AT_Dynamics-derivation.pdf}
    \vspace{-1em}
    \caption{Curve of the closest boundary point $\hat{x}(t)$ (in blue) of the data point $x$.}
    \label{fig:curve}
\vspace{-1em}
\end{figure}
% \end{wrapfigure}

An example of the curve of the closest boundary point is depicted in Figure~\ref{fig:curve}.
To understand how the distance between the decision boundary $\Gamma_{y_i} (t)$ and $x_i$ changes, it suffices to focus on the curve of the closest boundary point $\hat{x}_i(t)$. We define the speed of the decision boundary to be the time derivative of the robust radius as follows:

\begin{definition}[Speed of the decision boundary $s(x_i,t)$] \label{def: speed_of_bdr}
Under the setting of definition \ref{def: closest_pt}, define the relative speed of the decision boundary w.r.t. $x_i$ as $s(x_i,t) = \frac{d}{dt} R(x_i,t) = \frac{d}{dt}  \|\hat{x}_i(t)-x_i\|_p$.
\end{definition}

Note that the speed $s(x_i,t) > 0$ means that the robustness improves for $x_i$ at time $t$, which is desirable during adversarial training. The next proposition gives a closed-form expression for the speed given a training algorithm $\theta'(t)$.

\begin{proposition}[Closed-form expression of the speed] For $1 \leq p \leq \infty$,
% \setlength\abovedisplayskip{2pt}
% \setlength\belowdisplayskip{2pt}   
\begin{equation} \label{eq: expression_for_speed}
    s(x_i,t) = \frac{\nabla_\theta \phi^{y_i} (\hat{x}_i(t),\theta(t)) \cdot \theta'(t)}{\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q} 
\end{equation}
where $q$ satisfies that $1/q+1/p=1$. In particular, $q=2$ when $p=2$ and $q=1$ when $p=\infty$.
\end{proposition}

\paragraph{Remark}
The main assumption for Equation~\eqref{eq: expression_for_speed} is the local differentiability of $\phi^{y_i}(\cdot,\theta(t))$ at $\hat{x}_i(t)$.  The full assumptions and proof are left to Appendix~\ref{app: closed_expression_speed}. The key points of proving Equation~\eqref{eq: expression_for_speed} include the level set equation \citep{osher2004level,aghasi2011parametric} and the optimality condition for optimization problem~\eqref{eq: closest_pt}. Special care has been taken for $p=\infty$ since $L_\infty$ norm is not differentiable.

According to Equation~\eqref{eq: expression_for_speed}, the speed $s(x_i,t_0) $ is positive at time $t_0$ when $\nabla_\theta \phi^{y_i} (\hat{x}_i(t_0),\theta(t_0)) \cdot \theta'(t_0) >0$, i.e. the value of $\phi^{y_i}(\hat{x}_i(t_0))$ increases. This means that the boundary point $\hat{x}_i(t_0)$ will be correctly classified after the update. Also, the magnitude of the speed tends to be larger if $\|\nabla_x \phi^{y_i}(\hat{x}_i(t),\theta(t))\|_q$ is smaller, i.e. the margin function $\phi^{y_i}$ is flatter around $\hat{x}_i(t)$. In the remaining part of the paper, we will denote $s(x_i,t)$ and $R(x_i,t)$ as $s(x_i)$ and $R(x_i)$ when the indication is clear.

\textbf{Computing the closest boundary point}\quad 
To implement the Equation~\eqref{eq: expression_for_speed} in practice, we need to compute the closest boundary point $\hat{x}_i(t)$. We use the Fast Adaptive Boundary Attack (FAB) \citep{croce2020minimally} to approximate $\hat{x}_i(t)$. Note that here FAB only serves as an algorithm to approximate $\hat{x}_i(t)$, and can be decoupled from the remaining part of the framework. In our experiments we find that given enough number of iterations, FAB can reliably find the local optimum of Equation~\eqref{eq: closest_pt} where the expression for speed in Equation~\eqref{eq: expression_for_speed} is still valid. We give more details of how to check the local optimality condition of Equation~\eqref{eq: closest_pt} and the performance of FAB in Appendix~\ref{app: optimality}. 


\subsection{Dynamics of adversarial training} \label{ssec: Dynamics of adversarial training}
In this section, we numerically compute the speed of the decision boundary to understand the dynamics during training. More analysis of the dynamics are left to Appendix~\ref{app: more_dynamics}. 

We train a ResNet-18 \citep{he2016deep} on CIFAR-10 using 10-step PGD under $L_2$ perturbation with $\epsilon=0.5$ from a naturally pretrained model and evaluate it using 20-step PGD. The test accuracy is shown in Figure~\ref{fig: AT_acc}. We choose 512 points from the test set and at each iteration, we compute the robust radii and speed for correctly classified ones. We omit those points whose robust radii are larger than 1, which are considered very robust under $\epsilon=0.5$. The speed distribution over time is shown in Figure~\ref{fig: AT_speed_time}. We can observe that at the start of training (the first 100 iterations), the speed distribution is mostly positive and the robust accuracy increases drastically. Later, the speed distribution is centered around zero and the robustness improvement slows down. 

\input{\texhome/Speed_unnormalized_time}

\textbf{Non-converging dynamics of AT}\quad
In Figure~\ref{fig: AT_speed_time} we find that the variance of the speed distribution is never vanishing: the decision boundary always moves towards some data points while moving away from others. This indicates that AT does not converge. Despite the constant movement of the decision boundary, the average adversarial loss does converge. Therefore, the dynamics of the decision boundary w.r.t. each data point provides more information than an average of the surrogate loss. For comparison with AT, we adopt natural training (NT) whose test accuracy and speed distribution are shown in Figure~\ref{fig: clean_acc} and Figure~\ref{fig: clean_speed_time}. We observe that the speed distribution of the decision boundary during NT is effectively zero. This indicates that NT eventually does not move the decision boundary around correctly classified points anymore, which is different from AT. 


\textbf{Conflicting dynamics of AT}\quad Since the update of the parameters $\theta$ at each iteration is computed on one batch of the training data, we visualize the robust radii and speed on the training batch of each iteration in Figure~\ref{fig: interpretation_VR_trainBatch_all}. Observe that there is always a significant proportion of non-robust points (with $R(x_i)<0.5$) with negative speed, indicating the conflicting dynamics on the training batch. This is not desirable because ideally at each iteration, the vulnerable points in the training batch should be improved since the current update of $\theta$ is computed on them.
% \yc{This is also typical in other variants of AT, which is shown in appendix.} 
In Section~\ref{sec:dynamicalAT}, we will see that such conflicting dynamics can be alleviated: since the update rule has full access to the training batch, it is possible to design the update rule so that every vulnerable point in the training batch is made more robust. 


\input{\texhome/fig_intepret_train}




==> advML_workshop/s4_dynamicalAT.tex <==
\section{\algoName: \algoNameFull}\label{sec:dynamicalAT}

To remedy the conflicting dynamics issue and encourage robustness improvement on more vulnerable points, we propose \algoNameFull (\algoName), which customizes the dynamics of the decision boundary for each data point. We first introduce the design of the desirable dynamics in Section~\ref{ssec: dynamics_design}, and then present the algorithm in Section~\ref{ssec: realizing_dynamics}.
 
\subsection{Design of desirable dynamics} \label{ssec: dynamics_design}


% \setlength\abovedisplayskip{1pt}
% \setlength\belowdisplayskip{1pt}

Ideally, the decision boundary should move away from each vulnerable point. Moreover, given the limited capacity of the neural networks, robustness improvement on more vulnerable points should be encouraged more. Therefore, the desirable dynamics should satisfy the following conditions: 
\begin{list}{$\rhd$}{\topsep=0.ex \leftmargin=0.3in \rightmargin=0.in \itemsep =0.0in}
    \item \textbf{Condition 1:} $s(x_i) > 0 $ when $R(x_i) < r_0$ for some threshold $r_0$. 
    \item \textbf{Condition 2:} $s(x_i) \geq s(x_j)$ when $R(x_i) < R(x_j)$.
\end{list}

In particular, \textbf{Condition 2} considers customized manipulation of the decision boundary by encouraging smaller robust radii to improve faster. The goal of \algoName is to approximate both conditions and thus achieving fairer robustness to each data point as well as better overall robustness.
% under the limited model capacity.

% In particular, \textbf{Condition 2} considers a customized manupulation of the decision boundary. When satisfied, it robustifies each individual vulnerable point\yc{..fairness; dyna-cat; customized..}. % rather than focusing on the average robustness (or more accurately (un)weighted average of surrogate robustness) as in most prior works. 
% Consequently, \textbf{Condition 2} achieves a fairer robustness to individuals, leading to better overall robustness under a limited model capacity as well. % \yc{Not quite accurate: Previous work focus on surrogate loss, weighted average. We focus on improving radius faster.}


To design such desirable dynamics, we introduce a \textit{ratio function} $g(r)$, a non-increasing function that satisfies $g(r) > 0$ when $r < r_0$ for some threshold $r_0$. 
At each iteration, the speed $s(x_i)$ of the decision boundary w.r.t. $x_i$ should be approximately proportional to $g(R(x_i))$. In other words, $s(x_i) \approx \mu \cdot g(R(x_i))$ for some common scalar $\mu > 0$ for all data points. Since the effect of $g$ does not change if it is multiplied by a constant, we fix $g(0) = 1$. 


\textbf{Controlling the robustness level with the ratio function}\quad Instead of using a pre-defined perturbation length to control the robustness level, \algoName uses all of the closest boundary points, 
% with respect to all correctly classified data points during training
including those that are relatively far from the original ones. The ratio function $g$ controls the robustness level: if $g$ decays more slowly, \algoName will encourage robustness improvement even when the robust radius is large, and thus the model is robust to larger perturbation thresholds. On the other hand, if $g$ decays fast, the improvement on the non-robust points will be encouraged more.
% , so the model is unlikely to be able to withstand larger perturbation thresholds. 
How to calculate the optimal $g$ is still an open question. Therefore, we heuristically design different $g'$s and discuss more about them in Section~\ref{sec:exp_effect} and Appendix~\ref{app: further_exp_results}.

\subsection{\algoName: Realizing the desirable dynamics} \label{ssec: realizing_dynamics}
To customize the dynamics of the decision boundary for each data point, we propose to use a weighted average of loss on the closest boundary points and compute the weights to achieve the designed dynamics. Consider a batch $\mathcal{B}$ with size $n$ and denote $\mathcal{B}^{+}_\theta$ of size $m$ to be the set of correctly classified points in $\mathcal{B}$. We use the following loss function
\begin{equation} \label{eq: weighted loss general}
	L_\theta(\mathcal{B}) =  -\sum\nolimits_{i\in \mathcal{B}^{+}_\theta}c_i \phi^{y_i}(\hat{x}_i) + \lambda_{c}\frac{1}{n}\sum\nolimits_{i\in \mathcal{B}}l(x_i,y_i) 
\end{equation}
where the first term is the weighted margin loss on the closest boundary points  with weights $\{c_i\}$ to be determined. The second term is the cross-entropy loss on natural examples.

The speed $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$ depends on the weights $\mathbf{c} = (c_1,\cdots, c_m)^{T}$ in the following way: $\mathbf{c}$ determines the loss function by Equation~\ref{eq: weighted loss general}; the loss function, together with an optimization scheme, determines $\theta'(t)$ (for example, by Equation~\ref{eq: theta prime momentum weight decay general}); finally, $\theta'(t)$ determines the speed $\mathbf{s}$ by the closed-form expression~\ref{eq: expression_for_speed}. Since these dependencies are all linear, $\mathbf{s}$ is a linear function of $\mathbf{c}$, denoted by $\mathbf{s}(\mathbf{c})$. 


Our goal is to reverse engineer the weights $\mathbf{c}$ so that the speed $\mathbf{s}(\mathbf{c})$ approximates the designed dynamics specified by the ratio function $g$. Let the ratio values $\mathbf{g} = (g(R(x_1)),\cdots,g(R(x_{m})))^{T}$. 
% To approximate the desired dynamics given by $\mathbf{g}$, 
We solve the following optimization problem:
\vspace{-0.5em}
\begin{equation} \label{eq:opt_for_weight}
% \begin{aligned}
\setlength\abovedisplayskip{10pt}
\setlength\belowdisplayskip{2pt}
\min_{\mathbf{c}, \mu} \quad  \|\mathbf{s}(\mathbf{c}) - \mu \mathbf{g}\|^2_2 \quad
\textrm{s.t.} \quad \sum\nolimits_{i} c_i = 1, c_i\geq0, \mu \geq 0    \\
% \end{aligned}
\end{equation}

where $\mu$ is a scalar so that the solved $\mathbf{s}(\mathbf{c})$ is approximately a multiple of $\mathbf{g}$.
The problem~\eqref{eq:opt_for_weight} is a quadratic programming problem with linear constraints of size $m+1$, which is convex and can be solved efficiently and reliably. 
According to our experiments, the extra runtime of solving this quadratic programming is negligible.
We give the coefficient of this quadratic programming problem in Appendix~\ref{app: opt_for_weight}. The pseudocode of \algoName is shown in Appendix~\ref{app: algo_pseudo}. We also introduce a burn-in period where we only use the clean loss during the initial stage of the training to achieve a descent clean accuracy. This is necessary because the closest boundary points used by \algoName can only be found for correctly classified examples. 





% Let the ratio values $\mathbf{g} = (g(R(x_1)),\cdots,g(R(x_{m})))^{T}$ and $\mathbf{s} = (s(\hat{x}_1),\cdots,s(\hat{x}_m))^{T}$. 
% According to the speed expression \eqref{eq: expression_for_speed}, the expression of $\theta'_k$ in \eqref{eq: theta prime momentum weight decay general} and the loss function \eqref{eq: weighted loss general}, $\mathbf{s}$ is a linear function of the  weights $\mathbf{c}$ and we denote it as $\mathbf{s}(\mathbf{c})$. 

\textbf{Comparisons with related adversarial training methods}\quad 
Several existing adversarial training methods also leverage the vulnerability difference among data points. In particular, MMA\citep{Ding2020MMA} trains on the closest boundary points, which is similar to \algoName. However, MMA adopts uniform weights and thus does not necessarily improve robustness of every vulnerable point. On the other hand, weighted adversarial training methods
% \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware}
assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. More related works are left to Appendix~\ref{sec:related_work_app}.




==> advML_workshop/s5_related.tex <==
\section{Related Work}\label{sec:related}

\textbf{Controlling parameterized surface}\quad 
The decision boundary can be viewed as a parameterized surface in the input space. Controlling such surface has been studied in image segmentation\citep{li2011level,aghasi2011parametric} and shape modelling\citep{chen2019learning,park2019deepsdf}. As for adversarial training, the authors of \citep{Atzmon2019control} propose to maximize the distance between each data point and some point on the decision boundary, which is not the closest one. On the other hand, we study the movement of the decision boundary w.r.t. each data point by analyzing its closest boundary point, which is directly related to the 
robust radius. 

\textbf{Comparisons with related adversarial training methods}\quad 
There are several defense techniques including gradient regularization \citep{moosavi2019robustness,tramer2017ensemble}, certified denfense\citep{cohen2019certified,wong2018provable,balunovic2019adversarial} and adversarial training \citep{madry2017towards,zhang2019theoretically,gowal2020uncovering,wang2019improving,zhang2020attacks}, where the last one is the most related to this work. 
In particular, MMA\citep{Ding2020MMA} trains on the closest boundary points, which is similar to \algoName. However, MMA adopts uniform weights and thus does not consider the vulnerability difference among the points. On the other hand, weighted adversarial training methods \citep{zeng2020adversarial,liu2021probabilistic,zhang2021geometryaware} assign larger weights to more vulnerable data points with smaller robust radii. However, previous weighted AT methods rely on indirect approximation of the robust radius, which might not be optimal. For example, GAIRAT \citep{zhang2021geometryaware} uses the least number of steps to attack an clean example as an surrogate to its robust radius, which is shown to be heavily dependent on attack paths and thus likely to make wrong judgement on the robustness \citep{liu2021probabilistic}. As another approximation, the logit margin \citep{liu2021probabilistic,zeng2020adversarial} is used but a larger logit margin value does not necessarily correspond to a larger robust radius. In this paper, we directly find the closest boundary points along with the robust radii. Moreover, instead of simply assigning larger weights to points with smaller robust radii, we compute the weights so that more vulnerable points will be improved faster. 



% so that an example with a larger logit margin value is viewed as more robust. However, a larger logit margin value does not necessarily correspond to a larger robust radius. 


==> advML_workshop/s6_exp.tex <==
\section{Experiments}\label{sec:exp}
In this section, we empirically evaluate the proposed \algoName on the CIFAR-10 \citep{krizhevsky2009learning} dataset. We visualize its dynamics in Section~\ref{sec:exp_effect} and evaluate its robustness performance and compare it with several state-of-the-art baselines in Section~\ref{sec:exp_robust}. Implementation details are left to Appendix \ref{app: exp_settings}, including neural network architectures and training hyperparameters. 
% Further experimental results are presented in Appendix \ref{app: further_exp_results}.

\subsection{Realizing the desirable dynamics}
\label{sec:exp_effect}

\begin{figure}[!t]
    \centering
    \resizebox{\columnwidth}{!}{\input{\texhome/experiment_fig/Our_batch_scatter}}
    \vspace{-0.3em}
    \caption{Radius-speed plot of \algoName on the training batches for three randomly chosen iterations. Proportion of points with negative speed for these iterations are all below $2\%$.}
    \label{fig: performance_batch_VR_ours}
    \vspace{-1.5em}
\end{figure} 

\algoName computes the weights to approximate the desirable dynamics by solving the optimization problem \eqref{eq:opt_for_weight}. To verify the quality of this approximation, we consider the $L_2$ norm constrained perturbation and choose the ratio function $g(r) = 1 - r$ when $r \leq 1$ and $g(r)=0$ otherwise. 
In Figure~\ref{fig: performance_batch_VR_ours}, we visualize the speed and robust radii of points in the training batches of three randomly chosen iterations.
We observe that the speed is positive for most of the points and is approximately a decreasing function of the robust radius, which is consistent with the design of $g$. 
By comparing with the conflicting dynamics of AT in Figure~\ref{fig: interpretation_VR_trainBatch_all}, we conclude that \algoName alleviates the conflicts and achieves the desirable dynamics during training. 


\subsection{Robustness Evaluation}
\label{sec:exp_robust}
\textbf{Compared baselines}\quad
The baseline defense methods include: (1) standard adversarial training (AT) \citep{madry2017towards} which trains on the worst case adversarial examples; (2) TRADES \citep{zhang2019theoretically} which trades off between the clean and robust accuracy; (3) MMA \citep{Ding2020MMA} which trains on the closest adversarial examples with uniform weights; (4) GAIRAT \citep{zhang2021geometryaware} which reweights adversarial examples based on the least perturbation steps. Their hyperparameters are left to Appendix~\ref{app: exp_settings}. 

\textbf{Evaluation protocol}\quad
We evaluate \algoName and the baselines under $L_2$ and $L_\infty$ norm constrained perturbation. The final robust accuracy is reported on AutoAttack (AA) \citep{croce2020reliable}, which uses an ensemble of selected strong attacks. We also include the results under PGD attack with 40 iterations in Appendix~\ref{app: further_exp_results}. For all methods, we choose the hyperparameters to achieve the best robust accuracy under the commonly used perturbation length $\epsilon = 0.5$ for $L_2$ setting and $\epsilon=\frac{8}{255}$ for $L_\infty$ setting. We also evaluate on larger perturbation thresholds to better examine the robustness of the models.
% against unknown perturbation strength.

\textbf{Hyperparameters of \algoName}\quad 
We use the ratio function with $g(0) = 1, g(r_0) = 0, g(r_1) = - g_1$ with $g_1 \geq 0 $ and linearly interpolate them when $0\leq r \leq r_1$. When $r>r_1$, $g(r)$ was set to the constant $-g_1$. We allow $g$ to be negative when $r > r_1$ because we experimentally find that 'pulling back' the decision boundary if it is too far away from data points could help improve both clean and robust accuracy. Choices of $r_0, r_1, g_1$ and other hyperparameters are left to Appendix~\ref{app: exp_settings}.


\textbf{Performance}\quad 
The main evaluation results are shown in Table \ref{table: performance_L2_more_eps} and Table \ref{table: performance_Linf_more_eps}. The full results and the ablation study on the effect of the ratio function are left to Appendix~\ref{app: further_exp_results}. In the $L_2$ case, \algoName obtains higher robust accuracy over all baselines on all considered perturbation thresholds. In the $L_\infty$ case, \algoName obtains both higher clean accuracy and robust accuracy than AT, MMA and GAIRAT. We observe that GAIRAT achieves high robustness under PGD attacks (shown in Appendix~\ref{app: further_exp_results}) but has much lower robust accuracy under the stronger AA attack, which may be due to obfuscated gradient \citep{AthalyeC018}. On the other hand, the performance gap between PGD and AA is relatively small for \algoName. When compared with TRADES, \algoName shows higher clean accuracy and comparable robust accuracy under larger $\epsilon$, although \algoName has lower robust accuracy when $\epsilon = \frac{8}{255}$. This is partially due to the higher difficulty of approximating the closest boundary points in the $L_\infty$ case, and a better algorithm for this is left for future work. 
\input{\texhome/tab_L2_moreEps}
\input{\texhome/tab_Linf_moreEps}
% \input{\texhome/tab_moreEps}

==> advML_workshop/s7_conc.tex <==
\section{Conclusion and Discussion} \label{sec:conc}

This paper has proposed a general framework to study the relative movement of the decision boundary w.r.t. each data point given an training algorithm. Using this framework, we reveal the non-converging and conflicting dynamics of AT. To alleviate the conflicts, we propose \algoNameFull (\algoName) to control the decision boundary to move faster away from more vulnerable points, which shows promising results on robustness performance. The future direction includes (a) designing more efficient algorithms for finding the closest boundary points; (b) better design of the desirable dynamics; (c) combining \algoName with other methods such as TRADES; (d) using the proposed framework to study the dynamics of other training algorithms for further insights. 





==> advML_workshop/tab_L2_moreEps.tex <==
\begin{table}[!htbp]
\centering
\noindent
\caption{{Clean and robust accuracy on CIFAR-10 under $L_2$ attack}}
\resizebox{\columnwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=0.5$}  & {$\epsilon=1$} & {$\epsilon=1.5$}  & {$\epsilon=2$} \\
\midrule
AT & {$88.38 \pm 0.23$} & {$65.29 \pm 0.21$}  & {$33.71 \pm 0.16$}  & {$11.16 \pm 0.09$}  & {$2.4 \pm 0.17$}  & \\
TRADES & {$87.05 \pm 0.01$} & {$67.92 \pm 0.11 $}  & {$42.08 \pm 0.16$}  & {$19.33 \pm 0.38$} & {$6.62 \pm 0.16$}  & \\
MMA & {$\boldsymbol{88.40} \pm 0.14$} & {$65.62 \pm 0.23$}  & {$36.54 \pm 0.14$} & {$14.01 \pm 0.08$}  & {$3.49 \pm 0.10$}  & \\
\midrule
Ours & {$87.25 \pm 0.05$} & {$\boldsymbol{67.96} \pm 0.14$}   & {$\boldsymbol{43.48} \pm 0.23$}  & {$\boldsymbol{20.92} \pm 0.12$} & {$\boldsymbol{6.72} \pm 0.18$} &  \\
\bottomrule
\end{tabular}}
\label{table: performance_L2_more_eps}
\end{table}

==> advML_workshop/tab_Linf_moreEps.tex <==
\begin{table}[!htbp]
\vspace{-1em}
\centering
\noindent
\caption{{Clean and robust accuracy on CIFAR-10 under $L_\infty$ attack} }
\resizebox{\columnwidth}{!}{\begin{tabular}{lSSSSSS}
\centering
Defense & {Clean} & {$\epsilon=\frac{8}{255}$} & {$\epsilon=\frac{12}{255}$} & {$\epsilon=\frac{16}{255}$} & {$\epsilon=\frac{20}{255}$} \\
\midrule
AT & {$83.25 \pm 0.17$} & {$45.75 \pm 0.15$} & {$26.38 \pm 0.14$} & {$12.34 \pm 0.17$} & {$4.89 \pm 0.11$}& \\
TRADES & {$83.54 \pm 0.08$} & {$\boldsymbol{47.18} \pm 0.11$}  & {$29.03 \pm 0.19$}& {$15.07 \pm 0.11$}  & {$\boldsymbol{6.78} \pm 0.06$} & \\
MMA & {$84.25 \pm 0.28$} & {$41.48 \pm 0.31$} & {$23.63 \pm 0.25$} & {$11.97 \pm 0.20$} &{$5.11 \pm 0.12$} & \\
GAIRAT & {$81.31 \pm 0.23$} & {$32.98 \pm 0.11$}& {$16.19 \pm 0.02$} & {$6.89 \pm 0.18$}  & {$2.57 \pm 0.07$} & \\
\midrule
Ours & {$\boldsymbol{85.13} \pm 0.13$} & {$46.47 \pm 0.18$}  & {$\boldsymbol{29.38} \pm 0.24$} & {$\boldsymbol{15.14} \pm 0.16$} & {$6.45 \pm 0.21$} & \\
\bottomrule
\end{tabular}}
\label{table: performance_Linf_more_eps}
\vspace{-1em}
\end{table}

==> algo.tex <==
%%% wrapping algorithm inside a figure environment, so that we can adjust the spacing around it using \vspace{}

\begin{figure}[!htbp]
\vspace{-1em}
\centering
\begin{algorithm}[H] 
\caption{\algoNameFull (\algoName)}
\label{alg: main algo}
\hspace*{\algorithmicindent} \textbf{Input:} 
The training data set, ratio function $g$, norm type $p$, clean loss strength $\lambda_c$, number of epochs $T$ and number of batches $M$. $\mathcal{A}(x,y)$ denotes the approximate closest boundary point returned by an algorithm $\mathcal{A}$ (e.g. FAB) on the correctly classified data point $(x,y)$.  \\
\hspace*{\algorithmicindent} \textbf{Output:} adversarially robust network $f_\theta$
\begin{algorithmic}[1]
\For{epoch = $1,\cdots,T$}
    \For{mini-batch = $1,\cdots,M$}
        \State Sample a mini-batch $\mathcal{B} = \{(x_i,y_i\}_{i=1}^{n}$
        \State Make predictions on $\mathcal{B}$ and find correctly classified points $\mathcal{B}_{\theta}^{+}$
        \For{$(x_i,y_i)\in \mathcal{B}_{\theta}^{+}$ (in parallel)}
            \State Find the approximate closest boundary point $\hat{x}_i = \mathcal{A}(x_i,y_i)$ as in \eqref{eq: closest_pt}
            \State Compute the robust radius $R(x_i) = \|\hat{x}_i - x_i\|_p$
            \State Calculate the ratio value $g(R(x_i))$
        \EndFor
        \State Solve the optimization problem \eqref{eq:opt_for_weight} for weights $c_i$ for $i \in \mathcal{B}_{\theta}^{+}$ 
        \State Update $\theta$ using the loss function \eqref{eq: weighted loss general}
        % $\theta \gets \theta - \eta(\sum_{i\in B_1^{\text{adv}}}c_i\nabla_\theta l(\hat{x}_i,y_i)  + \lambda_c\sum_{i\in B}\frac{1}{N}\nabla_\theta l(x_i,y_i))$
    \EndFor
\EndFor

% \Function{ComputeWeight}{$x,y$} \Comment{{\small{return the summation of two variables}}}
%   \State $z = x + y$
%   \State \textbf{Return} $z$ 
% \EndFunction
\end{algorithmic}
\end{algorithm}

\vspace{-1em}
\end{figure}


==> experiment_fig/Our_batch_hist.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 100}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0930522158741951) rectangle (axis cs:0.130964314592326,0.0101324841380119);
\draw[draw=none,fill=color0] (axis cs:0,0.0101324841380119) rectangle (axis cs:0.523857258369306,0.113317184150219);
\draw[draw=none,fill=color0] (axis cs:0,0.1133171916008) rectangle (axis cs:0.654821525679423,0.216501891613007);
\draw[draw=none,fill=color0] (axis cs:0,0.216501891613007) rectangle (axis cs:0.785785887553959,0.319686591625214);
\draw[draw=none,fill=color0] (axis cs:0,0.319686591625214) rectangle (axis cs:1.83350040429257,0.422871291637421);
\draw[draw=none,fill=color0] (axis cs:0,0.422871291637421) rectangle (axis cs:1.44060746051559,0.526055991649628);
\draw[draw=none,fill=color0] (axis cs:0,0.526055991649628) rectangle (axis cs:0.654821572961632,0.629240691661835);
\draw[draw=none,fill=color0] (axis cs:0,0.629240691661835) rectangle (axis cs:1.17867883133094,0.732425391674042);
\draw[draw=none,fill=color0] (axis cs:0,0.732425391674042) rectangle (axis cs:1.30964314592326,0.835610091686249);
\draw[draw=none,fill=color0] (axis cs:0,0.835610091686249) rectangle (axis cs:1.17867883133094,0.938794791698456);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 500}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0894175097346306) rectangle (axis cs:0.325926569166786,0.0128550156950951);
\draw[draw=none,fill=color0] (axis cs:0,0.0128550156950951) rectangle (axis cs:0.325926569166786,0.115127541124821);
\draw[draw=none,fill=color0] (axis cs:0,0.11512752622366) rectangle (axis cs:1.19506408694488,0.217400044202805);
\draw[draw=none,fill=color0] (axis cs:0,0.217400074005127) rectangle (axis cs:1.52099065611167,0.319672584533691);
\draw[draw=none,fill=color0] (axis cs:0,0.319672584533691) rectangle (axis cs:2.49877072768424,0.421945095062256);
\draw[draw=none,fill=color0] (axis cs:0,0.421945095062256) rectangle (axis cs:1.73827528882382,0.52421760559082);
\draw[draw=none,fill=color0] (axis cs:0,0.52421760559082) rectangle (axis cs:1.08642205551489,0.626490116119385);
\draw[draw=none,fill=color0] (axis cs:0,0.626490116119385) rectangle (axis cs:0.760494995642261,0.728762686252594);
\draw[draw=none,fill=color0] (axis cs:0,0.728762686252594) rectangle (axis cs:0.108642205551489,0.831035196781158);
\draw[draw=none,fill=color0] (axis cs:0,0.831035196781158) rectangle (axis cs:0.217284411102978,0.933307707309723);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 1000}},
xmin=0, xmax=1,
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
xtick=\empty
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0245624426752329) rectangle (axis cs:0.373517160888316,0.0699288472533226);
\draw[draw=none,fill=color0] (axis cs:0,0.069928839802742) rectangle (axis cs:0.87153997335234,0.164420127868652);
\draw[draw=none,fill=color0] (axis cs:0,0.164420127868652) rectangle (axis cs:1.24505720296105,0.258911430835724);
\draw[draw=none,fill=color0] (axis cs:0,0.258911430835724) rectangle (axis cs:1.6185741086022,0.353402733802795);
\draw[draw=none,fill=color0] (axis cs:0,0.353402733802795) rectangle (axis cs:1.12055130595537,0.447894036769867);
\draw[draw=none,fill=color0] (axis cs:0,0.447894036769867) rectangle (axis cs:1.49406840794049,0.542385339736938);
\draw[draw=none,fill=color0] (axis cs:0,0.542385339736938) rectangle (axis cs:1.86758668799003,0.636876583099365);
\draw[draw=none,fill=color0] (axis cs:0,0.636876583099365) rectangle (axis cs:0.747034203970246,0.731367886066437);
\draw[draw=none,fill=color0] (axis cs:0,0.731367945671082) rectangle (axis cs:0.622528503308539,0.825859248638153);
\draw[draw=none,fill=color0] (axis cs:0,0.825859189033508) rectangle (axis cs:0.622528503308539,0.92035049200058);
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\end{groupplot}

\draw ({$(current bounding box.south west)!-0.01!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\LARGE{Speed}};
\end{tikzpicture}


==> experiment_fig/Our_batch_scatter.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 100}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.139259457588196 0.87974089384079
0.421387225389481 0.505936861038208
0.497758567333221 0.281495809555054
0.192086070775986 0.694953858852386
0.976208627223969 0.0887730941176414
0.553409993648529 0.440094947814941
0.439580053091049 0.442619472742081
0.968777179718018 0.246498510241508
0.879478633403778 0.321859002113342
0.927507281303406 0.132060289382935
0.725531160831451 0.677463829517365
0.250144422054291 0.624903559684753
0.282028943300247 0.938794791698456
0.392061352729797 0.590279817581177
0.226367816329002 0.709937810897827
0.253683537244797 0.509217083454132
0.264158725738525 0.527510821819305
0.143192574381828 0.847660481929779
0.0656776130199432 0.856230556964874
0.512509167194366 0.468835383653641
0.452651411294937 0.452691107988358
0.96679413318634 -0.0930522158741951
0.457594335079193 0.362852275371552
0.818558394908905 0.210012018680573
0.0865476429462433 0.760084748268127
0.92186176776886 0.419143319129944
0.229736253619194 0.822469353675842
0.454779326915741 0.55412769317627
0.569496870040894 0.675950586795807
0.605530679225922 0.753823578357697
0.756329953670502 0.356041789054871
0.449440777301788 0.525765717029572
0.401755213737488 0.489267826080322
0.729974925518036 0.641091227531433
0.864565491676331 0.158966660499573
0.569140493869781 0.492613941431046
0.195144489407539 0.906790733337402
0.607923448085785 0.39532533288002
0.704999208450317 0.15942719578743
0.83390611410141 0.280181169509888
0.655198633670807 0.403607189655304
0.58749520778656 0.285376042127609
0.645855844020844 0.349601417779922
0.147765323519707 0.784916758537292
0.640424787998199 0.415896952152252
0.516849458217621 0.365468591451645
0.552274227142334 0.3888900578022
0.628182530403137 0.356706947088242
0.450512319803238 0.634923756122589
0.660074591636658 0.393710017204285
0.116237349808216 0.841611802577972
0.560958743095398 0.501353740692139
0.950110077857971 0.0379549711942673
0.189407855272293 0.777242183685303
0.17595100402832 0.903630018234253
0.808530151844025 0.284991264343262
0.142146334052086 0.782856583595276
0.755055904388428 0.250042021274567
0.383216202259064 0.92495208978653
0.0799809321761131 0.819203019142151
0.261886149644852 0.78420078754425
0.554071724414825 0.41170459985733
0.932360053062439 0.0142253050580621
0.0659285113215446 0.894612729549408
0.150298565626144 0.690214574337006
0.263341963291168 0.644734263420105
0.123858392238617 0.710014164447784
0.447123974561691 0.581269323825836
0.839296758174896 0.0896879211068153
0.46270939707756 0.211884632706642
0.185274988412857 0.767150223255157
0.398056268692017 0.772571265697479
0.542429447174072 0.403975188732147
0.61186957359314 0.46583878993988
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 500}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.776936888694763 0.249753534793854
0.386116743087769 0.406365096569061
0.174472793936729 0.521653413772583
0.805141091346741 0.933307707309723
0.440240800380707 0.551619172096252
0.591361165046692 0.133534938097
0.455250889062881 0.401996105909348
0.332143425941467 0.372915893793106
0.467637568712234 0.814061284065247
0.724299252033234 0.130848690867424
0.158043280243874 0.647002637386322
0.566194474697113 0.347332745790482
0.473153501749039 0.482004195451736
0.267547637224197 0.527089238166809
0.71589583158493 0.430038511753082
0.658745765686035 0.457427114248276
0.144467324018478 0.657042145729065
0.422516047954559 0.367061853408813
0.78759354352951 0.379683077335358
0.370047807693481 0.349326610565186
0.131544753909111 0.42074191570282
0.590262830257416 0.158686131238937
0.888246536254883 0.231273204088211
0.985404491424561 0.173878386616707
0.404500156641006 0.519400238990784
0.335165202617645 0.72149384021759
0.23070877790451 0.558023869991302
0.436972916126251 0.331318795681
0.644021034240723 0.0856519564986229
0.630360901355743 0.435541301965714
0.447283953428268 0.239694103598595
0.180275335907936 0.505020081996918
0.510656476020813 0.335002541542053
0.405353397130966 0.287605851888657
0.464257538318634 0.453973650932312
0.303507149219513 0.453528463840485
0.311053872108459 0.504680037498474
0.690726935863495 0.261621564626694
0.170168474316597 0.674301147460938
0.388627707958221 0.569280743598938
0.561706483364105 0.616437673568726
0.448287129402161 0.329984992742538
0.162112429738045 0.625538289546967
0.247905418276787 0.34765100479126
0.495826065540314 0.558913290500641
0.703568994998932 0.673902451992035
0.25944322347641 0.407854646444321
0.677498459815979 0.390358507633209
0.402255445718765 0.240773573517799
0.329665958881378 0.497239798307419
0.689209342002869 0.216121166944504
0.936314046382904 0.426470637321472
0.0554389469325542 0.885870456695557
0.63409698009491 0.330398440361023
0.935300230979919 0.17045946419239
0.35245755314827 0.348024547100067
0.23744623363018 0.559127688407898
0.323607683181763 0.559788584709167
0.0888271629810333 0.495435357093811
0.127962559461594 0.374380618333817
0.468316853046417 0.234871447086334
0.158229857683182 0.637133896350861
0.716919124126434 0.129116103053093
0.144968807697296 0.523131608963013
0.849043250083923 0.0959296450018883
0.975417494773865 0.011977213434875
0.0905567705631256 0.728091776371002
0.403979033231735 0.260361164808273
0.202995106577873 0.577884078025818
0.182661727070808 0.340855956077576
0.98902815580368 0.225347593426704
0.693903625011444 0.238435164093971
0.587247252464294 0.324716359376907
0.190335050225258 0.475275486707687
0.786740481853485 0.152153328061104
0.426211625337601 0.371549278497696
0.177270129323006 0.292735397815704
0.736927688121796 0.246110171079636
0.446727216243744 0.363649725914001
0.449692755937576 0.485296905040741
0.345438122749329 0.340099722146988
0.8830726146698 0.00464663049206138
0.56570303440094 0.28088241815567
0.805004954338074 0.189938649535179
0.262816816568375 0.33413490653038
0.717803835868835 0.107261158525944
0.864565908908844 0.293800443410873
0.878847897052765 -0.0894175097346306
0.606184422969818 0.199088245630264
0.59554123878479 0.170070052146912
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={\Large{iter: 1000}},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.5,1},
xticklabels={0,0.5,1},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,0,1},
yticklabels={-1,0,1},
axis lines=left
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.57584023475647 0.338832080364227
0.225332260131836 0.623566269874573
0.968862056732178 0.346817523241043
0.311254441738129 0.513589560985565
0.568746745586395 0.515619337558746
0.366963326931 0.513030588626862
0.41833233833313 0.463166058063507
0.556143522262573 0.361476302146912
0.529341161251068 0.54360020160675
0.205069601535797 0.647709488868713
0.908150136470795 0.0687245801091194
0.710321962833405 0.378976941108704
0.898783683776855 0.167049989104271
0.161436930298805 0.74740469455719
0.479314923286438 0.819670855998993
0.0888834595680237 0.627499997615814
0.309117376804352 0.631774067878723
0.302228063344955 0.392113834619522
0.614017605781555 0.154380187392235
0.695720970630646 0.465875148773193
0.75020694732666 0.134846374392509
0.874695301055908 0.0960765555500984
0.498199701309204 0.408374339342117
0.710412740707397 0.193369522690773
0.336726933717728 0.338454991579056
0.538124024868011 0.0865073874592781
0.0881228446960449 0.633062362670898
0.771107912063599 0.309533357620239
0.369485050439835 0.374647527933121
0.319801241159439 0.614099442958832
0.744711935520172 0.0975610539317131
0.19185908138752 0.430443435907364
0.269707530736923 0.774192214012146
0.131259053945541 0.855269432067871
0.491700023412704 0.629065930843353
0.671019077301025 0.30482617020607
0.420025080442429 0.478932470083237
0.585492372512817 0.299596399068832
0.361166208982468 0.542346000671387
0.859290421009064 0.120165780186653
0.346621990203857 0.14356492459774
0.131627649068832 0.92035049200058
0.115172833204269 0.535668432712555
0.199532762169838 0.629831790924072
0.200127780437469 0.605798184871674
0.589739680290222 0.321029216051102
0.73112541437149 0.253543674945831
0.598318040370941 0.211257830262184
0.280894696712494 0.91473114490509
0.713802218437195 0.280924409627914
0.347708225250244 0.593869745731354
0.965838074684143 0.537938714027405
0.383636444807053 0.447239965200424
0.935863971710205 0.203516334295273
0.14890643954277 0.680480480194092
0.0562681667506695 0.802294194698334
0.749043345451355 0.179575711488724
0.423711746931076 0.486505329608917
0.844658136367798 0.166071742773056
0.661024570465088 0.563995838165283
0.54025536775589 0.434267282485962
0.565700888633728 0.227442294359207
0.520568788051605 0.592914402484894
0.131979018449783 0.673773288726807
0.876122951507568 0.00479763699695468
0.535711050033569 0.318562299013138
0.345073401927948 0.585593223571777
0.226624682545662 0.70534759759903
0.560894787311554 0.332505911588669
0.278737008571625 0.508535087108612
0.486066699028015 0.266474425792694
0.970355808734894 -0.0245624426752329
0.276687234640121 0.543783009052277
0.643745064735413 0.479749530553818
0.661679565906525 0.178459644317627
0.28415521979332 0.55865490436554
0.292061328887939 0.422659397125244
0.562201738357544 0.833523273468018
0.294146001338959 0.838525772094727
0.0868585333228111 0.749682188034058
0.510356962680817 0.273927867412567
0.669389963150024 0.297383904457092
0.678594410419464 0.222954750061035
0.17401809990406 0.670224070549011
0.25044584274292 0.683681547641754
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [line width=3pt, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!-0.02!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=0.0
]{\LARGE{Radius}};
\draw ({$(current bounding box.south west)!-0.01!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.75,
  text=black,
  rotate=90.0
]{\LARGE{Speed}};
\end{tikzpicture}


==> experiment_fig/old_figs/VR_Our_batch.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 1000},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.968902170658112 0.471921056509018
0.265831738710403 0.761655151844025
0.207096517086029 0.865517735481262
0.978850305080414 0.464377641677856
0.579137623310089 0.716730833053589
0.170609176158905 0.907945692539215
0.57406884431839 0.489615648984909
0.704443216323853 0.661161541938782
0.880915462970734 0.436875522136688
0.617282450199127 0.701224386692047
0.491142302751541 0.756028711795807
0.679420709609985 0.845314860343933
0.552240133285522 0.776899993419647
0.317299515008926 0.768919587135315
0.872411787509918 0.43258860707283
0.840914011001587 0.56850802898407
0.150133773684502 0.969549119472504
0.417496234178543 0.6882404088974
0.521487653255463 0.450512498617172
0.55248236656189 0.96494323015213
0.866532981395721 0.461429923772812
0.493246614933014 0.638788878917694
0.932202696800232 0.524523794651031
0.398445904254913 0.659211575984955
0.698145747184753 0.442851215600967
0.908521592617035 0.679588794708252
0.554396629333496 0.671484231948853
0.365486174821854 0.743131697177887
0.939813911914825 0.441165775060654
0.484436184167862 0.807662844657898
0.506584823131561 0.78305721282959
0.557701885700226 0.730745613574982
0.837874174118042 0.468014597892761
0.57797384262085 0.697672724723816
0.875149309635162 0.416225016117096
0.325212061405182 0.8119056224823
0.10592208057642 0.797015309333801
0.932617425918579 0.568060576915741
0.38191169500351 0.771024644374847
0.504081308841705 0.741605877876282
0.550743997097015 0.704563617706299
0.350751787424088 0.808251321315765
0.507640957832336 0.744328796863556
0.982051849365234 0.325904458761215
0.765538573265076 0.640039205551147
0.575354278087616 0.732706546783447
0.185031935572624 0.850288033485413
0.367810308933258 0.823543071746826
0.980478703975677 0.601333975791931
0.218625828623772 0.749875605106354
0.503026366233826 0.769070088863373
0.221693009138107 0.853348791599274
0.785702705383301 0.6805619597435
0.94809478521347 0.570730984210968
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 2000},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.686285018920898 0.42705625295639
0.0615661516785622 0.563854992389679
0.241954311728477 0.485845685005188
0.416544258594513 0.307454526424408
0.337028115987778 0.414351254701614
0.405839025974274 0.556506514549255
0.170722767710686 0.477037459611893
0.785026609897614 0.320982336997986
0.268998771905899 0.791122674942017
0.60291451215744 0.414353340864182
0.629599928855896 0.46928808093071
0.46087583899498 0.334945797920227
0.852693200111389 0.276088446378708
0.61442619562149 0.521552324295044
0.946889638900757 0.296243607997894
0.474078714847565 0.4337018430233
0.518937230110168 0.43837833404541
0.274294465780258 0.460310071706772
0.825393438339233 0.237894043326378
0.238793015480042 0.376264750957489
0.726541638374329 0.317493408918381
0.259722948074341 0.380860209465027
0.786027729511261 0.281686186790466
0.87212336063385 0.332919865846634
0.788526594638824 0.35707214474678
0.660025298595428 0.502157211303711
0.319070100784302 0.489344090223312
0.553589999675751 0.276347160339355
0.320250242948532 0.126843005418777
0.882053792476654 -0.0105694215744734
0.789165318012238 0.411822021007538
0.580239832401276 0.402895331382751
0.988625168800354 0.288963139057159
0.636602818965912 0.380388557910919
0.105431295931339 0.531212151050568
0.522475838661194 0.477761715650558
0.316566497087479 0.422446072101593
0.714325428009033 0.344346612691879
0.252095103263855 0.357361972332001
0.213565915822983 0.485814124345779
0.171012192964554 0.531851768493652
0.980316698551178 0.236534103751183
0.237607881426811 0.437606751918793
0.972442090511322 0.176817253232002
0.437472820281982 0.26302433013916
0.226046726107597 0.549436748027802
0.817433059215546 0.33748596906662
0.979077160358429 0.271529704332352
0.137930765748024 0.249359503388405
0.284113973379135 0.554310739040375
0.664010286331177 0.356822699308395
0.59231048822403 0.285280883312225
0.478119522333145 0.331890642642975
0.132800444960594 0.327489763498306
0.233926087617874 0.561864495277405
0.299452006816864 0.439720928668976
0.484994649887085 0.382210314273834
0.913117229938507 0.21067550778389
0.30350336432457 0.488638699054718
0.647739708423615 0.246691137552261
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 5000},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.234617620706558 0.500277936458588
0.211388573050499 0.566922128200531
0.32329535484314 0.562682032585144
0.216600358486176 0.61413711309433
0.714290618896484 0.431059122085571
0.476620048284531 0.48390394449234
0.633130371570587 0.457955777645111
0.387982189655304 0.666635096073151
0.513616561889648 0.651579678058624
0.744789242744446 0.480239599943161
0.926783263683319 0.442411839962006
0.38214510679245 0.643455624580383
0.609603524208069 0.62471866607666
0.845026135444641 0.490298002958298
0.386313319206238 0.535261571407318
0.320195615291595 0.689014315605164
0.81830632686615 0.434413462877274
0.381827533245087 0.303626865148544
0.89215487241745 0.226100206375122
0.601888239383698 0.635784327983856
0.621108412742615 0.518928289413452
0.718669414520264 0.632552683353424
0.650688230991364 0.743343532085419
0.781298160552979 0.417314797639847
0.0565415881574154 0.788086831569672
0.406360596418381 0.534204483032227
0.320979058742523 0.594069719314575
0.723450899124146 0.482482552528381
0.518937468528748 0.555695235729218
0.497240841388702 0.532648384571075
0.507625579833984 0.617978751659393
0.538388192653656 0.561995804309845
0.212709382176399 0.670163035392761
0.633820354938507 0.546750664710999
0.951570153236389 0.36523112654686
0.987678110599518 0.254214704036713
0.220633953809738 0.989354908466339
0.423308581113815 0.712631344795227
0.582043468952179 0.564983487129211
0.74614417552948 0.600103259086609
0.235945135354996 0.695272207260132
0.792845666408539 0.426515579223633
0.53634375333786 0.707691550254822
0.509329915046692 0.498223304748535
0.168549031019211 0.775674104690552
0.239719346165657 0.681831836700439
0.706962049007416 0.545371115207672
0.907131731510162 0.566266536712646
0.739783525466919 0.535915434360504
0.851179122924805 0.304119616746902
0.480980515480042 0.261775821447372
0.989102005958557 0.207495719194412
0.179618388414383 0.709552645683289
0.601204335689545 0.602224946022034
0.665476322174072 0.537301540374756
0.615343868732452 0.526150345802307
0.944430112838745 0.275361329317093
0.681396424770355 0.223040446639061
0.18194206058979 0.812609136104584
0.721267461776733 0.496574223041534
0.281321316957474 0.655366718769073
0.85386711359024 0.453131973743439
0.143009722232819 0.436275839805603
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.01!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=south,
  text=black,
  rotate=0.0
]{Radius};
\draw ({$(current bounding box.south west)!0.02!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=west,
  text=black,
  rotate=90.0
]{Speed};
\end{tikzpicture}


==> experiment_fig/old_figs/VR_ours_batch_w_hist.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{groupplot}[group style={group size=6 by 1}]
\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 100},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.25,0.5,0.75,1},
xticklabels={0.0,0.5,1.0,,},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.704999208450317 0.15942719578743
0.392061352729797 0.590279817581177
0.497758567333221 0.281495809555054
0.605530679225922 0.753823578357697
0.554071724414825 0.41170459985733
0.142146334052086 0.782856583595276
0.755055904388428 0.250042021274567
0.192086070775986 0.694953858852386
0.452651411294937 0.452691107988358
0.968777179718018 0.246498510241508
0.282028943300247 0.938794791698456
0.808530151844025 0.284991264343262
0.0656776130199432 0.856230556964874
0.553409993648529 0.440094947814941
0.645855844020844 0.349601417779922
0.569140493869781 0.492613941431046
0.143192574381828 0.847660481929779
0.150298565626144 0.690214574337006
0.398056268692017 0.772571265697479
0.607923448085785 0.39532533288002
0.147765323519707 0.784916758537292
0.17595100402832 0.903630018234253
0.449440777301788 0.525765717029572
0.447123974561691 0.581269323825836
0.552274227142334 0.3888900578022
0.439580053091049 0.442619472742081
0.729974925518036 0.641091227531433
0.932360053062439 0.0142253050580621
0.116237349808216 0.841611802577972
0.250144422054291 0.624903559684753
0.261886149644852 0.78420078754425
0.96679413318634 -0.0930522158741951
0.560958743095398 0.501353740692139
0.253683537244797 0.509217083454132
0.457594335079193 0.362852275371552
0.401755213737488 0.489267826080322
0.0659285113215446 0.894612729549408
0.660074591636658 0.393710017204285
0.628182530403137 0.356706947088242
0.640424787998199 0.415896952152252
0.569496870040894 0.675950586795807
0.383216202259064 0.92495208978653
0.756329953670502 0.356041789054871
0.818558394908905 0.210012018680573
0.61186957359314 0.46583878993988
0.264158725738525 0.527510821819305
0.655198633670807 0.403607189655304
0.450512319803238 0.634923756122589
0.195144489407539 0.906790733337402
0.879478633403778 0.321859002113342
0.0865476429462433 0.760084748268127
0.83390611410141 0.280181169509888
0.0799809321761131 0.819203019142151
0.516849458217621 0.365468591451645
0.229736253619194 0.822469353675842
0.950110077857971 0.0379549711942673
0.226367816329002 0.709937810897827
0.976208627223969 0.0887730941176414
0.927507281303406 0.132060289382935
0.542429447174072 0.403975188732147
0.185274988412857 0.767150223255157
0.421387225389481 0.505936861038208
0.58749520778656 0.285376042127609
0.46270939707756 0.211884632706642
0.139259457588196 0.87974089384079
0.839296758174896 0.0896879211068153
0.454779326915741 0.55412769317627
0.263341963291168 0.644734263420105
0.864565491676331 0.158966660499573
0.189407855272293 0.777242183685303
0.725531160831451 0.677463829517365
0.512509167194366 0.468835383653641
0.92186176776886 0.419143319129944
0.123858392238617 0.710014164447784
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 500},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.25,0.5,0.75,1},
xticklabels={0.0,0.5,1.0,,},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.25944322347641 0.407854646444321
0.590262830257416 0.158686131238937
0.464257538318634 0.453973650932312
0.561706483364105 0.616437673568726
0.332143425941467 0.372915893793106
0.591361165046692 0.133534938097
0.247905418276787 0.34765100479126
0.716919124126434 0.129116103053093
0.0554389469325542 0.885870456695557
0.677498459815979 0.390358507633209
0.144968807697296 0.523131608963013
0.690726935863495 0.261621564626694
0.59554123878479 0.170070052146912
0.644021034240723 0.0856519564986229
0.495826065540314 0.558913290500641
0.805004954338074 0.189938649535179
0.436972916126251 0.331318795681
0.473153501749039 0.482004195451736
0.849043250083923 0.0959296450018883
0.724299252033234 0.130848690867424
0.426211625337601 0.371549278497696
0.162112429738045 0.625538289546967
0.693903625011444 0.238435164093971
0.180275335907936 0.505020081996918
0.63409698009491 0.330398440361023
0.888246536254883 0.231273204088211
0.566194474697113 0.347332745790482
0.776936888694763 0.249753534793854
0.311053872108459 0.504680037498474
0.177270129323006 0.292735397815704
0.0888271629810333 0.495435357093811
0.786740481853485 0.152153328061104
0.455250889062881 0.401996105909348
0.703568994998932 0.673902451992035
0.587247252464294 0.324716359376907
0.404500156641006 0.519400238990784
0.144467324018478 0.657042145729065
0.448287129402161 0.329984992742538
0.170168474316597 0.674301147460938
0.805141091346741 0.933307707309723
0.388627707958221 0.569280743598938
0.446727216243744 0.363649725914001
0.127962559461594 0.374380618333817
0.935300230979919 0.17045946419239
0.864565908908844 0.293800443410873
0.985404491424561 0.173878386616707
0.0905567705631256 0.728091776371002
0.35245755314827 0.348024547100067
0.23070877790451 0.558023869991302
0.174472793936729 0.521653413772583
0.936314046382904 0.426470637321472
0.386116743087769 0.406365096569061
0.303507149219513 0.453528463840485
0.158229857683182 0.637133896350861
0.467637568712234 0.814061284065247
0.262816816568375 0.33413490653038
0.405353397130966 0.287605851888657
0.8830726146698 0.00464663049206138
0.449692755937576 0.485296905040741
0.370047807693481 0.349326610565186
0.630360901355743 0.435541301965714
0.717803835868835 0.107261158525944
0.335165202617645 0.72149384021759
0.658745765686035 0.457427114248276
0.975417494773865 0.011977213434875
0.510656476020813 0.335002541542053
0.689209342002869 0.216121166944504
0.202995106577873 0.577884078025818
0.403979033231735 0.260361164808273
0.606184422969818 0.199088245630264
0.440240800380707 0.551619172096252
0.323607683181763 0.559788584709167
0.98902815580368 0.225347593426704
0.267547637224197 0.527089238166809
0.23744623363018 0.559127688407898
0.447283953428268 0.239694103598595
0.736927688121796 0.246110171079636
0.78759354352951 0.379683077335358
0.468316853046417 0.234871447086334
0.158043280243874 0.647002637386322
0.402255445718765 0.240773573517799
0.878847897052765 -0.0894175097346306
0.56570303440094 0.28088241815567
0.71589583158493 0.430038511753082
0.131544753909111 0.42074191570282
0.329665958881378 0.497239798307419
0.345438122749329 0.340099722146988
0.190335050225258 0.475275486707687
0.422516047954559 0.367061853408813
0.182661727070808 0.340855956077576
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 3000},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.25,0.5,0.75,1},
xticklabels={0.0,0.5,1.0,,},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\addplot [draw=color0, fill=color0, mark=*, only marks]
table{%
x  y
0.0817365944385529 0.867674112319946
0.533936858177185 0.428688377141953
0.294490247964859 0.575457692146301
0.191696301102638 0.705106377601624
0.777195274829865 0.169598773121834
0.951595187187195 0.180614769458771
0.493152648210526 0.415251791477203
0.570287942886353 0.159825593233109
0.423713564872742 0.543446719646454
0.814855873584747 0.165298193693161
0.576456725597382 0.315379619598389
0.888468503952026 0.191853851079941
0.653435111045837 0.22555860877037
0.122432962059975 0.745577096939087
0.356743931770325 0.538100600242615
0.569653213024139 0.303878575563431
0.569445431232452 0.532717764377594
0.969858348369598 0.09162487834692
0.919908165931702 0.288053721189499
0.983428478240967 0.0386368110775948
0.226993948221207 0.534350633621216
0.46128648519516 0.483001679182053
0.812167346477509 0.184243068099022
0.113914214074612 0.90733814239502
0.983700454235077 0.422286838293076
0.43880707025528 0.309785306453705
0.543598413467407 0.277403861284256
0.47244855761528 0.491245210170746
0.650085866451263 0.41348671913147
0.371362298727036 0.479745149612427
0.585280239582062 0.352438002824783
0.26160055398941 0.465487897396088
0.182527959346771 0.570489048957825
0.327341109514236 0.489190250635147
0.935183882713318 0.0496866852045059
0.0773639604449272 0.684758722782135
0.479597151279449 0.567265033721924
0.785211443901062 0.0549652948975563
0.336012244224548 0.656233727931976
0.577840745449066 0.443245053291321
0.114977948367596 0.682622849941254
0.686502456665039 0.522340059280396
0.312052130699158 0.629898965358734
0.718758106231689 0.232464984059334
0.875719726085663 0.25407412648201
0.114390224218369 0.785102546215057
0.0545082986354828 0.944594740867615
0.0705606415867805 0.715467631816864
0.530273199081421 0.321661382913589
0.584746181964874 0.347295641899109
0.280913412570953 0.600384593009949
0.197391241788864 0.644949316978455
0.236994490027428 0.378778517246246
0.798084557056427 0.0915812030434608
0.510002255439758 0.372925519943237
0.374745756387711 0.395561009645462
0.136563122272491 0.457673341035843
0.580816686153412 0.495245665311813
0.506234109401703 0.454161554574966
0.277639627456665 0.596580028533936
0.324215263128281 0.527666866779327
0.492877215147018 0.285518914461136
0.691874027252197 0.394520133733749
0.078777588903904 0.774883270263672
0.127409636974335 0.711575865745544
0.633400738239288 0.409918874502182
0.0751356109976768 0.347895860671997
0.98067718744278 0.306284248828888
0.729027152061462 0.274086356163025
0.543085038661957 0.513598680496216
0.417235404253006 0.241217479109764
0.594324052333832 0.424429804086685
0.792836129665375 0.350332170724869
0.15471775829792 0.680841088294983
0.533702552318573 0.349337220191956
0.415899455547333 0.594696164131165
0.469830065965652 0.533640563488007
0.928201973438263 0.21082828938961
0.12568923830986 0.669020712375641
0.617589056491852 0.478675007820129
0.54864114522934 0.280780762434006
0.185902744531631 0.715623736381531
0.793601274490356 0.185111552476883
0.464082300662994 0.312457919120789
};
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
1 2.22044604925031e-16
};
\addplot [semithick, red, opacity=0.4]
table {%
0.5 -1
0.5 1
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 100},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=14.7,
xtick style={color=black},
xtick={0,5,10,15},
xticklabels={0.0,0.5,1.0,},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0930522158741951) rectangle (axis cs:1,0.0101324841380119);
\draw[draw=none,fill=color0] (axis cs:0,0.0101324841380119) rectangle (axis cs:4,0.113317184150219);
\draw[draw=none,fill=color0] (axis cs:0,0.1133171916008) rectangle (axis cs:5,0.216501891613007);
\draw[draw=none,fill=color0] (axis cs:0,0.216501891613007) rectangle (axis cs:6,0.319686591625214);
\draw[draw=none,fill=color0] (axis cs:0,0.319686591625214) rectangle (axis cs:14,0.422871291637421);
\draw[draw=none,fill=color0] (axis cs:0,0.422871291637421) rectangle (axis cs:11,0.526055991649628);
\draw[draw=none,fill=color0] (axis cs:0,0.526055991649628) rectangle (axis cs:5,0.629240691661835);
\draw[draw=none,fill=color0] (axis cs:0,0.629240691661835) rectangle (axis cs:9,0.732425391674042);
\draw[draw=none,fill=color0] (axis cs:0,0.732425391674042) rectangle (axis cs:10,0.835610091686249);
\draw[draw=none,fill=color0] (axis cs:0,0.835610091686249) rectangle (axis cs:9,0.938794791698456);
\addplot [semithick, red, opacity=0.4]
table {%
7.105427357601e-15 2.22044604925031e-16
14.7 2.22044604925031e-16
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 500},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=24.15,
xtick style={color=black},
xtick={0,10,20,30},
xticklabels={0.0,0.5,1.0,},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\draw[draw=none,fill=color0] (axis cs:0,-0.0894175097346306) rectangle (axis cs:3,0.0128550156950951);
\draw[draw=none,fill=color0] (axis cs:0,0.0128550156950951) rectangle (axis cs:3,0.115127541124821);
\draw[draw=none,fill=color0] (axis cs:0,0.11512752622366) rectangle (axis cs:11,0.217400044202805);
\draw[draw=none,fill=color0] (axis cs:0,0.217400074005127) rectangle (axis cs:14,0.319672584533691);
\draw[draw=none,fill=color0] (axis cs:0,0.319672584533691) rectangle (axis cs:23,0.421945095062256);
\draw[draw=none,fill=color0] (axis cs:0,0.421945095062256) rectangle (axis cs:16,0.52421760559082);
\draw[draw=none,fill=color0] (axis cs:0,0.52421760559082) rectangle (axis cs:10,0.626490116119385);
\draw[draw=none,fill=color0] (axis cs:0,0.626490116119385) rectangle (axis cs:7,0.728762686252594);
\draw[draw=none,fill=color0] (axis cs:0,0.728762686252594) rectangle (axis cs:1,0.831035196781158);
\draw[draw=none,fill=color0] (axis cs:0,0.831035196781158) rectangle (axis cs:2,0.933307707309723);
\addplot [semithick, red, opacity=0.4]
table {%
2.8421709430404e-14 2.22044604925031e-16
24.15 2.22044604925031e-16
};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={iter: 3000},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=15.75,
xtick style={color=black},
xtick={0,5,10,15,20},
xticklabels={0.0,0.5,1.0,,},
y grid style={white!69.0196078431373!black},
ymin=-1, ymax=1,
ytick style={color=black},
ytick={-1,-0.75,-0.5,-0.25,0,0.25,0.5,0.75,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0,,,}
]
\draw[draw=none,fill=color0] (axis cs:0,0.0386368110775948) rectangle (axis cs:5,0.129232615232468);
\draw[draw=none,fill=color0] (axis cs:0,0.129232615232468) rectangle (axis cs:8,0.21982841193676);
\draw[draw=none,fill=color0] (axis cs:0,0.219828397035599) rectangle (axis cs:12,0.31042417883873);
\draw[draw=none,fill=color0] (axis cs:0,0.310424149036407) rectangle (axis cs:12,0.401019960641861);
\draw[draw=none,fill=color0] (axis cs:0,0.401019990444183) rectangle (axis cs:15,0.491615772247314);
\draw[draw=none,fill=color0] (axis cs:0,0.491615742444992) rectangle (axis cs:12,0.582211494445801);
\draw[draw=none,fill=color0] (axis cs:0,0.58221161365509) rectangle (axis cs:7,0.672807395458221);
\draw[draw=none,fill=color0] (axis cs:0,0.672807335853577) rectangle (axis cs:8,0.763403177261353);
\draw[draw=none,fill=color0] (axis cs:0,0.763403177261353) rectangle (axis cs:2,0.853998959064484);
\draw[draw=none,fill=color0] (axis cs:0,0.853999018669128) rectangle (axis cs:3,0.94459480047226);
\addplot [semithick, red, opacity=0.4]
table {%
0 2.22044604925031e-16
15.75 2.22044604925031e-16
};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.01!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=south,
  text=black,
  rotate=0.0
]{Radius};
\draw ({$(current bounding box.south west)!0.02!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.5!(current bounding box.north west)$}) node[
  scale=0.6,
  anchor=west,
  text=black,
  rotate=90.0
]{Speed};
\end{tikzpicture}


==> experiment_fig/radius_distribution.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, font=\large},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\Large{radius}},
xmin=0, xmax=5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=0.906499451926922,
ytick style={color=black}
]
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.00012119859457016,0) rectangle (axis cs:0.144508928060532,0.411766890524049);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.5}
\addlegendentry{k=1}

\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.14450891315937,0) rectangle (axis cs:0.28889662027359,0.545705991157668);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.28889662027359,0) rectangle (axis cs:0.433284342288971,0.678114247219903);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.433284342288971,0) rectangle (axis cs:0.577672064304352,0.792153776379909);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.577672064304352,0) rectangle (axis cs:0.722059786319733,0.848025492008637);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.722059786319733,0) rectangle (axis cs:0.866447508335114,0.863332811358974);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:0.866447448730469,0) rectangle (axis cs:1.01083517074585,0.80286923135731);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.01083517074585,0) rectangle (axis cs:1.15522289276123,0.677348881252386);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.15522289276123,0) rectangle (axis cs:1.29961061477661,0.492130317113316);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.29961061477661,0) rectangle (axis cs:1.44399833679199,0.347476149252637);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.44399833679199,0) rectangle (axis cs:1.58838605880737,0.222721496547395);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.58838605880737,0) rectangle (axis cs:1.73277378082275,0.114039529160006);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.73277378082275,0) rectangle (axis cs:1.87716150283813,0.0711790349790643);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:1.87716150283813,0) rectangle (axis cs:2.02154922485352,0.0336761025707401);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.02154922485352,0) rectangle (axis cs:2.1659369468689,0.0137765874153028);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.1659369468689,0) rectangle (axis cs:2.31032466888428,0.00612292774013456);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.31032466888428,0) rectangle (axis cs:2.45471239089966,0.00306146387006728);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.45471239089966,0) rectangle (axis cs:2.59910011291504,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.59910011291504,0) rectangle (axis cs:2.74348783493042,0.000765365967516821);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:2.74348783493042,0) rectangle (axis cs:2.8878755569458,0.00153073193503364);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.000629313290119171,0) rectangle (axis cs:0.20014876127243,0.432014092923934);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,fill opacity=0.5}
\addlegendentry{k=2}

\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.200148746371269,0) rectangle (axis cs:0.399668157100677,0.495429042647959);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.399668216705322,0) rectangle (axis cs:0.599187612533569,0.536761979920304);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.599187612533569,0) rectangle (axis cs:0.798707067966461,0.541291536028653);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.798707127571106,0) rectangle (axis cs:0.998226583003998,0.557711467560902);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.998226523399353,0) rectangle (axis cs:1.1977459192276,0.537894469506224);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.19774580001831,0) rectangle (axis cs:1.39726531505585,0.44616904075973);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.39726543426514,0) rectangle (axis cs:1.59678483009338,0.392946065091915);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.59678483009338,0) rectangle (axis cs:1.79630422592163,0.330097342865398);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.79630422592163,0) rectangle (axis cs:1.99582374095917,0.250828534335736);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:1.99582386016846,0) rectangle (axis cs:2.19534301757812,0.186847664203475);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.19534301757812,0) rectangle (axis cs:2.39486265182495,0.127962110361838);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.39486265182495,0) rectangle (axis cs:2.5943820476532,0.0883279339399694);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.59438228607178,0) rectangle (axis cs:2.79390168190002,0.037369510513064);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.79390144348145,0) rectangle (axis cs:2.99342083930969,0.0232143928944791);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:2.99342107772827,0) rectangle (axis cs:3.19294047355652,0.015853731732815);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.19294023513794,0) rectangle (axis cs:3.39245963096619,0.00566204704743393);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.39245963096619,0) rectangle (axis cs:3.59197926521301,0.00283102014074863);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.59197950363159,0) rectangle (axis cs:3.79149889945984,0.00169861411423018);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:3.79149866104126,0) rectangle (axis cs:3.99101805686951,0.00113240940948679);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.000650271773338318,0) rectangle (axis cs:0.263168036937714,0.371470997289431);
\addlegendimage{ybar,ybar legend,draw=none,fill=color2,fill opacity=0.5}
\addlegendentry{k=3}

\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.263167977333069,0) rectangle (axis cs:0.525685787200928,0.460623984346566);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.525685787200928,0) rectangle (axis cs:0.788203477859497,0.476833788422071);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:0.788203477859497,0) rectangle (axis cs:1.05072128772736,0.44576509553637);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.05072128772736,0) rectangle (axis cs:1.31323897838593,0.450718245713403);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.31323885917664,0) rectangle (axis cs:1.57575666904449,0.396685908250042);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.57575678825378,0) rectangle (axis cs:1.83827447891235,0.303930884971575);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:1.83827447891235,0) rectangle (axis cs:2.10079216957092,0.247647387754617);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.10079193115234,0) rectangle (axis cs:2.36330962181091,0.213427021446706);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.36330986022949,0) rectangle (axis cs:2.62582778930664,0.157143381512121);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.62582778930664,0) rectangle (axis cs:2.88834547996521,0.10806431465656);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:2.88834524154663,0) rectangle (axis cs:3.1508629322052,0.075645020259592);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.15086317062378,0) rectangle (axis cs:3.41338086128235,0.0481786736177164);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.41338086128235,0) rectangle (axis cs:3.6758987903595,0.0220631108713293);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.67589855194092,0) rectangle (axis cs:3.93841624259949,0.01350803933207);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:3.93841648101807,0) rectangle (axis cs:4.20093441009521,0.0103561540824607);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.20093441009521,0) rectangle (axis cs:4.46345186233521,0.00405241548002493);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.46345186233521,0) rectangle (axis cs:4.72596979141235,0.00135080270640792);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.7259693145752,0) rectangle (axis cs:4.98848676681519,0.00135080516000831);
\draw[draw=none,fill=color2,fill opacity=0.5] (axis cs:4.98848724365234,0) rectangle (axis cs:5.25100517272949,0.00045026756880264);
\addplot [semithick, red, opacity=0.5, dashed, forget plot]
table {%
0.5 0
0.5 0.906499451926922
};
\end{axis}

\end{tikzpicture}


==> experiment_fig/ratio_function.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
% \tiny, \scriptsize, \small, \large, \Large, \LARGE, \huge, \Huge, \HUGE
\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, font=\large},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={\Large{radius}},
xmin=-0.260499999765307, xmax=5.25049999998882,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\Large{$g$}},
ymin=-0.0504999995231628, ymax=1.06049998998642,
% ymin=0, ymax=1.06049998998642,
ytick style={color=black}
]
\addplot [line width=3pt, color0]
table {%
-0.00999999977648258 1.00999999046326
0.0406060665845871 0.959393918514252
0.0912121310830116 0.908787846565247
0.141818180680275 0.858181834220886
0.19242425262928 0.807575762271881
0.243030324578285 0.756969690322876
0.293636381626129 0.706363618373871
0.344242453575134 0.655757546424866
0.394848525524139 0.605151474475861
0.445454597473145 0.554545402526855
0.49606066942215 0.50393933057785
0.546666741371155 0.453333258628845
0.597272753715515 0.402727246284485
0.647878885269165 0.352121114730835
0.698484897613525 0.301515102386475
0.749090969562531 0.250909030437469
0.799697041511536 0.200302958488464
0.850303113460541 0.149696886539459
0.900909185409546 0.0990908145904541
0.951515197753906 0.0484848022460938
1.00212132930756 0
1.05272734165192 0
1.10333347320557 0
1.15393948554993 0
1.20454549789429 0
1.25515151023865 0
1.3057576417923 0
1.35636365413666 0
1.40696978569031 0
1.45757579803467 0
1.50818181037903 0
1.55878794193268 0
1.60939407348633 0
1.66000008583069 0
1.71060621738434 0
1.7612122297287 0
1.81181836128235 0
1.86242437362671 0
1.91303038597107 0
1.96363651752472 0
2.01424264907837 0
2.06484866142273 0
2.11545467376709 0
2.16606092453003 0
2.21666693687439 0
2.26727294921875 0
2.31787896156311 0
2.36848497390747 0
2.41909098625183 0
2.46969699859619 0
2.52030301094055 0
2.57090926170349 0
2.62151527404785 0
2.67212128639221 0
2.72272729873657 0
2.77333354949951 0
2.82393932342529 0
2.87454533576965 0
2.92515134811401 0
2.97575759887695 0
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=1}
\addplot [line width=3pt, color1]
table {%
-0.00999999977648258 1.00499999523163
0.0406060665845871 0.979696989059448
0.0912121310830116 0.954393923282623
0.141818180680275 0.929090917110443
0.19242425262928 0.903787851333618
0.243030324578285 0.878484845161438
0.293636381626129 0.853181838989258
0.344242453575134 0.827878773212433
0.394848525524139 0.802575707435608
0.445454597473145 0.777272701263428
0.49606066942215 0.751969695091248
0.546666741371155 0.726666629314423
0.597272753715515 0.701363623142242
0.647878885269165 0.676060557365417
0.698484897613525 0.650757551193237
0.749090969562531 0.625454545021057
0.799697041511536 0.600151479244232
0.850303113460541 0.574848413467407
0.900909185409546 0.549545407295227
0.951515197753906 0.524242401123047
1.00212132930756 0.498939335346222
1.05272734165192 0.473636329174042
1.10333347320557 0.448333263397217
1.15393948554993 0.423030257225037
1.20454549789429 0.397727251052856
1.25515151023865 0.372424244880676
1.3057576417923 0.347121179103851
1.35636365413666 0.321818172931671
1.40696978569031 0.296515107154846
1.45757579803467 0.271212100982666
1.50818181037903 0.245909094810486
1.55878794193268 0.220606029033661
1.60939407348633 0.195302963256836
1.66000008583069 0.169999957084656
1.71060621738434 0.144696891307831
1.7612122297287 0.119393885135651
1.81181836128235 0.0940908193588257
1.86242437362671 0.0687878131866455
1.91303038597107 0.0434848070144653
1.96363651752472 0.0181817412376404
2.01424264907837 0
2.06484866142273 0
2.11545467376709 0
2.16606092453003 0
2.21666693687439 0
2.26727294921875 0
2.31787896156311 0
2.36848497390747 0
2.41909098625183 0
2.46969699859619 0
2.52030301094055 0
2.57090926170349 0
2.62151527404785 0
2.67212128639221 0
2.72272729873657 0
2.77333354949951 0
2.82393932342529 0
2.87454533576965 0
2.92515134811401 0
2.97575759887695 0
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=2}
\addplot [line width=3pt, color2]
table {%
-0.00999999977648258 1.00333333015442
0.0406060665845871 0.986464619636536
0.0912121310830116 0.969595968723297
0.141818180680275 0.952727258205414
0.19242425262928 0.935858607292175
0.243030324578285 0.918989896774292
0.293636381626129 0.902121186256409
0.344242453575134 0.88525253534317
0.394848525524139 0.868383824825287
0.445454597473145 0.851515114307404
0.49606066942215 0.834646463394165
0.546666741371155 0.817777752876282
0.597272753715515 0.800909101963043
0.647878885269165 0.78404039144516
0.698484897613525 0.767171680927277
0.749090969562531 0.750303030014038
0.799697041511536 0.733434319496155
0.850303113460541 0.716565608978271
0.900909185409546 0.699696898460388
0.951515197753906 0.682828307151794
1.00212132930756 0.665959596633911
1.05272734165192 0.649090886116028
1.10333347320557 0.632222175598145
1.15393948554993 0.615353465080261
1.20454549789429 0.598484873771667
1.25515151023865 0.581616163253784
1.3057576417923 0.564747452735901
1.35636365413666 0.547878742218018
1.40696978569031 0.531010031700134
1.45757579803467 0.514141440391541
1.50818181037903 0.497272729873657
1.55878794193268 0.480404019355774
1.60939407348633 0.463535308837891
1.66000008583069 0.446666657924652
1.71060621738434 0.429797947406769
1.7612122297287 0.412929236888885
1.81181836128235 0.396060526371002
1.86242437362671 0.379191875457764
1.91303038597107 0.362323224544525
1.96363651752472 0.345454514026642
2.01424264907837 0.328585803508759
2.06484866142273 0.311717092990875
2.11545467376709 0.294848442077637
2.16606092453003 0.277979671955109
2.21666693687439 0.26111102104187
2.26727294921875 0.244242370128632
2.31787896156311 0.227373659610748
2.36848497390747 0.21050500869751
2.41909098625183 0.193636357784271
2.46969699859619 0.176767647266388
2.52030301094055 0.159898996353149
2.57090926170349 0.143030226230621
2.62151527404785 0.126161575317383
2.67212128639221 0.109292924404144
2.72272729873657 0.092424213886261
2.77333354949951 0.0755555033683777
2.82393932342529 0.0586869120597839
2.87454533576965 0.0418182015419006
2.92515134811401 0.0249495506286621
2.97575759887695 0.00808078050613403
3.02636361122131 0
3.07696962356567 0
3.12757563591003 0
3.17818164825439 0
3.22878766059875 0
3.27939367294312 0
3.32999968528748 0
3.38060593605042 0
3.43121194839478 0
3.48181796073914 0
3.5324239730835 0
3.58303022384644 0
3.6336362361908 0
3.68424224853516 0
3.73484826087952 0
3.78545451164246 0
3.83606052398682 0
3.88666653633118 0
3.93727254867554 0
3.98787879943848 0
4.03848457336426 0
4.0890908241272 0
4.13969659805298 0
4.19030284881592 0
4.2409086227417 0
4.29151487350464 0
4.34212112426758 0
4.39272689819336 0
4.4433331489563 0
4.49393939971924 0
4.54454517364502 0
4.59515142440796 0
4.64575719833374 0
4.69636344909668 0
4.74696969985962 0
4.7975754737854 0
4.84818172454834 0
4.89878797531128 0
4.94939374923706 0
5 0
};
\addlegendentry{k=3}
\addplot [line width=3pt, red, opacity=0.5, forget plot]
table {%
-0.260499999765307 -2.77555756156289e-17
5.25049999998882 -2.77555756156289e-17
};
\addplot [line width=3pt, red, opacity=0.5, dashed, forget plot]
table {%
0.5 -0.0504999995231629
0.5 1.06049998998642
};
\end{axis}

\end{tikzpicture}

